Technical Design Report for the LUXE Experiment

This Technical Design Report presents a detailed description of all aspects of the LUXE (Laser Und XFEL Experiment), an experiment that will combine the high-quality and high-energy electron beam of the European XFEL with a high-intensity laser, to explore the uncharted terrain of strong-field quantum electrodynamics characterised by both high energy and high intensity, reaching the Schwinger field and beyond. The further implications for the search of physics beyond the Standard Model are also discussed.

==> Makefile <==
# Makefile for creating an ATLAS LaTeX document

# Copyright (C) 2002-2022 CERN for the benefit of the ATLAS collaboration
#------------------------------------------------------------------------------
# By default makes mydocument.pdf using target run_pdflatex.
# Replace mydocument with your main filename or add another target set.
# Adjust TEXLIVE if it is not correct, or pass it to "make new".
# Replace BIBTEX = biber with BIBTEX = bibtex if you use bibtex instead of biber.
# Adjust FIGSDIR for your figures directory tree.
# Adjust the %.pdf dependencies according to your directory structure.
# Use "make clean" to cleanup.
# Use "make cleanpdf" to delete $(BASENAME).pdf.
# "make cleanall" also deletes the PDF file $(BASENAME).pdf.
# Use "make cleanepstopdf" to remove PDF files created automatically from EPS files.
#   Note that FIGSDIR has to be set properly for this to work.

# Set the default target to run_pdflatex instead of run_latexmk to use explicit
# pdflatex/biber commands to compile.

# You can use the target version to check your TeX Live version.

#-------------------------------------------------------------------------------
# Check which TeX Live installation you have with the command pdflatex --version
TEXLIVE  = 2020
LATEX    = latex
PDFLATEX = pdflatex
# BIBTEX   = bibtex
BIBTEX   = biber
DVIPS    = dvips
DVIPDF   = dvipdf
TLVERS   = $(shell pdflatex --version | grep -Go 'TeX Live [0-9]*' | grep -Go '[0-9].*')
# TLOKAY   = $(shell test $(TLVERS) -ge $(TEXLIVE) && echo true)
TWIKI    = https://twiki.cern.ch/twiki/bin/view/AtlasProtected/PubComLaTeXFAQ

#-------------------------------------------------------------------------------
# The main document filename
BASENAME = mydocument

#-------------------------------------------------------------------------------
# Adjust this according to your top-level figures directory
# This directory tree is used by the "make cleanepstopdf" command
FIGSDIR  = figs
#-------------------------------------------------------------------------------

# EPSTOPDFFILES = `find . -name \*eps-converted-to.pdf`
rwildcard=$(foreach d,$(wildcard $1*),$(call rwildcard,$d/,$2) $(filter $(subst *,%,$2),$d))
EPSTOPDFFILES = $(call rwildcard, $(FIGSDIR), *eps-converted-to.pdf)

# Default target - make mydocument.pdf with latexmk.
default: run_latexmk
# Use pdflatex/biber instead to compile.
# default: run_pdflatex

.PHONY: run_latexmk
.PHONY: newdocument newdocumenttexmf newnotemetadata newpapermetadata newfiles
.PHONY: draftcover preprintcover newdata
.PHONY: version clean cleanpdf help

# Check TeX Live version
version:
	@echo "Checking version"
	@echo "TLVERS $(TLVERS), TEXLIVE $(TEXLIVE)"
	if [ $(TLVERS) -lt $(TEXLIVE) ]; then \
		echo "Your TeX Live version ($(TLVERS)) is older than $(TEXLIVE). Please consult $(TWIKI)"; \
	fi

# Standard pdflatex target
run_pdflatex: $(BASENAME).pdf
	@echo "Made $<"

# Remove -pdf option to run latex instead of pdflatex
run_latexmk:
	latexmk -pdf $(BASENAME)

#-------------------------------------------------------------------------------
# Specify the tex and bib file dependencies for running pdflatex
# If your bib files are not in the main directory adjust this target accordingly
#%.pdf:	%.tex *.tex bib/*.bib
%.pdf:	%.tex *.tex *.bib
	$(PDFLATEX) $<
	-$(BIBTEX)  $(basename $<)
	$(PDFLATEX) $<
	$(PDFLATEX) $<
#-------------------------------------------------------------------------------

# Default is to make a new paper
new: newnote

newpaper: TEMPLATE=atlas-paper
newpaper: newdocument newfiles newpapermetadata newauxmat

newpapertexmf: TEMPLATE=atlas-paper
newpapertexmf: newdocumenttexmf newfiles newpapermetadata newauxmat

newnote: TEMPLATE=atlas-note
newnote: newdocument newfiles newnotemetadata

newnotetexmf: TEMPLATE=atlas-note
newnotetexmf: newdocumenttexmf newfiles newnotemetadata

newbook: TEMPLATE=atlas-book
newbook: newdocument newfiles newpapermetadata

newbooktexmf: TEMPLATE=atlas-book
newbooktexmf: newdocumenttexmf newfiles newpapermetadata

draftcover:
	if [ $(TEXLIVE) -ge 2013 -a $(TEXLIVE) -lt 2100 ]; then \
	  sed 's/texlive=20[0-9][0-9]/texlive=$(TEXLIVE)/' template/atlas-draft-cover.tex \
	    >$(BASENAME)-draft-cover.tex; \
	else \
	  echo "Invalid value for TEXLIVE: $(TEXLIVE)"; \
	  cp  template/$(BASENAME)-draft-cover.tex $(BASENAME)-draft-cover.tex; \
	fi

preprintcover:
	sed 's/texlive=20[0-9][0-9]/texlive=$(TEXLIVE)/' template/atlas-preprint-cover.tex \
	  >$(BASENAME)-preprint-cover.tex
	#cp template/atlas-preprint-cover.tex $(BASENAME)-preprint-cover.tex

newdata:
	sed s/atlas-document/$(BASENAME)/ template/atlas-hepdata-main.tex | \
	sed 's/texlive=20[0-9][0-9]/texlive=$(TEXLIVE)/' >$(BASENAME)-hepdata-main.tex
	cp template/atlas-hepdata.tex $(BASENAME)-hepdata.tex

newdocument:
	if [ $(TEXLIVE) -ge 2013 -a $(TEXLIVE) -lt 2100 ]; then \
	  sed s/atlas-document/$(BASENAME)/ template/$(TEMPLATE).tex | \
	    sed 's/texlive=20[0-9][0-9]/texlive=$(TEXLIVE)/' >$(BASENAME).tex; \
	else \
	  echo "Invalid value for TEXLIVE: $(TEXLIVE)"; \
	  sed s/atlas-document/$(BASENAME)/ template/$(TEMPLATE).tex >$(BASENAME).tex; \
	fi

newdocumenttexmf:
	if [ $(TEXLIVE) -ge 2013 -a $(TEXLIVE) -lt 2100 ]; then \
	  sed s/atlas-document/$(BASENAME)/ template/$(TEMPLATE).tex | \
	  sed 's/texlive=20[0-9][0-9]/texlive=$(TEXLIVE)/' | \
	  sed 's/\\RequirePackage{latex\/atlaslatexpath}/% \\RequirePackage{latex\/atlaslatexpath}/' \
	  >$(BASENAME).tex; \
	else \
	  echo "Invalid value for TEXLIVE: $(TEXLIVE)"; \
	  sed s/atlas-document/$(BASENAME)/ template/$(TEMPLATE).tex >$(BASENAME).tex; \
	fi

newpapermetadata:
	cp template/atlas-paper-metadata.tex $(BASENAME)-metadata.tex

newnotemetadata:
	cp template/atlas-note-metadata.tex $(BASENAME)-metadata.tex

newfiles:
	echo "% Put you own bibliography entries in this file" > $(BASENAME).bib
	# touch $(BASENAME).bib
	touch $(BASENAME)-defs.sty

newauxmat:
	cp template/atlas-auxmat.tex $(BASENAME)-auxmat.tex
	cp template/atlas-hepdata.tex $(BASENAME)-hepdata.tex

run_latex: dvipdf

# Targets if you run latex instead of pdflatex
dvipdf:	$(BASENAME).dvi
	$(DVIPDF) -sPAPERSIZE=a4 -dPDFSETTINGS=/prepress $<
	@echo "Made $(basename $<).pdf"

dvips:	$(BASENAME).dvi
	$(DVIPS) $<
	@echo "Made $(basename $<).ps"

# Specify dependencies for running latex
#%.dvi:	%.tex tex/*.tex bibtex/bib/*.bib
%.dvi:	%.tex *.tex *.bib
	$(LATEX)    $<
	-$(BIBTEX)  $(basename $<)
	$(LATEX)    $<
	$(LATEX)    $<

%.bbl:	%.tex *.bib
	$(LATEX) $<
	$(BIBTEX) $<

help:
	@echo "To create a new paper/CONF Note/PUB Note draft give the command:"
	@echo "make newpaper [BASENAME=mydocument] [TEXLIVE=YYYY]"
	@echo "To create a new ATLAS note draft give the command:"
	@echo "make newnote [BASENAME=mydocument] [TEXLIVE=YYYY]"
	@echo "To create a long document (book) like a TDR:"
	@echo "make newbook [BASENAME=mydocument] [TEXLIVE=YYYY]"
	@echo ""
	@echo "To compile the paper give the command"
	@echo "make"
	@echo "If your bib files are not in the main directory, adjust the %.pdf target accordingly." 
	@echo ""
	@echo "To compile the document using latexmk give the command:"
	@echo "make run_latexmk"
	@echo "You can also adjust the 'default' target."
	@echo ""
	@echo "If atlaslatex is installed centrally, e.g. in ~/texmf:"
	@echo "make newpapertexmf|newnotetexmf|newbooktemf [BASENAME=mydocument] [TEXLIVE=YYYY]"
	@echo ""
	@echo "If you need a standalone draft cover give the commands:"
	@echo "make draftcover [BASENAME=mydocument] [TEXLIVE=YYYY]"
	@echo "pdflatex mydocument-draft-cover"
	@echo ""
	@echo "If you need a standalone preprint cover give the commands:"
	@echo "make preprintcover [BASENAME=mydocument] [TEXLIVE=YYYY]"
	@echo "pdflatex mydocument-preprint-cover"
	@echo ""
	@echo "If you need a document for HepData material give the commands:"
	@echo "make newdata [BASENAME=mydocument] [TEXLIVE=YYYY]"
	@echo "pdflatex mydocument-hepdata-main"
	@echo ""
	@echo "make clean    to clean auxiliary files (not output PDF)"
	@echo "make cleanpdf to clean output PDF files"
	@echo "make cleanps  to clean output PS files"
	@echo "make cleanall to clean all files"
	@echo "make cleanepstopdf to clean PDF files automatically made from EPS"
	@echo "make version to check your TeX Live version"
	@echo ""

clean:
	-rm *.dvi *.toc *.aux *.lof *.lot *.log *.out \
		*.bbl *.blg *.brf *.bcf *-blx.bib *.run.xml \
		*.cb *.ind *.idx *.ilg *.inx *.tdo \
		*.synctex.gz *~ *.fls *.fdb_latexmk .*.lb spellTmp

cleanpdf:
	-rm $(BASENAME).pdf
	-rm $(BASENAME)-draft-cover.pdf $(BASENAME)-preprint-cover.pdf
	-rm $(BASENAME)-hepdata-main.pdf

cleanps:
	-rm $(BASENAME).ps
	-rm $(BASENAME)-draft-cover.ps $(BASENAME)-preprint-cover.ps
	-rm $(BASENAME)-hepdata-main.ps

cleanall: clean cleanpdf cleanps

# Clean the PDF files created automatically from EPS files
cleanepstopdf: $(EPSTOPDFFILES)
	@echo "Removing PDF files made automatically from EPS files"
	-rm $^


==> acknowledgements/Makefile <==
# Makefile for creating ATLAS Acknowledegments

TEXLIVE  = 2020
PDFLATEX = pdflatex
BIBTEX   = biber

BASENAME = Acknowledgements-main

.PHONY: clean cleanpdf

run_pdflatex: $(BASENAME).pdf
	@echo "Made $<"

# Change TeX Live version
texlive: $(BASENAME).tex
	if [ $(TEXLIVE) -ge 2013 -a $(TEXLIVE) -lt 2100 ]; then \
	  echo "Changing texlive value in $<"; \
	  sed -i'.bak' 's/texlive=20[0-9][0-9]/texlive=$(TEXLIVE)/' $<; \
	else echo "Invalid value for TEXLIVE: $(TEXLIVE)"; fi; \

# Change biblatex backend
bibtex: $(BASENAME).tex
	if [ $(BIBTEX) = 'biber' -o $(BIBTEX) = 'bibtex' ]; then \
	  echo "Changing biblatex backend in $<"; \
	  sed -i'.bak' -e 's/backend=biber/backend=$(BIBTEX)/' -e 's/backend=bibtex/backend=$(BIBTEX)/' $<; \
	else echo "Invalid value for BIBTEX: $(BIBTEX)"; fi; \

# Standard LaTeX targets
$(BASENAME).pdf: $(BASENAME).tex
	$(PDFLATEX) $<
	-$(BIBTEX)  $(basename $<)
	$(PDFLATEX) $<
	$(PDFLATEX) $<

%.bbl: %.tex *.bib
	$(PDFLATEX) $*
	$(BIBTEX) $*

clean:
	-rm *.dvi *.toc *.aux *.log *.out *.blg *.bbl *.bcf *-blx.bib \
	 *.run.xml *.synctex.gz *~ *.fls *.fdb_latexmk .*.lb spellTmp 

cleanpdf:
	-rm $(BASENAME).pdf

cleanall: clean cleanpdf


==> authorlists/authorlist-inst.tex <==
\setcounter{Maxaffil}{2000} 
 \author{ I.~Levy}
 \affil {Department of Physics, Nuclear Research Centre-Negev, P.O. Box 9001, Beer Sheva 84190, Israel}
\author{N.~Cavanagh}
\author{K.~Fleck}
\author{G.~Sarri}
\author{M.~Streeter}
\affil{School of Mathematics and Physics, The Queen’s University of Belfast, BT7 1NN, Belfast, United Kingdom}
\author{M.~Bruschi}
\author{A.~Sbrizzi}
\affil{INFN, Bologna, Italy}
\author{U.~Acosta}
\author{B.~K{\"a}mpfer}
\affil{ Helmholtz-Zentrum Dresden-Rossendorf, 01328 Dresden, Germany\\
{\rm and}\\
TU~Dresden, 01062 Dresden, Germany}
\author{M.~Gostkin}
\author{A.I.~Titov}
\author{A.~Zhemchugov}
\affil{ Joint Institute for Nuclear Research ( JINR), Dubna 141980, Russia} 
\author{F.~Qu\'er\'e}
  \affil{LIDYL, CEA, CNRS, Universit\'e Paris-Saclay, CEA Saclay, 91 191 Gif-sur-Yvette, France}
\author{T.~Blackburn}
\affil{University of Gothenburg, SE-41296 Gothenburg, Sweden}
 \author{T.~Ma}
\author{Y.~Soreq}
  \affil{Physics Department, Technion—Israel Institute of Technology, Haifa 3200003, Israel}
  \author{M.~Altarelli}
  \affil{Max Planck Institute for Structure and Dynamics of Matter, Hamburg, 22761, Germany}
\author{R.~A{\ss}mann}
\author{T.~Behnke}
\author{O.~Borysov}
\author{R.~Brinkmann}
\author{F.~Burkart}
\author{K.~B{\"u}{\ss}er}
\author{W.~Decking}
%\author{B.~Heinemann$^{a,b}$}
\author{B.~Heinemann\footnote {\bf corresponding author: beate.heinemann@desy.de} \footnote{also at Albert-Ludwigs-Universit{\"a}t-Freiburg}}
\author{L.~Helary}
\author{M.~Hoffmann}
\author{X.~Huang}
\author{R.~Jacobs}
\author{J.~List}
%\author{W.~Lohmann$^{c}$}
\author{W.~Lohmann\footnote{also at BTU, Cottbus and RWTH, Aachen}}
\author{E.~Negodin}
\author{R.~Prasad}
\author{A.~Ringwald}
\author{S.~Schmitt}
\author{S.~Schuwalow}
\author{M.~Shchedrolosiev}
\author{D.~Thoden}
   \affil{Deutsches Elektronen-Synchrotron (DESY), Hamburg, 22607, Germany} 

%\author{M.~Zepf $^{d}$}
\author{M.~Zepf \footnote{also at Helmholtz Institut Jena,  07743 Jena, Germany}}
  \affil{Friedrich Schiller Universit{\"a}t Jena, Jena, 07743, Germany}
\author{A.~S{\"a}vert}
\author{D.~Seipt}
\author{T.~Teter}
  \affil{Helmholtz Institut Jena,  07743 Jena, Germany}
\author{M.~Firlej}
\author{T.~Fiutowski}
\author{M.~Idzik}
\author{J.~Moron} 
\author{K.~Swientek}
\affil{AGH University of Science and Technology, Faculty of Physics and Applied Computer 
Science, Krakow, Poland}

\author{M.~Borysova}
\author{H.~Lahno}
  \affil{ Institute for Nuclear Research NASU (KINR), Kyiv, 03680, Ukraine}
% \author{J.~Hallford$^{f}$}
\author{J.~Hallford\footnote{also at  Deutsches Elektronen-Synchrotron (DESY), Hamburg, 22607, Germany }}
\author{A.~Hartin}
\author{M.~Wing\footnote{also at  Deutsches Elektronen-Synchrotron (DESY), Hamburg, 22607, Germany }}
  \affil{University College London, London, WC1E 6BT, United Kingdom}
 \author{ A.~Fedetov}
\author{A.~Mironov}
  \affil{National Research Nuclear University MEPhI, Kashirskoe sh. 31, Moscow, 115409, Russia}
 \author{S.~Rykovanov}
  \affil{Skolkovo Institute of Science and Technology (Skoltech), Moscow 121205, Russia}
  \author{U.~Dosselli, M.~Morandin, M.~Zanetti}
  \affil{INFN, Padova, Italy}
 \author{B.~King}
\author{T.~Heinzl}
\author{A.~Ilderton}
\author{A.J.~Macleod}
\author{S.~Tang}
  \affil{University of Plymouth, Plymouth PL4 8AA, United Kingdom}

\author{O.~Davidi}
\author{G.~Perez}
\author{A.~Santra}
 \author{N.~Tal Hod}
  \affil{Weizmann Institute of Science, Rehovot, 7610001, Israel}
\author{Z.~Bai\footnote{ also at Weizmann Institute of Science, Rehovot, 7610001, Israel}}
\affil{Department of Physics, Southern University of Science and Technology, Shenzhen 518055, China}
\author{S.~Boogert}
  \affil{John Adams Institute at Royal Holloway, Department of Physics, Royal Holloway, Egham, TW20 0EX, Surrey, United Kingdom}
\author{H.~Abramowicz}
\author{Y.~Benhammou}
\author{S.~Huang}
\author{A.~Levanon}
\author{A.~Levy}
\author{I.~Pomerantz}
  \affil{Tel Aviv University, Tel Aviv, 6997801, Israel}



                                                           %




==> authorlists/authorlist.tex <==

\author[1]{H. Abramowicz}
\author[2,3]{U.~Acosta}
\author[4]{M. Altarelli}
\author[5]{R.~A{\ss}mann}
\author[6,7]{Z.~Bai}
\author[5]{T.~Behnke}
\author[1]{Y.~Benhammou}
\author[8]{T.~Blackburn}
\author[9]{S.~Boogert}
\author[5]{O.~Borysov}
\author[5,10]{M.~Borysova}
\author[5]{R.~Brinkmann}
\author[11]{M.~Bruschi}
\author[5]{F.~Burkart}
\author[5]{K.~B{\"u}{\ss}er}
\author[12]{N.~Cavanagh}
\author[6]{O.~Davidi}
\author[5]{W.~Decking}
\author[13]{U.~Dosselli}
\author[3]{N.~Elkina}
\author[14]{A.~Fedotov}
\author[15]{M.~Firlej}
\author[15]{T.~Fiutowski}
\author[12]{K.~Fleck}
\author[16]{M.~Gostkin}
\author[5]{C.~Grojean\thanks{also at HU Berlin}}
\author[5,17]{J.~Hallford}
\author[18,19] {H.~Harsh}
\author[17]{A.~Hartin}
%\author[3]{I.~Hartl}
\author[5,20]{B.~Heinemann\thanks{corresponding author: beate.heinemann@desy.de}}
\author[21]{T.~Heinzl}
\author[5]{L.~Helary}
\author[5,20]{M.~Hoffmann}
\author[1]{S.~Huang}
\author[5,15,20]{X.~Huang}
\author[15]{M.~Idzik}
\author[21]{A.~Ilderton}
\author[5]{R.~Jacobs}
\author[2,3]{B.~K{\"a}mpfer}
\author[21]{B.~King} 
\author[10]{H.~Lahno}
\author[1]{A.~Levanon}
\author[1]{A.~Levy}
\author[22]{I.~Levy}
\author[5]{J.~List}
\author[5]{W.~Lohmann\thanks{also at BTU Cottbus und RWTH Aachen}}
\author[23]{T.~Ma}
\author[21]{A.J.~Macleod}
\author[6]{V. Malka}
\author[5]{F.~Meloni}
\author[14]{A.~Mironov}
\author[13]{M.~Morandin}
\author[15]{J.~Moron}
\author[5]{E.~Negodin}
\author[6]{G.~Perez}
\author[1]{I.~Pomerantz}
\author[24]{R.P{\"o}schl}
\author[5]{R.~Prasad}
\author[25]{F.~Qu\'er\'e}
\author[5]{A.~Ringwald}
\author[26]{C.~R\"odel}
%\author[3]{M.~Saimpert}
\author[27]{S.~Rykovanov}
\author[18,19] {F. Salgado}
\author[6]{A.~Santra}
\author[12]{G.~Sarri}
\author[18]{A.~S{\"a}vert}
\author[28]{A.~Sbrizzi\thanks{also at University of Udine, Udine, Italy}}
\author[5]{S.~Schmitt}
\author[2,3]{U.~Schramm}
\author[5]{S.~Schuwalow}
\author[18]{D.~Seipt}
\author[29]{L.~Shaimerdenova}
\author[5]{M.~Shchedrolosiev}
\author[29]{M.~Skakunov}
\author[23]{Y.~Soreq}
\author[12]{M.~Streeter}
\author[15]{K.~Swientek}
%\author[6]{T.~Teter}
%\author[21]{A.~Titov}
\author[6]{N.~Tal~Hod}
\author[21]{S.~Tang}
\author[18,19]{T.~Teter}
\author[5]{D.~Thoden}
\author[16]{A.I.~Titov}
\author[29]{O.~Tolbanov}
\author[3]{G.~Torgrimsson}
\author[29]{A.~Tyazhev}
\author[5,17]{M.~Wing}
\author[13]{M.~Zanetti}
\author[29]{A.~Zarubin}
\author[3]{K.~Zeil}
\author[18,19]{M.~Zepf}
\author[16]{A.~Zhemchukov}

\affil[1]{Tel Aviv University, Tel Aviv, 6997801, Israel}
\affil[2]{TU~Dresden, 01062 Dresden, Germany}
\affil[3]{Helmholtz-Zentrum Dresden-Rossendorf, 01328 Dresden, Germany}
\affil[4]{Max Planck Institute for Structure and Dynamics of Matter, 22761 Hamburg, Germany}
\affil[5]{Deutsches Elektronen-Synchrotron (DESY), 22607 Hamburg, Germany}
\affil[6]{Weizmann Institute of Science, Rehovot, 7610001, Israel}
\affil[7]{Department of Physics, Southern University of Science and Technology, Shenzhen 518055, China}
%
\affil[8]{University of Gothenburg, SE-41296 Gothenburg, Sweden}
\affil[9]{John Adams Institute at Royal Holloway, Department of Physics, Royal Holloway, Egham, TW20 0EX, Surrey, UK}
\affil[10]{Institute for Nuclear Research NASU (KINR), Kyiv, 03680, Ukraine}
\affil[11]{INFN and University of Bologna, Bologna, Italy}
\affil[12]{School of Mathematics and Physics, The Queen’s University of Belfast, Belfast, BT7 1NN, UK}
\affil[13]{INFN and University of Padova, Padova, Italy}
\affil[14]{National Research Nuclear University MEPhI, Kashirskoe sh. 31, Moscow, 115409, Russia}
\affil[15]{Faculty of Physics and Applied Computer Science, AGH University of Science and Technology,  Krakow, Poland} 
\affil[16]{Joint Institute for Nuclear Research ( JINR), Dubna 141980, Russia}
\affil[17]{University College London, London, WC1E 6BT, UK}
\affil[18]{Helmholtz Institut Jena,  07743 Jena, Germany}
\affil[19]{Friedrich Schiller Universit{\"a}t Jena, 07743 Jena, Germany}
\affil[20]{Albert-Ludwigs-Universit{\"a}t Freiburg, 79085 Freiburg, Germany}
\affil[21]{University of Plymouth, Plymouth, PL4 8AA, UK}
\affil[22]{Department of Physics, Nuclear Research Centre-Negev, P.O. Box 9001, Beer Sheva 84190, Israel}
\affil[23]{Physics Department, Technion—Israel Institute of Technology, Haifa 3200003, Israel}
\affil[24]{Universit{\'e} Paris-Saclay, CNRS/IN2P3, IJCLab, 91405 Orsay, France}
\affil[25]{LIDYL, CEA, CNRS, Universit\'e Paris-Saclay, CEA Saclay, 91 191 Gif-sur-Yvette, France}
\affil[26]{Institute of Nuclear Physics, TU Darmstadt, 64289 Darmstadt, Germany}
\affil[27]{Skolkovo Institute of Science and Technology (Skoltech), Moscow 121205, Russia}
\affil[28]{INFN Trieste, Trieste, Italy}
\affil[29]{National Research Tomsk State University NI TSU, TSU, Russia}


%\newpage

==> bib/doc/Makefile <==
# Makefile for creating documentation for ATLAS LaTeX
# Usually called from a subdirectory

TEXLIVE  = 2020
LATEX    = latex
PDFLATEX = pdflatex
BIBTEX   = biber
DVIPS    = dvips
DVIPDF   = dvipdf

BASENAME = dummy

.PHONY: clean cleanpdf

run_pdflatex: $(BASENAME).pdf
	@echo "Made $<"

# Remove -pdf option to run latex instead of pdflatex
run_latexmk:
	latexmk -pdf $(BASENAME)

run_latex: $(BASENAME).dvi
	$(DVIPDF) -sPAPERSIZE=a4 -dPDFSETTINGS=/prepress $<
	@echo "Made $< and $(basename $<).pdf"

# Change TeX Live version
texlive: $(BASENAME).tex
	if [ $(TEXLIVE) -ge 2013 -a $(TEXLIVE) -lt 2100 ]; then \
	  echo "Changing texlive value in $<"; \
	  sed -i'.bak' 's/texlive=20[0-9][0-9]/texlive=$(TEXLIVE)/' $<; \
	else echo "Invalid value for TEXLIVE: $(TEXLIVE)"; fi; \

# Standard LaTeX targets
$(BASENAME).pdf: $(BASENAME).tex
	$(PDFLATEX) $<
	-$(BIBTEX)  $(basename $<)
	$(PDFLATEX) $<
	$(PDFLATEX) $<

%.bbl: %.tex *.bib
	$(PDFLATEX) $*
	$(BIBTEX) $*

clean:
	-rm *.dvi *.toc *.aux *.log *.out *.blg *.bbl *.bcf *-blx.bib \
	 *.run.xml *.synctex.gz *.fls *.fdb_latexmk *.listing .*.lb *~

cleanpdf:
	-rm $(BASENAME).pdf


==> bib/doc/atlas_latex/atlas_latex-text.tex <==
% !TEX root = atlas_latex.tex

%-------------------------------------------------------------------------------
% Body of the guide to the use of the ATLAS LaTeX package
%-------------------------------------------------------------------------------
\section{Introduction}
\label{sec:intro}
%-------------------------------------------------------------------------------

This collection of ATLAS \LaTeX\ templates, style files and documentation
can be used for papers, preprints and notes, both public and internal. 
All necessary files are collected in a single package called \Package{atlaslatex}.
The package is available from the web pages of the Publication Committee~\cite{pubcom} and from 
Git~\cite{pubcom-git}.

\ADOCnew{09-00-00} The package should work for \TeX\ Live versions from 2013 onwards.
\ADOCnew{II-JJ-KK} indicates the version number of ATLAS \LaTeX\ when new features are added.
\ADOCold{II-J-KK} indicates the version number when a feature is removed or made obsolete.

The collection replaces and improves on the previous packages.
In particular it supersedes:
\begin{itemize}\setlength{\parskip}{0pt}\setlength{\itemsep}{0pt}
\item \texttt{atlasnote-00-04-05}
\item \texttt{atlascover-00-00-11}
\item \texttt{atlaspreprint-00-00-05}
\item \texttt{atlasbib-00-00-04}
\end{itemize}
\Cref{sec:oldnote} summarises the changes that have been made and
how you can adapt your documents to use the new package.
\Cref{sec:oldcover} summarises the changes to the cover macros.

The package includes the \Package{atlasdoc} class, useful style files
and documentation of the package.
The package also defines a standard ATLAS style for papers.
This style should be used for paper drafts and for submission to the arXiv and the journal.
This option is the default. Add the option \Option{atlasstyle=false} to the \Package{atlasdoc} class if you do not want to use this style.
The documentation is provided as both PDF files and \LaTeX\ documents
that should provide examples of how to use the package and how to write
good \LaTeX.

The design principle is that you have a main document and 
the style files and \Package{atlasdoc} class are in a subdirectory \File{latex}.
The logos that are needed are kept in a \File{logos} directory.
These subdirectories can of course be links to a centrally maintained \texttt{latex} directory.
See below and \cref{sec:texmf} for how to proceed if you want to use and/or install
the package in a central place.

The usual procedure is that for each document that you create,
you first unpack the latest version of \Package{atlaslatex} and
then create your main document in the top-level directory.
This structure means that it is easier to update the style files if a new version of
\Package{atlaslatex} is released. 
Each document can then be independent of the \Package{atlaslatex} release.

%------------------------------------------------------------------------------
\section{Getting started}
%------------------------------------------------------------------------------

To create a new document you can issue one of the commands:
%
\begin{bashlisting}
make newpaper [BASENAME=mydocument] [TEXLIVE=YYYY]
make newnote [BASENAME=mydocument] [TEXLIVE=YYYY]
\end{bashlisting}
depending on whether you want to write a paper/CONF Note/Pub Note draft or
an ATLAS not draft.
%
The command copies \File{atlas-document.tex} and
\File{atlas-paper-metadata.tex} or \File{atlas-note-metadata.tex}
to \File{mydocument.tex} and \File{mydocument-metadata.tex}.%
\footnote{The \File{Makefile} should work for regular Linux and MacOSX distributions.
For Windows, you probably have to execute the tasks in the \File{Makefile} by hand.}
The selected \TeX\ Live version is set with the \Option{TEXLIVE} option. The default is 2020.
The \texttt{make newpaper|newnote} command also creates empty files \File{mydocument-defs.sty} and \File{mydocument.bib}.
By default the document will be an ATLAS note draft.
Use \texttt{make newpaper} for an ATLAS paper draft (including CONF and PUB notes).
% If you want it to be a paper draft, add the option \Option{PAPER} to the document class.
Replace the option \Option{PAPER} with \Option{CONF} or \Option{PUB} as appropriate.

In the \File{Makefile} you should change the \texttt{BASENAME} to the name of your document.
You can then compile your document with the command: \texttt{make}.
You can try the command \texttt{make run\_latexmk} instead,
which invokes \texttt{latexmk}, a Perl script that is cleverer than the \texttt{Makefile}.
You can also make this command the default.
Have a look at \File{Makefile} for other things you can adjust.

If you install \Package{atlaslatex} in a central directory such as \File{\$\{HOME\}/texmf} the basic command is one of:
%
\begin{bashlisting}
make newpapertexmf [BASENAME=mydocument] [TEXLIVE=YYYY]
make newnotetexmf [BASENAME=mydocument] [TEXLIVE=YYYY]
make newbooktexmf [BASENAME=mydocument] [TEXLIVE=YYYY]
\end{bashlisting}
%
See \cref{sec:texmf} for more details.

In order to make a new document of book form like a TDR, use one of the commands:
%
\begin{bashlisting}
make newbook [BASENAME=mydocument] [TEXLIVE=YYYY]
make newbooktexmf [BASENAME=mydocument] [TEXLIVE=YYYY]
\end{bashlisting}
%
By default, this will pass the option \Option{BOOK} to \Package{atlasdoc}.
Use \verb|make newbooktexmf| for a book with \Package{atlaslatex} in a central directory.

Note that you have to specify the language of your document as an option in the
\Macro{documentclass} command. Typical settings are
\begin{itemize}
\item UKenglish (or british);
\item USenglish (or american).
\end{itemize}

As mentioned above the default \TeX\ Live version is currently set to 2020.
This should be the only option you have to adjust if you use different versions of \LaTeX.
You should be able to always set a version lower than the one you have installed to maintain compatibility with older versions.
To test compatibility with arXiv, try a setting of 2020.
%This will, among other things, automatically switch from the \Package{newtx} fonts to \Package{txfonts} if you
%are using the ATLAS preprint style.

\ADOCnew{01-07-00} You should include the command \Macro{maketitle} after your\\
\verb|\begin{document}| if you want the document title to be printed.

Add the option \Option{atlasstyle=false} to the \Macro{documentclass} if you do not want to typeset your document in the ATLAS preprint style.

%------------------------------------------------------------------------------
\section{ATLAS \LaTeX\ and the Physics Office GitLab project}
%------------------------------------------------------------------------------

With the move of ATLAS software and documents to Git,
new opportunities are available to streamline the production of documents
and smooth the process of submitting them to arXiv and journals.
This project is called PO-GitLab in the following~\cite{atlas-PO-gitlab}.

In order for the new tools to work smoothly some file-naming conventions should be followed.
If the Physics Office set up the Git repository, the files should already have the correct names.
The conventions are documented on
\url{https://gitlab.cern.ch/atlas-physics-office/gitlab-integration/wikis/newproject}.
For paper drafts, in short:
\begin{itemize}
  \item the main file should have the name GROUP-YEAR-NUM-PAPER.tex;
  \item the metadata file should have the name GROUP-YEAR-NUM-PAPER-metadata.tex
  \item the auxiliary material should be included in a file with the name GROUP-YEAR-NUM-PAPER-auxmat.tex
\end{itemize}

In addition:
\begin{itemize}
  \item figures must be included using the \Macro{includegraphics} command;
\end{itemize}

%-------------------------------------------------------------------------------
\section{Title, author and document numbers}
\label{sec:metadata}
%-------------------------------------------------------------------------------

An ATLAS document usually collects a series of labels over time.
These include the reference code of the analysis, e.g.\ \texttt{BPHY-2013-04}, 
the ATLAS note number and the CERN preprint number.
In addition the abstract and title are needed on the front page of the document and also on various cover pages.
The editors of the document, the editorial board members and the contributors to the analysis
also need to be specified at some point.

While all this information can be collected in the main file of the document, 
it is probably better to put it all in a separate document.
By default this file is called \texttt{mydocument-metadata.tex}.

\ADOCnew{04-00-00} As the metadata needed for ATLAS notes and ATLAS papers are somewhat different,
separate templates are used.


%-------------------------------------------------------------------------------
\subsection{Authors and Contributors}
\label{sec:contribute}
%-------------------------------------------------------------------------------

You can include an author's ORCID using the \Macro{AtlasOrcid} macro:\\
\verb+\AtlasOrcid[0000-0002-03-9876]{John Postdoc}+.
This command will be used in the ATLAS Collaboration author lists.

The supporting documentation for an ATLAS note (not the paper draft) should contain a list of the contributors to the analysis.
A style file \Package{atlascontribute.sty} has been written to help with the creation of such a list.
The macros in the style file can also build the author list at the same time.
Two basic macros are used to add names to the author list and list of contributions:
\Macro{AtlasContributor} and \Macro{AtlasAuthorContributor}. 
The first macro adds a person to the list of contributors, while the second one also adds the person
to the author list. I assume that in almost all cases you will want to use \Macro{AtlasAuthorContributor}.
An optional argument can be added to \Macro{AtlasAuthorContributor}, which contains the author's ORCID.
The author's name becomes a link to the ORCID.
Typical commands are:
\begin{tcblisting}{listing only}
\AtlasAuthorContributor{Joe Student}{a}{fake background estimate.}
\AtlasAuthorContributor{Jane Student}{b}{top background estimate.}
\AtlasAuthorContributor[0000-0002-03-9876]{John Postdoc}{a}{editor of internal note.}
\AtlasContributor{Jo Helper}{useful contributions in a few places.}
\affil[a]{University of Nowhere}
\affil[b]{University of Somewhere}
\end{tcblisting}
If a person should be added to the author list, you also need to add an appropriate affiliation using the macro \Macro{affil}.
The optional argument is a letter or number that should also be given as the second argument to
\Macro{AtlasAuthorContributor}.

You can keep the list of authors and contributors separate
by using \Macro{author} for the authors and \Macro{AtlasContributor} for the contributors.
You print the list of contributors by giving the command \Macro{PrintAtlasContribute}.
Note that \Macro{PrintAtlasContribute} has an argument that gives the fraction of the line width
to be used for the name of the person.
The list should either be printed before the table of contents or after the conclusions
(i.e.\ where the Acknowledgements appear in a paper).

Note that the \Package{authblk} package assumes that you will also have affiliations for each author.
You can avoid them by using the syntax \verb|\author{[ ]{Author Name}}|.
Note that a space is needed in the optional argument.
This means that a space appears between the author name and the comma after it, which is not so nice.
Alternatively you can make the author list using the syntax:\\
\verb|\author{Joe Student \and Jane Student \and John Postdoc}| and avoid the use of the
\Package{authblk} package by giving the option \Option{authblk=false} to \Package{atlascontribute}.

Note that the \Package{atlascontribute} package requires that the packages 
\Package{array} and \Package{booktabs} be installed.
If the list of contributors is very long, it may spread over more than one page.
The \Package{tabular} environment does not like this.
Add the option \Option{longtable} to use \Package{longtable},
or the option \Option{xtab} to use \Package{xtab}.
This option of course also requires that the \Package{xtab} or \Package{longtable} package is installed.


%-------------------------------------------------------------------------------
\subsection{Special author lists}
%-------------------------------------------------------------------------------

Sometimes a PUB note has a special author list.
Hence a link to this list should be added to the front page.
This can be achieved with the following code snippet that should be used for the author:
\begin{tcblisting}{listing only}
% \usepackage[marginal,hang]{footmisc}
% \setlength{\footnotemargin}{0.5em}
\usepackage{authblk}
\author{The ATLAS Collaboration%
\thanks{The full author list can be found at:\\
  \url{https://atlas.web.cern.ch/Atlas/PUBNOTES/ATL-PHYS-PUB-2014-YYY/authorlist.pdf}}
}
\end{tcblisting}

\ADOCnew{01-07-00} The first two lines are needed if you do not use the standard ATLAS preprint style.
Note that \Package{atlasdoc} has to be loaded with the option \Option{maketitle=false}
and \Macro{maketitle} should be added after \verb|\begin{document}|.

\ADOCold{07-00-00} In order that the footnote and the copyright statement do not overlap,
you may need to pass the option \Option{copyrightoffset=1em} to the \Package{atlasdoc} class.


%-------------------------------------------------------------------------------
\subsection{Metadata commands}
%-------------------------------------------------------------------------------

The standard list of metadata commands are given below.
More are available for the draft cover page when a paper, CONF note or PUB note draft
is circulated to the collaboration.\\
See \texttt{template/atlas-document-metadata.tex} for more details.

\begin{itemize}
  \item \Macro{AtlasTitle\{<Title>\}} typesets the paper title. If not
    given, you get either an error or a dummy title will be produced.

  \item \Macro{author\{<Author>\}} typesets the paper author. If not
    explicitly given, \enquote{The ATLAS Collaboration} will be used by
    default. Note that the \verb|\author{}| command is pretty limited
    in case you want to display multiple author names and multiple
    affiliations. For this use case the \verb|authblk.sty| package is
    provided; this is a typical example of its use:
    \begin{verbatim}
\usepackage{authblk}
\renewcommand\Authands{, } % avoid ``. and'' for last author
\renewcommand\Affilfont{\itshape\small} % affiliation formatting

\author[a]{First Author}
\author[a]{Second Author}
\author[b]{Third Author}

\affil[a]{One Institution}
\affil[b]{Another Institution}
    \end{verbatim}
    See also \cref{sec:contribute} if you want to combine the creation of a list of authors and contributors.

    If you do not want each institute on a separate line, uncomment the lines in the metadata file:
    \begin{verbatim}
\makeatletter
\renewcommand\AB@affilsepx{, \protect\Affilfont}
\makeatother
    \end{verbatim}


  \item \Macro{AtlasAbstract\{<The abstract text>\}} typesets the
    abstract on the front page and cover page.

  \item \Macro{date\{<Date>\}} typesets the paper date. If not
    explicitly given, the current date (\verb|\today|) will be used.

  \item \Macro{AtlasVersion\{<Draft Version>\}} displays the draft
    version on the front page, a DRAFT banner on all the other page
    headings, and adds line numbers to all text to easy commenting and
    reviewing.
    Should be included when paper draft is circulated to ATLAS.
    Highly recommended for all documents in the draft stage.
    In the future, the steering of whether the document is a draft or not will be done
    using the option \Option{atlasdraft}.
    \ADOCnew{04-03-00} If \Option{atlasdraft=true} or \Macro{AtlasVersion} is not empty,
    the document is declared as a draft.

  \item \Macro{AtlasJournal\{<Journal Name>\}} displays the phrase \emph{to
    be submitted to Journal Name} at the bottom of the front page and
    on the cover page.
    Should be included when a paper draft is circulated to ATLAS.

  \item \Macro{AtlasRefCode\{<Reference code>\}} displays the ATLAS
    standard reference code, e.g.\ \texttt{BPHY-2014-03}, on the front page and
    the cover page. Not shown on the front page if the note number is given.

  \item \Macro{AtlasNote\{<Note number>\}} displays the note number
    for a CONF, PUB, INT or COM note, e.g.\ \texttt{ATLAS-CONF-2014-23},
    on the front page and cover page.
    If the note number is given, the reference code is not shown.

  \item \Macro{PreprintIdNumber\{<CERN preprint number>\}} displays the CERN
    preprint number on the front page.
    
  \item \Macro{AtlasDate\{<Date>\}} set by the Physics Office as the date of submission of a paper.

  \item \Macro{AtlasJournalRef\{<Journal reference>\}} displays the journal reference
    on the preprint front page.
    This should be used for the arXiv update after the paper has been published.

  \item \Macro{AtlasDOI\{<Journal reference>\}} displays the DOI
    on the preprint front page.
    This should be used for the arXiv update after the paper has been published.

  \item \Macro{arXivId\{<arXiv identifier>\}} displays the arXiv reference
    on the front page.

\end{itemize}
%
\texttt{template/atlas-document.tex} contains a basic skeleton that can be
used to start typing a new note using the \texttt{atlasdoc} class. Many of
the custom commands described above are used in this example file, in
order to demonstrate their use.

Links to supporting documentation should also be included on the cover page of draft papers circulated to ATLAS.
They can be included using
\verb|\AtlasCoverSupportingNote{Short title}{CDS link}|.
It is also possible to give a TWiki page instead, but this is deprecated.\\
As mentioned above, see \texttt{template/atlas-document-metadata.tex} for more details.


%-------------------------------------------------------------------------------
\section{The \texttt{atlasdoc} class}
\label{app:atlasdoc}
%-------------------------------------------------------------------------------

This document has been typeset using the \texttt{atlasdoc.cls} class.

The \texttt{atlasdoc} class can use either the standard \LaTeX\ \texttt{article} class
as its basis or the \KOMAScript\ \texttt{sctartcl} class.
All the usual commands and options you usually use
with \texttt{article}  or \texttt{scrartcl} should work with it. 
You turn on the use of \KOMAScript\ with the option \texttt{koma}.
For instance, a standard document can be produced using this simple preamble:
%
\begin{tcblisting}{listing only}
  \RequirePackage{latex/atlaslatexpath}
  \documentclass[UKenglish]{atlasdoc}
  \usepackage{atlaspackage}
  \usepackage{atlasphysics}
  \graphicspath{{logos/}{figs/}}
\end{tcblisting}
%
Note that the document language must be specified, otherwise \texttt{babel} will complain.

The \LaTeX\ packages that are used in the document are mostly specified in 
\texttt{latex/atlaspackage.sty}.

The style file \texttt{latex/atlasphysics.sty} defines a lot of useful
macros for particles and more. See the separate document
\texttt{atlas\_physics.pdf}~\cite{atlas-physics} for details.

If you do not want to use \Package{biblatex} you need to add the option \Option{biblatex=false} when you
include \texttt{atlaspackage}.
Have a look at the \texttt{latex/atlaspackage.sty} to see how \texttt{biblatex} is included.
In your main document you use \Macro{addbibresource} in the preamble to include your \texttt{.bib} files.
Note that the backend \Package{biber} returns with an error if it finds an empty \texttt{.bib} file.
A style file \File{latex/atlasbiblatex.sty} is available that adjusts the format of the references to the usual ATLAS conventions.

As mentioned above, you have to specify the document language as an option to \Package{atlasdoc}.
Several more options can be set.
In the following the default option is in boldface.
\begin{description}
\item[\Option{atlasstyle=true|{\normalfont false}}] turn on (default) or off the use of the ATLAS style for the document;
\item[\Option{atlasdraft={\normalfont true}|false}] this is a draft version of the document;
\item[\Option{coverpage}] include an ATLAS draft cover page;
\item[\Option{cernpreprint}] make the front page for a CERN preprint.
  The option \Option{preprint} works as well, but is deprecated;
\item[\Option{NOTE}] the document is an ATLAS note (default);
\item[\Option{PAPER}] the document is an ATLAS paper (draft);
\item[\Option{CONF}] the document is a CONF note;
\item[\Option{PUB}] the document is an PUB note;
\item[\Option{BOOK}] the document is book form like an LOI or TDR;
\item[\Option{HEPDATA}] a separate document with detailed tables etc.\ for HEPData;
\item[\Option{texlive=2020}] adjust if you use an older version of \TeX\ Live like 2013.
  A value less than 2013 adjusts a few \Package{biblatex} options.
  A value less than 2012 uses \Package{txfonts}.
\item[\Option{paper=a4|{\normalfont letter}}] set the paper size;
\item[\Option{titlesize=normal|{\normalfont small}}] use normal or reduced size fonts for the title page;
\item[\Option{tocdepth=2}] depth of table of contents. The default is to include subsections (2);
\item[\Option{floatopt=true|{\normalfont false}}] adjust the options (default) governing number and placement of floats on a page;
\item[\Option{tableheading=true|{\normalfont false}}] adjust table caption spacing for captions above the table;
\item[\Option{mathlines=true|{\normalfont false}}] put line numbers on equations;
\item[\Option{linenofix=true|{\normalfont false}}] fix line numbers around AMS math environments with using the \Package{linenomath} environment;
\item[\Option{texmf}] use the syntax \Macro{usepackage\{package\}}
  instead of \Macro{usepackage\{latex/package\}} to include packages.
  \emph{\ADOCold{10.0.0} With the move to the \Package{atlaslatexpath} style file, this option is obsolete}.
\item[\Option{newtx}] use the \Package{newtxtext} and \Package{newtxmath} packages for fonts 
  (default for \TeX Live > 2012);
\item[\Option{txfonts}] use the \Package{txfonts} package for fonts instead of the default
  (default for older \TeX Live versions);
\item[\Option{abstract=true|\normalfont{false}}] the document contains an abstract.
  This option is only needed together with the \Option{BOOK} option,
  if the book does not have an abstract;
\item[\Option{atlaslogo=true|{\normalfont false}}] show the ATLAS logo on the title page;
\item[\Option{cernlogo=true|{\normalfont false}}] show the CERN logo on the title page;
\item[\Option{cmslogo={\normalfont true}|false}] include the CMS logo on the title page;
\item[\Option{extralogo=\normalfont{filename}}] include an extra logo on the title page;
\item[\Option{showframe={\normalfont true}|false}] load the \Package{showframe} package, to display frames showing the boxes for text body, header, footer and margin;
\item[\Option{shownote={\normalfont true}|false}] show the PUB note number.
  This is turned off by default for the final version of PUB notes.
  It does not affect other document types.
\item[\Option{mhchem={\normalfont true}|false}] include \Package{mhchem} before \Package{xpatch} to avoid
  an error with \TeX\ Live 2014.
  \emph{\ADOCold{07-00-00} This option has no effect};
\item[\Option{datetop=true|{\normalfont false}}] put the date at the top of the title page;
  \emph{\ADOCnew{07-00-00} No date is printed if this option is set to false};
\item[\Option{titleextraheight=0em}] extra height that could be needed for the title, if it is very long.
  \emph{\ADOCold{07-00-00} This option has no effect};
\item[\Option{copyrightoffset=0em}] adjust the position of the copyright, if it is not completely correct.
  \emph{\ADOCold{07-00-00} This option has no effect};
\end{description}

\ADOCnew{11.4.0} The option \Option{tableheading} leads to better spacing of table captions above a table (the ATLAS default).
With this option, and in general,you should use \Macro{centering}
and not \Macro{begin\{center\}}\ldots\Macro{end\{center\}} to centre tables and figures.
If you want to place a caption explicitly you can use
the macros \Macro{captionabove} and \Macro{captionbelow}.

\ADOCnew{04-03-00} It is intended to replace using the definition of \Macro{AtlasVersion} to decide if this a final version of a document.
In a later version the default value will be set to \Option{false},
so that this option simply has to be removed when a document is final.

\ADOCnew{13.3.0} The options \Option{cmslogo} and \Option{extralogo} have been added to allow
the CMS Collaboration logo, or another logo, to be added to the CERN preprint page next to the ATLAS logo.
The logos are included with the same height as the ATLAS logo.
The extra logo should probably be added to the \File{logos} directory.
Using the option \Option{cmslogo} implies that the author and the copyright will be changed automatically.
If you use the option \Option{extralogo}, do not forget to adjust \Macro{author} (and copyright) accordingly,
if the paper is published together with another collaboration.

The \Option{atlaslogo} and \Option{cernlogo} options are for cases where a paper has a limited set of authors
and so should not necessarily include these logos.
In this case you may want to tweak the \Package{hyperref} document information,
the title page and also the draft label using the following commands:
\begin{verbatim}
% Author and title for the PDF file
\hypersetup{pdftitle={Limited author document},pdfauthor={J.~Smith et al.}}
% Tweak the title page
\AtlasHeading{System Paper}
\AtlasDraftHeading{DRAFT}
\end{verbatim}

The following options were removed.
% They are mostly still available in \Package{atlasdoc1}.
\begin{description}
\item[maketitle={\normalfont true}|false] turn on or off the creation of a title page within \Macro{AtBeginDocument}.
  \ADOCold{02-00-00} If the option is false, but you still want a title, give the command \Macro{maketitle} after
  \verb|\begin{document}|.
  This is the recommended way of proceeding;
\item[nomaketitle]\mbox{}
  \ADOCold{01-07-00}  do not create a title page; equivalent to \Option{maketitle=false};
\item[koma=true|{\normalfont false}] use the \KOMAScript\ base class \Package{scrartcl} instead of \Package{article};
  \ADOCold{02-00-00} No longer an option.
\item[\Option{letterpaper}] set the paper size to letter.
  \ADOCold{07-00-00} This option does not work anymore
  --- use \Option{paper=letter} instead;
\item[\Option{a4paper}] set the paper size to A4;
  \ADOCold{07-00-00} This option does not work anymore
  --- use \Option{paper=a4} instead;
\item[\Option{letter}] set the paper size to letter.
  \ADOCold{02-00-00} This option does not work anymore
  --- use \Option{paper=letter} instead;
\end{description}
Note that the options \Option{CONF} and \Option{PUB} get passed to \Package{atlascover.sty}
as they only influence the cover pages.
%The option \Option{BOOK} uses book instead of article as the base class.

The
\href{http://www.tex.ac.uk/cgi-bin/texfaq2html?label=floats}{UK List of FAQ}
recommends changing several default \LaTeX\ options so that there are fewer problems
with figure and table placement.
It is certainly worth reading that page for further advice.
As it is very hard to really test how well these options work
they can be turned on or off in \Package{atlasdoc} via the option \Option{floatopt=true|false}.
The default value is set to \Option{true}.

\ADOCnew{02-00-00} \KOMAScript\ elements are used to create the title pages.
In particular, \Macro{publishers} is used for the abstract and copyright.
The space and position for this may need to be adjusted,
if you have a very long title. 
It is very helpful to turn on the \Option{showframe} option when doing such adjustments.
\ADOCold{07-00-00} Use the options
\Option{titleextraheight} and \Option{copyrightoffset} to make adjustments.


%-------------------------------------------------------------------------------
\subsection{Packages, dependencies and \Package{atlaspackage}}
\label{sec:atlaspackage}
%-------------------------------------------------------------------------------

The \Package{atlasdoc} class depends on these packages, whose presence in
your system is required:
\begin{itemize}\setlength{\parskip}{0pt}\setlength{\itemsep}{0pt}
\item \Package{babel}: become language aware;
\item \Package{scrlayer-scrpage}: defines the header for draft mode
  and for auxiliary material documents.
  For \TeX\ Live 2014 and earlier \Package{scrpage2} is used instead.
\item \Package{fontenc}: output font encoding;
\item \Package{hyperref}: add hyperlinks and ability to click on cross-references;
\item \Package{graphicx}: include graphics in the document;
\item \Package{lineno}: add line numbers to documents;
\item \Package{newtxtext} and \Package{newtxmath}: the standard ATLAS document font.
  If this is not available, you can fall back to \Package{txfonts};
\item \Package{xcolor}: add colours to \LaTeX;
\item \Package{ifthen}: improved handling of conditionals;
\item \Package{kvoptions}: process options passed to packages.
%\item \Package{scrdate, scrtime}: Current date and time for use in the header.
\end{itemize}
These should be installed in any modern \LaTeX\ installation.
See \cite{latex-faq} for details on which collections are needed to get these packages
for your operating system.

% Note that under Ubuntu versions 12.04 and 14.04, \Package{lineno} can be found in the
% \Package{texlive-humanities} package!
If you cannot find the \Package{lineno} package, it is also included in the \File{obsolete} directory.
Copy it to your main directory, or to \verb|${HOME}/texmf/tex/latex| in order to make
it centrally available.

Both the class \Package{atlasdoc} and all style files:
\Package{atlasbiblatex}, \Package{atlascontribute}, \Package{atlascover}, \Package{atlaspackage}, \Package{atlasphysics}
and \Package{atlastodo} need the package \Package{kvoptions} 
so that they can process options where a value for an option should be set.

\Package{atlasdoc} and \Package{atlascover} both need \texttt{hyperref}. 
Have a look at one of these packages to see how to include it by hand.
You can also simply use \texttt{atlaspackage.sty}

The style file \texttt{atlaspackage.sty} includes further packages.
You can steer how many by using the option \Option{minimal}, \Option{default} or \Option{full}.
The minimal set is:
\begin{itemize}\setlength{\parskip}{0pt}\setlength{\itemsep}{0pt}
\item \texttt{mathtools}: extra useful maths environments -- this includes \Package{amsmath} and some bug fixes;
\item \texttt{inputenc}: allow ä, ö, ø, ß, etc. to be input directly;
\item \texttt{hyperref}: add hyperlinks and ability to click on cross-references;
\item \texttt{placeins}: adds commands to force figure and table output before a certain position in the text.
\end{itemize}

The default set adds in addition:
\begin{itemize}\setlength{\parskip}{0pt}\setlength{\itemsep}{0pt}
\item \texttt{booktabs}: nicer tables. Use \Macro{toprule}, \Macro{midrule} and \Macro{bottomrule} instead of \Macro{hline};
\item \texttt{csquotes}: smart quotes that incorporate language dependence;
\item \texttt{siunitx}: units package with extra functionality for tables;
\item \texttt{subfig}: more than one plot in a figure;
% \item \texttt{tocloft}: extra options for typesetting table of contents etc.;
\item \texttt{cleveref}: automatically include \enquote{Fig.}, \enquote{Section} etc. when cross-referencing;
\item \texttt{bookmark}: better construction of index or outline in PDF viewers.
\end{itemize}

Finally the full set includes further packages that may be useful:
\begin{itemize}\setlength{\parskip}{0pt}\setlength{\itemsep}{0pt}
\item \texttt{mhchem}: chemical elements and molecules;
\item \texttt{diffcoeff}: mathematics for physics;
\item \texttt{rotating} rotate figures, tables, etc.;
\item \texttt{xfrac} nicer fractions;
\item \texttt{multirow} construction for table cells that span more than one row of the table.
\item \texttt{longtable} newer version of \Package{supertabular}, which allows tabular environments to go over more than one page.
  As an alternative you can include the use the option \Option{xtab} to use the \Package{xtab} package instead.
\end{itemize}
The above packages are all included if you turn on the full set.
You can turn them on individually if you use the minimal or standard set.
If you pass the \Option{xtab} option, it will be included instead of \Package{longtable}.
\ADOCold{12.0} If you are using an older \TeX\ Live version (earlier than 2016),
you will probably get an error when using the \Option{full} option,
as the \Package{diffcoeff} package was first released in 2016.
If this is the case, include the packages you want by passing the appropriate options to \Package{atlaspackage}.
\ADOCnew{12.1} \Package{diffcoeff} will not be included for \TeX\ Live versions older than 2016 (defined by the \Option{texlive} option).

The full list of options is:
\begin{description}\setlength{\parskip}{0pt}\setlength{\itemsep}{0pt}
\item[\Option{biblatex=true|{\normalfont false}}] turn on/off use of \Package{biblatex} and \Package{biber/bibtex};
\item[\Option{backend={\normalfont bibtex}|biber}] specify the backend to use with \Package{biblatex}.
  Specify \Option{backend=bibtex} to use \Package{bibtex} instead;
\item[\Option{hyperref=true|{\normalfont false}}] turn on/off use of the \Package{hyperref} package;
\item[\Option{bookmark=true|{\normalfont false}}] turn on/off use of the \Package{bookmark} package;
\item[\Option{siunitx=true|{\normalfont false}}] turn on/off use of the \Package{siunitx} package;
\item[\Option{eVkern={\normalfont true}|false}] apply a kern of -0.1em to \si{\eV} in order to move \enquote{e} and \enquote{V} closer together.
  This option is set by default if you use the \Option{txfonts} fonts;
\item[\Option{percentspace={\normalfont true}|false}] include or not the default space between a number and the \% sign;
\item[\Option{cleveref=true|{\normalfont false}}] turn on/off use of the \Package{cleverref} package;
\item[\Option{capsref=true|{\normalfont false}}] capitalise Section, Figure etc.\ when using \Package{cleverref};
\item[\Option{abbrevref=true|{\normalfont false}}] abbreviate Fig.\ etc.\ when using \Package{cleverref};
\item[\Option{mhchem={\normalfont true}|false}] turn on/off use of the \Package{mhchem} package;
\item[\Option{diffcoeff={\normalfont true}|false}] turn on/off use of the \Package{diffcoeff} package;
\item[\Option{physics={\normalfont true}|false}] turn on/off use of the \Package{physics} package;
\item[\Option{rotating={\normalfont true}|false}] turn on/off use of the \Package{rotating} package;
\item[\Option{xfrac={\normalfont true}|false}] turn on/off use of the \Package{xfrac} package;
\item[\Option{multirow={\normalfont true}|false}] turn on/off use of the \Package{multirow} package;
\item[\Option{longtable={\normalfont true}|false}] turn on/off use of the \Package{longtable} package;
\item[\Option{xtab={\normalfont true}|false}] turn on/off use of the \Package{xtab} package;
\item[\Option{subcaption={\normalfont true}|false}] use \Package{subcaption} instead of \Package{subfig};
  \Package{subcaption} is supposed to be a newer, better and more general package than \Package{subfig} or
  \Package{subfigure};
  % It is probably best to only use it with \TeX\ Live 2012 or later;
\item[\Option{subfigure={\normalfont true}|false}] use the deprecated package \Package{subfigure} 
  instead of \Package{subfig};
\item[\Option{subfig=true|{\normalfont false}}] use the somewhat deprecated package \Package{subfig};
\item[\Option{texlive=2020}] set if you use an older version of \TeX\ Live like 2013.
  % A value less than 2013 adjusts a few \Package{biblatex} options.
  % A value less than 2012 uses \Package{txfonts} and the old (Version 1) option names for \Package{siunitx}.
  % A value less than 2010 uses the old option names for \Package{csquotes}.
  Use \Option{texlive=2020} to test options for arXiv submissions;
\item[\Option{txfonts={\normalfont true}|false}] load the \Package{txfonts} package and adjust loading of \Package{mathtools/amsmath} for duplicate symbols;
\item[\Option{lineno=true|{\normalfont false}}] load the \Package{lineno} package.
\end{description}

\File{lineno.sty} and \File{authblk.sty} are also provided in \File{obsolete},
just in case they are not in your standard \LaTeX\ installation
and for some reason you cannot download them from CTAN (\url{https://ctan.org}).

Depending on the font you use, you may find that the \enquote{e} and \enquote{V} in \si{\eV}, \si{\MeV} etc.\
are too far apart.
You can pass the option \Option{eVkern} to \Package{atlaspackage} in order to move them 0.1em closer together.\footnote{%
This option has no effect for \TeX\ Live 2011 and older, as \Package{siunitx}
adjusted the spacing internally using the parameter \Option{eVcorra}.}
This is the amount used in the \File{atlasunit.sty} for \Macro{gev} etc.
which is included by passing the option \Option{unit=true} to \Package{atlasphysics}.
If you use \Package{siunitx}, I recommend setting \Option{unit=false},
so that you use one consistent set of definitions throughout your document.

The \Package{siunitx}~\cite{siunitx} package puts a (non-breaking) small space between a number and the \% sign,
as for any other unit.
It says that this is as required by the SI system of units~\cite{SI}.
In Section~5.4.7 of the brochure one can find:
\begin{quotation}
  The internationally recognized symbol \% (percent) may be used with the SI.
  When it is used, a space separates the number and the symbol \%.
  The symbol \% should be used rather than the name \enquote{percent}.
  In written text, however, the symbol \% generally takes the meaning of “parts per hundred”.
\end{quotation}
However, conventions between publishers appear to differ~\cite{percentspace}.
Many people are used to there being no space and this is also the ATLAS convention.
Pass the option \Option{percentspace=true} to include the space.
% This option only works for \TeX\ Live versions 2011 and later.

There used to be a problem using the \Package{tikz} package with \Package{atlasnote}.
With \Package{atlasdoc} this problem seems to have gone away.
\Package{tikz} is not included in \Package{atlaspackage}.
If you want to use it, just add the usual \verb|\usepackage{tikz}| to your preamble.

Other packages that have been used at some point include:
\begin{description}\setlength{\parskip}{0pt}\setlength{\itemsep}{0pt}
\item \Package{savesym}: needed to avoid errors if \Package{txfonts} is used, 
  as \Package{txfonts} and \Package{amsmath} define the same symbols;
\item \texttt{footmisc}: extra footnote options. 
  These mess up the \Option{atlasstyle} settings.
\end{description}


%-------------------------------------------------------------------------------
\subsection{Cover pages}
\label{sec:cover}
%-------------------------------------------------------------------------------

The package also provides cover pages for the circulations of ATLAS drafts and 
for the front page for the CERN preprint version of an ATLAS paper.
A further cover page is provided for a document containing detailed tables associated with a preprint/paper.
The style file can be found in \texttt{latex/atlascover.sty}.

If you wish to use the \texttt{atlascover} package with the 
\texttt{atlasdoc} class, you should usually use the \texttt{coverpage} option of the class:
\begin{verbatim}
  \documentclass[coverpage,UKenglish]{atlasdoc}
\end{verbatim}
instead of the the usual \texttt{usepackage} command: this will ensure
that the cover page is produced before the title page of the document.

\ADOCnew{01-07-00} You can include \texttt{atlascover} with \Macro{usepackage} if you prefer.
\ADOCold{01-07-00} You need the option \texttt{maketitle=false}
and you should include the \Macro{maketitle} command after \verb|\begin{document}|.

The following options can be passed on to the \Package{atlascover} package:
\begin{description}
\item[\Option{coverpage}] outputs the standard ATLAS paper draft cover page;
\item[\Option{CONF}] the document is a CONF note;
\item[\Option{PUB}] the document is an PUB note;
\item[\Option{LANGEDIT}] prints the language editor's name and email address;
% \item[\Option{cernpreprint}] the title page should be in the form of a CERN preprint;
%   The option \Option{preprint} works as well, but is deprecated;
%\item[\Option{preprint}] the title page should be in the form of a CERN preprint;
% \item[\Option{auxmat}] the title page for a document containing auxiliary material from a paper;
\item[\Option{coverfontsize}] the base font size used for the cover (default is 11pt). Adjust this for long abstracts;
\item[\Option{twocolumn}] use this option if your document is formatted in two columns;
\item[\Option{atlasdoc}] this option is set by \Package{atlasdoc} and is not usually needed by the user.
\end{description}

\ADOCnew{01-04-00} If you use \Package{atlascover} standalone, use the option \Option{coverpage=true} to
actually output a cover page. 
This makes the use of options more consistent.
\ADOCnew{02-00-00} The options \Option{cernpreprint}, \Option{preprint}
and \Option{auxmat} are no longer available in \Package{atlascover}.
You should pass these to \Package{atlasdoc} instead, as the title pages are now part of the main class.

Some papers have a very long abstract, such that it does not fit on the cover page.
You can reduce the font size used on the cover by setting the option \Option{coverfontsize}.
The default value is 11pt. Try 10.5pt or 10pt instead to get the abstract onto the page.

It used to be the case that some journal styles, especially JHEP,
produced an ATLAS draft cover page that was offset.
You could use the options \Option{hoffset} and \Option{voffset} to move the text around.\\
JHEP needed \verb|hoffset=1in, voffset=1in|.\\
revtex (APS journals) looked better with  \verb|hoffset=-0.25in, voffset=-0.25in|.\\
\ADOCnew{01-04-00} These offsets are ignored,
as the problems with spurious offsets have been eliminated.

The option \Option{clearpage}, which used to exist, has no effect.


%-------------------------------------------------------------------------------
\section{ATLAS preprint style}
\label{sec:atlasstyle}
%-------------------------------------------------------------------------------

This style should be used for the preparation of paper drafts,
as well as for the submission of papers to the arXiv and journals.
The journals will then convert the documents to the style appropriate for the journal.
% As some experience has to be gained with this package,
% feedback on any problems that occur with the style are very welcome.

Documents are typeset by default in the standard ATLAS preprint style.
The use of this style can be turned off by using the option
\Option{atlasstyle=false}.
This style uses \KOMAScript\ as the base class.
Further settings include:
\begin{description}
\item[Layout:] \Option{DIV=14} and an extra \SI{5}{\mm} for the binding;
\item[Paragraph:] the paragraph indentation is set to zero and 
  there is a half-line separation between paragraphs;
\item[Figures and tables:] a small font size is used for the captions.
  Captions are not indented.
  They should be below both figures and tables;
\item[Font:] the default fonts are from the \Package{newtx} package.
  These are very similar to \Package{txfonts} that have been used up to now,
  but have a better spacing in a few cases;
\item[Section headers:] the standard serif font is used.
\end{description}

The default fonts for ATLAS documents are \Package{newtxtext} and \Package{newtxmath}.
These are more modern variants of the package \Package{txfonts} that has been used in
ATLAS documents in the past.
%However, arXiv currently uses an older version of \TeX\ Live (2011) that does not include the
%\Package{newtx} fonts. 
%In ATLAS papers, please add the option \Option{texlive=2011} to \Package{atlasdoc}.
%As soon as arXiv switches to a newer version of \TeX\ Live this option may have to be adjusted
%or will no longer be necessary.

In general, if you have problems with the \Package{newtx} fonts,
you can switch to \Package{txfonts} by including the option \Option{txfonts} with \Package{atlasdoc}.


%-------------------------------------------------------------------------------
\section{CERN preprints and arXiv}
\label{sec:preprint}
%-------------------------------------------------------------------------------

If you are writing an ATLAS paper and it has been approved by the collaboration,
you have to make a version with the CERN preprint title page and prepare the 
paper for submission to arXiv.

If your paper draft is within the PO-GitLab project, the following steps will be
performed by the Physics Office using the GitLab Continuous Integration tools.
Before asking the Physics Office to do this,
you should check that your paper draft follows the ATLAS conventions.

In order to turn the paper into a CERN preprint,
you should replace the option \Option{PAPER} by \Option{cernpreprint} in \Package{atlasdoc}.
The CERN preprint number is given via the macro \Macro{PreprintIdNumber}.
At the same time you should pass the option \Option{texlive=2020} to
\Package{atlasdoc}.
This is because arXiv contains a 2020 \TeX\ Live installation.
Summarising, a typical \Macro{documentclass} command would be:
\begin{tcblisting}{listing only}
\pdfoutput=1
\RequirePackage{latex/atlaslatexpath}
\documentclass[cernpreprint, atlasdraft=false, texlive=2020, UKenglish]{atlasdoc}
\end{tcblisting}
The \Macro{pdfoutput} command tells arXiv that a PDF file should be produced directly.
You should also turn off ATLAS draft cover page --- remove the option \Option{coverpage=true}.
% If you move the class and style files to the same directory as the main file,
% you need to add the option \Option{texmf} to the \Macro{documentclass}.

If your paper should include the CMS logo, pass the option \Option{cmslogo} to \Package{atlasdoc}.
If your paper should include another logo next to the ATLAS logo,
pass the filename of the other logo to \Package{atlasdoc} using the \Option{extralogo} option.

You can test whether your document compiles with \TeX\ Live 2020 by setting your \texttt{PATH} on \texttt{lxplus} to
{\small
\begin{verbatim}
export PATH=/cvmfs/sft.cern.ch/lcg/external/texlive/2020/bin/x86_64-linux:${PATH}
\end{verbatim}
}

Note that you should submit the \File{bbl} file and not the \File{bib} to arXiv.
Depending on which journal you submit to, you should turn on or off the printing of the titles in the bibliography.
Further details on how to proceed can be found on the Physics Office TWiki~\cite{atlas-physicsoffice} --- see
the Section on \enquote{Guidelines for paper submission}.
APS journals have special requirements on the directory structure and the filenames for figures.
This is handled by the PO-GitLab tools.
%JINST uses a very old version of \LaTeX\ (2004).
% Neither \Package{biblatex} nor \Package{siunitx} are available
% and \KOMAScript\ does not contain the \Macro{KOMAoptions} command.
% See the Physics Office TWiki~\cite{atlas-physicsoffice} for more information.

It also makes sense to clean up the metadata file at this point.
You get rid of line numbering by making sure that neither \Macro{AtlasVersion} nor \Macro{draftversion} are defined.
I recommend moving the relevant definitions into the main \TeX\ file so that the metadata file is no longer needed.
If you clean things up, the \Package{atlascover} package is no longer needed.
The metadata commands that are needed in addition to the title, author and abstract are:
\begin{itemize}
  \item \Macro{AtlasJournal\{<Journal Name>\}}
  \item \Macro{PreprintIdNumber\{<CERN preprint number>\}}
  \item \Macro{AtlasDate\{<Date>\}} set by the Physics Office
  \item \Macro{AtlasJournalRef\{<Journal reference>\}} once it exists
  \item \Macro{AtlasDOI\{<Journal reference>\}} once it exists
  \item \Macro{arXivId\{<arXiv identifier>\}} once it exists
\end{itemize}

More details on arXiv recommendations can be found at
\url{https://arxiv.org/help/submit_tex}.


%-------------------------------------------------------------------------------
\section{ATLAS TDR and LOI documents}
\label{sec:book}
%-------------------------------------------------------------------------------

If you include the option \Option{BOOK}, \Package{atlasdoc} uses the \Package{scrbook}
as the document class.
This option is geared to long documents such as TDRs and LOIs.
Such a document has various numbers which can be set as follows:
\begin{itemize}\setlength{\parskip}{0pt}\setlength{\itemsep}{0pt}
  \item \Macro{AtlasRefCode}: ATLAS reference code, e.g.\ ATLAS-TDR-099.
  \item \Macro{PreprintIdCode}: LHCC reference code, e.g.\ CERN-LHCC-2017-099.
  \item \Macro{AtlasDate}: Official date of the document.
\end{itemize}
The title will be typeset flushleft, rather than the usual centering.
A typical title would be:
\begin{verbatim}
  \AtlasTitle{Technical Design Report\\
  for the ATLAS Detector Upgrade}
\end{verbatim}

If you want to add images to the front and back covers,
the template contains commented out commands that allow you to do this.
The \Package{pdfpages} package seems to work very well for such things.
The images can be in \texttt{pdf}, \texttt{png} or \texttt{jpg} format.
Unlike \Macro{includegraphics} you should include the filename extension.

Note that the title page will only be correctly formatted if you use 
\TeX\ Live 2013 or newer. If you are using an older version add \Macro{flushleft}
to \Macro{AtlasTitle}.

%-------------------------------------------------------------------------------
\section{ATLAS notes}
\label{sec:note}
%-------------------------------------------------------------------------------

If you include the macro \Macro{AtlasNote} in your preamble,
the note number will be printed under \enquote{ATLAS NOTE} at the top of your document.
This can be used for any sort of ATLAS note, including CONF, PUB and INT notes.


%-------------------------------------------------------------------------------
\section{Auxiliary and HEPData material}
\label{sec:auxmat}
%-------------------------------------------------------------------------------

Many papers have extra plots and tables that should be made public,
but are not submitted to arXiv and the journal.
These should be collected in a file \File{mydocument-auxmat.tex},
which is included in the draft document during its circulation within ATLAS,
This is transparent for editors if they use use PO-GitLab system,
but has to be done manually for other papers.

Some papers have many pages of extra tables and plots that are mainly of use to theorists
who need extra information.
Such material should usually included in the paper draft until it is ready for
submission to arXiv and to the journal.
The default name for the file containing the information is \File{mydocument-hepdata.tex}.
At the submission stage it should be moved into a separate document.
A skeleton document created using the command \verb|make newdata BASENAME=...|.
The front page for this document is formatted using the \Option{HEPDATA} option.
If you use this option you should specify the arXiv preprint identifier
using the macro \Macro{arXivId} and the HEPData record using the macro
\Macro{HepDataRecord}.
This information is then included on the cover page in the form of clickable links.

Use of this option also adds the arXiv preprint identifier to the top
of every page of the document.

If you want to create an HEPData document with an older \TeX\ Live version such as 2013, 
use the command \texttt{make newdata TEXLIVE=2013}.


%-------------------------------------------------------------------------------
\section{Symbols in \texttt{atlasphysics.sty}}
\label{sec:atlasphysics}
%-------------------------------------------------------------------------------

Many useful symbols are defined in \texttt{atlasphysics.sty}.
While this used to be a very long file, it has now been split into several smaller files,
which can be included or not using options.
The definitions can be found in a separate document \File{atlas\_physics.pdf}.


%-------------------------------------------------------------------------------
\section{Snippets and templates for standard text}
\label{sec:atlassnippets}
%-------------------------------------------------------------------------------

The Publication Committee provides standard texts giving examples
for the description of the ATLAS detector, and the appropriate references,
as well as other text snippets that may be useful to avoid too much use of ATLAS jargon.
For example, the ATLAS detector description can be found in \File{template/atlas-detector.tex}

You can find some text snippets that can be used in papers in \File{latex/atlassnippets.sty}.
To use them, provide the \Option{snippets} option to \Package{atlasphysics}.
Text snippets can also be found on the web pages~\cite{pubcom-snippet}.
Comments and/or suggestions on improvements are very welcome and
should be given to the Publication Committee.

In addition, CP and analysis groups have started providing templates for supporting (INT) notes.
These are included in a subdirectory of the \File{template} directory.
For now (2018-10-29) there are some templates from the EXOT group.


%-------------------------------------------------------------------------------
\section{Adding notes}
\label{sec:todo}
%-------------------------------------------------------------------------------

When writing a paper, you or others often want to add notes so that things are not forgotten.

The \Package{atlastodo} package provides a macro \Macro{ATLnote} that can be used to define notes with separate colours for each author.
This macro uses the \Package{todonotes} package,
which is also used for language editor comments.
For example:
\begin{tcblisting}{listing only}
\ATLnote{JS}{Jane}{magenta!20}{magenta}
\end{tcblisting}
adds macros \Macro{JSnote} and \Macro{JSinote} for notes in the margin and inline.
Note that you must use the inline variant for notes inside captions and other floating objects.
Turn off the output of any notes by passing the option \Option{output=false}
to the \Package{atlastodo} package.

The following options can be passed on to the \Package{atlastodo} package:
\begin{description}
\item[\Option{output}\OptionTFT] turn off the output of any notes;
\item[\Option{shift}\OptionTFT] adjust the margin to allow more space for notes;
\item[\Option{version=2\textbar\normalfont{1}}] version number.
\end{description}

If you want a list of all the notes,
add \Macro{listoftodos} somewhere in your document.
The \Package{todonotes} package also include a macro \Macro{missingfigure}
that is very useful if you want to include a figure, but do not yet have the plot.

The following code produces the paragraph below.
\begin{tcblisting}{listing only}
Here is an \JSnote[example paragraph]{Illustration of macro}
that shows how to use the macro. If you want a comment
without it being associated with text omit the optional argument.
\JSnote{This is a comment without associated text.}
This is some fill text between the comments.
\JSnote[Text to be improved.]{This is a comment with assoicated text.}
If you prefer your comments to be inline use the \Macro{JSinote} macro.
\JSinote{Here is an inline comment.}
\end{tcblisting}
Here is an \JSnote[example paragraph]{Illustration of macro}
that shows how to use the macro. If you want a comment
without it being associated with text omit the optional argument.
\JSnote{This is a comment without associated text.}
This is some fill text between the comments.
\JSnote[Text to be improved.]{This is a comment with assoicated text.}
If you prefer your comments to be inline use the \Macro{JSinote} macro.
\JSinote{Here is an inline comment.}

\ADOCold{12.0} Version 1 of \Package{atlastodo} had two argument:
the first for the text to be commented on and the second for the comment.
\ADOCnew{13.0} Version 2 of \Package{atlastodo} has one option argument
for the text to be commented on and a required one for the comment.

As mentioned above, notes in captions and other floating objects must be inline.
If you include a note in a caption,
you should also provide a short caption that does not include the note.
If you do not you will get errors in the list of figures and/or tables.
Here is an example with a short caption:
\begin{tcblisting}{listing only}
\caption[A nice plot.]{A nice plot. \IBinote{This need to be improved.}}
\end{tcblisting}

%-------------------------------------------------------------------------------
\section{Language editor commands}%
\label{sec:langedit}
%-------------------------------------------------------------------------------

The \Package{todonotes} has been used to add a few macros that should be of use
for language editors. The commands are in the \Package{atlascomment} style file.
This file is included if the \Option{LANGEDIT} is passed to \Package{atlasdoc}.
The commands added are:
\begin{description}
  \item[\Macro{LEecomment}] adds a comment about a change, or suggested change.
\end{description}
The commands takes two arguments: the relevant text and the explanation/suggestion.

Such comments are probably also useful for paper editors.
Have a look at this style file and the \Package{todonotes} documentation on how
you can set up your own macros.


%-------------------------------------------------------------------------------
\section{Scripts}%
\label{sec:script}
%-------------------------------------------------------------------------------

Four scripts are provided in the \File{scripts} directory to help updating existing documents:
\begin{description}
  \item[\File{atlaslatex\_update.sh}] Script to update the \Package{atlaslatex} version
    to the latest master version in Git.
  \item[\File{atlaslatex\_2020.sh}] Script to update the \Package{atlaslatex} version
    to be compatible with the 2020 version of TeX Live and \LaTeX.
  \item[\File{atlaslatex\_selfupdate.sh}] Script to update the scripts themselves.
  \item[\File{tex\_dollars.py}] Script to change from use of \TeX\ primitive \verb|$...$|
    to the \LaTeX\ macro \verb|\(...\)|.
\end{description}
Have a look at the scripts for the available options.


%-------------------------------------------------------------------------------
\section{Miscellaneous \LaTeX{} tips}%
\label{sec:latex}
%-------------------------------------------------------------------------------

%-------------------------------------------------------------------------------
\subsection{Line numbers}

Line numbers can be printed using the \Package{lineno} package, 
which is included by default.
Line numbers are automatically turned on if you set \Macro{AtlasVersion} (or \Macro{draftversion})
or you pass the option \Option{atlasdraft=true} to \Package{atlasdoc}.
In general, you can turn them on and off in a document by using the \Macro{linenumbers} or \Macro{nolinenumbers} commands.
Note that if \Macro{AtlasVersion} or option \Option{atlasdraft=true} are set,
you will always get line numbers on the standard title page.
Hence, for papers, CONF and PUB notes it is important to comment out \Macro{AtlasVersion} in order to suppress the line numbers for the final version.

In order to avoid line numbers going slightly wrong around figures and tables,
separate the \Package{figure} and \Package{table} environment from the rest of the text using blank lines.

\ADOCnew{08-04-00} Line numbering around AMS Math \LaTeX\ environments such as \Package{align}
should just work.
The code that does this is inside \File{atlasdoc.cls}.
If this causes problems, pass the option \Option{linenofix=false} to \Package{atlasdoc}.
You can set the option \Option{mathlines=false} to turn off numbering the lines in equations.
% Some debugging of this option is still ongoing, so it is currently set to \Option{false}.

For older versions of \Package{atlaslatex},
if you use AMS Math \LaTeX\ environments line numbering may be interrupted around the environment.
Enclose the environment in a \Package{linenomath} environment to fix this problem:
\begin{tcblisting}{listing only}
\begin{linenomath}
\begin{equation*}
  E = m c^{2}
\end{equation*}
\end{linenomath}
\end{tcblisting}
If you are using the environment \Package{linenomath} you may have to set the option \Option{mathlines=false}to avoid spurious line numbers.


%-------------------------------------------------------------------------------
\subsection{Definitions}

You can use \verb|\ensuremath| in definitions, so that they will work
in both text mode and math mode, e.g.\
\verb|\newcommand{\UoneS}{\ensuremath{\Upsilon(\text{1S})}\xspace}| to get
\UoneS in either mode (\verb|\UoneS{}| or \verb|$\UoneS$|).

I highly recommend that you also terminate every definition with \Macro{xspace},
as then you can use the definitions without having to terminate them with
\enquote{\textbackslash\textvisiblespace} or \enquote{\{\}}.


%-------------------------------------------------------------------------------
\subsection{Figures}

Use the \Package{graphicx} package to include your plots and figures. 
The use of older packages like \Package{espfig} is deprecated.
Since the \Package{graphicx} package is required by the \Package{atlasdoc}
class, it is automatically loaded when using it, and there is no need
to explicitly include it in the document preamble.

Always include your graphics file without giving the file extension.
For instance, if you want to include the \File{figure.eps}
file, you should use a syntax like this:
\begin{verbatim}
  \includegraphics[width=\textwidth]{figure}
\end{verbatim}
This will allow you to compile your document using either \LaTeX{} or
pdf\LaTeX{} without changing your source file: you can in fact have
both \File{figure.eps} and \File{figure.pdf} in your working directory,
and the proper one will be picked up according to the processing method
you choose.

Figures should be in general be made available in either \texttt{eps} (or \texttt{pdf}) format.
\texttt{png} format can be used for event displays.
However, ATLAS papers should only include \texttt{pdf} figures (and \texttt{png}).
This also implies that pdf\LaTeX{} should be used for compilation.
% Additionally, a \texttt{pdf} version of the plots can be
% useful in case \verb|pdflatex| is used to produce a publication.
%Colour versions are appropriate for talks, and black-and-white
%versions are necessary for the publication itself.

It is a good habit to keep your graphics files in a separate
sub-directory (e.g.\ in \File{figures/}. 
In this case you can include them by mentioning it explicitly every time:
\begin{verbatim}
  \includegraphics[width=\textwidth]{figures/figure}
\end{verbatim}
or by telling the \Package{graphicx} package where to look
for them, by using this command:
\begin{verbatim}
  \graphicspath{{figures/}}
\end{verbatim}

If you use a modern version of \TeX\ Live, it creates PDF files automatically from EPS files
(if they do not exist) when you use \File{pdflatex}.
An EPS file with the name \File{picture1.eps} will lead to a PDF file with the name
\File{picture1-eps-converted-to.pdf}.
If you have a lot of figures in many different directories, you may want to clean up the PDF files every so often.
You can use the command \verb|make cleanepstopdf| to achieve this.
You should adjust the top-level figures directory in the \File{Makefile} accordingly.


%-------------------------------------------------------------------------------
\subsection{Subfigures}

An example figure can be seen in Figure~\ref{fig:example}.
The standard options to use for the positioning are \Option{htbp}.
If you get a couple of lines of text at the top of the page,
make sure the figure is separated from the rest of the text with blank lines and/or try dropping the \Option{h} option.

\begin{figure}[htbp]
  \centering
  \includegraphics[width=0.5\columnwidth]{AtlasExample}
  \caption{An example ATLAS figure.}
  \label{fig:example}
\end{figure}

A figure with subfigures can be made as shown in the example of
Figure~\ref{fig:subfigexample}. In this example the \Package{subfig} package is used.
The syntax with the \Package{subcaption} and \Package{subfigure} packages is very similar.
The following commands were used to produce Figure~\ref{fig:subfigexample}:
{\footnotesize
\begin{verbatim}
\begin{figure}[htbp]
  \centering
  \subfloat[One subfigure example]{
    \includegraphics[width=0.45\textwidth]{AtlasExample}
    \label{fig:SubfigureExample1}
  }
  \subfloat[Another subfigure example]{
    \includegraphics[width= 0.45\textwidth]{AtlasExample}
    \label{fig:SubfigureExample2}
  }
  \caption{Subfigure example.
    \protect\subref{fig:SubfigureExample1} shows the cross-section as a function of $E_{\text{T,jet}}$ and 
    \protect\subref{fig:SubfigureExample2} shows exactly the same thing!}
  \label{fig:subfigexample}
\end{figure}
\end{verbatim}
}

You refer to the main figure using the usual \verb|\ref| command, e.g.\ see \Fig{\ref{fig:subfigexample}}.
You can refer to the subfigures using either the syntax \verb|\ref{fig:subfiglabel}| 
(e.g.\ see \Fig{\ref{fig:SubfigureExample2}}) or\\
\verb|\ref{fig:mainfiglabel}\subref{fig:subfiglabel}|
(e.g.\ see \Fig{\ref{fig:subfigexample}\subref{fig:SubfigureExample1}}).
Note that if you use the \Package{subfig} package and want to use the labels of the subfigures in the caption,
you have to use the syntax \verb|\protect\subref{fig:SubfigureExample1}|.
The packages \Package{subfigure} and \Package{subcaption} do not need protect, but it does not do any harm.

\begin{figure}[htbp]
  \centering
  \subfloat[One subfigure example.]{
    \includegraphics[width=0.45\textwidth]{AtlasExample}
    \label{fig:SubfigureExample1}
  }
  \subfloat[Another subfigure example.]{
    \includegraphics[width= 0.45\textwidth]{AtlasExample}
    \label{fig:SubfigureExample2}
  }
  \caption{Subfigure example.
    \protect\subref{fig:SubfigureExample1} shows the cross-section as a function of $E_{\text{T,jet}}$ and 
    \protect\subref{fig:SubfigureExample2} shows exactly the same thing!}
  \label{fig:subfigexample}
\end{figure}


%-------------------------------------------------------------------------------
\subsection{Positions of figures and tables}

In an ATLAS paper, all figures and tables should be printed before the conclusions.
You can achieve this by using the macro \Macro{FloatBarrier} from the
\Package{placeins} package.

In general, as mentioned above, you should separate the figure and table environments from the text by blank lines.
This helps the line numbers. The standard options to use for the placement are \Option{[htbp]}.


%-------------------------------------------------------------------------------
\subsection{Math mode macros}%
\label{sec:math}
%-------------------------------------------------------------------------------

The correct \LaTeX\ macros for math mode are \textbackslash(\ldots\textbackslash)
and not \(\$\ldots\$\) (which are \TeX\ primitives),
even though the \TeX\ primitives are used by most people.
\ADOCnew{06-00-00} The standard ATLAS bibliography and template files use the correct \LaTeX\ macros and
the documentation, example files will also be adjusted to use them.

If you are using a version of \LaTeX\ from before 2015, you may have problems
if you use the \LaTeX\ delimiters in captions and want to make as list of tables or figures.
If this is the case, just switch to \TeX\ primitives in the caption (or subcaption).


%-------------------------------------------------------------------------------
\subsection{\pT or \ET, that is the question}

Bold math should be automatically invoked in titles.
This short section tests whether that works properly.
It is of course good if things like \pT and \ET are automatically in bold face in
a header and normal font in the text (and table of contents).

With the current setup, this works OK. 
However, if you just use the option \Option{koma}, which then typesets titles using a sans serif font,
the $p$ and $E$ are typeset with a serif font and \textsf{T} is typeset with a sans serif font,
which is probably not what one wants!
Work is still ongoing to find the optimal set of options
--- search for \texttt{detect} in the \Package{siunitx} manual, to see the complete set of possibilities.
This is not a problem for the ATLAS preprint style as it uses a serif font for the section titles.


%------------------------------------------------------------------------------
\section{Recommended packages}

A vast number of \LaTeX\ packages are available.
In this section I collect a few useful packages that I recommend using.

\begin{description}
  \item[cleveref] Means that constructs like \verb|Fig.~\ref{fig:one}| or
  \verb|\Fig{\ref{fig:one}}| are no longer necessary.
  Instead just use \verb|\cref{fig:one}|.
  The package decides if it is a figure, table or equation and
  adds the appropriate text.
  At the beginning of sentences use \Macro{Cref}.
  This package is included by default if you use \Package{atlaspackage}.
  You can customise its use with the \Option{capsref} and \Option{abbrevref} options.
  If you include the package yourself, use \Macro{usepackage\{cleveref\}} to get \enquote{fig.} etc. and
  use \Macro{usepackage[capitalize]\{cleveref\}} to get \enquote{Fig.} etc.

  \item[heppennames] A package that defines most elementary particle, mesons and baryons in a
  consistent way. Optionally the symbols can be upright or italic.
  The package is included if you pass the option \Option{hepparticle} to \Package{atlasphysics}.
  You can use the package \Package{hepnicenames} instead, which uses more intuitive names for the particles,
  but is not as systematic.

  \item[diffcoeff] A useful package for differentials.
  \ADOCnew{12.0.0} The package is included if you pass the option \Option{full} to \Package{atlaspackage}.
  If the document language is set to \Option{USenglish},
  a slanted \textit{d} is used in differentials,
  while an upright \textrm{d} is used for other languages.
  I recommend \Macro{dl2x} to get a nice spacing for the differential in an integral,\\
  % diffcoeff tweaks for older TeX Live versions.
  \ifthenelse{\AtlasTeXLiveVersion < 2018}{%
    \emph{Examples are not complete as \Package{diffcoeff} package not available for older versions of TeX Live.\\}}{}
  e.g.\ \verb|\int f(x) \dl2x| gives 
  \ifthenelse{\AtlasTeXLiveVersion < 2018}{XXX, while}{\(\int f(x) \dl2x\), while}\\
  \verb|\int f(x) \dl0x| or \verb|\int f(x) \dl x| gives  
  \ifthenelse{\AtlasTeXLiveVersion < 2018}{XXX.}{\(\int f(x) \dl0x\).}
    
  Alternatives are \Package{esdiff} and \Package{derivative},
  but the \Package{derivative} is probably too new to be used in papers.
  You can use a package such as \Package{braket} for Dirac notation etc.

  The package \Package{physics} can also be used for differentials, matrices and more.
  As the name suggests it is geared to physics usage.
  However, the \LaTeX\ community is not very enthusiastic about the way the package is written.
  
  The \Package{commath} package is another alternative,
  but I find the \Package{physics} package to be more reliable when different fonts are used.

  \item[todonotes] Very nice package for adding notes.
  It is used by the \File{atlastodo.sty} style file.
  See \File{atlascomment.sty} for a further example.
\end{description}


%------------------------------------------------------------------------------
\subsection{Other (useful) packages}

In this section I collect a few useful packages that may be useful when preparing a document.
Note that I have only had a cursory read of their documentation,
so some work amy be needed to get them working as they are supposed to.
\begin{description}
  \item[snapshot] As the first paragraph of the documentation quotes:
    \begin{quotation}
      The \Package{snapshot} package helps the owner of a \LaTeX\ document obtain a list of the external dependencies of the document,
      in a form that can be embedded at the top of the document.
      To put it another way, it provides a snapshot of the current processing context of the document,
      insofar as it can be determined from inside \LaTeX.
  \end{quotation}
  It can also be used to arrange that the document is processed with the same versions of everything.
  I tried the package once, and it gave an error compiling.
  However, even if the compilation gives and error
  you can look at the resulting \File{.dep} file to get a list of all packages and versions used in a document.
  This may be helpful for debugging problems.

  \item[changes] The \Package{changes} package is another way of recording changes and adding comments.
    The \Package{todonotes} package is used to do some of this and is integrated into the \Package{atlastodo} style file.
    The \Package{changes} is supposed to work much like change markup in LibreOffice, Microsoft Office etc.
\end{description}


%-------------------------------------------------------------------------------
\section{Remarks on units and symbols}%
\label{sec:siunitx}
%-------------------------------------------------------------------------------

It is highly recommended to use a units package to format your units properly.
The package \Package{siunitx} works very well and is the package of choice.
Alternatives include \Package{units} and \Package{hepunits},
which is based on \Package{SIunits}.

The basic command to use in \Package{siunitx} is \verb|\SI{20}{\GeV}| to get
\SI{20}{\GeV}. 
There are also several other useful commands for specifying ranges:
\verb|\numrange| for a range of numbers and \verb|SIrange| for a range of numbers with a unit. 
Options exist for specifying how they are formatted.
The options can be set for an individual command or for the whole document.
For example, in this document I have specified the options:\\
\verb|\sisetup{separate-uncertainty, range-units=single, list=units=single}|
and\\
\verb|\sisetup{group-digits=integer, group-minimum-digits=4, detect-all}|.

In addition several extra units are defined:
\begin{itemize}
\item \verb|\micron| for \si{\micron};
\item \verb|\mrad| for \si{\mrad};
\item \verb|\nb| for \si{\nb};
\item \verb|\pb| for \si{\pb};
\item \verb|\fb| for \si{\fb}.
\end{itemize}
Use the syntax \verb|\SI{20.3}{\per\fb}| to get \SI{20.3}{\per\fb}.

Some things to note about using \Package{siunitx}:
\begin{itemize}
\item It tries to isolate itself from other packages.
  If you just want to write \si{\GeV} in your text,
  then you must write \verb|\si{\GeV}|.
\item It also contains two new column specifiers for tables ``S'' and ``s'',
  which are extremely useful for formatting tables properly.
\end{itemize}

% The option names are somewhat different for \TeX\ Live 2009,
% as this contained \Package{siunitx} Version 1.
% You can use the older options by including \Package{atlaspackage} with the 
% option \Option{texlive=2009}.
% You also have to turn off the inclusion of \File{atlasunits.sty} by including the option \Option{units=false} with
% the \Package{atlasphysics} package.


%-------------------------------------------------------------------------------
\section{\texttt{atlaslatex} directories and Git}
\label{sec:gitsvn}
%-------------------------------------------------------------------------------

There is some flexibility in how you set up your directory structure for using \Package{atlaslatex}.
By default the \Package{atlaslatex} style files are in the \File{latex} subdirectory and the
logos are in \File{logos}. This structure assumes that you will make a separate directory tree
for each document that you create.
If you want to include these files in Git or SVN, note that you only need to add the
\File{latex}, \File{logos} and \File{bib} directories of the \Package{atlaslatex} package to Git.
In order to create a new document, you also need the \File{template} directory.
For a paper, you also need the \File{acknowledgements} directory.

If you want use a centrally installed \Package{atlaslatex} package, then you would usually unpack the\\
\File{atlaslatex-X.Y.Z.tds.zip} file into your \File{texmf} tree --- see \cref{sec:texmf}.

If you want to use another setup, you should adjust the directory in \File{latex/atlaslatexpath.sty} appropriately.
This would enable you to maintain a single copy of each \Package{atlaslatex} version and easily switch between versions.
For example, you specify:
\verb|\def\input@path{{../atlaslatex-10.0.0/latex/}}|
in \File{latex/atlaslatexpath.sty}
to use version 10.0.0 of the \Package{atlaslatex} package, which you have unpacked into the directory tree
\File{../atlaslatex-10.0.0}.
Such a structure makes it very easy to switch between \Package{atlaslatex} versions without breaking anything!

% If you want to use another setup, you should set the variable \Macro{ATLASLATEXPATH} appropriately
% at the beginning of your document. This would enable you to maintain a single copy of each 
% \Package{atlaslatex} version and easily switch between versions.
% For example, you give the command\\
% \verb|\newcommand*{\ATLASLATEXPATH}{../atlaslatex-01-08-00/}|
% to use version 01-08-00 of the \Package{atlaslatex} package, which you have unpacked into the directory tree
% \File{../atlaslatex-01-08-00}.
% Such a structure makes it very easy to switch between \Package{atlaslatex} versions without breaking anything!


%-------------------------------------------------------------------------------
\section{Platforms and \LaTeX\ versions}
\label{sec:version}
%-------------------------------------------------------------------------------

The \Package{atlasdoc} class should in principle work both with \LaTeX{} and pdf\LaTeX{}.
However, the collection is no longer tested with \LaTeX,
so I strongly recommend to use pdf\LaTeX, which is the default.

I would expect everything to work with \TeX\ Live 2013 or later.
You should just set the option \Option{texlive} appropriately.
This is best done in the document class, as the option is then passed to all other packages.
Examples of changes include some option names for \Package{siunitx}.

% If for example you have \TeX\ Live 2013, add the option \Option{texlive=2013} to the document class.
% This will then include \Package{siunitx} with the correct options for Version 1.
% It will also switch to \Option{unit=false} to \Package{atlasphysics}
% and use option \Option{txfonts} in \Package{atlasdoc}.

\ADOCnew{04-00-00} If you use the \Package{biblatex} package,
the default is to use the \texttt{biber} backend.
% For \TeX\ Live versions earlier than 2013, it may be better to use \texttt{bibtex}.
% To do this, pass the option \Option{backend=bibtex} to \Package{atlaspackage}.

The \Package{atlaslatex} package should work under Linux, macOS and Windows.
Details on the installations that I use for testing things
and how you should set up your system can be found on the PubCom LaTEX FAQ~\cite{latex-faq}.


%-------------------------------------------------------------------------------
\section{Installation of \Package{atlaslatex} in \File{texmf} tree}%
\label{sec:texmf}
%-------------------------------------------------------------------------------

As discussed above, the \texttt{atlasdoc} class and the style files can all be found in the 
\File{latex} subdirectory. The template documents are usually set up to pick up the style files from there.
If you want to use the centrally installed version,
you should first copy \File{Makefile}, the \File{template} directory and the \File{bib} directory from 
\File{\$\{HOME\}/texmf/source/atlaslatex} to the directory where you want to create your document.
For the main document, you can then use the command 
\texttt{make newpapertexmf}, \texttt{make newnotetexmf} or \texttt{make newbooktemmf} to get a template which uses the
centrally installed style files.

If you want to install the package in a central area, use the \File{atlaslatex-X.Y.Z.tds.zip} file.
Change your directory to \File{\$\{HOME\}/texmf} and unzip the file there.
% To do it by hand you can do:
% \begin{itemize}
% \item unpack the tarball;
% \item copy the \texttt{latex} directory to \File{\$\{HOME\}/texmf/tex/latex/atlaslatex};
% \item copy the contents of the \File{bib} directories 
%   to \texttt{\$\{HOME\}/texmf/bib}.
% \end{itemize}
% It is more complicated to checkout part of a Git repository.
% Hence the method described above is the recommended way of installing
% \Package{atlaslatex} in your \File{texmf} tree.
% You can also checkout the two directory trees from SVN:
% {\small
% \begin{verbatim}
% cd ~/texmf/tex/latex
% svn co svn+ssh://svn.cern.ch/reps/atlasgroups/pubcom/latex/atlaslatex/trunk/latex atlaslatex
% cd ~/texmf
% svn co svn+ssh://svn.cern.ch/reps/atlasgroups/pubcom/latex/atlaslatex/trunk/bibtex
% \end{verbatim}
% }
% The advantage of using SVN is that you can keep the package up to date, by just giving the command
% \verb|svn update| in the two directories.
% If you already have a \File{bibtex} directory,
% first move it out of the way, then checkout from SVN
% and then move the contents of the old directory back into the \File{bibtex} tree.

% Under Windows, it appears to be better to use \texttt{https} instead of \texttt{svn+ssh}.
% You should therefore checkout:\\
% \verb|https://svn.cern.ch/reps/atlasgroups/pubcom/latex/atlaslatex/trunk|

In the template files, you have to use the command
\texttt{make newpapertexmf} or \texttt{make newnotetexmf} or simply comment out the line
\verb|\RequirePackage{latex/atlaslatexpath}|
% \begin{center}
%   \begin{tabular}{ll}
%     From & To \\
%     \midrule
%     \verb|\newcommand*{\ATLASLATEXPATH}{latex/}|    & \verb|\newcommand*{\ATLASLATEXPATH}{}| \\
%   \end{tabular}
% \end{center}

If you are using traditional \BibTeX\ you also have to change\\
\verb|\bibliographystyle{bib/bst/atlasBibStyleWoTitle}| to\\
\verb|\bibliographystyle{atlasBibStyleWoTitle}|

The \Option{texmf} option in \Package{atlasphysics} is not strictly necessary if you use the class \Package{atlasdoc},
but it does not do any harm.


\appendix
\clearpage
%-------------------------------------------------------------------------------
\section{Makefile}
%-------------------------------------------------------------------------------
\label{sec:makefile}

This section documents what the \File{Makefile} does when it creates a new document
or compiles one.

When a new paper draft is created using the command\\
\texttt{make newpaper BASENAME=GROUP-YYYY-XX-PAPER}\\
the following files are created in the main directory.
If a template filename is given in the table
it is taken from the \texttt{template} directory,
otherwise empty files are created.
\begin{center}
  \begin{tabular}{ll}
    \mcc{\texttt{template}} & \mcc{\texttt{main}} \\
    \midrule
    \texttt{atlas-paper.tex} & \texttt{GROUP-YYYY-XX-PAPER.tex} \\
    \texttt{atlas-paper-metadata.tex} & \texttt{GROUP-YYYY-XX-PAPER-metadata.tex} \\
    \texttt{atlas-auxmat.tex} & \texttt{GROUP-YYYY-XX-PAPER-auxmat.tex} \\
    \texttt{atlas-hepdata.tex} & \texttt{GROUP-YYYY-XX-PAPER-hepdata.tex} \\
    & \texttt{GROUP-YYYY-XX-PAPER-defs.sty} \\
    & \texttt{GROUP-YYYY-XX-PAPER.bib}
  \end{tabular}
\end{center}
The following string substitutions are made in \texttt{GROUP-YYYY-XX-PAPER.tex}:
\begin{center}
  \begin{tabular}{ll}
    \mcc{Old string} & \mcc{New string} \\
    \midrule
    \texttt{atlas-document} & \texttt{GROUP-YYYY-XX-PAPER} \\
    \texttt{texlive=2020} & \texttt{texlive=YYYY} \\
  \end{tabular}
\end{center}
The \TeX\ Live version is changed to \texttt{YYYY} (if given). Otherwise it is set to 2020.

The same thing is done for an ATLAS supporting note made with the command\\
\texttt{make newnote BASENAME=GROUP-YYYY-XX-INT1},\\
except that the main file template is taken from
\texttt{atlas-note.tex},
the metadata template is taken from \texttt{atlas-note-metadata.tex},
and the auxiliary material and HEPData files are not created.

The standard sequence of commands to compile a document is
\texttt{pdflatex, biber, pdflatex, pdflatex}.
You can change the \texttt{\%.pdf} target if necessary.
Better is to use \texttt{latexmk} via the target \texttt{run\_latexmk}.
I recommend you set this as the default command.

%-------------------------------------------------------------------------------
\section{Journal templates}
%-------------------------------------------------------------------------------
\label{sec:journal}

This section contains some information on where the \LaTeX\ templates for the different journals can be found and how to use them.
With the advent of the ATLAS preprint style and its use for ATLAS publications, 
it should no longer be necessary to format papers in the style used by the journals.
However, for papers that are written by a limited number of authors
the journal may require that the paper be submitted using its style.

The directory \File{journal} contains a very basic paper outline with the preamble needed for different journals.
So far the \Package{atlaslatex} package has been tested with the classes for Elsevier and APS journals and the style file used for JHEP and JINST.
The journal templates turn off the use of \Package{biblatex}
by adding the option \Option{biblatex=false} to \Package{atlaspackage}.
I have not tested if it is possible to use \Package{biblatex}.

\begin{description}
\item[Elsevier]Elsevier uses the \texttt{elsarticle} class which should be already installed if you have a standard 
  \TeX\ Live distribution. 
  It can also be found at \url{http://www.elsevier.com/locate/latex}.
  
\item[APS]APS journals use REV\TeX. This is also usually installed.
  It can also be found at \url{https://journals.aps.org/revtex}.
  Note that you have to specify the author after \verb|\begin{document}| with this class.
  Hence you should comment out the definition in your metadata file,\\
  e.g.\ \File{mydocument-metadata.tex}.
  If you want line numbers in a document typeset using REV\TeX, it is best to use the class option \Option{linenumbers}.
  In addition you should include \Package{atlaspackage} with the option \Option{lineno=false}.
  
\item[JHEP]The package can be downloaded from \url{http://jhep.sissa.it/jhep/help/JHEP_TeXclass.jsp}.
  It contains a style file \File{jheppub.sty} as well as a \BibTeX\ style file \File{JHEP.bst}. 
  If the author of the paper is not the the ATLAS Collaboration,
  you should use the macros \Macro{author} and \Macro{affiliation} to specify the names and their instiutions (see the documentation)
  and should NOT include the \Package{authblk} package.

\item[JINST]The package can be downloaded from \url{https://jinst.sissa.it/jinst/help/helpLoader.jsp?pgType=author}.
  It contains a style file \File{jinstpub.sty} as well as a \BibTeX\ style file \File{JHEP.bst}.
  The information on authors is the same as for JHEP.
\end{description}


%-------------------------------------------------------------------------------
\section{From \texttt{atlasnote} to \texttt{atlasdoc}}
\label{sec:oldnote}
%-------------------------------------------------------------------------------

The \texttt{atlasdoc} class replaces and supersedes \texttt{atlasnote}.
The decision was taken to give the class a new name, as it is supposed to be
able to be used for (almost) all ATLAS documents.
Some small changes in the user setup are necessary to use the new
class, style files and templates.

All style files are collected in the \texttt{latex} subdirectory.
It is assumed that this directory is a direct subdirectory of you main \LaTeX\ file.
If you want to keep the style files in a central place you can either put them in
\verb|${HOME}/texmf/tex/latex| or create a link from your main directory to the location of
your \texttt{latex} directory.

The main changes the user has to make are:
\begin{itemize}
\item Change the class name from \texttt{atlasnote} to \texttt{latex/atlasdoc};
\item Specify the document language as an option: UKenglish or USenglish;
\item Add \verb|\usepackage{latex/atlaspackage}| at the beginning of the document;
\item Change \verb|\usepackage{atlasphysics}| to \verb|\usepackage{latex/atlasphysics}|; 
\item Use the macro \Macro{AtlasTitle} instead of \Macro{title}.
\end{itemize}

The language specification means that dates etc.\ are also formatted according to 
the document language. 
If you use the package \Macro{csquotes}, quotation symbols are also consistently and properly set
when you use \Macro{enquote}.

All the documentation uses \texttt{biblatex} and \texttt{biber} instead of traditional \BibTeX.
The templates provide information on how to make the change in your own document.
The default document settings also use \texttt{biblatex} and \texttt{biber}.

\ADOCnew{01-00-00} The same macro names are used in both \Package{atlasdoc} and
\Package{atlascover} so that title, journal, version number and abstract only need to be specified once.
This means that if you start from an old preamble the following changes should be made:
\begin{center}
  \begin{tabular}{ll}
    Old	& New\\
    \midrule
    \Macro{title} & \Macro{AtlasTitle}\\
    \Macro{draftversion} & \Macro{AtlasVersion}\\
    \Macro{atlasnote} & \Macro{AtlasNote}\\
    \Macro{journal} & \Macro{AtlasJournal}\\
    \Macro{abstracttext} & \Macro{AtlasAbstract}
  \end{tabular}
\end{center}
If you use the old macro names 
\Macro{draftversion}, \Macro{journal}, \Macro{abstracttext},
they will continue to work in the document itself, but not on the cover page.

When you want to circulate a draft with cover pages, 
you also need to set the macro \Macro{AtlasRefCode}.
This replaces \Macro{AtlasCoverNumber} as it is used in several places.

The class and style files have been cleaned up and things 
that were thought to no longer be necessary have been removed.
% These pieces have been collected in \texttt{obsolete/atlasnote-obsolete.sty} in case they are needed.
% If something important has got lost, please let me know.

The \Package{subfigure} package has been replaced with \Package{subfig}, as \Package{subfigure} is now deprecated.
If you use \Package{subfig}, then you have to use \Macro{subfloat} instead of \Macro{subfigure}.
If you want to continue to use \Package{subfigure} include \Package{atlaspackage} with the option
\Option{subfigure=true}. 
You should also comment out the \Macro{usepackage\{subfigure\}}.

Similarly, if you do not want to include \Package{siunitx} set
the option \Option{siunitx=false}.

The option \verb|\skipbeforetitle{<length>}| used to set the distance between
the title page header and the note title. 
Given that stretchable space is now used, such an option is no longer appropriate.
It can be given, but will be ignored.
%The default value should be fine for most notes, but in case you have a long list of
%authors or a lengthy abstract you can use this command to buy
%some extra space. Note that \verb|<length>| can also be negative
%(use it at your own risk!).

%-------------------------------------------------------------------------------
\section{History}
%-------------------------------------------------------------------------------

Quite a lot of people have contributed to the ATLAS \LaTeX\ templates over time.
Marco Delmastro set them up in the first place and added a number of improvements over time.
Mike Vetterli implemented several changes to the cover pages, including switching to two pages.
Cristina Oropeza, Vasia Mitsou, Chris Hays and Mike Vetterli all made contributions to the preprint cover page.

Sven Menke provided the code so that bold math works in titles correctly.
Thorsten Kuhl had the idea of defining \Macro{ATLASLATEXPATH}, which makes things much more flexible.
Some problems occurred with this scheme \TeX{} Live 2020.
As a result the use of \Macro{ATLASLATEXPATH} was replaced with the \File{atlaslatexpath.sty} style file.

Juan Pedro Araque has done most of the work setting up the PO-GitLab project.
This resulted in a much smoother submission process for papers and
an improved handling of auxiliary material.

Knut Zoch provided the code that fixed the line numbering problems with AMS Math \LaTeX\ environments.


%-------------------------------------------------------------------------------
\subsection{Changes in \texttt{atlaslatex-10.0.0}}
\label{sec:atlaslatex10}
%-------------------------------------------------------------------------------

\ADOCnew{10.0.0} switches to Semantic Versioning.

The major change in this version is in the way that the class and style files are included.
This had to be changed as the result of a bug introduced in the October 2020 update of \LaTeX.
The \LaTeX{} update led to options being ignored when passed to a document class or a style file,
if the filename contained a directory.
While this bug will probably be fixed at some point,
it in general appears to be better to adjust the macro \Macro{input@path}
to specify the directory that should be searched for the ATLAS \LaTeX{} packages.
Hence a new style file \File{atlaslatexpath.sty} has been introduced and should be loaded using
\begin{tcblisting}{listing only}
\RequirePackage{latex/atlaslatexpath}
\end{tcblisting}
before the \Macro{documentclass}.

This change implies that all main files have to be updated.
A script \File{scripts/atlaslatex\_2020.sh} is provided that should make the necessary changes.


%-------------------------------------------------------------------------------
\subsection{Changes in \texttt{atlaslatex-05-00-00}}
\label{sec:atlaslatex5}
%-------------------------------------------------------------------------------

\ADOCnew{05-00-00} is the first version set up
to be fully compatible with the PO-GitLab scheme for papers.

Separate (dummy) files for auxiliary material and HEPData tables are created for new papers.
The \verb|make auxmat| command has been renamed to \verb|make newdata|,
as the auxiliary material for the webpage is now separated
from a separate file for tables etc.\ for HEPData.


%-------------------------------------------------------------------------------
\subsection{Changes in \texttt{atlaslatex-04-00-00}}
\label{sec:atlaslatex4}
%-------------------------------------------------------------------------------

\ADOCnew{04-00-00} The \File{Makefile} for \Package{atlaslatex}
has been restructured to reduce duplications and make separate commands for a new paper and a new note.
\texttt{biber} is now the default backend for \Package{biblatex},
as this allows the use of the \enquote{related} field for Errata.
Errata are included in the ATLAS bibliography file.
Metadata for notes and papers are now separate templates to prepare for them being created directly from Glance.
This is the first version that is designed for the Glance/Git integration.
As the above changes are quite major, there is a jump in the main version number.


%-------------------------------------------------------------------------------
\subsection{Changes in \texttt{atlaslatex-02-00-00}}
\label{sec:atlaslatex2}
%-------------------------------------------------------------------------------

\ADOCnew{02-00-00} Only the \KOMAScript\ classes are supported.
At the same time, the option BOOK was introduced, which uses \Package{scrbook} as the base class.
This is more suitable for long documents such as a TDR.

Several options, which make maintenance more difficult have been removed:
\Option{maketitle}, \Option{nomaketitle}, \Option{koma}.
In addition, support for \TeX\ Live versions older than 2009 has been removed.
% A version of the class with these options, which should still work with \TeX\ Live 2007,
% but without the \Option{BOOK} option is available as \File{atlasdoc1.cls}.
% However, the class (\Package{atlasdoc1}) will not be actively maintained or developed any more.
% If you want to explicitly load the \Package{atlascover} package,
% you should load \Package{atlascover1} when using \Package{atlasdoc1}.

The options \Option{cernpreprint}, \Option{preprint} and \Option{auxmat} are no longer available
in \Package{atlascover}.
You should pass these to \Package{atlasdoc} instead, as the title pages are now part of the main class.


%-------------------------------------------------------------------------------
\subsection{Changes in \texttt{atlascover-01-00-00}}
\label{sec:oldcover}
%-------------------------------------------------------------------------------

\ADOCnew{01-00-00} The same macro names are used in both \Package{atlasdoc} and
\Package{atlascover} so that title, journal and version number only need to be specified once.
This means that if you start from an old cover page the following changes have to be made:
\begin{center}
  \begin{tabular}{ll}
    Old                            & New                   \\
    \midrule
    \Macro{AtlasCoverPaperTitle}   & \Macro{AtlasTitle}    \\
    \Macro{AtlasCoverNumber}       & \Macro{AtlasRefCode}  \\
    \Macro{AtlasCoverPaperVersion} & \Macro{AtlasVersion}  \\
    \Macro{AtlasCoverJournal}      & \Macro{AtlasJournal}  \\
    \Macro{AtlasCoverAbstract}     & \Macro{AtlasAbstract}
  \end{tabular}
\end{center}

Note that \Package{atlaspreprint} is integrated into \Package{atlascover} and not maintained as a separate style file.
To get the CERN preprint front page, you have to include the option \Option{cernpreprint} when you invoke \Package{atlasdoc}.
If you start from an old preprint front page the following changes have to be made:
\begin{center}
  \begin{tabular}{ll}
    Old                              & New                   \\
    \midrule
    \Macro{PreprintCoverPaperTitle} & \Macro{AtlasTitle}    \\
    \Macro{PreprintJournalName}     & \Macro{AtlasJournal}  \\
    \Macro{PreprintCoverAbstract}   & \Macro{AtlasAbstract}
  \end{tabular}
\end{center}
The following changes are needed for the macros:
\begin{itemize}
\item The macro \Macro{AtlasCoverEdBoardMember} only has one argument, as a generic email list now exists for every EdBoard.
\end{itemize}


==> bib/doc/atlas_physics/Makefile <==
#------------------------------------------------------------------------------
# Makefile to make atlas_physics documentation
#------------------------------------------------------------------------------

BASENAME1 = atlas_physics
BASENAME2 = atlas_hepphysics
TEXLIVE = 2020

.PHONY: clean cleanpdf

atlas_physics:
	make -f ../Makefile run_latexmk BASENAME=$(BASENAME1)

atlas_hepphysics:
	if [ $(TEXLIVE) -ge 2013 ]; then \
		make -f ../Makefile BASENAME=$(BASENAME2); \
	fi

texlive:
	make -f ../Makefile texlive BASENAME=$(BASENAME1) TEXLIVE=$(TEXLIVE)
	make -f ../Makefile texlive BASENAME=$(BASENAME2) TEXLIVE=$(TEXLIVE)

clean:
	make -f ../Makefile clean

cleanpdf:
	-rm $(BASENAME1).pdf
	-rm $(BASENAME2).pdf

cleanall: clean cleanpdf


==> bib/doc/atlas_physics/atlas_physics_body.tex <==
%-------------------------------------------------------------------------------
\section{\File{atlasphysics.sty} style file}
\label{sec:atlasphysics}
%-------------------------------------------------------------------------------

The \File{atlasphysics.sty} style file implements a series of useful
shortcuts to typeset a physics paper, such as particle
symbols.

Options are parsed with the \Package{kvoptions} package, which is included by default.
The style file can included in the preamble of your paper with the usual
syntax:
%
\begin{tcblisting}{listing only}
\usepackage{atlasphysics}
\end{tcblisting}
%
The file is actually split into smaller files,
which can be included or not using options.
The following options are available, where the default setting is given in parentheses:
\begin{description}
\item[BSM](false) BSM and SUSY particles.
\item[hion](false) Useful macros for heavy ion physics.
\item[jetetmiss](false) Useful macros for Jet/Etmiss publications.
\item[journal](true) Journal abbreviations and a few other definitions for references.
\item[math](false) A few extra maths definitions.
\item[misc](true) Miscellaneous definitions that are often used.
\item[other](false) Definitions that used to be in \File{atlasphysics.sty},
  but are probably too specialised to be needed by most people.
\item[particle](true) Standard Model particles and some combinations.
\item[hepparticle](false) Standard Model particles and some combinations using the \Package{hepparticle} package.
  This option will supersede \Option{particle} at some time.
\item[process](false) Some example processes.
  These are not included by default as the current choice is rather arbitrary
  and certainly not complete.
\item[hepprocess](false) Some example processes using the \Package{hepparticle} package.
  These are not included by default as the current choice is rather arbitrary
  and certainly not complete.
  This option will supersede \Option{process} at some time.
\item[unit](true) Units that used to be defined -- not needed if you use \Package{siunitx} or \Package{hepunits}.
\item[xref](true) Useful abbreviations for cross-references.
\item[texlive=YYYY](2020) Set if you use an older version of \TeX\ Live like 2013.
\item[texmf](true) Use the syntax \Macro{usepackage\{package\}}
  instead of \Macro{usepackage\{\textbackslash ATLASLATEXPATH package\}} to include packages.
  This is needed if you install \Package{atlaslatex} centrally,
  rather than in a \File{latex} subdirectory.
\end{description}
Note that \Option{BSM} and \Option{BSM=true} are equivalent.
Use the syntax \Option{option=false} to turn off an option.
\ADOCnew{10.0.0} \Macro{ATLASLATEXPATH} is no longer used,
so the option \Option{texmf} has been set to \Option{true}.

If the  option \Option{texmf} is included, the subfiles are included using the command:
\verb|\RequirePackage{atlasparticle}| etc. instead of \verb|\RequirePackage{\ATLASLATEXPATH atlasparticle}|.
\ADOCnew{10.0.0} This is now the default option.

All definitions are done in a consistent way using \verb|\newcommand*|.
All definitions use \verb|\ensuremath| where appropriate and are terminated with
\verb|\xspace|, so you can simply write {\verb|\ttbar production| instead of
\verb|\ttbar\ production| or \verb|\ttbar{} production| to get \enquote{\ttbar production}.

The \Package{hepparticles}~\cite{hepparticles} package has uniform definitions for many Standard Model and BSM particles.
In fact you should use the package \Package{heppennames} and/or \Package{hepnicenames},
which contain many predefined particles.
These packages load \Package{hepparticles}, which can then be used to define more particles if you need them.
One very nice feature of these packages is that you can switch between italic and upright symbols via an option.

See \cref{sec:old}} for details on changes that were introduced when
when going from version 00-04-05 of \Package{atlasnote}
to version 01-00-00 of \Package{atlaslatex}.
Let me know if you spot some other changes that are not documented here!

Changes to the contents that might affect existing documents are given in \cref{sec:change}.

The following sections list the macros defined in the various files.


==> bib/doc/atlas_physics/atlas_physics_changes.tex <==
\onecolumn
%-------------------------------------------------------------------------------
\section{Changes}
\label{sec:change}
%-------------------------------------------------------------------------------

\textbf{Version 05-08-00} of \Package{atlaslatex} includes a new \File{atlassnippets.sty} style file.
This is supposed to contain snippets of text that are useful in many papers and/or notes.

\textbf{Version 01-08-01} of \Package{atlaslatex} includes quite a few definitions from the Jet/Etmiss group.
A new style file has been created \File{atlasjetetmiss.sty} that is not included by default.
Some of the definitions from the Jet/ETmiss group are of more general use and so have been merged into existing style files:
\begin{description}
\item[atlasmisc.sty] List of Monte Carlo generators expanded:
  \Macro{POWHEGBOX}, \Macro{POWPYTHIA}.
  Add MC macros with suffix \enquote{V} for version number.
  \Macro{kt}, \Macro{antikt}, \Macro{Antikt}, \Macro{LO}, \Macro{NLO}, \Macro{NLL}, \Macro{NNLO},
  \Macro{muF}, \Macro{muR}.
  Added macros \Macro{Runone}, \Macro{Runtwo}, \Macro{Runthr},
  Added \Macro{radlength} and \Macro{StoB}.
  Added some standard \(b\)-tagging terms:
  \Macro{btag}, \Macro{btagged}, \Macro{bquark}, \Macro{bquarks}, \Macro{bjet}, \Macro{bjets}.
\item[atlasparticle.sty] Now includes \Macro{pp}, \Macro{enu}, \Macro{munu},
\item[atlasprocess.sty] Added \Macro{Zbb}, \Macro{Ztt},
  \Macro{Zlplm}, \Macro{Zepem}, \Macro{Zmpmm}, \Macro{Ztptm},
  \Macro{tWb}, \Macro{Wqqbar},
  \Macro{Wlnu}, \Macro{Wenu}, \Macro{Wmunu},
  \Macro{Wjets}, \Macro{Zjets}.
  The definition of \Macro{Hllll} was corrected.
\item[atlasheavyion.sty] \Macro{pp} moved to \File{atlasparticle.sty}.
\end{description}

This version also introduced the (optional) use of the \Package{heppennames} package.
The style files \File{atlashepparticle.sty} and \File{atlashepprocess.sty}
are intended to replace \File{atlasparticle.sty} and \File{atlasprocess.sty}.
Several particle definitions were removed from the \Package{atlasparticle} package,
as they just enable a few Greek letters: \(\pi\), \(\eta\) and \(\psi\) to be used directly in text mode.
In addition, the primed \(\Upsilon\) resonances, e.g.\ \(\Upsilon''\),
as well as \(D^{**}\) were removed.
as the official names are \Ups{3} etc.,

The definitions of \MeV, \GeV\ etc.\ in \texttt{atlasunit.sty} were updated in order to remove the \texttt{if} tests in them.
The \texttt{if} tests caused a problem in a paper draft, although the reason was not understood.
The new definitions do not introduce extra space before the unit in math mode.


%-------------------------------------------------------------------------------
\section{Old macros}
\label{sec:old}
%-------------------------------------------------------------------------------

With the introduction of \Package{atlaslatex} several macro names have been changed to make them more consistent.
A few have been removed. The changes include:
\begin{itemize}
\item Kaons now have a capital \enquote{K} in the macro name, e.g.\ \verb|\Kplus| for \Kplus;
\item \verb|\Ztau|, \verb|\Wtau|, \verb|\Htau| \verb|\Atau| have been replaced by
  \verb|\Ztautau|, \verb|\Wtautau|, \verb|\Htautau| \verb|\Atautau|;
\item \verb|\Ups| replaces \verb|\ups|;
  the use of \verb|\ups| to produce \(\Upsilon\) in text mode has been removed;
\item \verb|\cm| has been removed, as it was the only length unit defined for text and math mode;
\item \verb|\mass| has been removed, as \verb|\twomass| can do the same thing and the name is more intuitive;
\item \verb|\mA| has been removed as it conflicts with \Package{siunitx} Version 1, which uses the name
  for milliamp.
\item \Macro{mathcal} rather than \Macro{mathscr} is recommended for luminosity and aplanarity.
\end{itemize}

Quite a few macros are more related to \Zboson physics than they are to LHC physics and have
been moved to the \File{atlasother.sty} file, which is not included by default.
There are also macros for various decay processes, \File{atlasprocess.sty} which are not included by default,
but may be useful for how you can define your favourite process.

It used to be the case that you had to use \verb|\MET{}| rather than just \verb|\MET| to get the spacing right,
as somehow \Package{xspace} did not do a good job for \met.
However, with the latest version of the packages both forms work fine.
You can compare \MET and \MET\ and see that the spacing is correct in both cases.


==> bib/doc/atlas_physics/atlas_physics_defs.tex <==
% Files with references in BibTeX format and biblatex style options
\addbibresource{../../bib/ATLAS.bib}
\addbibresource{atlas_physics.bib}

\graphicspath{{../../logos/}}

% Useful macros for documentation
% \newcommand{\File}[1]{\texttt{#1}\xspace}
% \newcommand{\Macro}[1]{\texttt{\textbackslash #1}\xspace}
% \newcommand{\Option}[1]{\textsf{#1}\xspace}
% \newcommand{\Package}[1]{\texttt{#1}\xspace}

%-------------------------------------------------------------------------------
% Generic document information
%-------------------------------------------------------------------------------
% Set author and title for the PDF file
\hypersetup{pdftitle={ATLAS LaTeX guide},pdfauthor={Ian Brock}}

\AtlasTitle{Symbols defined in \File{atlasphysics.sty}}

\author{Ian C. Brock}
\affil{University of Bonn}

\AtlasAbstract{%
  This note lists the symbols defined in \File{atlasphysics.sty}.
  These provide examples of how to define your own symbols, as well as many symbols
  that are often used in ATLAS documents.

  This document was generated using version \ATPackageVersion\ of the ATLAS \LaTeX\ package.
  The \TeX\ Live version is set to \AtlasTeXLiveVersion.
  It uses the option \Option{atlasstyle}, which implies that the standard ATLAS preprint style is used.
  The language is set to \languagename.
}


==> bib/doc/atlas_physics/atlas_physics_list1.tex <==
\newpage
%-------------------------------------------------------------------------------
\section{\File{atlasjournal.sty}}

Turn on including these definitions with the option \Option{journal=true} and off with the option \Option{journal=false}.

\input{atlasjournal}


\newpage
%-------------------------------------------------------------------------------
\section{\File{atlasmisc.sty}}

Turn on including these definitions with the option \Option{misc=true} and off with the option \Option{misc=false}.

\input{atlasmisc}

\noindent A length \Macro{figwidth} is defined that is \SI{2}{\cm} smaller than \Macro{textwidth}.

\noindent Monte Carlo generators and PDFs have an optional argument
that allows you to include the version, e.g.\
\verb|\PYTHIA[8]| to produce \PYTHIA[8] or\\
\verb|\PYTHIA[(v8.160)]| to produce \PYTHIA[(v8.160)].

\noindent A macro \Macro{pTX} is included that allows you to add an extra subscript and/or a superscript to \pT.
e.g.\\
\verb|\pTX| to produce \pTX;\\
\verb|\pTX[2]| to produce \pTX[2];\\
\verb|\pTX[][\text{had}]| to produce \pTX[][\text{had}];\\
\verb|\pTX[3][\text{had}]| to produce \pTX[3][\text{had}].

\noindent A generic macro \verb|\twomass| is defined, so that for example
\verb|\twomass{\mu}{\mu}| produces \twomass{\mu}{\mu} and \verb|\twomass{\mu}{e}| produces \twomass{\mu}{e}.

A macro \verb|\dk| is also defined which makes it easier to write down decay chains.
For example
\begin{verbatim}
\[\eqalign{a \to & b+c\\
   & \dk & e+f \\
   && \dk g+h}
\]
\end{verbatim}
produces
\[\eqalign{a \to & b+c\cr
   & \dk & e+f \cr
   && \dk g+h}
\]
Note that \Macro{eqalign} is also redefined in this package so that \Macro{dk} works.

The following macro names have been changed:\\
\verb|\ptsq| \(\to\) \verb|\pTsq|.


\newpage
%-------------------------------------------------------------------------------
\section{\File{atlasxref.sty}}

Turn on including these definitions with the option \Option{xref=true} and off with the option \Option{xref=false}.

\input{atlasxref}

\noindent The following macros with arguments are also defined:
\begin{xtabular}{ll}
\verb|\App{1}|  & \App{1}\\
\verb|\Eqn{1}|  & \Eqn{1}\\
\verb|\Fig{1}|  & \Fig{1}\\
\verb|\Refn{1}|  & \Refn{1}\\
\verb|\Sect{1}| & \Sect{1}\\
\verb|\Tab{1}|  & \Tab{1}\\
\verb|\Apps{1}{4}| & \Apps{1}{4} \\
\verb|\Eqns{1}{4}| & \Eqns{1}{4} \\
\verb|\Figs{1}{4}| & \Figs{1}{4} \\
\verb|\Refns{1}{4}| & \Refns{1}{4} \\
\verb|\Sects{1}{4}| & \Sects{1}{4} \\
\verb|\Tabs{1}{4}| & \Tabs{1}{4} \\
\verb|\Apprange{1}{4}| & \Apprange{1}{4} \\
\verb|\Eqnrange{1}{4}| & \Eqnrange{1}{4} \\
\verb|\Figrange{1}{4}| & \Figrange{1}{4} \\
\verb|\Refrange{1}{4}| & \Refrange{1}{4} \\
\verb|\Sectrange{1}{4}| & \Sectrange{1}{4} \\
\verb|\Tabrange{1}{4}| & \Tabrange{1}{4}
\end{xtabular}

The idea is that you can adapt these definitions according to your own preferences (or those of a journal).
Note that the macros \Macro{Ref} and \Macro{Refs} were renamed to \Macro{Refn} and \Macro{Refns}
in \Package{atlaslatex} 08-00-00, as \Macro{Ref} is now defined in the \Package{hyperref} package.


\newpage
%-------------------------------------------------------------------------------
\section{\File{atlasbsm.sty}}

Turn on including these definitions with the option \Option{BSM} and off with the option \Option{BSM=false}.

The macro \Macro{susy} simply puts a tilde (\(\tilde{\ }\)) over its argument,
e.g.\ \verb|\susy{q}| produces \susy{q}.

For \susy{q}, \susy{t}, \susy{b}, \slepton, \sel, \smu and
\stau, L and R states are defined; for stop, sbottom and stau also the
light (1) and heavy (2) states.
There are four neutralinos and two charginos defined,
the index number unfortunately needs to be written out completely.
For the charginos the last letter(s) indicate(s) the charge:
\enquote{p} for \(+\), \enquote{m} for \(-\), and \enquote{pm} for \(\pm\).

\input{atlasbsm}


\newpage
%-------------------------------------------------------------------------------
\section{\File{atlasheavyion.sty}}

Turn on including these definitions with the option \Option{hion=true} and off with the option \Option{hion=false}.
The heavy ion definitions use the package \Package{mhchem} to help with the formatting of chemical elements.
This package is included by \File{atlasheavyion.sty}.

\input{atlasheavyion}

%The following symbols were removed or modified with respect to the original submission
%\input{atlasheavyion-mod}


\newpage
%-------------------------------------------------------------------------------
\section{\File{atlasjetetmiss.sty}}

Turn on including these definitions with the option \Option{jetetmiss=true} and off with the option \Option{jetetmiss=false}.

\input{atlasjetetmiss}

\noindent The macro \Macro{etaRange} produces what you would expect:
\verb|\etaRange{-2.5}{+2.5}| produces \etaRange{-2.5}{+2.5} while
\verb|\AetaRange{1.0}| produces \AetaRange{1.0}.
The macro \Macro{avg} can be used for average values:
\verb|\avg{\mu}| produces \avg{\mu}.


\newpage
%-------------------------------------------------------------------------------
\section{\File{atlasmath.sty}}

Turn on including these definitions with the option \Option{math=true} and off with the option \Option{math=false}.

\input{atlasmath}

\noindent The macro \Macro{spinor} is also defined.
\verb|\spinor{u}| produces \spinor{u}.


\newpage
%-------------------------------------------------------------------------------
\section{\File{atlasother.sty}}

Turn on including these definitions with the option \Option{other} and off with the option \Option{other=false}.

\input{atlasother}


==> bib/doc/atlas_physics/atlas_physics_list2.tex <==
\newpage
\onecolumn
%-------------------------------------------------------------------------------
\section{\File{atlassnippets.sty}}

Turn on including these definitions with the option \Option{snippets} and off with the option \Option{snippets=false}.

\input{atlassnippets}
\twocolumn


\newpage
%-------------------------------------------------------------------------------
\section{\File{atlasunit.sty}}

Turn on including these definitions with the option \Option{unit} and off with the option \Option{unit=false}.

\input{atlasunit}

\noindent Lower case versions of the units also exist, e.g.\ \verb|\tev|, \verb|\gev|, \verb|\mev|, \verb|\kev|, and
\verb|\ev|.

As mentioned above, it is highly recommended to use a units package instead of
these definitions. \Package{siunitx} is the preferred package; a good alternative is \Package{hepunits}.
If either of these packages are used \File{atlasunit.sty} is not needed.

Most units that are needed in ATLAS documents are already defined by \Package{siunitx} or
are defined in \File{atlaspackage.sty}.
A selection of them is given below.
In order to use them in your document the unit should be included in
\verb|\si| or \verb|\SI|:\\
\begin{xtabular}{ll}
\verb|\si{\TeV}| & \si{\TeV} \\
\verb|\si{\GeV}| & \si{\GeV} \\
\verb|\si{\MeV}| & \si{\MeV} \\
\verb|\si{\keV}| & \si{\keV} \\
\verb|\si{\eV}|  & \si{\eV} \\
\verb|\si{\TeVc}| & \si{\TeVc} \\
\verb|\si{\GeVc}| & \si{\GeVc} \\
\verb|\si{\MeVc}| & \si{\MeVc} \\
\verb|\si{\keVc}| & \si{\keVc} \\
\verb|\si{\eVc}|  & \si{\eVc} \\
\verb|\si{\TeVcc}| & \si{\TeVcc} \\
\verb|\si{\GeVcc}| & \si{\GeVcc} \\
\verb|\si{\MeVcc}| & \si{\MeVcc} \\
\verb|\si{\keVcc}| & \si{\keVcc} \\
\verb|\si{\eVcc}|  & \si{\eVcc} \\
\verb|\si{\nb}| & \si{\nb} \\
\verb|\si{\pb}| & \si{\pb} \\
\verb|\si{\fb}| & \si{\fb} \\
\verb|\si{\per\fb}| & \si{\per\fb} \\
\verb|\si{\per\pb}| & \si{\per\pb} \\
\verb|\si{\per\nb}| & \si{\per\nb} \\
\verb|\si{\ifb}| & \si{\ifb} \\
\verb|\si{\ipb}| & \si{\ipb} \\
\verb|\si{\inb}| & \si{\inb} \\
\verb|\si{\Hz}|  & \si{\Hz} \\
\verb|\si{\kHz}| & \si{\kHz} \\
\verb|\si{\MHz}| & \si{\MHz} \\
\verb|\si{\GHz}| & \si{\GHz} \\
\verb|\si{\degr}| & \si{\degr} \\
\verb|\si{\m}| & \si{\m} \\
\verb|\si{\cm}| & \si{\cm} \\
\verb|\si{\mm}| & \si{\mm} \\
\verb|\si{\um}| & \si{\um} \\
\verb|\si{\micron}| & \si{\micron} \\
\end{xtabular}


==> bib/doc/atlas_physics/atlasbsm.tex <==
\begin{xtabular}{ll}
\verb|\Azero| & \Azero \\
\verb|\hzero| & \hzero \\
\verb|\Hzero| & \Hzero \\
\verb|\Hboson| & \Hboson \\
\verb|\Hplus| & \Hplus \\
\verb|\Hminus| & \Hminus \\
\verb|\Hpm| & \Hpm \\
\verb|\Hmp| & \Hmp \\
\verb|\ggino| & \ggino \\
\verb|\chinop| & \chinop \\
\verb|\chinom| & \chinom \\
\verb|\chinopm| & \chinopm \\
\verb|\chinomp| & \chinomp \\
\verb|\chinoonep| & \chinoonep \\
\verb|\chinoonem| & \chinoonem \\
\verb|\chinoonepm| & \chinoonepm \\
\verb|\chinotwop| & \chinotwop \\
\verb|\chinotwom| & \chinotwom \\
\verb|\chinotwopm| & \chinotwopm \\
\verb|\nino| & \nino \\
\verb|\ninoone| & \ninoone \\
\verb|\ninotwo| & \ninotwo \\
\verb|\ninothree| & \ninothree \\
\verb|\ninofour| & \ninofour \\
\verb|\gravino| & \gravino \\
\verb|\Zprime| & \Zprime \\
\verb|\Zstar| & \Zstar \\
\verb|\squark| & \squark \\
\verb|\squarkL| & \squarkL \\
\verb|\squarkR| & \squarkR \\
\verb|\gluino| & \gluino \\
\verb|\stop| & \stop \\
\verb|\stopone| & \stopone \\
\verb|\stoptwo| & \stoptwo \\
\verb|\stopL| & \stopL \\
\verb|\stopR| & \stopR \\
\verb|\sbottom| & \sbottom \\
\verb|\sbottomone| & \sbottomone \\
\verb|\sbottomtwo| & \sbottomtwo \\
\verb|\sbottomL| & \sbottomL \\
\verb|\sbottomR| & \sbottomR \\
\verb|\slepton| & \slepton \\
\verb|\sleptonL| & \sleptonL \\
\verb|\sleptonR| & \sleptonR \\
\verb|\sel| & \sel \\
\verb|\selL| & \selL \\
\verb|\selR| & \selR \\
\verb|\smu| & \smu \\
\verb|\smuL| & \smuL \\
\verb|\smuR| & \smuR \\
\verb|\stau| & \stau \\
\verb|\stauL| & \stauL \\
\verb|\stauR| & \stauR \\
\verb|\stauone| & \stauone \\
\verb|\stautwo| & \stautwo \\
\verb|\snu| & \snu \\
\end{xtabular}


==> bib/doc/atlas_physics/atlasheavyion.tex <==
\begin{xtabular}{ll}
\verb|\NucNuc| & \NucNuc \\
\verb|\nn| & \nn \\
\verb|\pn| & \pn \\
\verb|\np| & \np \\
\verb|\PbPb| & \PbPb \\
\verb|\AuAu| & \AuAu \\
\verb|\CuCu| & \CuCu \\
\verb|\pNuc| & \pNuc \\
\verb|\pdA| & \pdA \\
\verb|\dAu| & \dAu \\
\verb|\pPb| & \pPb \\
\verb|\Npart| & \Npart \\
\verb|\avgNpart| & \avgNpart \\
\verb|\Ncoll| & \Ncoll \\
\verb|\avgNcoll| & \avgNcoll \\
\verb|\TA| & \TA \\
\verb|\avgTA| & \avgTA \\
\verb|\TPb| & \TPb \\
\verb|\avgTPb| & \avgTPb \\
\verb|\TAA| & \TAA \\
\verb|\avgTAA| & \avgTAA \\
\verb|\TAB| & \TAB \\
\verb|\avgTAB| & \avgTAB \\
\verb|\TpPb| & \TpPb \\
\verb|\avgTpPb| & \avgTpPb \\
\verb|\Gl| & \Gl \\
\verb|\GG| & \GG \\
\verb|\sqn| & \sqn \\
\verb|\lns| & \lns \\
\verb|\sumETPb| & \sumETPb \\
\verb|\sumETp| & \sumETp \\
\verb|\sumETA| & \sumETA \\
\verb|\RAA| & \RAA \\
\verb|\RCP| & \RCP \\
\verb|\RpA| & \RpA \\
\verb|\RpPb| & \RpPb \\
\verb|\dNchdeta| & \dNchdeta \\
\verb|\dNevtdET| & \dNevtdET \\
\verb|\ystar| & \ystar \\
\verb|\ycms| & \ycms \\
\verb|\ygappb| & \ygappb \\
\verb|\ygapp| & \ygapp \\
\verb|\fgap| & \fgap \\
\end{xtabular}


==> bib/doc/atlas_physics/atlashepparticle.tex <==
\begin{xtabular}{ll}
\verb|\pp| & \pp \\
\verb|\pbar| & \pbar \\
\verb|\ppbar| & \ppbar \\
\verb|\tbar| & \tbar \\
\verb|\ttbar| & \ttbar \\
\verb|\bbar| & \bbar \\
\verb|\bbbar| & \bbbar \\
\verb|\cbar| & \cbar \\
\verb|\ccbar| & \ccbar \\
\verb|\sbar| & \sbar \\
\verb|\ssbar| & \ssbar \\
\verb|\ubar| & \ubar \\
\verb|\uubar| & \uubar \\
\verb|\dbar| & \dbar \\
\verb|\ddbar| & \ddbar \\
\verb|\fbar| & \fbar \\
\verb|\ffbar| & \ffbar \\
\verb|\qbar| & \qbar \\
\verb|\qqbar| & \qqbar \\
\verb|\nbar| & \nbar \\
\verb|\nnbar| & \nnbar \\
\verb|\ee| & \ee \\
\verb|\epm| & \epm \\
\verb|\epem| & \epem \\
\verb|\mumu| & \mumu \\
\verb|\tautau| & \tautau \\
\verb|\leplep| & \leplep \\
\verb|\ellell| & \ellell \\
\verb|\enu| & \enu \\
\verb|\munu| & \munu \\
\verb|\lnu| & \lnu \\
\verb|\Zzero| & \Zzero \\
\verb|\Zboson| & \Zboson \\
\verb|\Wplus| & \Wplus \\
\verb|\Wminus| & \Wminus \\
\verb|\Wboson| & \Wboson \\
\verb|\Wpm| & \Wpm \\
\verb|\Wmp| & \Wmp \\
\verb|\taulep| & \taulep \\
\verb|\tauhad| & \tauhad \\
\verb|\tauhadvis| & \tauhadvis \\
\verb|\pizero| & \pizero \\
\verb|\piplus| & \piplus \\
\verb|\piminus| & \piminus \\
\verb|\pipm| & \pipm \\
\verb|\pimp| & \pimp \\
\verb|\etaprime| & \etaprime \\
\verb|\Kzero| & \Kzero \\
\verb|\Kzerobar| & \Kzerobar \\
\verb|\kaon| & \kaon \\
\verb|\Kplus| & \Kplus \\
\verb|\Kminus| & \Kminus \\
\verb|\KzeroL| & \KzeroL \\
\verb|\Kzerol| & \Kzerol \\
\verb|\Klong| & \Klong \\
\verb|\KzeroS| & \KzeroS \\
\verb|\Kzeros| & \Kzeros \\
\verb|\Kshort| & \Kshort \\
\verb|\Kstar| & \Kstar \\
\verb|\jpsi| & \jpsi \\
\verb|\Jpsi| & \Jpsi \\
\verb|\psip| & \psip \\
\verb|\chic| & \chic \\
\verb|\UoneS| & \UoneS \\
\verb|\chib| & \chib \\
\verb|\Dstar| & \Dstar \\
\verb|\Bd| & \Bd \\
\verb|\Bs| & \Bs \\
\verb|\Bu| & \Bu \\
\verb|\Bc| & \Bc \\
\verb|\Lb| & \Lb \\
\verb|\Bstar| & \Bstar \\
\verb|\BoBo| & \BoBo \\
\verb|\BodBod| & \BodBod \\
\verb|\BosBos| & \BosBos \\
\end{xtabular}


==> bib/doc/atlas_physics/atlashepprocess.tex <==
\begin{xtabular}{ll}
\verb|\btol| & \btol \\
\verb|\ctol| & \ctol \\
\verb|\btoctol| & \btoctol \\
\verb|\Jee| & \Jee \\
\verb|\Jmm| & \Jmm \\
\verb|\Jmumu| & \Jmumu \\
\verb|\Wjj| & \Wjj \\
\verb|\tjjb| & \tjjb \\
\verb|\Hbb| & \Hbb \\
\verb|\Hgg| & \Hgg \\
\verb|\Hll| & \Hll \\
\verb|\Hllll| & \Hllll \\
\verb|\Hmmmm| & \Hmmmm \\
\verb|\Heeee| & \Heeee \\
\verb|\Zll| & \Zll \\
\verb|\Zlplm| & \Zlplm \\
\verb|\Zee| & \Zee \\
\verb|\Zepem| & \Zepem \\
\verb|\Zmm| & \Zmm \\
\verb|\Zmpmm| & \Zmpmm \\
\verb|\Ztt| & \Ztt \\
\verb|\Ztptm| & \Ztptm \\
\verb|\Zbb| & \Zbb \\
\verb|\Wln| & \Wln \\
\verb|\Wen| & \Wen \\
\verb|\Wmn| & \Wmn \\
\verb|\Wlnu| & \Wlnu \\
\verb|\Wenu| & \Wenu \\
\verb|\Wmunu| & \Wmunu \\
\verb|\Wqqbar| & \Wqqbar \\
\verb|\Amm| & \Amm \\
\verb|\Ztautau| & \Ztautau \\
\verb|\Wtaunu| & \Wtaunu \\
\verb|\Atautau| & \Atautau \\
\verb|\Htautau| & \Htautau \\
\verb|\tWb| & \tWb \\
\verb|\Wjets| & \Wjets \\
\verb|\Zjets| & \Zjets \\
\verb|\Brjl| & \Brjl \\
\end{xtabular}


==> bib/doc/atlas_physics/atlasjetetmiss.tex <==
\begin{xtabular}{ll}
\verb|\topo| & \topo \\
\verb|\Topo| & \Topo \\
\verb|\topos| & \topos \\
\verb|\Topos| & \Topos \\
\verb|\insitu| & \insitu \\
\verb|\Insitu| & \Insitu \\
\verb|\LS| & \LS \\
\verb|\NLOjet| & \NLOjet \\
\verb|\Fastjet| & \Fastjet \\
\verb|\TwoToTwo| & \TwoToTwo \\
\verb|\largeR| & \largeR \\
\verb|\LargeR| & \LargeR \\
\verb|\akt| & \akt \\
\verb|\Akt| & \Akt \\
\verb|\AKT| & \AKT \\
\verb|\AKTFat| & \AKTFat \\
\verb|\AKTPrune| & \AKTPrune \\
\verb|\AKTFilt| & \AKTFilt \\
\verb|\KTSix| & \KTSix \\
\verb|\ca| & \ca \\
\verb|\CamKt| & \CamKt \\
\verb|\CASix| & \CASix \\
\verb|\CAFat| & \CAFat \\
\verb|\CAPrune| & \CAPrune \\
\verb|\CAFilt| & \CAFilt \\
\verb|\htt| & \htt \\
\verb|\mcut| & \mcut \\
\verb|\Nfilt| & \Nfilt \\
\verb|\Rfilt| & \Rfilt \\
\verb|\ymin| & \ymin \\
\verb|\fcut| & \fcut \\
\verb|\Rsub| & \Rsub \\
\verb|\mufrac| & \mufrac \\
\verb|\Rcut| & \Rcut \\
\verb|\zcut| & \zcut \\
\verb|\ftile| & \ftile \\
\verb|\fem| & \fem \\
\verb|\fpres| & \fpres \\
\verb|\fhec| & \fhec \\
\verb|\ffcal| & \ffcal \\
\verb|\central| & \central \\
\verb|\ecap| & \ecap \\
\verb|\forward| & \forward \\
\verb|\Npv| & \Npv \\
\verb|\Nref| & \Nref \\
\verb|\Navg| & \Navg \\
\verb|\avgmu| & \avgmu \\
\verb|\JES| & \JES \\
\verb|\JMS| & \JMS \\
\verb|\EMJES| & \EMJES \\
\verb|\GCWJES| & \GCWJES \\
\verb|\LCWJES| & \LCWJES \\
\verb|\EM| & \EM \\
\verb|\GCW| & \GCW \\
\verb|\LCW| & \LCW \\
\verb|\GSL| & \GSL \\
\verb|\GS| & \GS \\
\verb|\MTF| & \MTF \\
\verb|\MPF| & \MPF \\
\verb|\Njet| & \Njet \\
\verb|\njet| & \njet \\
\verb|\ETjet| & \ETjet \\
\verb|\etjet| & \etjet \\
\verb|\pTavg| & \pTavg \\
\verb|\ptavg| & \ptavg \\
\verb|\pTjet| & \pTjet \\
\verb|\ptjet| & \ptjet \\
\verb|\pTcorr| & \pTcorr \\
\verb|\ptcorr| & \ptcorr \\
\verb|\pTjeti| & \pTjeti \\
\verb|\ptjeti| & \ptjeti \\
\verb|\pTrecoil| & \pTrecoil \\
\verb|\ptrecoil| & \ptrecoil \\
\verb|\pTleading| & \pTleading \\
\verb|\ptleading| & \ptleading \\
\verb|\pTjetEM| & \pTjetEM \\
\verb|\ptjetEM| & \ptjetEM \\
\verb|\pThat| & \pThat \\
\verb|\pthat| & \pthat \\
\verb|\pTprobe| & \pTprobe \\
\verb|\ptprobe| & \ptprobe \\
\verb|\pTref| & \pTref \\
\verb|\ptref| & \ptref \\
\verb|\pToff| & \pToff \\
\verb|\ptoff| & \ptoff \\
\verb|\pToffjet| & \pToffjet \\
\verb|\ptoffjet| & \ptoffjet \\
\verb|\pTZ| & \pTZ \\
\verb|\ptZ| & \ptZ \\
\verb|\pTtrue| & \pTtrue \\
\verb|\pttrue| & \pttrue \\
\verb|\pTtruth| & \pTtruth \\
\verb|\pttruth| & \pttruth \\
\verb|\pTreco| & \pTreco \\
\verb|\ptreco| & \ptreco \\
\verb|\pTtrk| & \pTtrk \\
\verb|\pttrk| & \pttrk \\
\verb|\ptrk| & \ptrk \\
\verb|\pTtrkjet| & \pTtrkjet \\
\verb|\pttrkjet| & \pttrkjet \\
\verb|\ntrk| & \ntrk \\
\verb|\EoverP| & \EoverP \\
\verb|\Etrue| & \Etrue \\
\verb|\Etruth| & \Etruth \\
\verb|\Ecalo| & \Ecalo \\
\verb|\EcaloEM| & \EcaloEM \\
\verb|\asym| & \asym \\
\verb|\Response| & \Response \\
\verb|\Rcalo| & \Rcalo \\
\verb|\Rcalom| & \Rcalom \\
\verb|\RcaloEM| & \RcaloEM \\
\verb|\RMPF| & \RMPF \\
\verb|\EcaloCALIB| & \EcaloCALIB \\
\verb|\RcaloCALIB| & \RcaloCALIB \\
\verb|\EcaloEMJES| & \EcaloEMJES \\
\verb|\RcaloEMJES| & \RcaloEMJES \\
\verb|\EcaloGCWJES| & \EcaloGCWJES \\
\verb|\RcaloGCWJES| & \RcaloGCWJES \\
\verb|\EcaloLCWJES| & \EcaloLCWJES \\
\verb|\RcaloLCWJES| & \RcaloLCWJES \\
\verb|\Rtrack| & \Rtrack \\
\verb|\rtrk| & \rtrk \\
\verb|\Rtrk| & \Rtrk \\
\verb|\rtrackjet| & \rtrackjet \\
\verb|\rtrackjetiso| & \rtrackjetiso \\
\verb|\rtrackjetnoniso| & \rtrackjetnoniso \\
\verb|\rtrackjetisoratio| & \rtrackjetisoratio \\
\verb|\gammajet| & \gammajet \\
\verb|\deltaphijetgamma| & \deltaphijetgamma \\
\verb|\rapjet| & \rapjet \\
\verb|\etajet| & \etajet \\
\verb|\phijet| & \phijet \\
\verb|\etadet| & \etadet \\
\verb|\etatrk| & \etatrk \\
\verb|\Rmin| & \Rmin \\
\verb|\DeltaR| & \DeltaR \\
\verb|\DetaDphi| & \DetaDphi \\
\verb|\Deta| & \Deta \\
\verb|\Drap| & \Drap \\
\verb|\DetaOneTwo| & \DetaOneTwo \\
\verb|\DyDphi| & \DyDphi \\
\verb|\DeltaRdef| & \DeltaRdef \\
\verb|\DeltaRydef| & \DeltaRydef \\
\verb|\DeltaRtrk| & \DeltaRtrk \\
\verb|\JVF| & \JVF \\
\verb|\cJVF| & \cJVF \\
\verb|\RpT| & \RpT \\
\verb|\JVT| & \JVT \\
\verb|\ghostpt| & \ghostpt \\
\verb|\ghostptavg| & \ghostptavg \\
\verb|\ghostfm| & \ghostfm \\
\verb|\ghostfmi| & \ghostfmi \\
\verb|\ghostdensity| & \ghostdensity \\
\verb|\ghostrho| & \ghostrho \\
\verb|\Aghost| & \Aghost \\
\verb|\Amu| & \Amu \\
\verb|\Amui| & \Amui \\
\verb|\jetarea| & \jetarea \\
\verb|\jetareafm| & \jetareafm \\
\verb|\jetareai| & \jetareai \\
\verb|\Rkt| & \Rkt \\
\verb|\pTmuslope| & \pTmuslope \\
\verb|\ptmuslope| & \ptmuslope \\
\verb|\pTnpvslope| & \pTnpvslope \\
\verb|\ptnpvslope| & \ptnpvslope \\
\verb|\pTmuunc| & \pTmuunc \\
\verb|\ptmuunc| & \ptmuunc \\
\verb|\pTnpvunc| & \pTnpvunc \\
\verb|\ptnpvunc| & \ptnpvunc \\
\verb|\sumPt| & \sumPt \\
\verb|\sumpt| & \sumpt \\
\verb|\sumpTtrk| & \sumpTtrk \\
\verb|\sumpttrk| & \sumpttrk \\
\verb|\nPUtrk| & \nPUtrk \\
\verb|\mjet| & \mjet \\
\verb|\mlead| & \mlead \\
\verb|\mleadavg| & \mleadavg \\
\verb|\Mjet| & \Mjet \\
\verb|\massjet| & \massjet \\
\verb|\masscorr| & \masscorr \\
\verb|\mthresh| & \mthresh \\
\verb|\mjetavg| & \mjetavg \\
\verb|\masstrkjet| & \masstrkjet \\
\verb|\width| & \width \\
\verb|\wcalo| & \wcalo \\
\verb|\wtrk| & \wtrk \\
\verb|\shapeV| & \shapeV \\
\verb|\pTsubjet| & \pTsubjet \\
\verb|\ptsubjet| & \ptsubjet \\
\verb|\sjone| & \sjone \\
\verb|\sjtwo| & \sjtwo \\
\verb|\msubjone| & \msubjone \\
\verb|\msubjtwo| & \msubjtwo \\
\verb|\pTsubji| & \pTsubji \\
\verb|\ptsubji| & \ptsubji \\
\verb|\pTsubjone| & \pTsubjone \\
\verb|\ptsubjone| & \ptsubjone \\
\verb|\pTsubjtwo| & \pTsubjtwo \\
\verb|\ptsubjtwo| & \ptsubjtwo \\
\verb|\Rsubjets| & \Rsubjets \\
\verb|\DRsubjets| & \DRsubjets \\
\verb|\yij| & \yij \\
\verb|\dcut| & \dcut \\
\verb|\dmin| & \dmin \\
\verb|\dij| & \dij \\
\verb|\Dij| & \Dij \\
\verb|\Donetwo| & \Donetwo \\
\verb|\Dtwothr| & \Dtwothr \\
\verb|\yonetwo| & \yonetwo \\
\verb|\ytwothr| & \ytwothr \\
\verb|\yonetwoDef| & \yonetwoDef \\
\verb|\ytwothrDef| & \ytwothrDef \\
\verb|\xj| & \xj \\
\verb|\jetFunc| & \jetFunc \\
\verb|\tauone| & \tauone \\
\verb|\tautwo| & \tautwo \\
\verb|\tauthr| & \tauthr \\
\verb|\tauN| & \tauN \\
\verb|\tautwoone| & \tautwoone \\
\verb|\tauthrtwo| & \tauthrtwo \\
\verb|\dip| & \dip \\
\verb|\diponetwo| & \diponetwo \\
\verb|\diptwothr| & \diptwothr \\
\verb|\diponethr| & \diponethr \\
\verb|\mtaSup| & \mtaSup \\
\verb|\mcalo| & \mcalo \\
\verb|\mcomb| & \mcomb \\
\verb|\ECFOne| & \ECFOne \\
\verb|\ECFTwo| & \ECFTwo \\
\verb|\ECFThr| & \ECFThr \\
\verb|\ECFThrNorm| & \ECFThrNorm \\
\verb|\DTwo| & \DTwo \\
\verb|\CTwo| & \CTwo \\
\verb|\FoxWolfRatio| & \FoxWolfRatio \\
\verb|\PlanarFlow| & \PlanarFlow \\
\verb|\Angularity| & \Angularity \\
\verb|\Aplanarity| & \Aplanarity \\
\verb|\KtDR| & \KtDR \\
\verb|\Qw| & \Qw \\
\verb|\NConst| & \NConst \\
\end{xtabular}


==> bib/doc/atlas_physics/atlasjournal.tex <==
\begin{xtabular}{ll}
\verb|\AcPA| & \AcPA \\
\verb|\ARevNS| & \ARevNS \\
\verb|\CPC| & \CPC \\
\verb|\EPJ| & \EPJ \\
\verb|\EPJC| & \EPJC \\
\verb|\FortP| & \FortP \\
\verb|\IJMP| & \IJMP \\
\verb|\JETP| & \JETP \\
\verb|\JETPL| & \JETPL \\
\verb|\JaFi| & \JaFi \\
\verb|\JHEP| & \JHEP \\
\verb|\JMP| & \JMP \\
\verb|\MPL| & \MPL \\
\verb|\NCim| & \NCim \\
\verb|\NIM| & \NIM \\
\verb|\NIMA| & \NIMA \\
\verb|\NP| & \NP \\
\verb|\NPB| & \NPB \\
\verb|\PL| & \PL \\
\verb|\PLB| & \PLB \\
\verb|\PR| & \PR \\
\verb|\PRC| & \PRC \\
\verb|\PRD| & \PRD \\
\verb|\PRL| & \PRL \\
\verb|\PRep| & \PRep \\
\verb|\RMP| & \RMP \\
\verb|\ZfP| & \ZfP \\
\verb|\collab| & \collab \\
\end{xtabular}


==> bib/doc/atlas_physics/atlasmath.tex <==
\begin{xtabular}{ll}
\verb|\boxsq| & \boxsq \\
\verb|\grad| & \grad \\
\end{xtabular}


==> bib/doc/atlas_physics/atlasmisc.tex <==
\begin{xtabular}{ll}
\verb|\pT| & \pT \\
\verb|\pt| & \pt \\
\verb|\pTX| & \pTX \\
\verb|\ET| & \ET \\
\verb|\eT| & \eT \\
\verb|\et| & \et \\
\verb|\HT| & \HT \\
\verb|\pTsq| & \pTsq \\
\verb|\MET| & \MET \\
\verb|\met| & \met \\
\verb|\sumET| & \sumET \\
\verb|\EjetRec| & \EjetRec \\
\verb|\PjetRec| & \PjetRec \\
\verb|\EjetTru| & \EjetTru \\
\verb|\PjetTru| & \PjetTru \\
\verb|\EjetDM| & \EjetDM \\
\verb|\Rcone| & \Rcone \\
\verb|\abseta| & \abseta \\
\verb|\Ecm| & \Ecm \\
\verb|\rts| & \rts \\
\verb|\sqs| & \sqs \\
\verb|\Nevt| & \Nevt \\
\verb|\zvtx| & \zvtx \\
\verb|\dzero| & \dzero \\
\verb|\zzsth| & \zzsth \\
\verb|\RunOne| & \RunOne \\
\verb|\RunTwo| & \RunTwo \\
\verb|\RunThr| & \RunThr \\
\verb|\kt| & \kt \\
\verb|\antikt| & \antikt \\
\verb|\Antikt| & \Antikt \\
\verb|\pileup| & \pileup \\
\verb|\Pileup| & \Pileup \\
\verb|\btag| & \btag \\
\verb|\btagged| & \btagged \\
\verb|\bquark| & \bquark \\
\verb|\bquarks| & \bquarks \\
\verb|\bjet| & \bjet \\
\verb|\bjets| & \bjets \\
\verb|\mh| & \mh \\
\verb|\mW| & \mW \\
\verb|\mZ| & \mZ \\
\verb|\mH| & \mH \\
\verb|\ACERMC| & \ACERMC \\
\verb|\ALPGEN| & \ALPGEN \\
\verb|\AMCatNLO| & \AMCatNLO \\
\verb|\BLACKHAT| & \BLACKHAT \\
\verb|\CALCHEP| & \CALCHEP \\
\verb|\COLLIER| & \COLLIER \\
\verb|\COMPHEP| & \COMPHEP \\
\verb|\EVTGEN| & \EVTGEN \\
\verb|\FEYNRULES| & \FEYNRULES \\
\verb|\GGTOVV| & \GGTOVV \\
\verb|\GOSAM| & \GOSAM \\
\verb|\HATHOR| & \HATHOR \\
\verb|\Herwig| & \Herwig \\
\verb|\HERWIG| & \HERWIG \\
\verb|\HERWIGpp| & \HERWIGpp \\
\verb|\HRES| & \HRES \\
\verb|\JIMMY| & \JIMMY \\
\verb|\MADSPIN| & \MADSPIN \\
\verb|\MADGRAPH| & \MADGRAPH \\
\verb|\MGNLO| & \MGNLO \\
\verb|\MCatNLO| & \MCatNLO \\
\verb|\MCFM| & \MCFM \\
\verb|\METOP| & \METOP \\
\verb|\OPENLOOPS| & \OPENLOOPS \\
\verb|\POWHEG| & \POWHEG \\
\verb|\POWHEGBOX| & \POWHEGBOX \\
\verb|\POWHEGBOXRES| & \POWHEGBOXRES \\
\verb|\PHOTOS| & \PHOTOS \\
\verb|\PHOTOSpp| & \PHOTOSpp \\
\verb|\PROPHECY| & \PROPHECY \\
\verb|\PROTOS| & \PROTOS \\
\verb|\Pythia| & \Pythia \\
\verb|\PYTHIA| & \PYTHIA \\
\verb|\RECOLA| & \RECOLA \\
\verb|\Sherpa| & \Sherpa \\
\verb|\SHERPA| & \SHERPA \\
\verb|\TOPpp| & \TOPpp \\
\verb|\VBFNLO| & \VBFNLO \\
\verb|\MGNLOHER| & \MGNLOHER \\
\verb|\MGNLOPY| & \MGNLOPY \\
\verb|\MGHER| & \MGHER \\
\verb|\MGPY| & \MGPY \\
\verb|\POWHER| & \POWHER \\
\verb|\POWPY| & \POWPY \\
\verb|\SHERPABH| & \SHERPABH \\
\verb|\SHERPAOL| & \SHERPAOL \\
\verb|\ABM| & \ABM \\
\verb|\ABKM| & \ABKM \\
\verb|\CT| & \CT \\
\verb|\CTEQ| & \CTEQ \\
\verb|\GJR| & \GJR \\
\verb|\HERAPDF| & \HERAPDF \\
\verb|\LUXQED| & \LUXQED \\
\verb|\MSTW| & \MSTW \\
\verb|\MMHT| & \MMHT \\
\verb|\MSHT| & \MSHT \\
\verb|\NNPDF| & \NNPDF \\
\verb|\PDFforLHC| & \PDFforLHC \\
\verb|\AUET| & \AUET \\
\verb|\AZNLO| & \AZNLO \\
\verb|\FXFX| & \FXFX \\
\verb|\GEANT| & \GEANT \\
\verb|\MENLOPS| & \MENLOPS \\
\verb|\MEPSatLO| & \MEPSatLO \\
\verb|\MEPSatNLO| & \MEPSatNLO \\
\verb|\MINLO| & \MINLO \\
\verb|\Monash| & \Monash \\
\verb|\Perugia| & \Perugia \\
\verb|\Prospino| & \Prospino \\
\verb|\UEEE| & \UEEE \\
\verb|\LO| & \LO \\
\verb|\NLO| & \NLO \\
\verb|\NLL| & \NLL \\
\verb|\NNLO| & \NNLO \\
\verb|\muF| & \muF \\
\verb|\muQ| & \muQ \\
\verb|\muR| & \muR \\
\verb|\hdamp| & \hdamp \\
\verb|\NLOEWvirt| & \NLOEWvirt \\
\verb|\ra| & \ra \\
\verb|\la| & \la \\
\verb|\rarrow| & \rarrow \\
\verb|\larrow| & \larrow \\
\verb|\lapprox| & \lapprox \\
\verb|\rapprox| & \rapprox \\
\verb|\gam| & \gam \\
\verb|\stat| & \stat \\
\verb|\syst| & \syst \\
\verb|\radlength| & \radlength \\
\verb|\StoB| & \StoB \\
\verb|\alphas| & \alphas \\
\verb|\NF| & \NF \\
\verb|\NC| & \NC \\
\verb|\CF| & \CF \\
\verb|\CA| & \CA \\
\verb|\TF| & \TF \\
\verb|\Lms| & \Lms \\
\verb|\Lmsfive| & \Lmsfive \\
\verb|\kperp| & \kperp \\
\verb|\Vcb| & \Vcb \\
\verb|\Vub| & \Vub \\
\verb|\Vtd| & \Vtd \\
\verb|\Vts| & \Vts \\
\verb|\Vtb| & \Vtb \\
\verb|\Vcs| & \Vcs \\
\verb|\Vud| & \Vud \\
\verb|\Vus| & \Vus \\
\verb|\Vcd| & \Vcd \\
\end{xtabular}


==> bib/doc/atlas_physics/atlasother.tex <==
\begin{xtabular}{ll}
\verb|\etpt| & \etpt \\
\verb|\etptsig| & \etptsig \\
\verb|\begL| & \begL \\
\verb|\lowL| & \lowL \\
\verb|\highL| & \highL \\
\verb|\Epsb| & \Epsb \\
\verb|\Epsc| & \Epsc \\
\verb|\Mtau| & \Mtau \\
\verb|\swsq| & \swsq \\
\verb|\swel| & \swel \\
\verb|\swsqb| & \swsqb \\
\verb|\swsqon| & \swsqon \\
\verb|\gv| & \gv \\
\verb|\ga| & \ga \\
\verb|\gvbar| & \gvbar \\
\verb|\gabar| & \gabar \\
\verb|\Zzv| & \Zzv \\
\verb|\Abb| & \Abb \\
\verb|\Acc| & \Acc \\
\verb|\Aqq| & \Aqq \\
\verb|\Afb| & \Afb \\
\verb|\GZ| & \GZ \\
\verb|\GW| & \GW \\
\verb|\GH| & \GH \\
\verb|\GamHad| & \GamHad \\
\verb|\Gbb| & \Gbb \\
\verb|\Rbb| & \Rbb \\
\verb|\Gcc| & \Gcc \\
\verb|\Gvis| & \Gvis \\
\verb|\Ginv| & \Ginv \\
\end{xtabular}


==> bib/doc/atlas_physics/atlasparticle.tex <==
\begin{xtabular}{ll}
\verb|\pp| & \pp \\
\verb|\pbar| & \pbar \\
\verb|\ppbar| & \ppbar \\
\verb|\tbar| & \tbar \\
\verb|\ttbar| & \ttbar \\
\verb|\bbar| & \bbar \\
\verb|\bbbar| & \bbbar \\
\verb|\cbar| & \cbar \\
\verb|\ccbar| & \ccbar \\
\verb|\sbar| & \sbar \\
\verb|\ssbar| & \ssbar \\
\verb|\ubar| & \ubar \\
\verb|\uubar| & \uubar \\
\verb|\dbar| & \dbar \\
\verb|\ddbar| & \ddbar \\
\verb|\fbar| & \fbar \\
\verb|\ffbar| & \ffbar \\
\verb|\qbar| & \qbar \\
\verb|\qqbar| & \qqbar \\
\verb|\nbar| & \nbar \\
\verb|\nnbar| & \nnbar \\
\verb|\ee| & \ee \\
\verb|\epm| & \epm \\
\verb|\epem| & \epem \\
\verb|\mumu| & \mumu \\
\verb|\tautau| & \tautau \\
\verb|\leplep| & \leplep \\
\verb|\ellell| & \ellell \\
\verb|\enu| & \enu \\
\verb|\munu| & \munu \\
\verb|\lnu| & \lnu \\
\verb|\taulep| & \taulep \\
\verb|\tauhad| & \tauhad \\
\verb|\tauhadvis| & \tauhadvis \\
\verb|\Zzero| & \Zzero \\
\verb|\Zboson| & \Zboson \\
\verb|\Wplus| & \Wplus \\
\verb|\Wminus| & \Wminus \\
\verb|\Wboson| & \Wboson \\
\verb|\Wpm| & \Wpm \\
\verb|\Wmp| & \Wmp \\
\verb|\pizero| & \pizero \\
\verb|\piplus| & \piplus \\
\verb|\piminus| & \piminus \\
\verb|\pipm| & \pipm \\
\verb|\pimp| & \pimp \\
\verb|\etaprime| & \etaprime \\
\verb|\Kzero| & \Kzero \\
\verb|\Kzerobar| & \Kzerobar \\
\verb|\kaon| & \kaon \\
\verb|\Kplus| & \Kplus \\
\verb|\Kminus| & \Kminus \\
\verb|\KzeroL| & \KzeroL \\
\verb|\Kzerol| & \Kzerol \\
\verb|\Klong| & \Klong \\
\verb|\KzeroS| & \KzeroS \\
\verb|\Kzeros| & \Kzeros \\
\verb|\Kshort| & \Kshort \\
\verb|\Kstar| & \Kstar \\
\verb|\jpsi| & \jpsi \\
\verb|\Jpsi| & \Jpsi \\
\verb|\psip| & \psip \\
\verb|\chic| & \chic \\
\verb|\UoneS| & \UoneS \\
\verb|\chib| & \chib \\
\verb|\Dstar| & \Dstar \\
\verb|\Bd| & \Bd \\
\verb|\Bs| & \Bs \\
\verb|\Bu| & \Bu \\
\verb|\Bc| & \Bc \\
\verb|\Lb| & \Lb \\
\verb|\Bstar| & \Bstar \\
\verb|\BoBo| & \BoBo \\
\verb|\BodBod| & \BodBod \\
\verb|\BosBos| & \BosBos \\
\end{xtabular}


==> bib/doc/atlas_physics/atlasprocess.tex <==
\begin{xtabular}{ll}
\verb|\btol| & \btol \\
\verb|\ctol| & \ctol \\
\verb|\btoctol| & \btoctol \\
\verb|\Jee| & \Jee \\
\verb|\Jmm| & \Jmm \\
\verb|\Jmumu| & \Jmumu \\
\verb|\Wjj| & \Wjj \\
\verb|\tjjb| & \tjjb \\
\verb|\Hbb| & \Hbb \\
\verb|\Hgg| & \Hgg \\
\verb|\Hll| & \Hll \\
\verb|\Hllll| & \Hllll \\
\verb|\Hmmmm| & \Hmmmm \\
\verb|\Heeee| & \Heeee \\
\verb|\Zll| & \Zll \\
\verb|\Zlplm| & \Zlplm \\
\verb|\Zee| & \Zee \\
\verb|\Zepem| & \Zepem \\
\verb|\Zmm| & \Zmm \\
\verb|\Zmpmm| & \Zmpmm \\
\verb|\Ztt| & \Ztt \\
\verb|\Ztptm| & \Ztptm \\
\verb|\Zbb| & \Zbb \\
\verb|\Wln| & \Wln \\
\verb|\Wen| & \Wen \\
\verb|\Wmn| & \Wmn \\
\verb|\Wlnu| & \Wlnu \\
\verb|\Wenu| & \Wenu \\
\verb|\Wmunu| & \Wmunu \\
\verb|\Wqqbar| & \Wqqbar \\
\verb|\Amm| & \Amm \\
\verb|\Ztautau| & \Ztautau \\
\verb|\Wtaunu| & \Wtaunu \\
\verb|\Atautau| & \Atautau \\
\verb|\Htautau| & \Htautau \\
\verb|\tWb| & \tWb \\
\verb|\Wjets| & \Wjets \\
\verb|\Zjets| & \Zjets \\
\verb|\Brjl| & \Brjl \\
\end{xtabular}


==> bib/doc/atlas_physics/atlassnippets.tex <==
\begin{xtabular}{lp{10cm}}
\verb|\AntiktSnippet| & \AntiktSnippet \\
\verb|\TopoclusteringSnippet| & \TopoclusteringSnippet \\
\verb|\GroomingSnippet| & \GroomingSnippet \\
\verb|\FastSimSnippet| & \FastSimSnippet \\
\verb|\PileupSnippet| & \PileupSnippet \\
\end{xtabular}


==> bib/doc/atlas_physics/atlasunit.tex <==
\begin{xtabular}{ll}
\verb|\electronvolt| & \electronvolt \\
\verb|\TeV| & \TeV \\
\verb|\GeV| & \GeV \\
\verb|\MeV| & \MeV \\
\verb|\keV| & \keV \\
\verb|\eV| & \eV \\
\verb|\TeVc| & \TeVc \\
\verb|\GeVc| & \GeVc \\
\verb|\MeVc| & \MeVc \\
\verb|\keVc| & \keVc \\
\verb|\eVc| & \eVc \\
\verb|\TeVcc| & \TeVcc \\
\verb|\GeVcc| & \GeVcc \\
\verb|\MeVcc| & \MeVcc \\
\verb|\keVcc| & \keVcc \\
\verb|\eVcc| & \eVcc \\
\verb|\ifb| & \ifb \\
\verb|\ipb| & \ipb \\
\verb|\inb| & \inb \\
\verb|\degr| & \degr \\
\end{xtabular}


==> bib/doc/atlas_physics/atlasxref.tex <==
\begin{xtabular}{ll}
\end{xtabular}


==> bib/doc/atlas_tables/Makefile <==
#------------------------------------------------------------------------------
# Makefile to make atlas_tables documentation
#------------------------------------------------------------------------------

BASENAME = atlas_tables
TEXLIVE = 2020

.PHONY: clean cleanpdf

atlas_tables:
	make -f ../Makefile run_latexmk BASENAME=$(BASENAME); \

texlive:
	make -f ../Makefile texlive BASENAME=$(BASENAME) TEXLIVE=$(TEXLIVE)

clean:
	make -f ../Makefile clean
	
cleanpdf:
	-rm $(BASENAME).pdf

cleanall: clean cleanpdf
	

==> bib/doc/atlas_tables/cross-sections_charm-ET1.tex <==
% Charm differential cross sections d sigma / dY in bins of ET
\sisetup{round-mode=figures, round-precision=2,
  group-digits=integer, group-minimum-digits=4}
\begin{tabular}{%
    S[table-format=2.0, table-number-alignment=right,
    round-mode=places, round-precision=0]@{$\,:\,$}
    S[table-format=2.0, table-number-alignment=left,
    round-mode=places, round-precision=0]
    S[table-format=4.2, table-number-alignment=right,
    round-mode=figures, round-precision=3]@{$\,\pm\,$}
    S[table-format=3.2, table-number-alignment=right,
    round-mode=figures, round-precision=2]@{$\,$}l}
  \toprule
  \multicolumn{2}{c}{\ET} &
  \multicolumn{3}{c}{$\dif\sigma / \dif\ET$}\\
  \multicolumn{2}{c}{\mbox{}} & \multicolumn{3}{c}{[\si{\pico\barn\per\GeV}]}\\
  \midrule
 4.2 & 8.0  & 3634.06 & 114.491  & \numpmerr{+201.404 }{-181.511}{2}  \\
 8.0 & 11.0 & 719.458 & 21.9334  & \numpmerr{+43.3087 }{-39.7824}{2}  \\
11.0 & 14.0 & 214.572 & 9.71991  & \numpmerr{+20.5413 }{-19.6464}{2}  \\
14.0 & 17.0 & 85.7584 & 6.03401  & \numpmerr{+10.0875 }{-8.99952}{2}  \\
17.0 & 20.0 & 35.4095 & 3.91591  & \numpmerr{+5.5349  }{-5.41347}{2}  \\
20.0 & 25.0 & 14.1253 & 2.72552  & \numpmerr{+3.46528 }{-3.22476}{2}  \\
25.0 & 35.0 & 2.37786 & 0.968562 & \numpmerr{+0.849647}{-0.855525}{2} \\
  \bottomrule
\end{tabular}


==> bib/doc/atlas_tables/cross-sections_charm-ET2.tex <==
% Charm differential cross sections d sigma / dY in bins of ET
\sisetup{round-mode=figures, round-precision=2,
  group-digits=integer, group-minimum-digits=4}
\begin{tabular}{%
    S[table-format=2.0, table-number-alignment=right,
    round-mode=places, round-precision=0]@{$\,:\,$}
    S[table-format=2.0, table-number-alignment=left,
    round-mode=places, round-precision=0]
    S[table-format=4.1, table-alignment=right,
    round-mode=figures, round-precision=3]@{$\,\pm\,$}
    S[table-format=3.1, table-alignment=right,
    round-mode=figures, round-precision=2]@{$\,$}r}
  \toprule
  \multicolumn{2}{c}{\ET} &
  \multicolumn{3}{c}{$\dif\sigma / \dif\ET$}\\
  \multicolumn{2}{c}{[\si{\GeV}]} & \multicolumn{3}{c}{[\si{\pico\barn\per\GeV}]}\\
  \midrule
 4.2 & 8.0  & 3634.06                    & 114.491                    & \numpmRF{+201.404 }{-181.511 }{2}  \\
 8.0 & 11.0 & 719.458                    & 21.9334                    & \numpmerr{+43.3087 }{-39.7824 }{0} \\
11.0 & 14.0 & {\numRF{214.572}{2}\phdo}  & {\numRF{9.71991}{1}\phdo}  & \numpmerr{+20.5413 }{-19.6464 }{0} \\
14.0 & 17.0 & {\numRF{85.7584}{2}\phdo}  & {\numRF{6.03401}{1}\phdo}  & \numpmerr{+10.0875 }{-8.99952 }{0} \\
17.0 & 20.0 & {\numRF{35.4095}{3}}       & {\numRF{3.91591}{2}}       & \numpmerr{+5.5349  }{-5.41347 }{1} \\
20.0 & 25.0 & 14.1253                    & 2.72552                    & \numpmerr{+3.46528 }{-3.22476 }{1} \\
25.0 & 35.0 & {\numRF{2.37786}{2}}       & {\numRF{0.968562}{1}}      & \numpmerr{+0.849647}{-0.855525}{1}  \\
  \bottomrule
\end{tabular}


==> bib/doc/atlas_tables/cross-sections_charm-eta1.tex <==
\renewcommand{\arraystretch}{1.4}
\sisetup{round-mode = places}
\centering
\begin{tabular}{%
S@{\,:\,}S
r@{\,}@{$\pm$}@{\,}l@{\,}l
}
\toprule
\multicolumn{2}{c}{\etajet} & \multicolumn{3}{c}{\diffetab} \\
\multicolumn{2}{c}{} & \multicolumn{3}{c}{[\si{\pico\barn}]} \\
\midrule
{\num{-1.6}} & -1.1 & \numRP{0.574}{3} & \num[round-precision=3]{0.094} &
$^{\numRP{+0.035}{3}}_{\numRP{-0.031}{3}}$ \\
{\num{-1.1}} & -0.8 & \numRP{1.213}{2} & \num[round-precision=2]{0.211} &
$^{\numRP{+0.162}{2}}_{\numRP{-0.162}{2}}$ \\
{\num{-0.8}} & -0.5 & \numRP{2.141}{2} & \num[round-precision=2]{0.219} &
$^{\numRP{+0.223}{2}}_{\numRP{-0.123}{2}}$ \\
{\num{-0.5}} & -0.2 & \numRP{2.326}{2} & \num[round-precision=2]{0.210} &
$^{\numRP{+0.284}{2}}_{\numRP{-0.214}{2}}$ \\
{\num{-0.2}} & +0.1 & \numRP{2.641}{2} & \num[round-precision=2]{0.220} &
$^{\numRP{+0.283}{2}}_{\numRP{-0.233}{2}}$ \\
{\num{+0.1}} & +0.5 & \numRP{3.160}{2} & \num[round-precision=2]{0.211} &
$^{\numRP{+0.232}{2}}_{\numRP{-0.172}{2}}$ \\
{\num{+0.5}} & +1.4 & \numRP{2.881}{2} & \num[round-precision=2]{0.154} &
$^{\numRP{+0.201}{2}}_{\numRP{-0.301}{2}}$ \\
\bottomrule
\end{tabular}


==> bib/doc/atlas_tables/cross-sections_charm-eta2.tex <==
\renewcommand{\arraystretch}{1.4}
\sisetup{round-mode = places, round-precision = 2}
\centering
\begin{tabular}{%
    S[table-format=3.2, table-number-alignment = right]@{\,:\,}S
    S[round-mode = places, round-precision = 2,
    table-format = 1.3, table-number-alignment = right]
    @{\(\,\pm\,\)}
    S[round-mode = places, round-precision = 2,
    table-format = 1.3, table-number-alignment = left]
    @{\,}l
    }
\toprule
\multicolumn{2}{c}{\etajet} & \multicolumn{3}{c}{\diffetab} \\
\multicolumn{2}{c}{} & \multicolumn{3}{c}{[\si{\pico\barn}]} \\
\midrule
-1.6 & -1.1 & {\numRP{0.574}{3}} & {\numRP{0.094}{3}} & \(^{\numRP{+0.035}{3}}_{\numRP{-0.031}{3}}\) \\
-1.1 & -0.8 & 1.213 & 0.211 & \(^{\num{+0.162}}_{\num{-0.162}}\) \\
-0.8 & -0.5 & 2.141 & 0.219 & \(^{\num{+0.223}}_{\num{-0.123}}\) \\
-0.5 & -0.2 & 2.326 & 0.210 & \(^{\num{+0.284}}_{\num{-0.214}}\) \\
-0.2 & +0.1 & 2.641 & 0.220 & \(^{\num{+0.283}}_{\num{-0.233}}\) \\
+0.1 & +0.5 & 3.160 & 0.211 & \(^{\num{+0.232}}_{\num{-0.172}}\) \\
+0.5 & +1.4 & 2.881 & 0.154 & \(^{\num{+0.201}}_{\num{-0.301}}\) \\
\bottomrule
\end{tabular}


==> bib/doc/atlas_tables/cross-sections_charm-x1.tex <==
% Charm differential cross sections d sigma / dY in bins of xda
\sisetup{round-mode=figures, round-precision=2,
  group-digits=integer, group-minimum-digits=4}
\sisetup{scientific-notation=fixed, fixed-exponent=0}
\begin{tabular}{%
    S[table-format=1.5, table-number-alignment=right,
    round-mode=figures, round-precision=1]@{$\,:\,$}
    S[table-format=1.5, table-number-alignment=left,
    round-mode=figures, round-precision=1]
    S[table-format=8.0, table-number-alignment=right,
    round-mode=figures, round-precision=3]@{$\,\pm\,$}
    S[table-format=6.0, table-number-alignment=right,
    round-mode=figures, round-precision=2]@{$\,$}r}
  \toprule
  \multicolumn{2}{c}{$x$} &
  \multicolumn{3}{c}{$\dif\sigma / \dif x$}\\
  \multicolumn{2}{c}{\mbox{}} & \multicolumn{3}{c}{[\si{\pico\barn}]}\\
  \midrule
0.00008 & 0.00020 & 1.08474e+07 & 867945  & \numpmerr{+761437 }{-647690 }{2}  \\
0.00020 & 0.00060 & 1.08385e+07 & 388976  & \numpmerr{+567443 }{-441257 }{2}  \\
0.00060 & 0.00160 & 4.974e+06   & 135404  & \numpmerr{+256385 }{-233376 }{2}  \\
0.00160 & 0.00500 & 1.21664e+06 & 31162.1 & \numpmerr{+68948.1}{-62459.6}{2} \\
0.00500 & 0.01000 & 256870      & 12232.7 & \numpmerr{+18363.7}{-16463.7}{2} \\
0.01000 & 0.10000 & 10652.6     &  791.21 & \numpmerr{+913.118}{-815.675}{2} \\
  \bottomrule
\end{tabular}


==> bib/doc/atlas_tables/cross-sections_charm-x2.tex <==
% Charm differential cross sections d sigma / dY in bins of xda
\sisetup{round-mode=figures, round-precision=2,
  group-digits=integer, group-minimum-digits=4}
\sisetup{scientific-notation=fixed, fixed-exponent=0}
\begin{tabular}{%
    S[table-format=1.5, table-number-alignment=right,
    round-mode=figures, round-precision=1]@{$\,:\,$}
    S[table-format=1.5, table-number-alignment=left,
    round-mode=figures, round-precision=1]
    S[table-format=5.1, table-alignment=right,
    round-mode=figures, round-precision=4]@{$\,\pm\,$}
    S[table-format=3.1, table-alignment=right,
    round-mode=figures, round-precision=2]@{$\,$}r}
  \toprule
  \multicolumn{2}{c}{$x$} &
  \multicolumn{3}{c}{$\dif\sigma / \dif x$}\\
  \multicolumn{2}{c}{\mbox{}} & \multicolumn{3}{c}{[\si{\nano\barn}]}\\
  \midrule
0.00008 & 0.00020                 & {\numRF{1.08474e+04}{2}\phdo}  & {\numRF{867945e-3}{1}\phdo}  & \numpmerr{+761437 e-3}{-647690 e-3}{1} \\
0.00020 & 0.00060                 & {\numRF{1.08385e+04}{3}\phdo}  & {\numRF{388976e-3}{1}\phdo}  & \numpmerr{+567443 e-3}{-441257 e-3}{1} \\
0.00060 & {\numRF{0.0016}{2}\pho} & {\numRF{4.974e+03}{3}\phdo}    & 135404e-3                    & \numpmerr{+256385 e-3}{-233376 e-3}{2} \\
{\numRF{0.0016}{2}\pho} & 0.00500 & {\numRF{1.21664e+03}{4}\phdo}  & 31162.1e-3                   & \numpmerr{+68948.1e-3}{-62459.6e-3}{2} \\
0.00500 & 0.01000                 & {\numRF{256870e-03}{3}\phdo}   & 12232.7e-3                   & \numpmerr{+18363.7e-3}{-16463.7e-3}{2} \\
0.01000 & 0.10000                 & {\numRF{10652.6e-03}{3}}       & {\numRF{791.21e-3}{1}}       & \numpmerr{+913.118e-3}{-815.675e-3}{1} \\
  \bottomrule
\end{tabular}


==> chapters/Overview_and_Scientific_Objectives.tex <==

%===============================================================================
\chapterauthors{B. Heinemann \\ DESY, 22761 Hamburg (Germany)}{B.King \\ University of Plymouth, Plymouth (UK)}
\date{\today}

\begin{chaptabstract}
    This chapter presents an overview of all aspects of LUXE (Laser Und XFEL Experiment), an experiment that will combine the high-quality and high-energy electron beam of the European XFEL with a high-intensity laser to explore the uncharted terrain of strong-field quantum electrodynamics characterised by both high energy and high intensity. The chapter  also illustrates the physics performance that will be achieved using a few selected example measurements.
\end{chaptabstract}

\tableofcontents
%===============================================================================
%\begin{refsection}
%\part{Motivation}
%===============================================================================
\section{Introduction and Scientific Motivation}
\label{sec:theory}

The LUXE experiment and its scientific motivation have previously been described in a Conceptual Design Report (CDR)~\cite{luxecdr}. In this technical design report a brief recap of the scientific motivation is presented but the main focus is on the updated technical design of the experiment, including options for a staged installation. 

There are two main layouts foreseen. The first (and initial) mode will collide the electron beam of the European XFEL directly with a high-power laser. In a second mode, first the electron beam is converted to a photon beam and that photon beam then interacts with the laser, directly scattering light off light. In these interactions, photons, electrons and positrons can be produced and a set of detectors is designed to measure their multiplicities and energies. 
\newline
The main aims of the LUXE experiment are:
\begin{itemize}
    \item  measure the interactions of real photons with electrons and positrons [BEATE, BEN PLEASE CHECK: ELECTRONS AND POSITRONS OR ELECTRONS AND PHOTONS?]at field strengths where the coupling to charges becomes non-perturbative;
    \item make precision measurements of electron-photon and photon-photon interactions in a transition from the perturbative to the non-perturbative regime of quantum electrodynamics (QED);
   \item use strong-field QED (SFQED) processes to design a sensitive search for new particles beyond the Standard Model that couple to photons.
\end{itemize}

QED has been tested to a very high precision in systems with weak electromagnetic (EM) fields. For example, precision measurements of the electron anomalous magnetic moment \cite{Hanneke_2011} agree with the predictions of QED \cite{Aoyama:2019ryr} to an accuracy of around one part in a billion. However, in strong EM fields, QED predicts many phenomena that are yet to be confirmed experimentally. One reason is the high value of the natural EM field strength scale occurring in QED, the Schwinger Limit: $\mathcal{E}_{\textrm{cr}}=m^{2}c^{3}/(e\hbar)=1.32\times 10^{18}\,\textrm{Vcm}^{-1}$, which is currently orders of magnitude above any terrestrially producible field strength. However, in the rest frame of a high-energy probe charge, the EM field strength $\mathcal{E}$ is boosted by the Lorentz factor, $\gamma$, to $\mathcal{E}_{\ast}=\gamma \mathcal{E}(1+\cos\theta)$ where the collision angle at LUXE is $\theta=17.2\;\textrm{degrees}$. In this way, by colliding the $16.5\,\textrm{GeV}$ \euxfel electron beam with intense photon pulses produced by the laser, the electron rest-frame field at LUXE can reach and exceed the Schwinger Limit and hence strong-field QED phenomena can be accessed.
\newline
The implementation of this project greatly expands the scope of the E144 experiments, performed at SLAC in the 1990's \cite{Bamber:1999zt}, leveraging on the huge progress of high-power laser and accelerator technologies in the last three decades.
\newline
QED in intense EM fields \cite{Fedotov:2022ely}, such as will be probed at LUXE, can arise in numerous settings. In astrophysics pair creation can accompany gravitational collapse of black holes \cite{Ruffini:2009hg} and affect the propagation of cosmic rays \cite{nikishov62}. Some neutron stars are so strongly magnetised, that their magnetospheres probe the Schwinger limit \cite{Kouveliotou:1998ze,Harding_2006,Turolla:2015mwa}. In particle physics, in beam-beam collisions at future high-energy lepton colliders, strong-field effects are expected to feature prominently \cite{yakimenko2019prospect,Bucksbaum:2020}, and probing of the Coulomb field of heavy ions can be sensitive to strong-field effects \cite{Akhmadaliev:2001ik}. Strong fields, albeit in non-relativistic systems where the field strength scale is set by the ionisation potential, are the target of much investigation in the atomic and molecular physics communities (see e.g. \cite{ivanov}).
\newline
%
What separates SFQED phenomena apart from regular QED is the dependency on the dimensionless charge-field coupling. In a plane wave EM background, which approximates well the situation in a laser pulse as will be tested by LUXE, this coupling can be described with the classical nonlinearity parameter $\xi=|e|\mathcal{E}_{L}\lambdabar_{e}/\hbar \omega_{L}$: the work done by the EM field over a Compton wavelength in units of the EM field photon energy ($|e|$ is the charge of a positron, $\lambdabar_{e}$ the reduced Compton wavelength of an electron and $\hbar\omega_{L}$ the energy of a laser photon). Therefore, $\xi$ quantifies how many laser photons interact with the charge in a given QED process, with the probability of $n$ laser photons scaling as $\sim\xi^{2n}$. In weak fields, probabilities of QED events scale as $\sim \xi^{2}$, with higher-order interactions with the background being suppressed. But clearly when $\xi \sim O(1)$, this perturbative hierarchy breaks down, and all numbers of interactions between the charge and laser background must be taken into account. Hence in sufficiently strong fields, the probability of processes depend in a  non-perturbative way on the EM field. This parameter is sometimes referred to as the `intensity parameter', because it can be written $\xi = \sqrt{I_{L}/I_{\textrm{cr}}}(m_e c^{2}/\hbar \omega_{L})$, where $I_{L}/I_{\textrm{cr}}$ is the ratio of the laser intensity to the intensity of a field at the Schwinger limit and $m_e$ is the electron mass. 
\newline
\newline
\subsection{The nonlinear Compton Process}
A key target process of the LUXE experiment is nonlinear (inverse\footnote{The process is the ``nonlinear inverse Compton process'' but in the field it is commonly called the ``nonlinear Compton process''.}) Compton (NLC) scattering, depicted in Fig.~\ref{fig:NLCdiag}, where an electron or positron absorbs $n$ optical photons, $\gamma_L$, from the laser background and converts them into a single, high-energy gamma photon:
\[
e^\pm +n\gamma_{L} \to e^{\pm} + \gamma.
\]
This process has a classical limit. How much QED deviates from the classical limit, is in part quantified by the `quantum nonlinearity parameter', $\chi$, which for an incident electron can be written as $\chi_{e} = \mathcal{E}_{\ast}/\mathcal{E}_{\textrm{cr}}$ i.e. the ratio of the laser EM field, in the rest frame of the electron, to the Schwinger limit.  
\begin{figure}[ht]
   \centering
   \includegraphics*[width=6cm]{figures_chapt2/NLC1b.eps}
   \caption{The nonlinear Compton process. Left: an electron `dressed' in the laser background (double solid lines) emits a single high energy photon, $\gamma$. Right: a sum of Compton processes where the electron interacts with $n$ laser photons $\gamma_{L}$ (dashed lines), and emits a single high energy photon. 
   \label{fig:NLCdiag}}
\end{figure}
The magnitude of nonlinear and quantum effects, can be clearly seen in the position of the `Compton edge' \cite{Harvey:2009ry} in electron and photon spectra, where $\chi$ quantifies the electron recoil when it emits a photon. The ratio, $u$, of the photon energy to the incident electron energy at the Compton edge in nonlinear QED, nonlinear classical electrodynamics and linear QED respectively, is:
\[
u_{\textsf{\scriptsize nonlin.QED}} = \frac{2\eta}{2\eta + 1 + \xi^{2}}; \quad u_{\textsf{\scriptsize nonlin.class.}} = \frac{2\eta}{1 + \xi^{2}}; \quad
u_{\textsf{\scriptsize lin.QED}} = \frac{2\eta}{2\eta + 1},
\]
where $\eta=\gamma \hbar \omega_{L} (1+\cos\theta)/m_{e}c^{2}$ is the `energy' parameter (from the definitions above, it is easily seen that $\chi_{e} = \eta \xi$, so that the preceding expressions for $u$ can be written in terms of $\chi_{e}$).  For typical LUXE parameters around $\xi=1$, the position of the edge predicted by these three theories differs by $O(100\,\textrm{MeV})$. Therefore measurement of the position of the Compton edge allows quantum and nonlinear effects to be to differentiated.
\newline
\newline
\subsection{The nonlinear Breit-Wheeler Process}
Another key target process of the LUXE experiment, is nonlinear Breit-Wheeler (NBW) pair-creation:
\[
\gamma + n\gamma_{L} \to e^{+} + e^{-},
\]
depicted in Fig.~\ref{fig:NBWdiag}. This is a purely quantum effect with no classical analogue and hence requires the quantum nonlinearity parameter of the photon, $\chi_{\gamma}$, to fulfill $\chi_{\gamma}\sim O(1)$ in order to proceed, where $\chi_{\gamma} = (\mathcal{E}_{L}/\mathcal{E}_{\textrm{cr}})(\hbar \omega_{\gamma}/m_{e}c^{2})(1+\cos\theta)$; here $\hbar\omega_{\gamma}$ is the energy of the gamma photon and $\mathcal{E}_{L}$ is the laser field strength (both taken in the laboratory frame). Although linear Breit-Wheeler pair production was recently observed in Coulomb fields in heavy ion collisions \cite{STAR:2019wlg}, LUXE would provide the first observation of the nonlinear process in the non-perturbative regime, using real photons.
\begin{figure}[ht]
   \centering
   \includegraphics*[width=6cm]{figures_chapt2/NBW1.eps}
   \caption{The nonlinear Breit-Wheeler process. Left: a high energy photon $\gamma$ produces an electron-positron pair that is `dressed' in the laser background (double solid lines). Right: a sum of Breit-Wheeler processes involving $n$ laser photons $\gamma_{L}$ (dashed lines). 
   \label{fig:NBWdiag}}
\end{figure}
The non-perturbative nature of this process is exposed in the $\xi \gg 1$, $\chi_{\gamma} \ll 1$ limit, where the rate scales as:
\[
\Gamma_{\tiny\textrm{BW}} \propto \frac{\mathcal{E}_{L}}{\mathcal{E}_{\textrm{cr}}}\exp\left[-\frac{8}{3}\frac{m_e}{\omega_{\gamma}(1+\cos\theta)}\frac{\mathcal{E}_{\textrm{cr}}}{\mathcal{E}_{L}}\right],
\]
and we recall the charge-field coupling $\xi \propto \mathcal{E}_{L}$. The Breit-Wheeler rate has a similarity to the Schwinger process in a static electric field $\mathcal{E}_{S}$ (see e.g. \cite{Hartin:2018sha})
\[
\Gamma_{\tiny\textrm{S}} \propto \left(\frac{\mathcal{E}_{S}}{\mathcal{E}_{\textrm{cr}}}\right)^{2}\exp\left[-\pi\frac{\mathcal{E}_{\textrm{cr}}}{\mathcal{E}_{S}}\right].
\]
\newline
\newline

\subsection{The nonlinear Trident Process}
Another target process of LUXE is the nonlinear trident process, depicted in Fig.~\ref{fig:tridentDiag}, which combines a nonlinear Compton step and a nonlinear Breit-Wheeler pair-creation step off the radiated photon:
\[
e^{-} + n \gamma_{L} \to e^{-} + \gamma \qquad \textrm{and} \qquad \gamma + n'\gamma_{L} \to e^{+} + e^{-},
\]
where the number of background laser photons in the Breit-Wheeler step, $n'$, will in general be different to the number of photons involved in the Compton step, $n$. 
\begin{figure}[ht]
   \centering
   \includegraphics*[width=3cm]{figures_chapt2/triT1.eps}
   \caption{The nonlinear trident process. Double lines represent electrons and positrons dressed in the laser background.
   \label{fig:tridentDiag}}
\end{figure}
Although this process was measured in the E144 experiment \cite{Burke:1997ew}, it was done in the perturbative, multiphoton regime. LUXE will measure this in the non-perturbative, all-order regime, as a test of SFQED. In order to achieve this, a new approximation framework has been developed around  locally monochromatic rates \cite{Heinzl:2020ynb}, which have been built into a bespoke numerical simulation code called \textsc{Ptarmigan} \cite{ptarmigan} that models the laser interaction point and was rigorously benchmarked with direct calculations from QED \cite{Blackburn:2021rqm,Blackburn:2021cuq}.
\newline
\subsection{Beyond the Standard Model}
There is significant experimental evidence for new physics beyond the Standard Model \cite{McCullough:2018knz,Strategy:2019vxc}. Possible explanation of these experimental signals includes the existence of new, light degrees of freedom, which are weakly coupled to the Standard Model and potentially long-lived. Axion-like particles (ALPs), which are generalisations of the posited axion that solves the strong-CP problem \cite{Peccei:1977hh, Peccei:1977ur, Wilczek:1977pj, Weinberg:1977ma}, can couple to two photons and hence produce a signal in the LUXE experiment. A `secondary production' mechanism will be used, which involves using high-energy photons generated via the nonlinear Compton process, propagating downstream to a beam dump, in which ALPs can be created (via the Primakoff effect) and then decay on the other side of the dump to two photons, see Fig.~\ref{fig:BSM}. A detector is then placed to detect the photons, reject backgrounds due to e.g. neutrons and to measure the energies and angles of the photons. This aspect of LUXE is called LUXE-NPOD  (LUXE New Physics search with Optical Dump)
and described in more detail in Ref.~\cite{Bai:2021dgm}. 

\begin{figure}[ht]
   \centering
   \includegraphics*[height=4.2cm]{figures_chapt2/BSMDetector_pointing_upper.png}
   \caption{Schematic drawing of Compton photons hitting the beam dump. A small fraction of them may be converted to ALPs which then may decay again to two photons.
   \label{fig:BSM}}
\end{figure}

It will be sensitive to the pseudoscalar ALP couplings in the region of $10^{-5}\,\textrm{GeV}^{-1}$ for pseudoscalar masses around $\sim 200\,\textrm{MeV}$, a parameter space as yet unexplored by running experiments. It also presents a novel and complementary way compared to classic dump experiments, e.g. compared to dumping the electron beam directly this method results in significantly lower backgrounds. 
\newline
\subsection{Expected Particle Spectra}
The \textsc{Ptarmigan}~\cite{ptarmigan} MC generator is used to predict particle rates and spectra for the purpose of optimising the design of the experiment. Fig.~\ref{fig:rates} shows the number of particles produced in the Compton and Breit-Wheeler processes. The parameters for the figures are the same as those in Tables~\ref{tab:xfelepara} and~\ref{tab:laser} with the exception of the bunch length which was assumed to be of 40~$\mu$m instead of $5-10$~$\mu$m. The impact on physics observables of interest is at most 25\%.

\begin{figure}[ht]
   \centering
   \includegraphics*[width=0.45\textwidth]{figures_chapt2/TDR_5_5_part1.pdf}
   \includegraphics*[width=0.48\textwidth]{figures_chapt2/TDR_5.8_Npositrons_xi.pdf}
   \caption{Left: Number of electrons and photons in \elaser collisions as function of $\xi$. Right: Number of positrons in \elaser and \glaser collisions as function of $\xi$. Shown are the expected results based on \textsc{Ptarmigan} for two phases (\phaseone and \phasetwo) of the experiment that differ by the laser power, see Sec.~\ref{sec:laser}.
   \label{fig:rates}}
\end{figure}

The energy spectra for electrons and photons predicted by \textsc{Ptarmigan} for the Compton process for the LUXE parameters are shown in Fig.~\ref{fig:elspec} for various values of $\xi$. At low $\xi$ the Compton edges are clearly visible. With increasing $\xi$ they become less and less pronounced and the electron energy spectrum extends to lower energies and, correspondingly, the photon energy spectrum extends to higher energies. The goal is to measure both the electron and the photon energy spectra and to determine the position of the edges.

\begin{figure}[ht]
   \centering
   \includegraphics*[width=0.48\textwidth]{figures_chapt2/TDR_5.6_electron_spectrum.pdf}
   \includegraphics*[width=0.48\textwidth]{figures_chapt2/TDR_5.6_photon_spectrum.pdf}
   \caption{Electron and photon energy spectra for the Compton process in the \elaser mode for four values of $\xi$ in \phaseone. The distributions are normalised per bunch crossing.
   \label{fig:elspec} }
\end{figure}

Fig.~\ref{fig:posspec} shows the energy spectra of positrons, resulting from the Breit-Wheeler process, for the \elaser and \glaser modes. The detectors are designed to reconstruct these spectra with good precision. \newline

\begin{figure}[ht]
   \centering
   \includegraphics*[width=0.48\textwidth]{figures_chapt2/TDR_5.9_photon_energy_elaser_BKmodified.pdf}
   \includegraphics*[width=0.48\textwidth]{figures_chapt2/TDR_5.9_photon_energy_gamma_BKmodified.pdf}
   \caption{Positron energy spectra for the Breit-Wheeler process in the \elaser mode (left) and the \glaser mode (right) for two values of $\xi$ in \phaseone. The distributions are normalised to equal area.
   \label{fig:posspec}}
\end{figure}

\section{European XFEL Accelerator}
A very high-quality electron beam with a design energy of up to $\sim 17.5$~GeV is delivered by the linear accelerator of the European XFEL (\euxfel\!\!). The \euxfel has been operating since 2017. 

The beam consists of bunch trains which contain up to 2700 individual bunches, and the rate of bunch trains is normally 10~Hz. Only one of the bunches within a train will be used for the LUXE experiment as the laser operates with a frequency of 1~Hz only (the other 9~Hz will be used to measure the backgrounds). The properties of the individual bunches at the LUXE interaction point (IP) are summarised in Table~\ref{tab:xfelepara}. For the purpose of this document, electron beam energies of 16.5 and 14.0~GeV are assumed. For LUXE, the higher the energy the better but it is also interesting to perform the measurement at several energies. The accelerator is designed for a bunch charge of 1~nC but mostly operates at 0.25~nC, corresponding to $1.5\times 10^9$ electrons. 

\begin{table}[htbp]
\begin{center}
\begin{tabular}{l|r}
Parameter          & Value \\ \hline
Beam Energy [GeV]  & $16.5$\\
Bunch Charge [nC]  & 0.25   \\ 
Repetition Rate [Hz]    & 10 \\ 
Spotsize at the IP [$\mu$m]        & $5-20$  \\ 
Bunch length [$\mu$m]        & $5-10$  \\ 
Normalised projected emittance [mm mrad] & 1.4 \\
Energy spread $\delta E/E$ (\%) & 0.1\\
%Physics data taking time [$10^7$s per year] & $1.3$ & $0.25$, $0.50$\\ \hline
\end{tabular}
\caption{Electron beam parameters for the \euxfel as assumed for the design of the LUXE experiment. The electron beam spot size at the LUXE interaction point IP can be adjusted. The bunch length is expected to be about 5-10~$\mu$m, depending on the bunch charge and electron energy.
\label{tab:xfelepara}}
\end{center}
\end{table}

The electron bunch for LUXE is extracted with a fast kicker magnet and then directed towards an annex of the XS1 building where the LUXE experiment can be housed. A sketch of the \euxfel fan and the end of the LINAC is shown in Fig.~\ref{fig:XFEL_sketch}. The red circle indicates the location of the XS1 building. 

\begin{figure}[ht]
   \centering
   \includegraphics*[height=4.2cm]{figures_chapt2/XFEL_position.png}
   \caption{Schematic drawing of the \euxfel fan. The location foreseen for the extraction of the beam for the LUXE experiment is circled in red. The SASE1, SASE2 and SASE3 undulators and the experimental hall are also shown.
   \label{fig:XFEL_sketch}}
\end{figure}

The 2022 operations schedule of the \euxfel is shown in Fig.~\ref{fig:euxfelops} for illustration. Previous years (except 2020 which was impacted by the COVID19 pandemic) were comparable. 

\begin{figure}
    \centering
    \includegraphics*[width=0.9\textwidth]{figures_chapt2/OAO_2022_new.png}
    \caption{Operations Schedule of the \euxfel for 2022.}
    \label{fig:euxfelops}
\end{figure}

It is seen that in 2021 the winter shutdown extends over about two months (including the break during the holiday season) and there is another 2-week shutdown in the summer during which there is access to the experimental area of LUXE. Otherwise, there are short access opportunities on Mondays during which short access is possible. In total, there are 28 weeks of photon delivery in 2021 at three different energies: 16 weeks at $E=14$~GeV, 6 weeks each at $E=11.5$~GeV and  $E=16.5$~GeV. 

Another aspect to consider is the fraction of time where stable physics data taking is possible. In 2021 (which again is representative also for other years) the facility delivered photons to the photon science experiments for 4032 hours ($1.45\times 10^7$s). A breakdown of the hours of the facility is shown in Fig.~\ref{fig:euxfelhour}


\begin{figure}
    \centering
    \includegraphics*[width=0.9\textwidth]{figures_chapt2/XFEL_Hours_2021}
    \caption{Operational modes of the \euxfel accelerator and the number of hours spent in each mode in 2021. Stable physics running corresponds to ``X-ray delivery''. Source: European XFEL Annual Report 2021}
    \label{fig:euxfelhour}
\end{figure}

%\begin{table}
%\begin{center}
%\begin{tabular}{l|r}
%Operations Mode          & Hours in 2019\\ \hline
%Scheduled downtime  & 2280\\
%Setup, tuning, unscheduled & 1176   \\ 
%Facility development   & 1656 \\ 
%Photon delivery        & 3648  \\ 
%Total operating & 6480 \\
%%Physics data taking time [$10^7$s per year] & $1.3$ & $0.25$, %$0.50$\\ \hline
%\end{tabular}
%\caption{Operational modes of the \euxfel accelerator and the %number of hours spent in each mode in 2019. Stable physics running %corresponds to ``photon delivery''.
%\label{tab:euxfel19}}
%\end{center}
%\end{table}

Based on this past performance, we assume that LUXE will have an opportunity for physics data taking for $1.3\times 10^7$~s, and considering a data taking efficiency of LUXE of 75\% and a similar splitting between the various energies as in 2021, about $5\times 10^6$~s are provided at $E_e=14$~GeV and $2\times 10^{6}$~s at $E_e=16.5$~GeV. Data will also be taken at $E=11.5$~GeV but no  simulations of the QED processes for LUXE have yet been performed at this energy.

Furthermore we assume that normally we have a two-week access each year in the summer period and an access of 4-6 weeks each year in the winter period. Additionally, in 2025 there is a six-month shutdown planned during which a variety of work will be performed at the \euxfel facility. Among the plans is the construction of the beam extraction for the 2nd fan of the European XFEL, which LUXE can benefit from until the 2nd fan construction commences in about 2030. 

\section{Laser and Diagnostics}

As it shall be detailed in Chapter 3, the laser will be installed in a small building at the ground level, directly above the beam extraction tunnel. A Titanium Sapphire laser with a wavelength of 800~nm and a pulse length of 25-30~fs will be used. Initially a laser with 40~TW power will be utilised (termed ``phase-0''), and in a later phase it will be upgraded to 350~TW (``phase-1'').

\textbf{The paragraph below needs revision by Ben and Beate}

The polarisation of the laser will normally be linear. However, at present, calculations for linear polarisation are not yet fully available and thus the physics prospects shown are based on the assumption of circular polarisation unless otherwise stated. A discussion of the impact can be found in Ref.~\cite{luxecdr}.

\textbf{The paragraph above needs revision by Ben and Beate}

The laser beam will be transported down to the experimental area to an interaction chamber via a pipe with a diameter of 45~cm. Inside the interaction chamber it will be focused tightly to a waist $w_0$ (the FWHM of the laser) between 3 and 150~$\mu$m, depending on the $\xi$ value targeted. Inside the chamber the laser photons cross the electron beam at an approximate angle\footnote{The exact angle will depend upon the choice of off-axis parabola.} of 20$^\circ$ and with a repetition rate of 1~Hz. 

A summary of the laser parameters and expected $\xi$ and $\chi$ values is presented in Table~\ref{tab:laser}. Fig.~\ref{fig:megaplot} shows the $\xi$ and $\chi$ values that can be accessed at LUXE at the various beam energies.

\begin{table}[ht]
\begin{center}
\begin{tabular}{|l|c|c|}
\hline
\textbf{Laser parameters} &  phase-0 & phase-1\\
\hline
%&  \\ 
%  \textbf{Laser energy after compression (J)}  & 1.2 & 1.2 & 9 \\
Fraction of ideal Gaussian intensity in focus (\%) & \multicolumn{2}{c|}{50}\\   
Laser central wavelength (nm) & \multicolumn{2}{c|}{800}\\
Laser pulse duration (fs)  & \multicolumn{2}{c|}{25-30}\\  
Laser focal spot waist $w_0$ ($\mu$m)  & \multicolumn{2}{c|}{$\geq 3$} \\ 
    Laser repetition rate (Hz) & \multicolumn{2}{c|}{1- 10}\\  
   Electron-laser crossing angle (rad)  &  \multicolumn{2}{c|}{0.35}\\  
   \hline
Laser energy after compression (J) & 1.2 & 10 \\
Laser power (TW) & 40 & 350 \\
Peak intensity in focus ($\times10^{20}$~W/cm$^{2}$)  & $< 1.33$ & $\leq 12$ \\  
    Dimensionless peak intensity, $\xi$ &  $<7.9$ &  $<23.6$\\   
     \hline
      \multicolumn{3}{c}{}   \\
      \hline
    \textbf{Quantum parameter} & phase-0 & phase-1\\  
 \hline
    $\chi_e$ for $E_e=14.0$~GeV  &  $<1.28$ &  $<3.77$\\ 
    $\chi_e$ for $E_e=16.5$~GeV  &  $<1.50$ &  $<4.45$\\  
    \hline
    \hline
\end{tabular}
\vspace{1.2cm}
\caption{Laser parameters for the two phases of the LUXE experiment, and the quantum parameter $\chi_e$ is given for two different electron energies. All values are for circular polarisation with peak field parameters $\xi$ and $\chi$ increasing by a factor of $\sqrt{2}$ for linearly polarised laser irradiation. For focal spot the lowest value targeted is given, and the peak intensity ($\xi$ and $\chi_e$) values given correspond to this waist value. The laser pulse is expected to be Gaussian in all three dimensions in the focal point. The laser is expected to operate at 1 Hz repetition rate, a 10 Hz repetition rate is in principle available at lower intensities.}\label{tab:laser}
\end{center}
\end{table}

\begin{figure}[t]
    \centering
    \includegraphics*[width=0.9\textwidth]{figures_chapt2/chivsxi_nochiline.png}
    \caption{Quantum parameter $\chi$ versus the laser intensity parameter $\xi$. The blue lines show the values accessible at the LUXE experiment for three different energy values of the \euxfel accelerator. Also shown are previous (E144 \cite{Bula:1996st,Burke:1997ew}, Astra-Gemini  \cite{Cole:2017zca,Poder:2018ifi}) and planned (E320 and ELI-NP) experiments [BEATE, BEN: REFERENCES FOR E320 AND ELI-NP?].}
    \label{fig:megaplot}
\end{figure}

The laser will be synchronised with the electron beam via a system~\cite{Synchroxfel,Schulz} developed by DESY for the synchronisation of lasers used by the so-called ``pump and probe'' experiments at the \euxfel\!\!. The system designed at DESY has demonstrated the stable synchronisation of two RF signals to better than 13~fs, compared to a requirement of 25~fs given the electron and laser bunch lengths and their relative collision angle of $20^\circ$.

In addition, an elaborate diagnostics system has been designed with the goal to characterise the intensity to better than 1\% relatively (shot by shot) and 5\% absolutely. It relies on a variety of devices that measure the energy, fluence and other properties of the laser beam. The diagnostics is based on the beam after the interaction. A sketch of the diagnostics is shown in Fig.~\ref{fig:laserdiag}. 


\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.9\textwidth, angle=0]{figures_chapt2/diag_full_setup2.png}
    \vspace{1.2cm}
    \caption{Schematic diagram of the proposed intensity tagging diagnostics. The laser beam will be  attenuated and imaged on the return path to the diagnostics. (a) Layout of the laser shot tagging diagnostics in the laser area. (b) Focus diagnostic for the spot size measurement at the interaction point. (c) Set-up for an \textit{in situ} laser intensity measurement at the IP. }
    \label{fig:laserdiag}
\end{figure}

\label{sec:laser}

%\printbibliography[heading=subbibintoc]
%\end{refsection}

\newpage
\section{LUXE detectors}

The LUXE experiment is designed to analyse electron-laser and photon-laser interactions that occur at the interaction point inside the interaction chamber. Furthermore, it is also planned to use it for searches of axion-like particles resulting from photons interacting in the photon beam dump via the Primakoff effect. However, this latter part of the experiment is not yet as advanced and is considered an upgrade that will be installed at a later point, see Ref.~\cite{luxecdr}. Here, only the setup relevant to the studies of the QED interactions is discussed.

In order to fully characterise these interactions it is necessary to measure the multiplicities of particles produced as well as their energy spectra. The particles of interest are electrons, photons and positrons and the fluxes of these particles vary strongly depending on the running mode and the location. In general, the experiment is designed such that it has redundancy in many of the measurements which will allow cross-checks and cross-calibrations between the different approaches. A full simulation of the experimental area was performed with \geant to decide on the technologies for the detectors. A more elaborate discussion of the rates of signal and background can be found in Sec.~5.3 of the CDR~\cite{luxecdr} and in Chapters 3 to 10 of this TDR.
%and in the  notes~\cite{luxenotescin,luxenotecher,luxenotetrk,luxindividual &technicalenotecalo,luxenotegpr,luxenotegsp,luxenotebsc}. 

A sketch of the layout of the experiment for the \elaser and the \glaser modes are shown in Fig.~\ref{fig:layoutdet}. 

\begin{figure}[htbp]
\centering
\includegraphics[width=0.48\textwidth]{figures_chapt2/detector_conceptual_layout_trident_color_wide_with_BSM.pdf} 
\includegraphics[width=0.48\textwidth]{figures_chapt2/detector_conceptual_layout_bppp_color_wide.pdf} 
\caption{Schematic layouts for the \elaser and \glaser setup. Shown are the magnets, detectors and main shielding and absorbing elements.[BEATE AND BEN: IN THE GAMMA-LASER SETUP SHOULD THE $e^{-}$ DETECTOR BE IDENTIFIED AS CALICE INSTEAD OF TBD?] ] %The gamma profiler not shown, it is envisaged at the location of the last shielding before the backscattering calorimeter, see Fig. \ref{fig:fig1_gammaray_spectrometer}.
} 
\label{fig:layoutdet} 
\end{figure}
There are three separate areas in the LUXE experiment that are required for the strong-field QED aspects of the research program:
\begin{itemize}
    \item Target area: this area is only relevant for the \glaser mode. A target chamber is installed for the purpose of converting the electron beam to a photon beam either via bremsstrahlung on a tungsten target or via inverse Compton scattering [IS INV. C. SCATT. DESCRIBED IN ANOTHER TDR CHAPTER??] on a low-intensity laser beam. Behind the target chamber there is a dipole magnet to separate electrons, photons and positrons. A scintillation screen and camera and a Cherenkov detector is installed to measure the electron flux which can be used to reconstruct the energy spectrum and measure the flux of electrons after the bremsstrahlung process. In the \elaser mode the magnet is turned off and the electrons proceed to the IP. 
    
    \item IP Area: at the IP, electrons, positrons and photons are expected to be produced. Behind the IP there is a dipole magnet to separate these three particles physically in the horizontal plane. Behind the magnet on the left-hand side ($x>0$, the ``positron side''), for both the \elaser and \glaser setup there is a system to measure the number of positrons and their energy spectrum. It consists of a tracker~\cite{luxenotetrk} and a calorimeter~\cite{luxenotecalo}. On the right-hand side ($x<0$, the ``electron side''), in the \elaser case there is a scintillator screen with a camera~\cite{luxenotescin}and a Cherenkov detector ~\cite{luxenotecher}. The positron rates vary between $10^{-4}$ and $10^4$ per bunch crossing, and thus the technology chosen must be able to achieve an excellent background rejection (ideally $<10^{-3}$ per bunch crossing) to facilitate measurements at very low multiplicities, and achieve a good linearity at high multiplicities. A tracker followed by a calorimeter was chosen as these technologies are adequate for such particle multiplicities and are very effective at reducing backgrounds from stray secondary and tertiary particles. On the electron side the particle flux is much higher for the \elaser setup and can reach values as high as $10^9$ per bunch crossing. Therefore the technologies used here are designed to be adequate for such high fluxes. It is important that the position resolution in these detectors is high so that the energy resolution is better than 2\% in order to be able to resolve the Compton edges, see Ref.~\cite{luxenotecher}. The technologies chosen are Cherenkov detectors and scintillation screens. 
    
    In the \glaser case, we expect $e^+e^-$ pairs to be produced with fluxes between $10^{-4}$ and $\sim 10$ $e^\pm$ per BX. Thus, here a tracker and a calorimeter is used on both the positron and the electron side. Due to the low multiplicity of electrons and positrons it is possible to combine the electron and positron and thus reconstruct the energy of the initial photon event by event.  
    \item Photon Area: any photons that are produced at the IP in the \elaser mode (the Compton photons) or that fly through the IP area undisturbed in the \glaser mode end up in the photon detection system which is designed to measure the photon flux, angular and energy spectrum. The energy spectrum is determined using  a \textit{Gamma Spectrometer}~\cite{luxenotegsp} consisting of a small tungsten target which converts photons to $e^+e^-$ pairs, a dipole magnet that separates them, and two scintillation screens (with cameras) that measure the electron and positron energy spectra. It is followed by a \textit{Gamma Profiler}~\cite{luxenotegpr}, made up of two sapphire strip detectors which are designed to measure the size of the photon beam in the horizontal and transverse direction. For a linearly polarised beam the photon spot size in the two planes can be used to get an independent measurement of $\xi$. The sapphire detector granularity is chosen such that this can be obtained for each shot with a precision of 5\%. Finally there is a \textit{Gamma Flux Monitor}~\cite{luxenotebsc}, which consists of lead-glass calorimeter blocks that were originally designed for the HERA-b experiment but were never used there. It will measure the overall photon flux and also serve as a type of luminosity monitor as the photon flux is a very good measure of the overlap between the electron beam and the laser for the \elaser setup. The Gamma Profiler and the Gamma Spectrometer are also sensitive to the photon flux. 
\end{itemize}

Three beam dumps are required to dump the electron or photon beams. They are designed to reduce back-scattering in the IP and photon area sections where signal particle rates are low. Furthermore, shielding components are placed to further reduce the background radiation based on a full simulation of the experimental area with the \geant program~\cite{Allison:2006ve, Allison:2016lfl}.

A common data acquisition system is used. For 10~Hz of data taking, the data rate is about 200 MB/s and is dominated by the scintillation screens. The readout of each detector and of each laser diagnostic is controlled by a dedicated PC which is connected to a central ``Trigger Logic Unit'' (TLU), which was developed within the EU AIDA-2020 project, which receives a clock from the \euxfel accelerator and distributes the signal to the detectors and the laser. A central PC receives data from the TLU and builds the events and enables monitoring of the data. The data are then written to tape storage. 

The LUXE experiment is very modular in that it consists of a series of independent pieces which are readily accessible when access to the tunnel is allowed. It is thus possible to stage the installation, depending on when a given detector piece is needed and/or ready. For all components, it is foreseen that the installation is prepared and tested very well on the surface ahead of time so that the time needed for installation in the tunnel is minimised. 

The readout boards are mostly placed in a counting room on the 2nd floor that is accessible during \euxfel operation.

Given the possible uncertainties on the time scales on which all the detectors can be ready, it is prudent to consider a \textit{minimal} version of the LUXE experiment which could be ready for first data. A conceptual sketch of such a minimal version is shown in Fig.~\ref{fig:luxebare}.

\begin{figure}[htbp]
\centering
\includegraphics[width=0.48\textwidth]{figures_chapt2/detector_conceptual_layout_barebones_color_wide.pdf} 
\includegraphics[width=0.48\textwidth]{figures_chapt2/detector_conceptual_layout_barebones_color_wide_withtracker.pdf} 
\caption{Schematic layouts for a minimal (left) and a next-to-minimal (right) version of the LUXE experiment for the \elaser setup. Shown are the magnets, detectors and main shielding and absorbing elements. %The gamma profiler not shown, it is envisaged at the location of the last shielding before the backscattering calorimeter, see Fig. \ref{fig:fig1_gammaray_spectrometer}.
} 
\label{fig:luxebare} 
\end{figure}

This minimal version could be used for a first measurement of the Compton process via the measurement of the electron spectrum with the scintillation screen and/or Cherenkov detector. Additionally, the already existing prototype of the CALICE~\cite{Irles:2019ikz} calorimeter could be installed on the positron side and could be used to measure the number of positrons within the limited energy range of about $4-8$~GeV~\footnote{The existing prototype of the CALICE calorimeter is only 18~cm long and thus cannot cover the entire energy spectrum. However, it is planned to construct a 36~cm prototype by 2024 which could be used and would cover about 80\% of the spectrum.}. Additionally, the back-scattering calorimeter provides a measure of the photon flux. It is important to stress that such a minimal version is only able to cover a fraction of the LUXE physics programme but it would already allow some physics measurements, even if several detectors are delayed due to e.g.\! delayed delivery of components, missing resources or technical difficulties. However, both the physics scope and the precision will be very limited compared to the design shown in Fig.~\ref{fig:layoutdet} as discussed in Sec.~\ref{sec:physics}.

In principle, any scenario between the bare minimum and full version should be conceivable depending on the readiness of the components. For instance, if available, tracker half-layers could be installed in front of the calorimeter (see next-to-minimal version in Fig.~\ref{fig:luxebare}).

The data taking strategy needs to be optimised to achieve the best overall precision. For the Compton process the statistical uncertainties are negligible even for a single shot, since the number of electrons and photons exceed 1 million per shot (see Fig.~\ref{fig:rates}), yielding a 0.1\% statistical uncertainty. Thus these measurements can be made within minutes of data taking once the experiment is commissioned. For the Breit-Wheeler process the particles rates are significantly lower, and are $\ll 1$ at low $\xi \leq 2$, see Fig.~\ref{fig:rates}. Furthermore, the measurements of this process will be subject to a significant systematic uncertainty of 20-40\% due to the uncertainty on the laser intensity, see Sec.~\ref{sec:physics}. Therefore it seems reasonable to take data at a given laser intensity for a time period that allows a statistical uncertainty of better than 10\% to be achieved. Assuming no background, for \phaseone (\phasetwo) this can be achieved within a single day for $\xi\geq 1.5$ ($\xi\geq 1.2$). At lower $\xi$, it is important to collect statistics for an extended period of time. For instance a 30\% uncertainty at $\xi=1$ requires at least 10 days of data taking for \phaseone.   
Based on these consideration we assume that about 80\% of the data taking will be devoted to the low-$\xi$ region ($\xi<2$) and only 20\% to data taking at high $\xi$. 

At the highest $\xi$ values, the particle rates are actually rather too high than too low in the \elaser mode. Here, the rates can be reduced by large factors by defocusing the electron beam. For instance, by increasing the beam spot size in the transverse plane from 5 to 20~$\mu$m, at the highest $\xi$ the rate can be reduced by a factor of 10.

\section{Physics Prospects}
\label{sec:physics}

The \textsc{Ptarmigan} Monte Carlo event generator is used to assess the physics sensitivity of the experiment as described in Sec.~\ref{sec:theory}. Unless otherwise stated, it is assumed that the full experiment as shown in Fig.~\ref{fig:layoutdet} is available. 

Three important goals of the experiment are the measurement of the following observables as function of the $\xi$-parameter: i) the Compton edges; ii) the number of photons radiated per electron in \elaser collisions and iii) the rate of positrons in \glaser and \elaser collisions. 

The Compton edges are measured in the IP area on the electron side by the scintillation screen and the Cherenkov detector, and in the photon area by the Gamma Spectrometer~\footnote{In the Gamma Spectrometer the photon spectrum is inferred by inverting the measured energy spectra of electrons and positrons created by photon conversion.}. Examples of these reconstructed spectra are shown in Fig.~\ref{fig:elspec}. The edge is then identified based on a so-called finite-impulse-response-filter (FIR) method, which was proposed in the context of kinematic edge reconstruction at the International Linear Collider (ILC)~\cite{Tsai:1974}. The edge position as a function of $\xi$ is shown in Fig.~\ref{fig:resultscom} compared to the theoretical prediction of \sfqed, the linear (purely perturbative) QED prediction (Klein-Nishina formula) and the classical prediction (Thomson scattering). The Klein-Nishina prediction would yield a fixed value of 12~GeV for all $\xi$ while the full QED calculation increases versus $\xi$ approaching the classical prediction at high $\xi$. It is seen that a 2.5\% uncertainty in $\xi$ affects the Compton edge position by at most 0.5\%. The experimental uncertainties are expected to be about 2\% for the Compton edge position due to the uncertainty on the absolute energy scale.

Another interesting measurement is the relative fraction of photons radiated per electron versus $\xi$. As can be seen from the right-hand plot of Fig.~\ref{fig:resultscom}, whereas the leading-order perturbative result scales with $\xi^{2}$, the effect of the non-perturbative  coupling between the electron and the laser field can be seen as a suppression of the photon emission rate. Statistical uncertainties are expected to be negligible. The 2.5\% uncertainty on $\xi$ results in an uncertainty on the relative fraction of photons produced of up to 4\%. Thus the relative systematic uncertainty on the photon and electron flux normalisation should be kept below 2\% to avoid this being the dominant source. 

\begin{figure}[htbp]
\centering
\begin{minipage}[c]{0.45\textwidth}
\centering
\includegraphics[width=\textwidth]{figures_chapt2/ComptonEdgePlot1f.pdf}
%\includegraphics[width=0.9\textwidth]{fig/ComptonEdgePlot1eBar.pdf}
\includegraphics[width=0.9\textwidth]{figures_chapt2/ComptonEdgePlot1eBar2B.pdf}
%\caption{test}
%\label{fig:sample_figure}
\end{minipage}
\begin{minipage}[c]{0.45\textwidth}
\includegraphics[width=\textwidth]{figures_chapt2/Compton_Money_Plot_Errors_v2c.pdf}
\end{minipage}
\caption{Expected experimental results for the measurement of the Compton edge in the electron energy spectrum in \elaser interactions (left) and the ratio of the number of photons produced per electron as a function of $\xi$ (right). A 2.5\% uncertainty on $\xi$, corresponding to a 5\% uncertainty on the laser intensity, is illustrated in orange as uncertainty on the theoretical nonlinear QED prediction. The uncertainties on the data points illustrate a 2\% uncertainty on the electron energy scale. The predictions of the Klein-Nishina formula and a nonlinear classical predictions (Thomson scattering) are also shown. The bottom panels show the ratio to the central nonlinear QED prediction, and the uncertainty due to the uncertainty on $\xi$, and (on the right only) due to other uncertainties in the theoretical prediction.[BEATE AND BEN: MEANING OF THE "NUMBER OF CYCLES" IN THIS AND FOLLOWING FIGURE?]
} 
\label{fig:resultscom} 
\end{figure}

Another important measurement is the positron multiplicity versus $\xi$ for \glaser interactions. The goal is to observe Breit-Wheeler $e^+e^-$ production from collisions of real photons, and to measure the predicted non-perturbative effects at high $\xi$. 

Fig.~\ref{fig:resultsbw} shows the expected results for the Breit-Wheeler process. The left figure shows the theoretical prediction and illustrates the importance of the uncertainty on $\xi$. Due to the very steep dependence of the $e^+$ rate on $\xi$, a 2.5\% error in $\xi$ can lead to a 20\%-60\% error on the number of positrons measured (with the error increasing, for lower positron counts). 
The uncertainties represent those anticipated if there is an irreducible background of $0.01$ particles per BX and for each $\xi$ value 10 days of data taking are used. A correlated uncertainty on the prediction arises from a 2.5\% uncertainty on the absolute value of $\xi$ (see left figure). In addition an uncertainty shot-by-shot of 1\% on the laser intensity, corresponding to 0.5\% on $\xi$, will result in an uncorrelated error between the data points of about 10\% at low $\xi$ decreasing to about 5\% at high $\xi$. 


\begin{figure}[htbp]
\centering
\includegraphics[width=0.48\textwidth]{figures_chapt2/NBW_Money_Plot_Errors_v2b.pdf}
\raisebox{+0.2\height}{\includegraphics[width=0.48\textwidth]{figures_chapt2/glaser_err_ratio_bg001.png}}
\caption{Left: Number of positrons produced in \glaser collisions as a function of $\xi$ as expected in the full QED calculation (solid line) and in the purely perturbative calculation (dashed line). Also shown is the impact of a 2.5\% uncertainty on $\xi$ (wide orange band). The bottom two panels show the ratio to the full QED prediction to make the uncertainties visible (the blue band is the difference between the full QED theory calculation and simulation).
Right: Number of positrons produced in \glaser collisions as function of $\xi$, normalized by the laser waist for phase-0 and phase-1. The data uncertainties shown represent the statistical uncertainties corresponding to 10 days of data taking and a background of 0.01 particles per bunch crossing. Also shown is a 40\% correlated uncertainty to illustrate the impact of the uncertainty on $\xi$. [MEANING OF $\xi^{22}$ IN TOP LEFT? TICKS ON LOWER AXIS OF RIGHT SIDE?]} 
\label{fig:resultsbw} 
\end{figure}

A minimal LUXE experiment, as illustrated in Fig.~\ref{fig:luxebare},  would be able to measure the Compton edge, as shown in Fig.~\ref{fig:resultscom}, although likely the uncertainty on the theoretical prediction would be larger due to a less well-known laser intensity (since the Gamma Profiler cannot constrain it). And, the measurement could only be performed with electrons and not with photons due to a missing Gamma Spectrometer. It would also be able to measure the positron rate albeit in a restricted energy range and likely with a larger uncertainty due to inferior background rejection.

Fig.~\ref{fig:resultsextra} shows the expected positron rates in the \elaser mode in the restricted energy range compared to the full range, and also shows a comparison of the positron rates with the electron energy of 14~GeV versus 16.5~GeV. It is seen that the shape of the distribution is not changed significantly by reducing the positron energy range. The lower electron beam energy reduces the particle rates by factors of 5-10 depending on $\xi$. [E-LASER (PLOTS)  OR GAMMA-LASER (CAPTION)? ]

\begin{figure}[htbp]
\centering
\includegraphics[width=0.48\textwidth]{figures_chapt2/TDR_CALICE.pdf}
\includegraphics[width=0.48\textwidth]{figures_chapt2/TDR_16.5GeV_14.0GeV.pdf}
\caption{Left: Number of positrons produced in \glaser collisions as function of $\xi$ for a restricted energy range (CALICE: 4-8 GeV) and the full energy range. 
Right: Number of positrons produced in \glaser collisions as function of $\xi$ for an electron beam energy of 16.5~GeV compared to 14~GeV. 
%\BH{Note to reviewers: will update plots so they extend to lower xi and also show the relevant ratios.}
} 
\label{fig:resultsextra} 
\end{figure}

\section{Conclusion}
LUXE will pioneer a region of QED and be able to measure the transition from the perturbative to the nonperturbative regime in various observables. It makes use of the existing \euxfel accelerator electron beam and a high-intensity laser to study the strong-field regime which is relevant for a variety of astrophysical phenomena, atomic physics and future high energy electron accelerators. Detectors are designed to achieve a high signal efficiency and a good background rejection. Risks due to delays of components (during the difficult pandemic period) are mitigated by planning  for redundancy in the measurements and for a staged installation.

==> chapters/testgithub.tex <==
testitest
shelltestitest

==> chapters10/organisation.tex <==

\subsection{Human and financial resources}

In terms of human resources the project requires 0.5 FTE for engineering, 1.0 FTE of a technician and 1.5 FTE of a postdoc and physicist each, integrated over 3 years (2022 -- 2024) as detailed in Table~\ref{tab:fte}.
\begin{table}
    \centering
    \caption{Summary of the FTE foreseen for the construction and installation of the LUXE GFM.}
    \vspace{0.2cm}    
    \begin{tabular}{p{2.5cm}|p{1.5cm}|p{1.5cm} |p{1.5cm}|p{1.5cm} }
         Year & 2021 & 2022& 2023 & 2024\\\hline
         Employment & existing / to hire	& existing / to hire & existing / to hire	& existing / to hire\\\hline
         Engineers  & 0/0 &	0/0.5 &	0/0	& 0/0\\
         Technicians & 0/0 &	0/0	&0/0.5&	0/0.5\\
         Physicist & 	1/0	&0.5/0&	0.5/0&	0.5/0 \\
         Postdocs & 0/0	&0/0.5&	0/0.5&	0/0.5 \\
\hline
\hline
         Sum              & 1/0	&0.5/1&	0.5/1.0&	0.5/1.0 \\ 
        \hline
    \end{tabular}
    \label{tab:fte}
\end{table}

The budget for the construction of the GFM detector is estimated and summarised in Table~\ref{tab:cost}. The price for PMTs coupled with voltage dividers comes from Hamamatsu quotations and for laser diagnostics from the ThorLabs website. QF is a quality factor (see Appendix) which quantifies the level of confidence in a price estimate.

\begin{table}
    \centering
    \caption{Summary of the budget required for the construction of the LUXE GFM, based on cost estimates for the still missing components. In addition the quality factor for each component and the average QF in the last line are given.}
    \vspace{0.2cm}
    \begin{tabular}{ p{4.5cm}|p{1.9cm}|p{0.8cm}|p{3cm} }
        Component  & Cost (kEur) & QF &Comment\\\hline
         Mechanical frame & 5 & 5& DESY\\
         Lead Glass blocks  & free & 0 & Available\\
         8 PMTs, 8 voltage dividers & 12 &2 & For 1 or 2 PMTs the QU Fund could be used, for others - N/D \\
         CAEN V1730SB 16/8 Channel 14 bit 500 MS/s Digitizer & 15 & 0 & Available\\
         Diagnostic Laser diode and Laser driver, fibers & 10 & 3 & N/D \\ 
         DAQ hardware, power supplies, cables, PCBs & 5 & 1 &  HV is available, others - N/D \\
         Tooling    & 10&3 & DESY \\
\hline
\hline
         Sum              & 57 &   2 &        \\\hline
    \end{tabular}
    \label{tab:cost}
\end{table}

\subsection{Schedule and milestones}

The readiness for installation is planned for January 2024. But it can fit in all three LUXE scenarios.
The global milestones for the GFM are (Fig.~\ref{fig:GM_milestones}):

\begin{enumerate}
    \item Finalise the design by February 2022;
    \item Assemble a detector module prototype by August 2022;
    \item Test the advanced detector module prototype by the end of 2022;
    \item Assemble the full detector and install by the forth quarter of 2023;
    \item Commission by first quarter of 2024.
\end{enumerate}


\begin{figure}[ht!]
  \begin{center}
    \includegraphics[width=0.9\textwidth]{figures_chapt10/milestones181121.png}
      \end{center}
    \caption{Milestones and timeline for the GFM delivery and installation.}
    \label{fig:GM_milestones}
\end{figure}

\subsection{Risk management}
This section discusses the main risk factors, how/if they impact cost and/or schedule, their probability and how they are mitigated.  There are two dimensions, the impact and the probability. We separate the impact on the cost and on the schedule and use the following terms for impact risks:

\begin{itemize}
    \item Insignificant: Risk is easily mitigated by day to day process;
    \item Minor: Delays up to 10\% of the schedule. Cost increase up to 10\% of budget;
    \item Moderate: Delays up to 30\% of the schedule. Cost increase up to 30\% of budget; 
    \item Major: Delays up to 50\% of schedule. Cost increase up to 50\% of budget;
    \item Catastrophic: project abandoned.
\end{itemize}

The probability of a risk to be realised is quantified as, rare: ($<3$\%), unlikely (3--10\%), moderate (10--50\%), likely (50--90\%) or certain ($>90\%$). 

\begin{table}[]
    \centering
    \caption{Risk description for the GFM, potential impact on cost and schedule, probability to occur and strategy on how to mitigate the risk.}
\begin{tabular}{p{0.2\linewidth}|p{0.15\linewidth}|p{0.1\linewidth}|p{0.1\linewidth}|p{0.25\linewidth}}
         Description & Cost & Schedule & Prob. & Strategy\\\hline \hline
         Not radiation hard crystals &Insignificant &Minor &Moderate & Exchange-friendly design\\\hline
         Sub-optimal design identified in TB&Minor &Minor &Unlikely& Detailed simulation; use tested existing technologies wherever possible\\    \hline  
         Full detector: components failure&Insignificant &Minor &Unlikely & Develop components testing procedure in the lab before assembly. Design to provide for easy exchange of faulty elements.\\   \hline
         Full detector: design flaws&Insignificant &Minor &Unlikely& Detailed simulation; Build mechanical and technological prototypes in advance\\   \hline
         Installation, commissioning&Insignificant &Minor &Unlikely& Exchange-friendly design\\         
         \hline
         \end{tabular}
         \label{tab:risks}
\end{table}

Table~\ref{tab:risks} shows a summary of the risks. Considering the fact that the available crystals were stored for many years at a warehouse there was a risk, with potential high impact on schedule and cost, that because of ageing and/or sub-optimal storage they would not be in working conditions. This risk was mitigated in the recent lab and beam tests (see Section~\ref{sec:tests}).  Another risk is due to the lack of accurate information about the chemical composition of the lead-glass crystals and their radiation tolerance. Future beam-tests will clarify this aspect. The other risks mentioned in Table~\ref{tab:risks} can be easily mitigated and have no impact on the cost or schedule of the LUXE experiment.


\subsection{Responsibilities}
The responsibilities are shared by one senior physicist from KINR, Ukraine and the LUXE group at DESY. The work concerning simulation, \geant and MC, documentation, lab tests and beam-tests are the responsibility of the physicist from KINR and starting from 2022 also one postdoc employed by the LUXE team at DESY. 
In 2022 the engineering drawings of the detector (CAD model) will be produced with the help of an engineer from DESY.
To produce the supporting structure, technical support will be required but can be outsourced.
The help from technicians and the lab space at DESY will be needed to assemble the detector. 

==> chapters11/organisation.tex <==
\label{sec:organisation}

\subsection{Human and financial resources}

\subsubsection*{DAQ, DQM and slow control system costs}
The following human resources are required for delivery of the DAQ, DQM and slow control systems.  The costs associated with the DAQ hardware are given in Table~\ref{tab:cost}.

\begin{itemize}
    \item 0.2 FTE/yr physicist for oversight and communication with detector responsibles.
    \item 0.3 FTE/yr physicist/engineer for technical work, responsible for timing and synchronisation (TLU).
    \item 1 FTE/yr post-doc/engineer for DAQ software, EUDAQ2 (including DQM).
    \item 0.5 FTE/yr PhD student to support above, particularly software.
    \item Some effort for the DQM software is included in the full-time DAQ software post and some effort for the slow control system is included in the full-time common software post.  We therefore estimate that a further 0.5 FTE/yr physicist/engineer is needed to also work on the slow control and DQM systems for development and redundancy.
\end{itemize}

It is assumed that for completion of the DAQ system, the above effort is required for 3\,years.  Once data-taking starts, the above effort is expected to be reduced by 50\%.  Effort will be required for maintenance, new developments and on-call activities.  It is expected that data taking will be covered by a shift system and so expert help will not be constantly required.


\begin{table}[]
    \centering
    \caption{Cost estimates for the DAQ hardware. The comment discusses the source of the price.}
    \begin{tabular}{|l|c|c|c|l|}
        \hline
        Component  & Quantity & \vtop{\hbox{\strut Unit cost} \hbox{\strut (kEur)}} & \vtop{\hbox{\strut Total cost} \hbox{\strut (kEur)}} & Comment\\\hline
%%%        TLU & 4 & 4 & 16 & \vtop{\hbox{\strut From recent} \hbox{\strut production}}\\ \hline
        TLU & 15 & 3.3 & 50 & \vtop{\hbox{\strut From recent} \hbox{\strut production}}\\ \hline
        Fanout & 4 & 2 & 8 & --\\ \hline
        DAQ PC & 2 & 1 & 2 & PC costs\\ \hline
        Storage buffer & 1 & 20 & 20 & DELL website \\ \hline
    \end{tabular}
    \label{tab:cost}
\end{table}


\subsubsection*{Computing and software costs}
The following human resources are required for support of the common computing infrastructure and software:
\begin{itemize}
    \item 0.5 FTE/yr physicist for oversight, organisation of the procurement of storage and computing resources in conjunction with DESY IT, and communication with detector responsibles.
    \item 0.5 FTE/yr physicist/engineer to develop and maintain the LUXE simulation.
    \item 0.5 FTE/yr physicist/engineer for technical work on computing, grid, etc.
    \item 1 FTE/yr physicist/engineer for technical work on the common software. These responsibilities include for example the design, implementation and maintenance of a conditions database, and the maintenance of the combined positron reconstruction from the tracker and calorimeter inputs.
    \item 0.5 FTE/yr physicist/engineer dedicated to the development and maintenance of an overall software framework for the experiment.
\end{itemize}
The above effort is initially required for 3\,years until data taking starts.  At the start of data taking, a similar level of effort will be required, although it is expected that some aspects will be covered by PhD students. 

No costs are expected for the distribution of LUXE software, which will use freely-available public repositories\footnote{\url{https://github.com/LUXEsoftware}}. 

The expected costs for the storage of data and MC simulated events is summarised in Table~\ref{tab:computing_storage_costs}, assuming no compression for the data from the cameras and laser diagnostics.

The estimated cost for robust storage resources (i.e.\ backed-up disks or tapes) is of 50~\euro/TB on disk and 16.5~\euro/TB on tape. 

\begin{table}[hbt]
    \centering
    \caption{Size estimates for the various data formats per year of operation, assuming robust disk- or tape-based storage and the maximum event size for data events at a single site.}
    \def\arraystretch{1.2}
    \begin{tabular}{|l|c|c|c|}
        \hline
        Type of data                   & \vtop{\hbox{\strut Data size} \hbox{\strut (PB)}}  & \vtop{\hbox{\strut Disk cost} \hbox{\strut (kEur)}} & \vtop{\hbox{\strut Tape cost} \hbox{\strut (kEur)}} \\
        \hline
        Raw data (filled BX)           & 0.46      & --  & 7.8 \\
        Raw data (empty BX)            & 0.01      & --  & 0.2 \\
        Reconstructed data & 0.40   & 50  & -- \\
        \hline
        Simulated data (1:1 filled BX) & 0.54      & 70  & -- \\
        \hline
        Total                          & 1.42      & 120 & 8.0\\
        \hline
    \end{tabular}
    \label{tab:computing_storage_costs}
\end{table}



\subsection{Schedule and milestones}

The 3-year schedules for the DAQ system, DQM and slow control systems and the computing and hardware is shown in Fig.~\ref{fig:DAQ-schedule}.

\begin{figure}[hbt]
\centering
    \includegraphics[trim={1.5cm 11cm 5.cm 1.5cm},clip,width=0.99\textwidth]{figures_chapt11/Excel_timescales-detectors-forMatthew-includingDAQ-reorder_Mar2022_CorrectDataTaking.pdf}
    \caption{Schedule.}
    \label{fig:DAQ-schedule}
\end{figure}

%%% Computing milestones (to be included in the figure):
%%% \begin{itemize}
%%%    \item End 2022: Definition of RAW data byte-stream format for the LUXE detectors
%%%    \item 2022-2023: Design and implementation of data-taking conditions database 
%%%    \item End 2024: Procurement of initial storage resources
%%% \end{itemize}

\subsection{Risk management}

The major risk for each subject is given in Table~\ref{tab:risks} and discussed below.

It is expected that the simulation will undergo updates and improvements, even during data taking.  A risk is that the simulation is not of sufficient accuracy for the start of data analysis.  This will lead to possible delays in the first results and/or less precise measurements, but should not affect the start-up of the experiment.  To mitigate this, parts of the simulation need to be prioritised.

The main risk for the DAQ is that all systems are not fully integrated.  To try and ensure this does not happen, integration has started early, both testing in the lab and in beam tests.  The TLU has been used already by several detectors, as has EUDAQ2 and work continues.  Should this risk be realised, it would mean a slip in the schedule and the costs would be the extra effort needed to ensure integration is done within an extra 6\,months.  This may result in more work needed offline to ensure that the data is merged correctly.

The DQM and slow control monitoring require  software and the implementation of the checks within the software.  Delays in their operation may lead to delays in data taking or less efficient data taking as safe and continuous operation is not possible.

Computing risks are related to possible failures of computing hardware.  As the PCs, networks, etc.\ will make use of standard equipment, then (average) failure rates will be known and spares should be readily available.

The most important risk related to the software development affects the implementation of the detector condition database, which is required to be completed before the start of the data taking. Delays in the implementation might lead to loss, or poor quality of the reconstructed data.

Other minor risks affecting software development are related to the potential lack of a coherent software framework at the start of the data taking, because of the limited person power that will be available in this field. This can generally lead to poorly efficient workflows. The likelihood is considered to be relatively high. It is not expected to have an impact on the quality of the results released by the experiment, but rather on their timeliness.

\begin{table}[h]
    \centering
    \caption{Risk for the DAQ: description, potential impact on cost and schedule, probability to occur and strategy on how to mitigate the risk.}
\begin{tabular}{|p{0.22\linewidth}|p{0.12\linewidth}|p{0.1\linewidth}|p{0.12\linewidth}|p{0.3\linewidth}|}
         \hline
         Description & Cost & Schedule & Prob. & Strategy\\\hline
         Simulation not accurate & 0 kEUR & 0.0 & Moderate & Prioritise parts of simulation. \\ \hline
         Not all systems integrated in DAQ & 50 kEUR & 0.25 & Moderate & Start early.  May need extra integration offline. \\ \hline
         Slow control and/or DQM not ready & 50 kEUR & 0.25 & Moderate & Start early.  May need to do more manual checks. \\ \hline
         Conditions database not ready & 50 kEUR & 0.25 & Moderate & Start early. Decide on a minimum set of conditions. \\ \hline
         Integration in  software framework not complete & 0 kEUR & 0.0 & High & Choose well-known framework. \\
         \hline
         \end{tabular}
         \label{tab:risks}
\end{table}


\subsection{Responsibilities}

Each of the discussed activities has the following institutes taking responsibility for them.

\subsubsection*{DAQ, DQM and slow control systems}

\begin{itemize}
    \item \textbf{DAQ:} Primary responsibility lies with UCL, with contributions from DESY and also other institutes developing detectors.
    \item \textbf{DQM:} This is coordinated by UCL, with input from other institutes developing detectors.
    \item \textbf{Slow control:} Primary responsibility lies with DESY, with input from UCL.
\end{itemize}

\subsubsection*{Computing and software costs}

\begin{itemize}
    \item \textbf{Simulation:} The primary coordinating institute is DESY, but contributions are needed from sub-detector groups. 
    \item \textbf{Computing:} This is the responsibility of DESY.
\end{itemize}

==> chapters12/acknowledge.tex <==
The authors would like to thank..

==> chapters12/organisation.tex <==

\subsection{Human and financial resources}
\label{sec:ressources}
The human and financial resources are estimated assuming a schedule relative to the point in time $T_0$, where funding for the LUXE experiment is released, with more than three years until the experiment is ready for data-taking. No explicit assumptions are made about the schedule at which a long \euxfel shutdown could happen.\\

The cost model is made such that one separates core invest and material costs (in kEUR) and person power (in FTE) that is assumed to come from local resources (i.e. DESY groups, M or FH). The core invest estimates are based on (preliminary) quotes from vendors or on experience from experts at DESY. The estimates of the person power requirements come from experts. Overheads, escalation or contingency are not included. 

In the LUXE CDR~\cite{luxecdr}, different work packages were introduced to describe the deliverables needed by the experiment. The financial resources are based on a similar structure. Each estimate come with a confidence level index, 1 being the most reliable and 4 being the least reliable:

\begin{itemize}

      \item Confidence level 1:  Quote from a company

      \item Confidence level 2: Preliminary estimate from experts

      \item Confidence level 3: Preliminary estimate after consultation with experts

      \item Confidence level 4: Less reliable estimates, based on other methods

\end{itemize}      

%Table~\ref{TC:Annex:Resources_WP61} shows the financial resources for the workpackage 1.1, technical coordination - outside building, which summarises the costs associated to the new building and the infrastructure that will need to be constructed outside of XS1. 

%\begin{landscape}% Landscape page
%\begin{table}[h]
% \tiny
%\begin{tabular}{lp{50mm}llp{50mm}}
%\hline
%Item 	                & Description  																	& Res. (kE) & Confidence  & Comments \\
%\hline 
%\hline 


%\hline
%1 New outside building 					& Container building, contains lab space for clean room (100m2), service room (20m2),  and offices (control room, etc..) (180 m2)									&  995 		 		  &    2 	    & Based on discussion with Denny Drossmann, engineer responsible for design and construction of Innovation Village: 1.95kE/m2 for office and 6.05kE/m2 for lab (price taking into account inflation to beginning of 2022)\\      
%\hline     
%2 CR computers and desk equipment     & Computer and desk equipment for experimental control room in surface building of XS1				&  10 				  &    3 	     & Numbers estimated from survey of computers, screens,.. in IBISS  \\
  
%\hline 
%3 Electrical cabinet in surface building 		& Cabinets to host back-end electronics											&  25 		 		  &    3 	 	& 5keuros per cabinet (5 pieces), estimated with Daniel Thoden (engineer MEA)  \\  


%\hline 
%\hline
%\end{tabular}
%\caption{Resources required for workpackage 1.1, technical coordination - New building. Confidence rules:1 - Quote from a company; 2 - Preliminary estimate from experts; 3 - Preliminary estimate after consultation with experts;4 – Less reliable estimates, based on other methods.}
%\label{TC:Annex:Resources_WP61}
%\end{table}
%\end{landscape}% Landscape page
% \end{adjustwidth}

% \newpage

%Table~\ref{TC:Annex:Resources_WP62} shows the financial resources for the workpackage 1.2, technical coordination - Installation/Experiment, which summarises item related to the electron beam-line. 

%\begin{landscape}% Landscape page
%\begin{table}[h]
%\begin{tabular}{lp{50mm}llp{50mm}}
%\hline
%Item 							    & Description  																	& Res. (kE) & Confidence   & Comments \\
%\hline 
%\hline                                                                                                                                      
%1 Electron beam line 				& Including equipment (monitor, pumps,etc...)									&  300 		 		  &    2 	    & Machine experts said that beam line with instrument is 10k/m (assuming 30m)  \\      
%\hline
          
%2 Dumps 							& HICS dump and photon dumps													&  300		 		  &    2	 	& Machine experts said that one dump is around 100k. \\
%\hline

%4 Dipole power supplies 			& Power supplies to power TDC magnets.											&  105		 		  &    1	 	& Discussion with MKK. Each HVPS would be ~35k. \\
%\hline

%5 Dipole cabling+ cooling			& services to TDC magnets														&  150		 		  &    4	 	& extrapolated from machine CDR. \\

%\hline

%6 Magnet support and adjustment plate			& 8k/pieces												         	&  24		 		  &    2	 	& Discussion with K. Gadow (FH engineer). \\

%\hline

%7 IP Chamber gate valve +control system			& IP Chamber gate valve +control system														&  50		 		  &    2	 	& Estimate from Matt Zepf. \\

%\hline

%7(bis) IP Chamber vacuum tank			&  Taken into account in Laser note! Shown here for information! Not accounted for in our pricing.														&  40		 		  &    2	 	& Estimate from K. Gadow(FH engineer) \\

%\hline

%8 Target vacuum chambers			& 20k each, chambers with movable targets													&  40		 		  &    2	 	& Discussion with K. Gadow(FH engineer). \\

%%%%\caption{Resources required for workpackage 1.2, technical coordination - Installation/Experiment. Confidence rules:1 - Quote from a company; 2 - Preliminary estimate from experts; 3 - Preliminary estimate after consultation with experts;4 – Less reliable estimates, based on other methods.}
%\label{TC:Annex:Resources_WP62}
%\end{table}
%\end{landscape}% Landscape page

%Tables~\ref{TC:Annex:Resources_WP63.1} and~\ref{TC:Annex:Resources_WP63.2} shows the financial resources for the workpackage 1.3, technical coordination - service/Experiment, which summarises item related to the services needed in the experiment. 

% \newpage
%\begin{landscape}% Landscape page
%\begin{table}[h]
%\begin{tabular}{lp{50mm}llp{50mm}}
%%\hline
%Item 							    & Description  																	& Res. (kE) & Confidence   & Comments \\
%\hline 
%\hline                                                                                                                                      
%5 Networking 		 				& Network Infrastructure to experiment 											&  70		 		  &    2	 	    & Discussion with Kars Ohrenberg (IT). Estimate valid for about 100 device connected to network. \\
%\hline

%6 Cooling and cabling  				& Cooling and cabling of experiment including counting room.					&  100		 		  &    3	    & Discussion with Daniel Thoden (MEA engineer) and extrapolated from Matt Zepf AC quote. \\
%\hline

%7 UPS						 		& Battery for emergency urgent experiment										&  15		 		  &    4	 	    & 1 Schneider electric 10kW UPS (with battery pack) that can run for 20min at full capacity. \\
%\hline

%\hline
%\end{tabular}
%\caption{Resources required for workpackage 1.3, first part, technical coordination - Service/Experiment. Confidence rules:1 - Quote from a company; 2 - Preliminary estimate from experts; 3 - Preliminary estimate after consultation with experts;4 – Less reliable estimates, based on other methods.}
%\label{TC:Annex:Resources_WP63.1}
%\end{table}
%\end{landscape}% Landscape page

% \newpage
%\begin{landscape}% Landscape page
%\begin{table}[h]
%\begin{tabular}{lp{50mm}llp{50mm}}
%\hline
%Item 							    & Description  																	& Res. (kE) & Confidence  & Comments \\
%\hline 
%\hline  

% 8 Small optic table for detectors			& Table to hold all IP detectors.												& 15 				  &    1            & Estimated by Noam and Weiz workshop. Should be moved to detector common note.\\
%\hline

%8 Mechanical tray and base platform	& Detector installation structure (12 pieces, 6k each).											& 72 				  &    2            & Estimated by Noam and Weizmann workshop.\\
%\hline

%9 Vacuum chamber for magnets	& Chamber from magnet (2 pieces needed, 65k each)															& 130 				  &    2            & Estimated by Noam and Weizmann workshop. Compared to CDR added 2 other chambers for other magnets. \\
%\hline

%10 Movable stage							& Or equivalent device to move positron side tracker.									& 30 				            &    1      & Noam Quote from company. \\


%\hline
%11 Support structure 	& Concrete supporting elements to hold instruments, magnets, etc.				&  30 		 		  &    2     & Estimation after design made from Karsten Gadow (FH engineer)- March 2022  \\  
%\hline 

%12 Movable bridges 				& Way to access instruments										   &  0		 		  &    2	      & Estimation from Karsten Gadow (FH engineer).
%\hline 
%13 Shielding 				& Concrete elements to shield beam-line								    	& 0						 		  &    2	      &  Estimation after design made from Karsten Gadow (blocks recycled) - March 2022   \\

%\hline

%14 Vacuum Pumps 				& Pumps for vacuum chambers								    	& 65						 		  &    1	      &  1 for each of the 5 vacuum chambers (IP, target*2, magnets*2), 13k for each quote from M.Zepf.    \\

%you \hline

% \hline
% 16 Pandora detectors				& 	Radiation detectors (*5, dumps,IP, electronics)			    	& ??						 		  &    2	      &  Need to be checked with Albrecht?    \\
%\hline
%\hline
%\end{tabular}
%%\caption{Resources required for workpackage 1.3, second part, technical coordination - Service/Experiment. Confidence rules:1 - Quote from a company; 2 - Preliminary estimate from experts; 3 - Preliminary estimate after consultation with experts;4 – Less reliable estimates, based on other methods.}
%\label{TC:Annex:Resources_WP63.2}
%\end{table}
%\end{landscape}% Landscape page

% \newpage

%Table~\ref{TC:Annex:Resources_WP64} shows the financial resources for the workpackage 1.4, technical coordination - Infrastructure Laser, which summarises item related to the Laser infrastructure. 

%\begin{landscape}% Landscape page
%\begin{table}[h]
%\begin{tabular}{lp{50mm}llp{50mm}}
%\hline
%%Item 							    & Description  																	& Res. (kE) & Confidence  & Comments \\
%\hline
%1 Laser clean room+AC						& 100 m2									&  180 		 		  &    1 	    & Quote from LOEMAT company at 1000 Euro/m2 and 800 Euros/m2(clim) .\\      
  %\hline     

% 2 Clean room						& Laser clean room to be install in XS1 UG02									&  500 		 		  &    3 	    & Based on discussion with U. Schneekloth: 500 for 300m3 class 6. For class 8 would be 200 - 300. Quote from LOEMAT company at 1000 Euro/m2 and 800 Euros/m2(clim), but seems low .\\      
%   \hline
        
% 3 Air Conditioning 					& AC for Laser area																&  250		 		  &    1	 	& Company quote to M. Zepf \\


% \hline                                                                                                                1 Non permanent building						& contains clean room, service room, and control room (300 m2)									&  250 		 		  &    3 	    & Based on future discussion with Denny Drossmann innovation village .\\      
%   \hline     

% 2 Clean room						& Laser clean room to be install in XS1 UG02									&  500 		 		  &    3 	    & Based on discussion with U. Schneekloth: 500 for 300m3 class 6. For class 8 would be 200 - 300. Quote from LOEMAT company at 1000 Euro/m2 and 800 Euros/m2(clim), but seems low .\\      
%   \hline
        
% 3 Air Conditioning 					& AC for Laser area																&  250		 		  &    1	 	& Company quote to M. Zepf \\
%\hline
%2 Water supply 						& Installation costs															&  20		 		  &    2	 	    & estimate from M. Zepf. \\
%\hline

%3 Cabling supply 					& Installation costs															&  20		 		  &    2	 	    & estimate from M. Zepf. \\
%\hline

%4 UPS						 		& Battery for emergency urgent experiment										&  15		 		  &    4	 	    & 1 Schneider electric 10kW UPS (with battery pack) that can run for 20min at full capacity. \\
%     \hline

%5 Laser beam line					& Laser vacuum pipe, turbo-pump, gatevalves to go from Surface to UG03									&  108 		 		  &    2 	     & estimate from M. Zepf.\\      
 % \hline
        
% 6 Vacuum Pumps 				& Pumps laser beam line							    	& 26						 		  &    1	      &  2 turbo pumps 13k each    \\
        
        %   \hline

%7 Interlocks system					& Interlocks system									&  50 		 		  &    4 	     & estimate after discussion with machine experts.\\      
%\hline
% 8 Monitoring hazardous system					& Monitor hazardous things around laser.								&  ?? 		 		  &    2 	     & estimate from K. Gadow.\\      
%\hline    
  
% 2 Gamma chamber and ICS beamline 	& Vacuum chamber for ICS with beam pipe											&  15		 		  &    2	 	& 		Q1 22	&  Q4 22    & estimate from M. Zepf. \\


%\hline
%\hline
%\end{tabular}
%\caption{Resources required for workpackage 1.4, technical coordination - Infrastructure/Laser. Confidence rules:1 - Quote from a company; 2 - Preliminary estimate from experts; 3 - Preliminary estimate after consultation with experts;4 – Less reliable estimates, based on other methods.}
%\label{TC:Annex:Resources_WP64}
%\end{table}
%\end{landscape}% Landscape page

% \newpage

% Table~\ref{TC:Annex:Resources_WP65} shows the financial resources for the workpackage 1.5, technical coordination - Installation Laser, which summarises item related to the Laser beam-lines. 

% \begin{landscape}% Landscape page
% \begin{table}[]
% \begin{tabular}{lp{50mm}llp{50mm}}
% \hline
% Item 							    & Description  																	& Res. (kE) & Confidence   & Comments \\
% \hline 
% \hline                                                                                                                                      
% 1 Laser beam line					& Laser vacuum pipe to go from Surface to UG03									&  108 		 		  &    2 	   & estimate from M. Zepf.\\      
%         \hline
  
% % 2 Gamma chamber and ICS beamline 	& Vacuum chamber for ICS with beam pipe											&  15		 		  &    2	  & estimate from M. Zepf. \\

% \hline

% \hline
% \end{tabular}
% \caption{Resources required for workpackage 1.5, technical coordination - Installation/Laser. Confidence rules:1 - Quote from a company; 2 - Preliminary estimate from experts; 3 - Preliminary estimate after consultation with experts;4 – Less reliable estimates, based on other methods.}
% \label{TC:Annex:Resources_WP65}
% \end{table}
% \end{landscape}% Landscape page

%\newpage

The total capital investment cost of the infrastructure combined amounts to about $3349\,\text{kEUR}$, out of which $23\%$ falls in confidence level  1, 65\% level 2, and 6\% for levels 3 and 4 respectively.
% Most of the hardware cost is expected to be spent during the second year after $T_0$, when equipment and components are ordered and delivered.\\
A time plan for the expenditure of this capital is given by Fig.~\ref{fig:luxeinfcostmap}


\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{fig/ProjectManagement/LUXEInfrastructureInvestMap.png}
    \caption{LUXE technical infrastructure spending profile.}
    \label{fig:luxeinfcostmap}
\end{figure}


The preliminary person-power needed to complete the design, and construction integrated over three years from $T_0$ is the following:

\begin{itemize}
    \item 5 FTE-years from M for LUXE beamline (4 (power, water, electrical, beam instrumentation)+1(interlock), charged to FH budget)
    \item 2 FTE-years for the Magnet, vacuum, dumps systems
    \item 3 FTE-years for Laser cleanroom design and the tranport line.
    \item 2 FTE-years for Detector support structures, Service room, Control room	
\end{itemize}

We are currently assuming the following FTE map for the coming years from $T_0$, flat distribution for FH, and peaking for M  for installation:
\begin{itemize}
    \item Y1: 2.34 (FH)  + 0.34 (M, LUXE)  
   \item Y Y2: 2.34 (FH) + 0.34 (M, LUXE) 
    \item YY3: 2.34 (FH) + 3.34 (M, LUXE) 
 \end{itemize}   
%5The different actors (DESY groups, external groups or companies) that needs to be involved to be able to deliver each of the previous items are summarized in Appendix~\ref{sec:Appendix:responsibilities}. 



==> chapters12/organisation_annex.tex <==

\subsection{Human and financial resources}
\label{sec:ressources}


The human and financial resources are estimated assuming a schedule relative to the point in time $T_0$, where funding for the LUXE experiment is released, with more than three years until the experiment is ready for data-taking. No explicit assumptions are made about the schedule at which a long \euxfel shutdown could happen.\\

The cost model is made such that one separates core invest and material costs (in kEUR) and person power (in FTE) that is assumed to come from local resources (i.e. DESY groups, M or FH). The core invest estimates are based on (preliminary) quotes from vendors or on experience from experts at DESY. The estimates of the person power requirements come from experts. Overheads, escalation or contingency are not included. 

In the LUXE CDR~\cite{luxecdr}, different work packages were introduced to describe the deliverables needed by the experiment. The financial resources are based on a similar structure. Each estimate come with a confidence level index, 1 being the most reliable and 4 being the least reliable:

\begin{itemize}

      \item Confidence level 1:  Quote from a company

      \item Confidence level 2: Preliminary estimate from experts

      \item Confidence level 3: Preliminary estimate after consultation with experts

      \item Confidence level 4: Less reliable estimates, based on other methods

\end{itemize}  

Table~\ref{TC:Annex:Resources_WP61} shows the financial resources for the workpackage 1.1, technical coordination - outside building, which summarises the costs associated to the new building and the infrastructure that will need to be constructed outside of XS1. 

\begin{landscape}% Landscape page
\begin{table}[h]
\small
\begin{tabular}{lp{50mm}llp{50mm}}
\hline
Item 	                & Description  																	& Res. (kE) & Confidence  & Comments \\
\hline 
\hline 


\hline
1 New outside building 					& Container building, contains lab space for clean room (100m2), service room (20m2),  and offices (control room, etc..) (180 m2)									&  995 		 		  &    2 	    & Based on discussion with Denny Drossmann, engineer responsible for design and construction of Innovation Village: 1.95kE/m2 for office and 6.05kE/m2 for lab (price taking into account inflation to beginning of 2022)\\      
\hline     
2 CR computers and desk equipment     & Computer and desk equipment for experimental control room in surface building of XS1				&  10 				  &    3 	     & Numbers estimated from survey of computers, screens,.. in IBISS  \\
  
\hline 
3 Electrical cabinet in surface building 		& Cabinets to host back-end electronics											&  25 		 		  &    3 	 	& 5keuros per cabinet (5 pieces), estimated with Daniel Thoden (engineer MEA)  \\  


\hline 
\hline
\end{tabular}
\caption{Resources required for workpackage 1.1, technical coordination - New building. Confidence rules:1 - Quote from a company; 2 - Preliminary estimate from experts; 3 - Preliminary estimate after consultation with experts;4 – Less reliable estimates, based on other methods.}
\label{TC:Annex:Resources_WP61}
\end{table}
\end{landscape}% Landscape page
% \end{adjustwidth}

% \newpage

Table~\ref{TC:Annex:Resources_WP62} shows the financial resources for the workpackage 1.2, technical coordination - Installation/Experiment, which summarises item related to the electron beam-line. 

\begin{landscape}% Landscape page
\begin{table}[h]
\tiny
\begin{tabular}{lp{50mm}llp{50mm}}
\hline
Item 							    & Description  																	& Res. (kE) & Confidence   & Comments \\
\hline 
\hline                                                                                                                                      
1 Electron beam line 				& Including equipment (monitor, pumps,etc...)									&  300 		 		  &    2 	    & Machine experts said that beam line with instrument is 10k/m (assuming 30m)  \\      
\hline
          
2 Dumps 							& HICS dump and photon dumps													&  300		 		  &    2	 	& Machine experts said that one dump is around 100k. \\
\hline

3 Experimental dipoles 				& 3 experimental dipoles (target, IP, gamma spectrometer)						&  390		 		  &    1	 	& Quote from Efremov institute Dec. 2021 for 3 TDC magnets.\\
\hline

4 Dipole power supplies 			& Power supplies to power TDC magnets.											&  105		 		  &    1	 	& Discussion with MKK. Each HVPS would be ~35k. \\
\hline

5 Dipole cabling+ cooling			& services to TDC magnets														&  150		 		  &    4	 	& extrapolated from machine CDR. \\

\hline

6 Magnet support and adjustment plate			& 8k/pieces												         	&  24		 		  &    2	 	& Discussion with K. Gadow (FH engineer). \\

\hline

7 IP Chamber gate valve +control system			& IP Chamber gate valve +control system														&  50		 		  &    2	 	& Estimate from Matt Zepf. \\

\hline

7(bis) IP Chamber vacuum tank			&  Taken into account in Laser note! Shown here for information! Not accounted for in our pricing.														&  40		 		  &    2	 	& Estimate from K. Gadow(FH engineer) \\

\hline

8 Target vacuum chambers			& 20k each, chambers with movable targets													&  40		 		  &    2	 	& Discussion with K. Gadow(FH engineer). \\

\hline
\hline
\end{tabular}
\caption{Resources required for workpackage 1.2, technical coordination - Installation/Experiment. Confidence rules:1 - Quote from a company; 2 - Preliminary estimate from experts; 3 - Preliminary estimate after consultation with experts;4 – Less reliable estimates, based on other methods.}
\label{TC:Annex:Resources_WP62}
\end{table}
\end{landscape}% Landscape page

Tables~\ref{TC:Annex:Resources_WP63.1} and~\ref{TC:Annex:Resources_WP63.2} shows the financial resources for the workpackage 1.3, technical coordination - service/Experiment, which summarises item related to the services needed in the experiment. 

% \newpage
\begin{landscape}% Landscape page
\begin{table}[h]
\small
\begin{tabular}{lp{50mm}llp{50mm}}
\hline
Item 							    & Description  																	& Res. (kE) & Confidence   & Comments \\
\hline 
\hline                                                                                                                                      
1 Electrical cabinet in UG02 		& Cabinets to host back-end electronics											&  10 		 		  &    3 	    & 5keuros per cabinet (2 pieces), estimated with Daniel Thoden (MEA engineer)  \\      

\hline

3 Electrical cabinet in UG03 		& Front end electronic in experimental area										&  25 		 		  &    3 	    & 5keuros per cabinet (5 pieces), estimated with Daniel Thoden (MEA engineer), probably need shielded ones...  \\   
   \hline
       
4 Gas outlet+pipes+detectors					& Gas outlet+pipes+sniffer in experimental area									&  20		 		  &    3	 	    & Discussion with Daniel Thoden (MEA engineer), and adding ~10k for gas sniffer (O2, sniffer). \\
\hline

5 Networking 		 				& Network Infrastructure to experiment 											&  70		 		  &    2	 	    & Discussion with Kars Ohrenberg (IT). Estimate valid for about 100 device connected to network. \\
\hline

6 Cooling and cabling  				& Cooling and cabling of experiment including counting room.					&  100		 		  &    3	    & Discussion with Daniel Thoden (MEA engineer) and extrapolated from Matt Zepf AC quote. \\
\hline

7 UPS						 		& Battery for emergency urgent experiment										&  15		 		  &    4	 	    & 1 Schneider electric 10kW UPS (with battery pack) that can run for 20min at full capacity. \\
\hline

\hline
\end{tabular}
\caption{Resources required for workpackage 1.3, first part, technical coordination - Service/Experiment. Confidence rules:1 - Quote from a company; 2 - Preliminary estimate from experts; 3 - Preliminary estimate after consultation with experts;4 – Less reliable estimates, based on other methods.}
\label{TC:Annex:Resources_WP63.1}
\end{table}
\end{landscape}% Landscape page

% \newpage
\begin{landscape}% Landscape page
\begin{table}[h]
\small
\begin{tabular}{lp{50mm}llp{50mm}}
\hline
Item 							    & Description  																	& Res. (kE) & Confidence  & Comments \\
\hline 
\hline  

% 8 Small optic table for detectors			& Table to hold all IP detectors.												& 15 				  &    1            & Estimated by Noam and Weiz workshop. Should be moved to detector common note.\\
\hline

8 Mechanical tray and base platform	& Detector installation structure (12 pieces, 6k each).											& 72 				  &    2            & Estimated by Noam and Weizmann workshop.\\
\hline

9 Vacuum chamber for magnets	& Chamber from magnet (2 pieces needed, 65k each)															& 130 				  &    2            & Estimated by Noam and Weizmann workshop. Compared to CDR added 2 other chambers for other magnets. \\
\hline

10 Movable stage							& Or equivalent device to move positron side tracker.									& 30 				            &    1      & Noam Quote from company. \\


\hline
11 Support structure 	& Concrete supporting elements to hold instruments, magnets, etc.				&  30 		 		  &    2     & Estimation after design made from Karsten Gadow (FH engineer)- March 2022  \\  
\hline 

12 Movable bridges 				& Way to access instruments										   &  0		 		  &    2	      & Estimation from Karsten Gadow (FH engineer).  \\
\hline 
13 Shielding 				& Concrete elements to shield beam-line								    	& 0						 		  &    2	      &  Estimation after design made from Karsten Gadow (blocks recycled) - March 2022   \\

\hline

14 Vacuum Pumps 				& Pumps for vacuum chambers								    	& 65						 		  &    1	      &  1 for each of the 5 vacuum chambers (IP, target*2, magnets*2), 13k for each quote from M.Zepf.    \\

\hline

% \hline
% 16 Pandora detectors				& 	Radiation detectors (*5, dumps,IP, electronics)			    	& ??						 		  &    2	      &  Need to be checked with Albrecht?    \\
\hline
\hline
\end{tabular}
\caption{Resources required for workpackage 1.3, second part, technical coordination - Service/Experiment. Confidence rules:1 - Quote from a company; 2 - Preliminary estimate from experts; 3 - Preliminary estimate after consultation with experts;4 – Less reliable estimates, based on other methods.}
\label{TC:Annex:Resources_WP63.2}
\end{table}
\end{landscape}% Landscape page

% \newpage

Table~\ref{TC:Annex:Resources_WP64} shows the financial resources for the workpackage 1.4, technical coordination - Infrastructure Laser, which summarises item related to the Laser infrastructure. 

\begin{landscape}% Landscape page
\begin{table}[h]
\small
\begin{tabular}{lp{50mm}llp{50mm}}
\hline
Item 							    & Description  																	& Res. (kE) & Confidence  & Comments \\
\hline
1 Laser clean room+AC						& 100 m2									&  180 		 		  &    1 	    & Quote from LOEMAT company at 1000 Euro/m2 and 800 Euros/m2(clim) .\\      
  \hline     

% 2 Clean room						& Laser clean room to be install in XS1 UG02									&  500 		 		  &    3 	    & Based on discussion with U. Schneekloth: 500 for 300m3 class 6. For class 8 would be 200 - 300. Quote from LOEMAT company at 1000 Euro/m2 and 800 Euros/m2(clim), but seems low .\\      
%   \hline
        
% 3 Air Conditioning 					& AC for Laser area																&  250		 		  &    1	 	& Company quote to M. Zepf \\


% \hline                                                                                                                1 Non permanent building						& contains clean room, service room, and control room (300 m2)									&  250 		 		  &    3 	    & Based on future discussion with Denny Drossmann innovation village .\\      
%   \hline     

% 2 Clean room						& Laser clean room to be install in XS1 UG02									&  500 		 		  &    3 	    & Based on discussion with U. Schneekloth: 500 for 300m3 class 6. For class 8 would be 200 - 300. Quote from LOEMAT company at 1000 Euro/m2 and 800 Euros/m2(clim), but seems low .\\      
%   \hline
        
% 3 Air Conditioning 					& AC for Laser area																&  250		 		  &    1	 	& Company quote to M. Zepf \\
\hline
2 Water supply 						& Installation costs															&  20		 		  &    2	 	    & estimate from M. Zepf. \\
\hline

3 Cabling supply 					& Installation costs															&  20		 		  &    2	 	    & estimate from M. Zepf. \\
\hline

4 UPS						 		& Battery for emergency urgent experiment										&  15		 		  &    4	 	    & 1 Schneider electric 10kW UPS (with battery pack) that can run for 20min at full capacity. \\
        \hline

5 Laser beam line					& Laser vacuum pipe, turbo-pump, gatevalves to go from Surface to UG03									&  108 		 		  &    2 	     & estimate from M. Zepf.\\      
        \hline
        
% 6 Vacuum Pumps 				& Pumps laser beam line							    	& 26						 		  &    1	      &  2 turbo pumps 13k each    \\
        
        %   \hline

7 Interlocks system					& Interlocks system									&  50 		 		  &    4 	     & estimate after discussion with machine experts.\\      
        \hline
% 8 Monitoring hazardous system					& Monitor hazardous things around laser.								&  ?? 		 		  &    2 	     & estimate from K. Gadow.\\      
        \hline    
  
% 2 Gamma chamber and ICS beamline 	& Vacuum chamber for ICS with beam pipe											&  15		 		  &    2	 	& 		Q1 22	&  Q4 22    & estimate from M. Zepf. \\


\hline
\hline
\end{tabular}
\caption{Resources required for workpackage 1.4, technical coordination - Infrastructure/Laser. Confidence rules:1 - Quote from a company; 2 - Preliminary estimate from experts; 3 - Preliminary estimate after consultation with experts;4 – Less reliable estimates, based on other methods.}
\label{TC:Annex:Resources_WP64}
\end{table}
\end{landscape}% Landscape page

% \newpage

% Table~\ref{TC:Annex:Resources_WP65} shows the financial resources for the workpackage 1.5, technical coordination - Installation Laser, which summarises item related to the Laser beam-lines. 

% \begin{landscape}% Landscape page
% \begin{table}[]
% \begin{tabular}{lp{50mm}llp{50mm}}
% \hline
% Item 							    & Description  																	& Res. (kE) & Confidence   & Comments \\
% \hline 
% \hline                                                                                                                                      
% 1 Laser beam line					& Laser vacuum pipe to go from Surface to UG03									&  108 		 		  &    2 	   & estimate from M. Zepf.\\      
%         \hline
  
% % 2 Gamma chamber and ICS beamline 	& Vacuum chamber for ICS with beam pipe											&  15		 		  &    2	  & estimate from M. Zepf. \\

% \hline

% \hline
% \end{tabular}
% \caption{Resources required for workpackage 1.5, technical coordination - Installation/Laser. Confidence rules:1 - Quote from a company; 2 - Preliminary estimate from experts; 3 - Preliminary estimate after consultation with experts;4 – Less reliable estimates, based on other methods.}
% \label{TC:Annex:Resources_WP65}
% \end{table}
% \end{landscape}% Landscape page

\newpage


The total capital investment cost of the infrastructure combined amounts to about $3349\,\text{kEUR}$, out of which $23\%$ falls in confidence level  1, 65\% level 2, and 6\% for levels 3 and 4 respectively.
% Most of the hardware cost is expected to be spent during the second year after $T_0$, when equipment and components are ordered and delivered.\\
A time plan for the expenditure of this capital is given by Fig.~\ref{fig:luxeinfcostmap}


\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{fig/ProjectManagement/LUXEInfrastructureInvestMap.png}
    \caption{LUXE technical infrastructure spending profile.}
    \label{fig:luxeinfcostmap}
\end{figure}


The preliminary person-power needed to complete the design, and construction integrated over three years from $T_0$ is the following:

\begin{itemize}
    \item 5 FTE-years from M for LUXE beamline (4 (power, water, electrical, beam instrumentation)+1(interlock), charged to FH budget)
    \item 2 FTE-years for the Magnet, vacuum, dumps systems
    \item 3 FTE-years for Laser cleanroom design and the tranport line.
    \item 2 FTE-years for Detector support structures, Service room, Control room	
\end{itemize}

We are currently assuming the following FTE map for the coming years from $T_0$, flat distribution for FH, and peaking for M  for installation:
\begin{itemize}
    \item Y1: 2.34 (FH)  + 0.34 (M, LUXE)  
   \item Y Y2: 2.34 (FH) + 0.34 (M, LUXE) 
    \item YY3: 2.34 (FH) + 3.34 (M, LUXE) 
 \end{itemize}   

The different actors (DESY groups, external groups or companies) that needs to be involved to be able to deliver each of the previous items are summarized in Appendix~\ref{sec:Appendix:responsibilities}. 

\subsection{Milestones}

The schedule is given with respect to $T_0$, the point in time, where the funding for LUXE is secured until three years from that point where the installation and commissioning phase is complete and the system is ready for data-taking.

Table~\ref{TC:Annex:Milestone_WP11} shows the milestones that were determined for the LUXE workpackage 1.1, technical coordination - infrastructure.

\newcounter{mycounter}

% \begin{landscape}% Landscape page
\begin{table}[h]
\begin{tabular}{lp{60mm}cp{40mm}}
\hline
Name	&	Milestone	& Target Date	& Estimated time for completion (Months)\\
\hline\hline

IN\stepcounter{mycounter}\themycounter & Finish Support Structure Design				& Q2/Y1	 & 6 \\
IN\stepcounter{mycounter}\themycounter & Company Decision on Support structure Order	& Q4/Y1	 & 3 \\
IN\stepcounter{mycounter}\themycounter & Finish support structure construction			& Q3/Y2	 & 2 \\
IN\stepcounter{mycounter}\themycounter & Finish Shielding Design	        			& Q1/Y2	 & 6 \\
IN\stepcounter{mycounter}\themycounter & XS1 ready for beamline installation			& Q1/Y2	 & 0 \\


IN\stepcounter{mycounter}\themycounter & Finish new building Design			        	& Q3/Y1	 & 6 \\
IN\stepcounter{mycounter}\themycounter & Company Decision on new building           	& Q1/Y2	 & 6 \\
IN\stepcounter{mycounter}\themycounter & Finish support new building        			& Q1/Y3	 & 12 \\

IN\stepcounter{mycounter}\themycounter & Finish Control Room Design				     	& Q2/Y3	 & 1 \\
IN\stepcounter{mycounter}\themycounter & Finish Control Room Construction				& Q2/Y3	 & 1 \\

IN\stepcounter{mycounter}\themycounter & Outside building ready                         & Q2/Y3	 & 0 \\

\hline\hline
\hline
\end{tabular}
\caption{Major Milestones required for workpackage 1.1, technical coordination - infrastructure.}
\label{TC:Annex:Milestone_WP11}
\end{table}
% \end{landscape}% Landscape page

Table~\ref{TC:Annex:Milestone_WP12} shows the milestones that were determined for the LUXE workpackage 1.2, technical coordination - Installation/Experiment.


\begin{table}[h]
\begin{tabular}{lp{60mm}cp{40mm}}
\hline
Name	&	Milestone	& Target Date	& Time for completion (Months)\\
\hline\hline

IN\stepcounter{mycounter}\themycounter	 &	LUXE electron vacuum beamline design finalization	& Q1/Y1	& 12   \\
IN\stepcounter{mycounter}\themycounter &	LUXE electron vacuum beamline delivery				& Q4/Y2	& 3    \\
IN\stepcounter{mycounter}\themycounter &	LUXE electron vacuum beamline installed				& Q3/Y4	& 1    \\
IN\stepcounter{mycounter}\themycounter &	LUXE electron vacuum beamline running				& Q4/Y4	& 1    \\
IN\stepcounter{mycounter}\themycounter &	Electron beam dump design finished					& Q2/Y2	& 12   \\
IN\stepcounter{mycounter}\themycounter &	E-Beam Dump Received								& Q4/Y3	& 6    \\
IN\stepcounter{mycounter}\themycounter &	E-Beam Dump installed								& Q4/Y3	& 1    \\
IN\stepcounter{mycounter}\themycounter &	photon beam dump design finished					& Q2/Y2	& 12   \\
IN\stepcounter{mycounter}\themycounter &	ph-beam dump received								& Q4/Y3	& 6    \\
IN\stepcounter{mycounter}\themycounter &	ph-beam dump installed								& Q4/Y3	& 1    \\
IN\stepcounter{mycounter}\themycounter &	Magnet design finished								& Q1/Y1	& 9    \\
IN\stepcounter{mycounter}\themycounter &	Magnet Tender Decision								& Q1/Y1	& 3    \\
IN\stepcounter{mycounter}\themycounter &	Magnets received @DESY								& Q3/Y3	& 18   \\
IN\stepcounter{mycounter}\themycounter &	Magnets tested										& Q1/Y4	& 6    \\
IN\stepcounter{mycounter}\themycounter &	Magnets installed									& Q2/Y4	& 1    \\
IN\stepcounter{mycounter}\themycounter &	magnet HV system design finished					& Q2/Y2	& 9    \\
IN\stepcounter{mycounter}\themycounter &	Magnet HV system received							& Q3/Y2	& 3    \\
IN\stepcounter{mycounter}\themycounter &	Magnet HV system tested								& Q4/Y2	& 3    \\
IN\stepcounter{mycounter}\themycounter &	Magnet HV system installed							& Q1/Y3	& 1    \\
IN\stepcounter{mycounter}\themycounter &	Detector installation Plan finalized				& Q3/Y2	& 3    \\
IN\stepcounter{mycounter}\themycounter &	Receive all detectors @DESY							& Q1/Y4	& 1    \\
IN\stepcounter{mycounter}\themycounter &	Install detectors in XS1							& Q2/Y4	& 1    \\
IN\stepcounter{mycounter}\themycounter &	Finish design of Vacuum chamber						& Q3/Y3	& 9    \\
IN\stepcounter{mycounter}\themycounter &	Receive vacuum magnet chamber						& Q1/Y4	& 1    \\
IN\stepcounter{mycounter}\themycounter &	Install vacuum magnet chamber						& Q1/Y4	& 1    \\
IN\stepcounter{mycounter}\themycounter &	Fiducialisation of all items for alignment			& Q1/Y4	& 10   \\
IN\stepcounter{mycounter}\themycounter &	align experiment									& Q2/Y4	& 2 	\\

\hline\hline
\hline
\end{tabular}
\caption{Major Milestones required for workpackage 1.2, technical coordination - Installation/Experiment.}
\label{TC:Annex:Milestone_WP12}
\end{table}


Table~\ref{TC:Annex:Milestone_WP13} shows the milestones that were determined for the LUXE workpackage 1.3, technical coordination - Service/Experiment.


\begin{table}[h]
\begin{tabular}{lp{60mm}cp{40mm}}
\hline
Name	&	Milestone	& Target Date	& Time for completion (Months)\\
\hline\hline

IN\stepcounter{mycounter}\themycounter    &	Service Room Design finished	                   & Q3/Y1   &	1\\
IN\stepcounter{mycounter}\themycounter    &	Service Room Ready	                               & Q1/Y3   &	2\\
IN\stepcounter{mycounter}\themycounter    &	Final specifications of the electrical cabinets	   & Q3/Y2   &	3\\
IN\stepcounter{mycounter}\themycounter    &	electrical cabinets delivered	                   & Q4/Y3   &	3\\
IN\stepcounter{mycounter}\themycounter    &	electrical cabinets installed	                   & Q4/Y3   &	1\\
IN\stepcounter{mycounter}\themycounter    &	Finish design of electrical services	           & Q3/Y2   &	6\\
IN\stepcounter{mycounter}\themycounter    &	electrical services installed	                   & Q2/Y3   &	1\\
IN\stepcounter{mycounter}\themycounter    &	Finish Design of Cooling services	               & Q3/Y2   &	6\\
IN\stepcounter{mycounter}\themycounter    &	Colling services installed	                       & Q2/Y3   &	1\\
IN\stepcounter{mycounter}\themycounter    &	Finish design of gas services	                   & Q3/Y2   &	6\\
IN\stepcounter{mycounter}\themycounter    &	Gas services installed	                           & Q2/Y3   &	1\\
IN\stepcounter{mycounter}\themycounter    &	Finish IT services Design	                       & Q3/Y2   &	6\\
IN\stepcounter{mycounter}\themycounter    &	IT services installation	                       & Q2/Y3   &	1\\
IN\stepcounter{mycounter}\themycounter    &	DAQ installed	                                   & Q2/Y3   &	2\\
IN\stepcounter{mycounter}\themycounter    &	Detector back-end installed	                       & Q2/Y3   &	1\\

\hline\hline
\hline
\end{tabular}
\caption{Major Milestones required for workpackage 1.3, technical coordination - Service/Experiment.}
\label{TC:Annex:Milestone_WP13}
\end{table}


Table~\ref{TC:Annex:Milestone_WP14} shows the milestones that were determined for the LUXE workpackage 1.4, technical coordination - Infrastructure/Laser.


\begin{table}[h]
\begin{tabular}{lp{60mm}cp{40mm}}
\hline
Name	&	Milestone	& Target Date	& Time for completion (Months)\\
\hline\hline

IN\stepcounter{mycounter}\themycounter    &	Finish laser cleanroom specifications	 &   Q1/Y1	& 12\\
IN\stepcounter{mycounter}\themycounter    &	laser cleanroom company decision	     &   Q2/Y1	& 5\\
IN\stepcounter{mycounter}\themycounter    &	Finish laser cleanroom design	         &   Q4/Y1	& 6\\
IN\stepcounter{mycounter}\themycounter    &	cleanroom construction	                 &   Q2/Y3	& 3\\
IN\stepcounter{mycounter}\themycounter    &	cleanroom equipped	                     &   Q2/Y3	& 1\\
IN\stepcounter{mycounter}\themycounter    &	Finish Laser AC specifications	         &   Q1/Y1	& 12\\
IN\stepcounter{mycounter}\themycounter    &	Decide Laser AC company	                 &   Q4/Y1	& 3\\
IN\stepcounter{mycounter}\themycounter    &	Finish Laser AC design	                 &   Q1/Y2	& 3\\
IN\stepcounter{mycounter}\themycounter    &	Laser AC installed	                     &   Q2/Y3	& 1\\
IN\stepcounter{mycounter}\themycounter    &	Finish design of Laser transport line	 &   Q2/Y1	& 6\\
IN\stepcounter{mycounter}\themycounter    &	Laser transport line constructed	     &   Q4/Y1	& 2\\
IN\stepcounter{mycounter}\themycounter    &	Laser transport line installed	         &   Q1/Y2	& 1\\

\hline\hline
\hline
\end{tabular}
\caption{Major Milestones required for workpackage 1.4,  technical coordination - Infrastructure/Laser.}
\label{TC:Annex:Milestone_WP14}
\end{table}

Table~\ref{TC:Annex:Milestone_WP15} shows the milestones that were determined for the LUXE workpackage 1.5, technical coordination - Installation/Laser.


\begin{table}[h]
\begin{tabular}{lp{60mm}cp{40mm}}
\hline
Name	&	Milestone	& Target Date	& Time for completion (Months)\\
\hline\hline
% IN\stepcounter{mycounter}\themycounter &	Finish 40TW Laser Movement Plan	        & Q4/Y1 &	1\\
IN\stepcounter{mycounter}\themycounter &	Receive Phase 0 Laser to XS1	                & Q4/Y3 &	6\\
IN\stepcounter{mycounter}\themycounter &	Commision Phase 0 Laser	                        & Q1/Y4 &	3\\
% IN\stepcounter{mycounter}\themycounter &	Decommission Phase 0 Laser	                    & Q4/Y4 &	1\\
% IN\stepcounter{mycounter}\themycounter &	Phase 1 Laser installed	                & Q1/Y5 &	6\\
% IN\stepcounter{mycounter}\themycounter &	Phase 1 Laser commissioned	            & Q3/Y5 &	3\\
IN\stepcounter{mycounter}\themycounter &	Finish design of IP chamber						& Q3/Y3	& 9    \\
IN\stepcounter{mycounter}\themycounter &	Receive IP chamber						& Q3/Y3	& 1    \\
IN\stepcounter{mycounter}\themycounter &	Install IP chamber						& Q2/Y4	& 1    \\

% IN\stepcounter{mycounter}\themycounter &	Finish IP chamber movement plan	        & Q4/Y2 &	6\\
% IN\stepcounter{mycounter}\themycounter &	IP chamber in XS1	                    & Q1/Y3 &	2\\
IN\stepcounter{mycounter}\themycounter &	IP chamber commissioned	                & Q3/Y4 &	2\\
% IN\stepcounter{mycounter}\themycounter &	Finish gamma ICS chamber Movement plan	& Q4/Y4 &	6\\
% IN\stepcounter{mycounter}\themycounter &	ICS chamber in XS1	                    & Q1/Y5 &	1\\
% IN\stepcounter{mycounter}\themycounter &	ICS chamber commissioned	            & Q1/Y5 &	1\\

\hline\hline
\hline
\end{tabular}
\caption{Major Milestones required for workpackage 1.5, , technical coordination - Installation/Laser.}
\label{TC:Annex:Milestone_WP15}
\end{table}





\subsection{Risk management}

The risks to the LUXE technical coordination project associated with the Milestones above are estimated based on the following scale:

\begin{itemize}
    \item Insignificant: Risk is easily mitigated by day to day process. 
    \item Minor: Delays up to 10\% of schedule. Cost increase up to 10\% of budget. 
    \item Moderate: Delays up to 30\% of schedule. Cost increase up to 30\% of budget. 
    \item Major: Delays up to 50\% of schedule. Cost increase up to 50\% of budget. 
    \item Catastrophic: project abandoned
\end{itemize}


The probability of a risk to be realized is quantified as, rare: ($<3$\%), unlikely (3-10\%), moderate (10-50\%), likely (50-90\%) or certain ($>90\%$).\\

Table~\ref{tab:risks1} and~\ref{tab:risks2} lists the risks associated with the milestones foreseen for the LUXE experiment.\\

\begin{table}[htb!]
    \centering
    \caption{Risk description, potential impact on cost and schedule, probability to occur and strategy on how to mitigate the risk. Part 1.}
\begin{tabular}{p{0.2\linewidth}|p{0.1\linewidth}|p{0.1\linewidth}|p{0.1\linewidth}|p{0.2\linewidth}|p{0.2\linewidth}}
        \hline
Risk description & Impact on Cost & Impact on Schedule & Probability to occur & Actions required & Mitigation\\
        \hline
All installations have to be done at the same time during the shutdown period & low & moderate & likely & careful planing, hiring and training people & try to use earlier shutdowns or downscope experiment\\        \hline

Magnet delivery late & low & low & moderate  & Finalize magnet specs, and see if adequate one(s) are available or need to be ordered & Downscope initial experiment (e.g. suboptimal magnet or e-laser mode only)\\        \hline

Electron vacuum line delivery late & low & moderate & low & finish design and order ASAP & Delay installation of beam-line and data-taking\\        \hline

Electron vacuum line damaged during installation & low & low & low & careful planing, hiring and training people & Repair beam-line and delay data-taking\\        \hline

Electron beam-dumps delivery late & low & moderate & low & finish design and order ASAP & Only install e-laser configuration\\        \hline

Electron beam-dumps damaged during installation & low & moderate & low & careful planing, hiring and training people & Repair beam-dump, only install e-laser configuration\\        \hline

Photon beam-dump delivery late & low & moderate & low & finish design and order ASAP & Consider simpler beam dump, or dump beam in final wall.\\        \hline

Photon beam-dump damaged during installation & low & moderate & low & careful planing, hiring and training people & Repair beam-dump, consider simpler beam dump, or dump beam in final wall\\        \hline
         \hline
         \end{tabular}
         \label{tab:risks1}
\end{table}

\begin{table}[htb!]
    \centering
    \caption{Risk description, potential impact on cost and schedule, probability to occur and strategy on how to mitigate the risk. Part 2.}
\begin{tabular}{p{0.2\linewidth}|p{0.12\linewidth}|p{0.12\linewidth}|p{0.12\linewidth}|p{0.2\linewidth}|p{0.2\linewidth}}
        \hline
Risk description & Impact on Cost & Impact on Schedule & Probability to occur & Actions required & Mitigation\\
\hline
New building delivery late & low & low & low & finish design and order ASAP & Delay installation of laser and back-end electronics\\        \hline

\hline
Laser transport line delivery late & low & negligible & low & finish design and order ASAP & Delay installation of transport-line\\        \hline

Laser transport line damaged during installation & low & low & low & careful planing, hiring and training people & Installation in earlier shutdown\\        \hline

Laser system component(s) damaged during or prior to installation & low & negligible & moderate & careful planning and trained personell & Repair or work with degregated laser\\        \hline

IP Chamber damaged during or prior to installation & low & moderate & low & careful planning and trained personel & Repair chamber or get a new one\\        \hline

Detector damaged during installation & low & negligible & low & careful planning and trained personel & Repair detector, work with suboptimal detector configuration\\        \hline

Supporting structure construction late & low & low & low & Finish design early & Installation in earlier shutdown\\        \hline

Services to experiment installed late & low & negligible & low & Finish design early & Installation in earlier shutdown, stage service installation\\        \hline
         \hline
         \end{tabular}
         \label{tab:risks2}
\end{table}


\subsection{Responsibilities}
The responsibility and human resources for the development, construction and installation of the LUXE experiment system will be taken by the FH division in DESY Hamburg. Certain aspects of the construction and installation in the experimental area require access to the Machine group such as electrical and gas system installations in the experimental area as well as lifting the detector systems into the LUXE area by crane. The laser system is a joint responsibility of the FH DESY and Jena institute. Further details are given in Appendix~\ref{sec:Appendix:responsibilities}.\\




\subsection{DESY Infrastructure Resource Vetting}
\label{sec:desy_vetting}

The LUXE experiment will require the development, construction and installation of different elements that are detailed in chapter~\ref{chapt12}. This requires a collaborative effort between several DESY technical groups, notably from M-groups, in addition to personnel from FH. The following list shows which technical groups are leading and helping to deliver each of the main components. Personnel from ZBAU, IT and IPP are also expected to contribute throughout the lists but are not specifically reported.


\begin{itemize}
\item \textbf{Technical infrastructure and safety UG03:} Collaborative effort from all the technical groups.
\item \textbf{Safety:} D3, D5, MR with contributions from MEA, MPS, EuXFEL GmbH.
\item \textbf{The electron beam line} (including beam dumps, magnets and interaction chambers): MEA, MKK, MVS with contributions from MDI, MCS, MSK, MPC, MPS, D3, D5, EuXFEL GmbH.
\item \textbf{Laser infrastructure and beamline:} MEA with contributions from MKK, EuXFEL GmbH.
\item \textbf{Surface building} (including service and control room):  EuXFEL GmbH with contributions from MEA, MPS, MKK.
\end{itemize}

Following the CD0 decision by the DESY directorate in November 2021, the resources needed by  the LUXE experiment were detailed and then discussed with the relevant DESY groups which need to be involved. A summary of the answers received so far is given in fig.~\ref{fig:vettingtable}.

The technical groups with a major contributions or roles:
\begin{itemize}
    \item MKK will be responsible for the technical infrastructure of the experiment (water cooling, electricity, etc). Original estimates for power consumption and cooling needs were communicated to MKK. A first critical check of the estimates and needs indicate that some additional investment might be needed to meet both power and cooling demands by LUXE, beyond what has been included in the current cost estimate. For the installation of the beamline in the tunnel, the currently installed cooling power will be marginal, and most likely an update of the installations will be needed. For the experiment itself, about 200 kW of cooling power will be needed in the experimental area, and a similar power will be needed for the surface installation (laser \& laser building). Currently the electrical installation is judged to likely be sufficient, but a more careful study will be needed. 
    \item MKK estimated that the total investment needed to update the electrical and cooling power could be as much as 1.5 Mo EUR in 2022 costs. A more careful study on how already existing resources could be used, and how synergies with the ASPECT proposal which is currently under study for the same physical location at the \euxfel as the LUXE experiment is ongoing. 
    \item MEA will be involved in different areas including alignment \& survey, laser interlock, experiment magnets, experiment integration, transport \& logistics. In total 2 FTE-years spread over 4 years are deemed sufficient for the tasks. 
    \item MVS will be responsible for the LUXE beamline vacuum system. A major challenge will be the interface between the beam-line vacuum, and the large volume laser transport system. Differential pumping will be needed, to decouple the laser vacuum from the machine vacuum. MVS agrees with the strategy and - under the assumption that the system will be built by external companies - will be able to supervise and advise tha activities with 0.5 FTE in total.
    \item XFEL/Bau: The only major construction project will be the laser building located on the \euxfel grounds at Osdorfer Born. The building will be financed by LUXE, and constructed under responsibility of the \euxfel company. A detailed specification of the building was communicated to \euxfel, and will form the basis of a concrete planning proposal. Preliminary estimates done by DESY and based on recently erected buildings at DESY amount to about 1 Mo EUR construction costs of the building, but are not yet confirmed by the \euxfel company. 
    \item IT will provide the IT infrastructure at the experimental site. This includes the establishment of sufficient IT infrastructure at the experiment and the surface location, and adequate band-width to transfer data from the experiment to central storage on the DESY site. The resource estimate was originally done by the IT group. The estimate does not include the support of the operation of the experiment.
\end{itemize}

The LUXE experiment will be operated by DESY and be located at the \euxfel premises. Safety issues are therefore to be addressed from early on by both relevant groups from DESY and from \euxfel. The overall concept has been developed together with SAVE, the other involved groups are MEA for the laser, MPS for the interlock, D3 for radiation protection and D5 for gases. The safety concept is an integral part of the project definition. 
\begin{itemize}
  \item MPS is responsible for radiation interlocks and risk assessments. The group asked to be involved as soon as possible in the design of the experiment and confirmed that the budget allocated for the radiation interlocks and the integrated 0.5 FTE-year person-power will be enough to realize the project.
  \item SAVE will be essential in defining safety concepts of the experiment. They will be involved from the beginning, assessing and verifying that the concept can be implemented. No major concerns were raised with the plans presented by LUXE. The exact responsibilities will have to be defined, once the experiment is approved.
\end{itemize}

A number of technical groups will be involved with relatively small contributions, of typically a fraction of a FTE-year.

\begin{itemize}
\item MPC will be involved with the dipole magnet power supplies used in the experiment. The resource estimate was originally done by the MPC group.
\item MCS will be involved in the beamline control system used in the experiment. MCS approved the estimate.
\item MSK will be involved in the synchronization of the \euxfel with the laser system. The resource estimate was originally done by the MSK group, and \item MDI will be involved in the design of the beam instrumentation. The resource estimate was developed by the project engineer. Given the modest amount of beam instrumentation that is currently planned to be installed, no concerns were raised by the group after the estimate was submitted.
\end{itemize}

The directorate of the EuXFEL welcomes the initiative and is generally supportive. 

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figures/fig_appendix_ProjectManagement/VettingTable.png}
    \caption{Responses from LUXE resource vetting at DESY.}
    \label{fig:vettingtable}
\end{figure}


\subsection*{Responsibilities required for each of the different work-package}

In the following tables the groups identified for each of the items required in the construction of the experiment are shown. The estimates presented here and also in Section~\ref{sec:ressources} still require further confirmations with each working groups.
\label{sec:Appendix:responsibilities}
\begin{landscape}% Landscape page
\begin{table}[]
\tiny
\begin{tabular}{|p{0.1\linewidth}|p{0.1\linewidth}|p{0.07\linewidth}|p{0.015\linewidth}|p{0.02\linewidth}|p{0.02\linewidth}|p{0.02\linewidth}|p{0.02\linewidth}|p{0.02\linewidth}|p{0.02\linewidth}|p{0.02\linewidth}|p{0.02\linewidth}|p{0.02\linewidth}|p{0.015\linewidth}|p{0.015\linewidth}|p{0.015\linewidth}|p{0.015\linewidth}|p{0.015\linewidth}|p{0.015\linewidth}|p{0.015\linewidth}|p{0.02\linewidth}|p{0.02\linewidth}|p{0.04\linewidth}|}
\hline

Workpackage & Item &  & FH & MEA & ZBAU & MDI & MVS & MCS & MSK & MPS & MPC & MKK & D3 & D5 & IT & IPP & MR & ZM3 & ZM5 & \euxfel Company & External company & Other institute\\ 
\multirow{19}{*}{\shortstack[l]{1) Electron beam \\line}} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\ 
\hline
\cline{2-23}

 & \multirow{3}{*}{\shortstack[l]{Beampipe Apertures\\ and transition}} & Design & Or & Or &  &  & And &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\ 
 &  & Construction &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & Or &  &  & Or & \\ 
 &  & Installation & Or & Or &  &  & And &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\ 
\cline{2-23}

 & \multirow{3}{*}{\shortstack[l]{Beamline support \\and vibration}} & Design & Or & Or &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\ 
 &  & Construction &  & And &  &  &  &  &  &  &  &  &  &  &  &  &  & Or & Or &  & Or & \\ 
 &  & Installation & Or & Or &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\ 
\cline{2-23}

 & \multirow{3}{*}{\shortstack[l]{Alignment and Survey}} & Design & And & And &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\ 
 &  & Construction &  & And &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\ 
 &  & Installation & And & And &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\ 
\cline{2-23}

 & \multirow{3}{*}{\shortstack[l]{Transport}} & Design & Or & Or &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\ 
 &  & Construction &  & And &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & And &  & \\ 
 &  & Installation & Or & Or &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & And &  & \\ 
\cline{2-23}

 & \multirow{3}{*}{\shortstack[l]{Beam monitors}} & Design &  &  &  & And &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\ 
 &  & Construction &  &  &  & Or &  &  &  &  &  &  &  &  &  &  &  &  &  &  & Or & \\ 
 &  & Installation &  & And &  & And & And &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\ 
\cline{2-23}

 & \multirow{3}{*}{\shortstack[l]{Beam controls / ctrl\\ system and timing}} & Design &  &  &  &  &  & And & And & And &  &  &  &  &  &  &  &  &  &  &  & \\ 
 &  & Construction &  &  &  &  &  & And & And & And &  &  &  &  &  &  &  &  &  &  &  & \\ 
 &  & Installation &  &  &  &  &  & And & And & And &  &  &  &  &  &  &  &  &  &  &  & \\ 
%  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\ 

\multirow{19}{*}{\shortstack[l]{2) Beam dumps}} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\ 
\hline

 & \multirow{3}{*}{\shortstack[l]{Electron-laser \\ electron dump}} & Design & And &  &  &  &  &  &  &  &  &  & And &  &  &  &  &  &  &  &  & Dubna\\ 
 &  & Construction &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & Dubna\\ 
 &  & Installation & Or & Or &  &  &  &  &  &  &  &  & And &  &  &  &  &  &  &  &  & \\ 
 \cline{2-23}

 & \multirow{3}{*}{\shortstack[l]{Gamma-laser \\ electron dump}} & Design & And &  &  &  &  &  &  &  &  &  & And &  &  &  &  &  &  &  &  & Dubna\\ 
 &  & Construction &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & Dubna\\ 
 &  & Installation & Or & Or &  &  &  &  &  &  &  &  & And &  &  &  &  &  &  &  &  & \\ 
 \cline{2-23}

 & \multirow{3}{*}{\shortstack[l]{Final photon dump}} & Design & And &  &  &  &  &  &  &  &  &  & And &  &  &  &  &  &  &  &  & Dubna\\ 
 &  & Construction &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & Dubna\\ 
 &  & Installation & Or & Or &  &  &  &  &  &  &  &  & And &  &  &  &  &  &  &  &  & \\ 
 \cline{2-23}

 & \multirow{3}{*}{\shortstack[l]{Shielding}} & Design & Or & Or &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & Dubna\\ 
 &  & Construction & Or & Or &  &  &  &  &  &  &  &  & And &  &  &  &  &  &  &  & And & \\ 
 &  & Installation & Or & Or &  &  &  &  &  &  &  &  & And &  &  &  &  &  &  &  & And & \\ 
 \cline{2-23}

 & \multirow{3}{*}{\shortstack[l]{Monitoring}} & Design & And & And &  &  &  &  &  &  &  &  & And &  &  &  &  &  &  &  &  & \\ 
 &  & Construction & And &  &  &  &  &  &  &  &  &  & And & And  &  &  &  &  &  &  &  & \\ 
 &  & Installation & And &  &  &  &  &  &  &  &  &  & And & And &  &  &  &  &  &  &  & \\ 
 \cline{2-23}

 & \multirow{3}{*}{\shortstack[l]{Services}} & Design & And &  &  &  &  &  &  &  &  & And &  &  &  &  &  &  &  &  &  & \\ 
 &  & Construction & And &  &  &  &  &  &  &  &  & And &  &  &  &  &  &  &  &  &  & \\ 
 &  & Installation & And &  &  &  &  &  &  &  &  & And &  &  &  &  &  &  &  &  &  & \\ 
 \cline{2-23}

 & \multirow{3}{*}{\shortstack[l]{Transport}} & Design & Or & Or & And &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\ 
 &  & Construction &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\ 
 &  & Installation & Or & Or & And &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\ 
 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\ 
 
 \hline

\hline
\end{tabular}
\caption{Identified responsibilities for the different items required by the LUXE experiment, for the design, construction and installation. When a group is needed it is assigned with "And". If two groups can achieve the same task they are assigned and "Or".}
% \label{TC:Annex:Resources_WP65}
\end{table}
\end{landscape}% Landscape page

\begin{landscape}% Landscape page
\begin{table}[]
\tiny
\begin{tabular}{|p{0.1\linewidth}|p{0.1\linewidth}|p{0.07\linewidth}|p{0.015\linewidth}|p{0.02\linewidth}|p{0.02\linewidth}|p{0.02\linewidth}|p{0.02\linewidth}|p{0.02\linewidth}|p{0.02\linewidth}|p{0.02\linewidth}|p{0.02\linewidth}|p{0.02\linewidth}|p{0.015\linewidth}|p{0.015\linewidth}|p{0.015\linewidth}|p{0.015\linewidth}|p{0.015\linewidth}|p{0.015\linewidth}|p{0.015\linewidth}|p{0.02\linewidth}|p{0.02\linewidth}|p{0.04\linewidth}|}
\hline

Workpackage & Item &  & FH & MEA & ZBAU & MDI & MVS & MCS & MSK & MPS & MPC & MKK & D3 & D5 & IT & IPP & MR & ZM3 & ZM5 & \euxfel Company & External company & Other institute\\
\multirow{7}{*}{\shortstack[l]{3) Experiment \\magnets}} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\ 
\hline
\cline{2-23}
 &\multirow{3}{*}{\shortstack[l]{Procurement tests \\and measurements}} & Design &  & And &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\ 
 &  & Construction &  & And &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\ 
 &  & Installation &  & And &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\ 
 \cline{2-23}
 

 &\multirow{3}{*}{\shortstack[l]{Power network}} & Design &  &  &  &  &  &  &  &  &  & And &  &  &  &  &  &  &  &  &  & \\ 
 &  & Construction &  &  &  &  &  &  &  &  &  & And &  &  &  &  &  &  &  &  &  & \\ 
 &  & Installation &  &  &  &  &  &  &  &  &  & And &  &  &  &  &  &  &  &  &  & \\ 
  \cline{2-23}

 &\multirow{3}{*}{\shortstack[l]{Power supplies}} & Design &  &  &  &  &  &  &  &  & And &  &  &  &  &  &  &  &  &  &  & \\ 
 &  & Construction &  &  &  &  &  &  &  &  &  & And &  &  &  &  &  &  &  &  &  & \\ 
 &  & Installation &  &  &  &  &  &  &  &  &  & And &  &  &  &  &  &  &  &  &  & \\ 
  \cline{2-23}
 &\multirow{3}{*}{\shortstack[l]{Cooling}} & Design &  &  &  &  &  &  &  &  & And &  &  &  &  &  &  &  &  &  &  & \\ 
 &  & Construction &  &  &  &  &  &  &  &  &  & And &  &  &  &  &  &  &  &  &  & \\ 
 &  & Installation &  &  &  &  &  &  &  &  &  & And &  &  &  &  &  &  &  &  &  & \\ 
  \cline{2-23}

 &\multirow{3}{*}{\shortstack[l]{Cabling}} & Design &  &  &  &  &  &  &  &  & And &  &  &  &  &  &  &  &  &  &  & \\ 
 &  & Construction &  &  &  &  &  &  &  &  & And &  &  &  &  &  &  &  &  &  &  & \\ 
 &  & Installation &  &  &  &  &  &  &  &  & And &  &  &  &  &  &  &  &  &  &  & \\ 
  \cline{2-23}

 &\multirow{3}{*}{\shortstack[l]{Vacuum chambers\\ and Exit windows}} & Design &  &  &  &  & And &  &  &  &  &  &  &  &  &  &  &  &  &  &  & Weizmann\\ 
 &  & Construction &  &  &  &  & And &  &  &  &  &  &  &  &  &  &  &  &  &  &  & Weizmann\\ 
 &  & Installation & And & And &  &  & And &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\ 
  \cline{2-23}

 &\multirow{3}{*}{\shortstack[l]{Survey and positions}} & Design & And & And &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\ 
 &  & Construction &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\ 
 &  & Installation & And & And &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\ 
 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\ 
  \cline{2-23}

 
 

 \hline

\hline
\end{tabular}
\caption{Identified responsibilities for the different items required by the LUXE experiment, for the design, construction and installation. When a group is needed it is assigned with "And". If two groups can achieve the same task they are assigned and "Or".}
% \label{TC:Annex:Resources_WP65}
\end{table}
\end{landscape}% Landscape page




\begin{landscape}% Landscape page
\begin{table}[]
\tiny
\begin{tabular}{|p{0.1\linewidth}|p{0.1\linewidth}|p{0.07\linewidth}|p{0.015\linewidth}|p{0.02\linewidth}|p{0.02\linewidth}|p{0.02\linewidth}|p{0.02\linewidth}|p{0.02\linewidth}|p{0.02\linewidth}|p{0.02\linewidth}|p{0.02\linewidth}|p{0.02\linewidth}|p{0.015\linewidth}|p{0.015\linewidth}|p{0.015\linewidth}|p{0.015\linewidth}|p{0.015\linewidth}|p{0.015\linewidth}|p{0.015\linewidth}|p{0.02\linewidth}|p{0.02\linewidth}|p{0.04\linewidth}|}
\hline

Workpackage & Item &  & FH & MEA & ZBAU & MDI & MVS & MCS & MSK & MPS & MPC & MKK & D3 & D5 & IT & IPP & MR & ZM3 & ZM5 & \euxfel Company & External company & Other institute\\
% \hline
% \multirow{19}{*}{\shortstack[l]{1) Electron beam \\line}} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\ 
% \hline
% \cline{2-23}

%  & \multirow{3}{*}{\shortstack[l]{Beampipe Apertur\\ and transition}} & Design & Or & Or &  &  & And &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\ 
%  &  & Construction &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & Or &  &  & Or & \\ 
%  &  & Installation & Or & Or &  &  & And &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\ 
% \cline{2-23}
\multirow{12}{*}{\shortstack[l]{4) Technical \\infrastructure\\ UG03}} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\ 
\hline
\cline{2-23}
 &\multirow{3}{*}{\shortstack[l]{Power network}} & Design &  &  &  &  &  & And &  &  & And & And &  &  &  &  &  &  &  &  &  & \\ 
 &  & Construction &  &  &  &  &  & And &  &  & And & And &  &  &  &  &  &  &  &  &  & \\ 
 &  & Installation &  &  &  &  &  & And &  &  & And & And &  &  &  &  &  &  &  &  &  & \\ 
 \cline{2-23}
 & Air conditioning & Design &  &  &  &  &  & And &  &  &  & And &  &  &  &  &  &  &  &  &  & \\ 
 &  & Construction &  &  &  &  &  & And &  &  &  & And &  &  &  &  &  &  &  &  &  & \\ 
 &  & Installation &  &  &  &  &  & And &  &  &  & And &  &  &  &  &  &  &  &  &  & \\ 
  \cline{2-23}

 & \multirow{3}{*}{\shortstack[l]{Liquids and\\ gas supply}} & Design &  & And &  &  &  & And &  &  &  &  &  &  &  &  &  &  &  &  &  & \\ 
 &  & Construction &  & And &  &  &  & And &  &  &  &  &  &  &  &  &  &  &  &  & And & \\ 
 &  & Installation &  & And &  &  &  & And &  &  &  &  &  &  &  &  &  &  &  &  & And & \\ 
  \cline{2-23}

 & \multirow{3}{*}{\shortstack[l]{Cabling (detector \\signal+beam \\monitoring)}} & Design & And &  &  & And &  &  &  &  &  &  &  &  &  &  &  &  &  &  & And & \\ 
 &  & Construction &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & And & And & \\ 
 &  & Installation &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & And & And & \\ 
  \cline{2-23}

 & \multirow{3}{*}{\shortstack[l]{Cable tray}} & Design &  &  &  & And &  &  &  &  &  &  &  &  &  &  &  &  &  & And & And & \\ 
 &  & Construction &  &  &  & And &  &  &  &  &  &  &  &  &  &  &  &  &  & And & And & \\ 
 &  & Installation &  &  &  & And &  &  &  &  &  &  &  &  &  &  &  &  &  & And & And & \\ 
  \cline{2-23}

 & \multirow{3}{*}{\shortstack[l]{Networking}} & Design &  &  &  & And &  &  &  &  &  &  &  &  & And &  &  &  &  &  &  & \\ 
 &  & Construction &  &  &  & And &  &  &  &  &  &  &  &  & And &  &  &  &  &  &  & \\ 
 &  & Installation &  &  &  & And &  &  &  &  &  &  &  &  &  &  &  &  &  &  & And & \\ 
  \cline{2-23}

 & \multirow{3}{*}{\shortstack[l]{Front-end racks}} & Design & And &  &  & And & And &  & And &  &  &  &  &  &  &  &  &  &  &  &  & \\ 
 &  & Construction & And &  &  & And & And &  & And &  &  &  &  &  &  &  &  &  &  &  &  & \\ 
 &  & Installation & And &  &  & And & And &  & And &  &  &  &  &  &  &  &  &  &  &  &  & \\ 
  \cline{2-23}

 & \multirow{3}{*}{\shortstack[l]{Detector movable \\structure}} & Design & And &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\ 
 &  & Construction &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & And & \\ 
 &  & Installation & And &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\ 
  \cline{2-23}

 & \multirow{3}{*}{\shortstack[l]{Detector support \\structure}} & Design & And &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\ 
 &  & Construction & And &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\ 
 &  & Installation & And &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\ 
  \cline{2-23}

 & \multirow{3}{*}{\shortstack[l]{Positioning and \\survey}} & Design & And & And &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\ 
 &  & Construction &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\ 
 &  & Installation & And & And &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\ 
  \cline{2-23}

 & \multirow{3}{*}{\shortstack[l]{Environment \\monitoring \\(temp and  hum..)}} & Design &  &  &  &  &  &  &  &  &  & And &  &  &  &  &  &  &  &  &  & \\ 
 &  & Construction &  &  &  &  &  &  &  &  &  & And &  &  &  &  &  &  &  &  &  & \\ 
 &  & Installation &  &  &  &  &  &  &  &  &  & And &  &  &  &  &  &  &  &  &  & \\ 
  \cline{2-23}

 & \multirow{3}{*}{\shortstack[l]{Development of \\integration concept}} & Design & And & And &  &  &  &  &  &  &  &  &  &  &  & And &  &  &  &  &  & \\ 
 &  & Construction &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\ 
 &  & Installation &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\ 
 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\ 
 
 \hline

\hline
\end{tabular}
\caption{Identified responsibilities for the different items required by the LUXE experiment, for the design, construction and installation. When a group is needed it is assigned with "And". If two groups can achieve the same task they are assigned and "Or".}
% \label{TC:Annex:Resources_WP65}
\end{table}
\end{landscape}% Landscape page


% \begin{landscape}% Landscape page
% \begin{table}[]
% \tiny
% \begin{tabular}{|p{0.1\linewidth}|p{0.1\linewidth}|p{0.07\linewidth}|p{0.015\linewidth}|p{0.02\linewidth}|p{0.02\linewidth}|p{0.02\linewidth}|p{0.02\linewidth}|p{0.02\linewidth}|p{0.02\linewidth}|p{0.02\linewidth}|p{0.02\linewidth}|p{0.02\linewidth}|p{0.015\linewidth}|p{0.015\linewidth}|p{0.015\linewidth}|p{0.015\linewidth}|p{0.015\linewidth}|p{0.015\linewidth}|p{0.015\linewidth}|p{0.02\linewidth}|p{0.02\linewidth}|p{0.04\linewidth}|}
% \hline

% Workpackage & Item &  & FH & MEA & ZBAU & MDI & MVS & MCS & MSK & MPS & MPC & MKK & D3 & D5 & IT & IPP & MR & ZM3 & ZM5 & XFEL Company & External company & Other institute\\

%  \multirow{9}{*}{\shortstack[l]{5) Service room }}  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\ 

%  & \multirow{3}{*}{\shortstack[l]{Power network}} & Design &  &  &  &  &  &  &  &  &  & And &  &  &  &  &  &  &  &  &  & \\ 
%  &  & Construction &  &  &  &  &  &  &  &  &  & And &  &  &  &  &  &  &  &  &  & \\ 
%  &  & Installation &  &  &  &  &  &  &  &  &  & And &  &  &  &  &  &  &  &  &  & \\ 
% \cline{2-23}
%  &\multirow{3}{*}{\shortstack[l]{Air conditioning}} & Design &  &  &  &  &  &  &  &  &  & And &  &  &  &  &  &  &  &  &  & \\ 
%  &  & Construction &  &  &  &  &  &  &  &  &  & And &  &  &  &  &  &  &  &  &  & \\ 
%  &  & Installation &  &  &  &  &  &  &  &  &  & And &  &  &  &  &  &  &  &  &  & \\ 
% \cline{2-23}
%  &\multirow{3}{*}{\shortstack[l]{Liquids and \\gas supply}} & Design &  & And &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\ 
%  &  & Construction &  &  &  &  &  &  &  &  &  & And &  &  &  &  &  &  &  &  & And & \\ 
%  &  & Installation &  &  &  &  &  &  &  &  &  & And &  &  &  &  &  &  &  &  & And & \\ 
% \cline{2-23}
%  &\multirow{3}{*}{\shortstack[l]{Cabling}} & Design & And &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & And & \\ 
%  &  & Construction &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & And & And & \\ 
%  &  & Installation &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & And & And & \\ 
% \cline{2-23}
%  &\multirow{3}{*}{\shortstack[l]{Cable tray}} & Design &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & And & \\ 
%  &  & Construction &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & And & And & \\ 
%  &  & Installation &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & And & And & \\ 
% \cline{2-23}
%  &\multirow{3}{*}{\shortstack[l]{Networking}} & Design &  &  &  &  &  &  &  &  &  &  &  &  & And &  &  &  &  &  &  & \\ 
%  &  & Construction &  &  &  &  &  &  &  &  &  &  &  &  & And &  &  &  &  &  &  & \\ 
%  &  & Installation &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & And & \\ 
% \cline{2-23}
%  &\multirow{3}{*}{\shortstack[l]{Front-end racks}} & Design & And &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\ 
%  &  & Construction & And &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\ 
%  &  & Installation & And &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\ 
% \cline{2-23}
%  &\multirow{3}{*}{\shortstack[l]{Environment \\monitoring}} & Design &  &  &  &  &  &  &  &  &  & And &  &  &  &  &  &  &  &  &  & \\ 
%  &  & Construction &  &  &  &  &  &  &  &  &  & And &  &  &  &  &  &  &  &  &  & \\ 
%  &  & Installation &  &  &  &  &  &  &  &  &  & And &  &  &  &  &  &  &  &  &  & \\ 
% \cline{2-23}
%  &\multirow{3}{*}{\shortstack[l]{Development of \\integration concept}} & Design & And & And &  &  &  &  &  &  &  &  &  &  &  & And &  &  &  &  &  & \\ 
%  &  & Construction &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\ 
%  &  & Installation &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\ 

%  \hline

% \hline
% \end{tabular}
% \caption{Identified responsibilities for the different items required by the LUXE experiment, for the design, construction and installation. When a group is needed it is assigned with "And". If two groups can achieve the same task they are assigned and "Or".}
% % \label{TC:Annex:Resources_WP65}
% \end{table}
% \end{landscape}% Landscape page



\begin{landscape}% Landscape page
\begin{table}[]
\tiny
\begin{tabular}{|p{0.1\linewidth}|p{0.1\linewidth}|p{0.07\linewidth}|p{0.015\linewidth}|p{0.02\linewidth}|p{0.02\linewidth}|p{0.02\linewidth}|p{0.02\linewidth}|p{0.02\linewidth}|p{0.02\linewidth}|p{0.02\linewidth}|p{0.02\linewidth}|p{0.02\linewidth}|p{0.015\linewidth}|p{0.015\linewidth}|p{0.015\linewidth}|p{0.015\linewidth}|p{0.015\linewidth}|p{0.015\linewidth}|p{0.015\linewidth}|p{0.02\linewidth}|p{0.02\linewidth}|p{0.04\linewidth}|}
\hline

Workpackage & Item &  & FH & MEA & ZBAU & MDI & MVS & MCS & MSK & MPS & MPC & MKK & D3 & D5 & IT & IPP & MR & ZM3 & ZM5 & \euxfel Company & External company & Other institute\\

\multirow{10}{*}{\shortstack[l]{5) Surface building \\(include service \\and control room ) }} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\ 
\hline
\cline{2-23}
 &\multirow{3}{*}{\shortstack[l]{Building }} & Design & And &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  And &  And & \\ 
 &  & Construction &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  And &  And & \\ 
 &  & Installation &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\ 
\cline{2-23}
 &\multirow{3}{*}{\shortstack[l]{Power network}} & Design &  &  &  &  &  & And &  &  & And & And &  &  &  &  &  &  &  &  &  & \\ 
 &  & Construction &  &  &  &  &  & And &  &  & And & And &  &  &  &  &  &  &  &  &  & \\ 
 &  & Installation &  &  &  &  &  & And &  &  & And & And &  &  &  &  &  &  &  &  &  & \\ 
 \cline{2-23}
 & Air conditioning & Design &  &  &  &  &  & And &  &  &  & And &  &  &  &  &  &  &  &  &  & \\ 
 &  & Construction &  &  &  &  &  & And &  &  &  & And &  &  &  &  &  &  &  &  &  & \\ 
 &  & Installation &  &  &  &  &  & And &  &  &  & And &  &  &  &  &  &  &  &  &  & \\ 
 \cline{2-23}

 & \multirow{3}{*}{\shortstack[l]{Liquids and\\ gas supply}} & Design &  & And &  &  &  & And &  &  &  &  &  &  &  &  &  &  &  &  &  & \\ 
 &  & Construction &  & And &  &  &  & And &  &  &  &  &  &  &  &  &  &  &  &  & And & \\ 
 &  & Installation &  & And &  &  &  & And &  &  &  &  &  &  &  &  &  &  &  &  & And & \\ 
  \cline{2-23}

 & \multirow{3}{*}{\shortstack[l]{Cabling}} & Design & And &  &  & And &  &  &  &  &  &  &  &  &  &  &  &  &  &  & And & \\ 
 &  & Construction &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & And & And & \\ 
 &  & Installation &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & And & And & \\ 
  \cline{2-23}

 & \multirow{3}{*}{\shortstack[l]{Cable tray}} & Design &  &  &  & And &  &  &  &  &  &  &  &  &  &  &  &  &  & And & And & \\ 
 &  & Construction &  &  &  & And &  &  &  &  &  &  &  &  &  &  &  &  &  & And & And & \\ 
 &  & Installation &  &  &  & And &  &  &  &  &  &  &  &  &  &  &  &  &  & And & And & \\ 
  \cline{2-23}

 & \multirow{3}{*}{\shortstack[l]{Networking}} & Design &  &  &  & And &  &  &  &  &  &  &  &  & And &  &  &  &  &  &  & \\ 
 &  & Construction &  &  &  & And &  &  &  &  &  &  &  &  & And &  &  &  &  &  &  & \\ 
 &  & Installation &  &  &  & And &  &  &  &  &  &  &  &  &  &  &  &  &  &  & And & \\ 
  \cline{2-23}

 & \multirow{3}{*}{\shortstack[l]{Front-end racks}} & Design & And &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\ 
 &  & Construction & And &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\ 
 &  & Installation & And &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\ 
  \cline{2-23}
 & \multirow{3}{*}{\shortstack[l]{Environment \\monitoring \\(temp and  hum..)}} & Design &  &  &  &  &  &  &  &  &  & And &  &  &  &  &  &  &  &  &  & \\ 
 &  & Construction &  &  &  &  &  &  &  &  &  & And &  &  &  &  &  &  &  &  &  & \\ 
 &  & Installation &  &  &  &  &  &  &  &  &  & And &  &  &  &  &  &  &  &  &  & \\ 
  \cline{2-23}

 & \multirow{3}{*}{\shortstack[l]{Development of \\integration concept}} & Design & And & And &  &  &  &  &  &  &  &  &  &  &  & And &  &  &  &  &  & \\ 
 &  & Construction &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\ 
 &  & Installation &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\ 
 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\ 

 \hline

\hline
\end{tabular}
\caption{Identified responsibilities for the different items required by the LUXE experiment, for the design, construction and installation. When a group is needed it is assigned with "And". If two groups can achieve the same task they are assigned and "Or".}
% \label{TC:Annex:Resources_WP65}
\end{table}
\end{landscape}% Landscape page


\begin{landscape}% Landscape page
\begin{table}[]
\tiny
\begin{tabular}{|p{0.1\linewidth}|p{0.1\linewidth}|p{0.07\linewidth}|p{0.015\linewidth}|p{0.02\linewidth}|p{0.02\linewidth}|p{0.02\linewidth}|p{0.02\linewidth}|p{0.02\linewidth}|p{0.02\linewidth}|p{0.02\linewidth}|p{0.02\linewidth}|p{0.02\linewidth}|p{0.015\linewidth}|p{0.015\linewidth}|p{0.015\linewidth}|p{0.015\linewidth}|p{0.015\linewidth}|p{0.015\linewidth}|p{0.015\linewidth}|p{0.02\linewidth}|p{0.02\linewidth}|p{0.04\linewidth}|}
\hline

Workpackage & Item &  & FH & MEA & ZBAU & MDI & MVS & MCS & MSK & MPS & MPC & MKK & D3 & D5 & IT & IPP & MR & ZM3 & ZM5 & \euxfel Company & External company & Other institute\\


\multirow{16}{*}{\shortstack[l]{6) Laser \\infrastructure\\ and beamline}} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\  

\hline
\cline{2-23}
 &\multirow{3}{*}{\shortstack[l]{Laser clean room}} & Design & And &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & And & \\ 
 &  & Construction &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & And & \\ 
 &  & Installation &  & And &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & And & \\ 
\cline{2-23}
 &\multirow{3}{*}{\shortstack[l]{Laser service room}} & Design & And &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & And & \\ 
 &  & Construction &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & And & \\ 
 &  & Installation &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & And & \\ 
\cline{2-23}
 &\multirow{3}{*}{\shortstack[l]{Power network}} & Design &  &  &  &  &  & And &  &  & And & And &  &  &  &  &  &  &  &  &  & \\ 
 &  & Construction &  &  &  &  &  & And &  &  & And & And &  &  &  &  &  &  &  &  &  & \\ 
 &  & Installation &  &  &  &  &  & And &  &  & And & And &  &  &  &  &  &  &  &  &  & \\ 
 \cline{2-23}
 & Air conditioning & Design &  &  &  &  &  & And &  &  &  & And &  &  &  &  &  &  &  &  &  & \\ 
 &  & Construction &  &  &  &  &  & And &  &  &  & And &  &  &  &  &  &  &  &  &  & \\ 
 &  & Installation &  &  &  &  &  & And &  &  &  & And &  &  &  &  &  &  &  &  &  & \\ 
  \cline{2-23}
  & \multirow{3}{*}{\shortstack[l]{Liquids and\\ gas supply}} & Design &  & And &  &  &  & And &  &  &  &  &  &  &  &  &  &  &  &  &  & \\ 
 &  & Construction &  & And &  &  &  & And &  &  &  &  &  &  &  &  &  &  &  &  & And & \\ 
 &  & Installation &  & And &  &  &  & And &  &  &  &  &  &  &  &  &  &  &  &  & And & \\ 
  \cline{2-23}

 & \multirow{3}{*}{\shortstack[l]{Cabling}} & Design & And &  &  & And &  &  &  &  &  &  &  &  &  &  &  &  &  &  & And & \\ 
 &  & Construction &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & And & And & \\ 
 &  & Installation &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & And & And & \\ 
  \cline{2-23}

 & \multirow{3}{*}{\shortstack[l]{Cable tray}} & Design &  &  &  & And &  &  &  &  &  &  &  &  &  &  &  &  &  & And & And & \\ 
 &  & Construction &  &  &  & And &  &  &  &  &  &  &  &  &  &  &  &  &  & And & And & \\ 
 &  & Installation &  &  &  & And &  &  &  &  &  &  &  &  &  &  &  &  &  & And & And & \\ 
  \cline{2-23}

 & \multirow{3}{*}{\shortstack[l]{Networking}} & Design &  &  &  & And &  &  &  &  &  &  &  &  & And &  &  &  &  &  &  & \\ 
 &  & Construction &  &  &  & And &  &  &  &  &  &  &  &  & And &  &  &  &  &  &  & \\ 
 &  & Installation &  &  &  & And &  &  &  &  &  &  &  &  &  &  &  &  &  &  & And & \\ 
  \cline{2-23}

 & \multirow{3}{*}{\shortstack[l]{Front-end racks}} & Design & And &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\ 
 &  & Construction & And &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\ 
 &  & Installation & And &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\ 
  \cline{2-23}
 & \multirow{3}{*}{\shortstack[l]{Environment \\monitoring \\(temp and  hum..)}} & Design &  &  &  &  &  &  &  &  &  & And &  &  &  &  &  &  &  &  &  & \\ 
 &  & Construction &  &  &  &  &  &  &  &  &  & And &  &  &  &  &  &  &  &  &  & \\ 
 &  & Installation &  &  &  &  &  &  &  &  &  & And &  &  &  &  &  &  &  &  &  & \\ 
  \cline{2-23}

 &\multirow{3}{*}{\shortstack[l]{Mirrors structure}} & Design &  &  & And &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & Jena\\ 
 &  & Construction &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & And &  &  &  & \\ 
 &  & Installation &  & And &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\ 
\cline{2-23}
 &\multirow{3}{*}{\shortstack[l]{Beampipe and\\  apertures and\\ transition}} & Design &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & Jena\\ 
 &  & Construction &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & And &  &  &  & \\ 
 &  & Installation &  & And &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\ 
\cline{2-23}
 &\multirow{3}{*}{\shortstack[l]{Beamline support}} & Design &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & Jena\\ 
 &  & Construction &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & And &  &  &  & \\ 
 &  & Installation &  & And &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\ 
\cline{2-23}
 &\multirow{3}{*}{\shortstack[l]{Positioning \\and survey}} & Design & And & And &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & Jena\\ 
 &  & Construction &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\ 
 &  & Installation & And & And &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\ 
\cline{2-23}
 &\multirow{3}{*}{\shortstack[l]{Beam monitors}} & Design &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & Jena\\ 
 &  & Construction &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & And &  &  &  & \\ 
 &  & Installation &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\ 
\cline{2-23}
 & \multirow{3}{*}{\shortstack[l]{Development of \\integration concept}} & Design & And & And &  &  &  &  &  &  &  &  &  &  &  & And &  &  &  &  &  & \\ 
 &  & Construction &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\ 
 &  & Installation &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\ 
 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\ 



 \hline

\hline
\end{tabular}
\caption{Identified responsibilities for the different items required by the LUXE experiment, for the design, construction and installation. When a group is needed it is assigned with "And". If two groups can achieve the same task they are assigned and "Or".}
% \label{TC:Annex:Resources_WP65}
\end{table}
\end{landscape}% Landscape page



\begin{landscape}% Landscape page
\begin{table}[]
\tiny
\begin{tabular}{|p{0.1\linewidth}|p{0.1\linewidth}|p{0.07\linewidth}|p{0.015\linewidth}|p{0.02\linewidth}|p{0.02\linewidth}|p{0.02\linewidth}|p{0.02\linewidth}|p{0.02\linewidth}|p{0.02\linewidth}|p{0.02\linewidth}|p{0.02\linewidth}|p{0.02\linewidth}|p{0.015\linewidth}|p{0.015\linewidth}|p{0.015\linewidth}|p{0.015\linewidth}|p{0.015\linewidth}|p{0.015\linewidth}|p{0.015\linewidth}|p{0.02\linewidth}|p{0.02\linewidth}|p{0.04\linewidth}|}
\hline

Workpackage & Item &  & FH & MEA & ZBAU & MDI & MVS & MCS & MSK & MPS & MPC & MKK & D3 & D5 & IT & IPP & MR & ZM3 & ZM5 & \euxfel Company & External company & Other institute\\

\multirow{5}{*}{\shortstack[l]{7) Interaction\\ Chamber}} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\ 
\hline
\cline{2-23}
 &\multirow{3}{*}{\shortstack[l]{Vacuum system}} & Design & And &  &  &  & And &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\ 
 &  & Construction &  &  &  &  & And &  &  &  &  &  &  &  &  &  &  &  &  &  & And & \\ 
 &  & Installation & And & And &  &  & And &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\ 
\cline{2-23}
 &\multirow{3}{*}{\shortstack[l]{Services}} & Design &  & And &  &  &  &  &  &  &  & And &  &  & And &  &  &  &  &  &  & \\ 
 &  & Construction &  & And &  &  &  &  &  &  &  & And &  &  & And &  &  &  &  &  &  & \\ 
 &  & Installation &  & And &  &  &  &  &  &  &  & And &  &  & And &  &  &  &  &  &  & \\ 
\cline{2-23}
 &\multirow{3}{*}{\shortstack[l]{Inner components}} & Design & And &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & Jena\\ 
 &  & Construction & And &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & Jena\\ 
 &  & Installation & And &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & Jena\\ 
\cline{2-23}
 &\multirow{3}{*}{\shortstack[l]{Monitoring}} & Design & And &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & Jena\\ 
 &  & Construction & And &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & Jena\\ 
 &  & Installation & And &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & Jena\\ 
\cline{2-23}
 &\multirow{3}{*}{\shortstack[l]{Positioning \\and survey}} & Design & And & And &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\ 
 &  & Construction &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\ 
 &  & Installation & And & And &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\ 
\hline
\end{tabular}
\caption{Identified responsibilities for the different items required by the LUXE experiment, for the design, construction and installation. When a group is needed it is assigned with "And". If two groups can achieve the same task they are assigned and "Or".}
% \label{TC:Annex:Resources_WP65}
\end{table}
\end{landscape}% Landscape page



\begin{landscape}% Landscape page
\begin{table}[]
\tiny
\begin{tabular}{|p{0.1\linewidth}|p{0.1\linewidth}|p{0.07\linewidth}|p{0.015\linewidth}|p{0.02\linewidth}|p{0.02\linewidth}|p{0.02\linewidth}|p{0.02\linewidth}|p{0.02\linewidth}|p{0.02\linewidth}|p{0.02\linewidth}|p{0.02\linewidth}|p{0.02\linewidth}|p{0.015\linewidth}|p{0.015\linewidth}|p{0.015\linewidth}|p{0.015\linewidth}|p{0.015\linewidth}|p{0.015\linewidth}|p{0.015\linewidth}|p{0.02\linewidth}|p{0.02\linewidth}|p{0.04\linewidth}|}
\hline

Workpackage & Item &  & FH & MEA & ZBAU & MDI & MVS & MCS & MSK & MPS & MPC & MKK & D3 & D5 & IT & IPP & MR & ZM3 & ZM5 & \euxfel Company & External company & Other institute\\
\multirow{4}{*}{\shortstack[l]{8) Safety }} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\ 
\hline
\cline{2-23}
 &\multirow{3}{*}{\shortstack[l]{Interlocks}} & Design &  & And &  &  &  &  &  & And &  &  & And &  &  &  & And &  &  &  &  & \\ 
 &  & Construction &  & And &  &  &  &  &  & And &  &  & And &  &  &  & And &  &  &  &  & \\ 
 &  & Installation &  & And &  &  &  &  &  & And &  &  & And &  &  &  & And &  &  &  &  & \\ 
\cline{2-23}
 &\multirow{3}{*}{\shortstack[l]{Radiation \\protection\\ monitoring}} & Design &  &  &  &  &  &  &  &  &  &  & And &  &  &  & And &  &  &  &  & \\ 
 &  & Construction &  &  &  &  &  &  &  &  &  &  & And &  &  &  & And &  &  &  &  & \\ 
 &  & Installation &  &  &  &  &  &  &  &  &  &  & And &  &  &  & And &  &  &  &  & \\ 
\cline{2-23}
 &\multirow{3}{*}{\shortstack[l]{Other safety \\monitorings}} & Design &  &  &  &  &  &  &  &  &  &  &  & And &  &  &  &  &  &  &  & \\ 
 &  & Construction &  &  &  &  &  &  &  &  &  &  &  & And &  &  &  &  &  &  &  & \\ 
 &  & Installation &  &  &  &  &  &  &  &  &  &  &  & And &  &  &  &  &  &  &  & \\ 
\cline{2-23}
 &\multirow{3}{*}{\shortstack[l]{Safety concepts}} & Design &  &  &  &  &  &  &  &  &  &  &  &  &  &  & And &  &  & And &  & \\ 
 &  & Construction &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\ 
 &  & Installation &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\

\hline
\end{tabular}
\caption{Identified responsibilities for the different items required by the LUXE experiment, for the design, construction and installation. When a group is needed it is assigned with "And". If two groups can achieve the same task they are assigned and "Or".}
% \label{TC:Annex:Resources_WP65}
\end{table}
\end{landscape}% Landscape page





\subsection*{Extra figures}
\label{sec:Appendix:Extrafig}
\begin{figure}[ht]
   \centering
   \includegraphics*[height=8cm]{fig/TechnicalInfrastructure/XFELSupport} \hspace{2 cm} 
   \includegraphics*[height=8cm]{fig/TechnicalInfrastructure/XFELShieldingBlocksElements}
   
   \caption{CAD drawing of the building elements used in the construction of the experiment, (Top) support structure element, (Bottom) concrete blocks used for shielding.
   \label{fig:LUXE_CAD_SupportAndShieldingElements}}
\end{figure}


==> chapters12/projectmanagement.tex <==
% Discuss here how PM is structured in LUXE

This chapter contains an overview of the LUXE project management and project organisation of the LUXE experiment, as well as a summary of the major items planning and resources scheduling. 

\section{Project Structure}
\label{ref:proj_structure}

\begin{table}
\begin{center}
\begin{tabular}{|c|c|p{5cm}|}
    \hline
    \textbf{WP \#} & \textbf{WP Name} & \textbf{Description}\\\hline
    1 & Laser, Optics, Diagnostics & LUXE Terawatt optical laser system, beamline optics, diagnostics suite\\\hline
    2 & Vacuum Systems & Electron and Laser beam pipes, chambers, pumps, control software \\\hline
    3 & Magnets & Experiment dipole magnets, power and cooling \\\hline
    4 & Beam Dumps & Electron and photon beam dumps, shielding, cooling \\\hline
    5 & Detectors & LUXE particle detectors \\\hline
    6 & Electron Beam Control & Beam monitoring, control, timing \\\hline
    7 & DAQ, Computing, Core Software & Data acquisition, reconstruction, processing, storage \\\hline
    8 & Theory, MC, Simulation & SFQED Signal simulation, Geant 4 detector simulation \\\hline
    9 & Surface Building & Building hosting the Laser cleanroom, control room, counting room \\\hline
    10 & Service Infrastructure & Building media services for XS1 and surface building \\\hline
    11 & Laser Cleanroom & Cleanroom interior \\\hline
    12 & Experiment Integration & Integration concept for the experiment, integrated design \\\hline
    13 & Operations & Experiment operations concept \\\hline
    14 & Safety & LUXE safety concept and safety-related infrastructure \\\hline
    15 & Technical Coordination & Central cordination and support of activities in all WP \\\hline
    16 & Project Management & Project organization, planning, tracking, resources, documentation, risks \\\hline
\end{tabular}
\caption{LUXE WBS highest level elements. }
\label{tab:wbs}
\end{center}
\end{table}

The LUXE project structure is defined by its two base project management documents, namely the work breakdown structure (WBS) and the product breakdown structure (PBS). The WBS lists and groups tasks that need to be completed to realize, operate and maintain the LUXE experimental complex. The PBS is a structured list of all components and deliverables of the LUXE experimental complex. Both WBS and PBS are closely linked. Table~\ref{tab:wbs} summarizes the highest level of the LUXE WBS elements. The WBS structure intends to mirror the areas of responsibilities of technical service groups during lifecycle of the experiment. Each WBS element, or work package, is provided with a scoping statement that precisely describes the scope of each task and the desired outcome. Finally, each WBS element is linked to one or several deliverables, i.e. an element of the PBS. For the sake of brevity, the scoping statements and list of deliverables have been omitted. \\

The WBS is used as basis for all further project management activities and documents. The tasks listed in the WBS enter the schedule and resource estimates, and are linked to the project documentation using a so-called project lifecycle management (PLM) tool.\\

\section{Organisational Structure}

\begin{figure}
    \centering
    \includegraphics[width=0.75\textwidth]{fig/ProjectManagement/LUXEOrganigram.png}
    \caption{LUXE Organigram.}
        \label{fig:organigram}
\end{figure}

The LUXE organisational structure is summarized in the organigram shown in fig.~\ref{fig:organigram}. 

\begin{table}
\begin{center}
\begin{tabular}{|c|p{7cm}|}
    \hline
    \textbf{Area} & \textbf{Responsible Institutes} \\\hline
    Technical Infrastructure & Deutsches Elektronen-Synchrotron (DESY) \\\hline
    Laser \& Diagnostics & Friedrich-Schiller University Jena, Helmholtz Institute Jena, (Laser, diagnostics, overall coordination) Deutsches Elektronen-Synchrotron (DESY), (Infrastructure), Tel Aviv University, (IP chamber)\\\hline
    Positron Detection Systen & AGH-University of Technology (AGH-UST) Cracow, Institute of Space Science (ISS) Bucharest, Tel Aviv University (TAU) (Electromagnetic Calorimeter) Weizmann Institute of Science (Pixel Tracker) \\\hline
    Electron Detection System & University College London (UCL) (Scintillator Screen \& Camera system), Deutsches Elektronen-Synchrotron (DESY) \\\hline
    Photon Detection System & INFN Bologna, INFN Padova, The Queen’s University of Belfast (Gamma Beam Profiler), The Queen’s University of Belfast (Gamma Ray Spectrometer) Deutsches Elektronen-Synchrotron (DESY) (Gamma Backscattering Calorimeter) \\\hline
    DAQ, Core Software \& Computing & Deutsches Elektronen-Synchrotron (DESY), University College London (UCL), Weizmann Institute of Science \\\hline
    Theory \& Monte Carlo & University of Gothenburg, University of Plymouth + contributors \\\hline
    Technical Coordination \& Project Management & Deutsches Elektronen-Synchrotron (DESY) \\\hline
\end{tabular}
\caption{Areas of responsibility in LUXE.}
\label{tab:resp}
\end{center}
\end{table}


Table~\ref{tab:resp} summarizes different areas of responsibility for areas within the LUXE experimental complex.


\section{Resource-Loaded Schedule}

The LUXE project schedule is driven mainly by the design, procurement and production lead times of the major elements in the experimental complex, namely the laser cleanroom surface building and laser system as well as the dipole magnets, beam dumps and interaction vacuum chamber (see fig. \ref{fig:majitemtimeline}). The installation schedule of the LUXE experiment is primarily driven by the \euxfel shutdown schedule, which foresees each year an end-of-year shutdown (duration of order one month) and a short summer shutdown (duration of order two weeks). In addition an extended long shutdown for six months is foreseen in the second half of the year 2025.Preliminary installation works will start in the shorter summer and end-of-year shutdowns in the years leading up to 2025 and the main installation of the long-lead-time major beamline elements and detectors will take place in the long shutdown in 2025.\\

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{fig/ProjectManagement/LUXEMajorItemsTimeline.png}
    \caption{LUXE major items timeline.}
    \label{fig:majitemtimeline}
\end{figure}


The order of the installation works and duration of individual tasks as listed in tab.~\ref{TC:Annex:Milestone_WP11} to~\ref{TC:Annex:Milestone_WP15} and shown in fig.~\ref{fig:luxeschedule} has been discussed with the main contributing engineer of the LUXE project. The main boundary conditions to consider for the installation are the availability of space in the LUXE cavern, availability of transport such as forklift and crane, limited allowed number of workers, especially respecting parallel works on the XTD20 extraction beamline during the 2025 shutdown, as well as the ordering and manufacturing schedule of the long lead-time components in the beamline.



\begin{figure}[htbp!]
\centering
\includegraphics[width=0.75\textwidth]{fig/ProjectManagement/LUXEInstallSchedule.png}
\includegraphics[width=0.75\textwidth]{fig/ProjectManagement/LUXEInstallSchedule_LongShutdown.png} 
\caption{LUXE overall installation schedule (top). Detailed installation schedule in 2025 long shutdown (bottom).} 
\label{fig:luxeschedule} 
\end{figure}


\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{fig/ProjectManagement/LUXEInfrastructureFTEmap.png}
    \caption{LUXE technical infrastructure FTE timeline by DESY technical groups.}
    \label{fig:luxeinfftemap}
\end{figure}

Fig.~\ref{fig:luxeinfftemap} shows the preliminary timeline of the DESY technical person-power needed for the design as well as the supervision of the manufacturing and installation of the LUXE technical infrastructure. The per-year FTE-need average is 2-3 FTE/year in FH and 1-2 FTE/year in the M-division, resulting in an integrated 8 FTE-years required in FH and 6 FTE-years in the M-division, in agreement with earlier estimates. The basis of estimate for this timeline is the list of tasks necessary to complete the infrastructure as shown in section~\ref{sec:Appendix:responsibilities}. Each task is fractionally assigned to one or several DESY groups according to the expertise profile needed. The scenario assumed in the timeline shown is that any task which lies in the expertise of FH technical personnel is completed to a major fraction by the FH personnel and technical personnel of other DESY groups is only used where necessary. A preliminary estimate of the duration, FTE and group participation needed for the individual tasks were made in discussion with the main contributing LUXE engineer and received feedback by the technical note review panel, resulting in fig.~\ref{fig:luxeschedule}. It should be emphasized that further discussions with the relevant experts from the accelerator groups are required to arrive at a more granular and precise estimate.

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{fig/ProjectManagement/LUXEInfrastructureInvestMap.png}
    \caption{LUXE technical infrastructure spending profile.}
    \label{fig:luxeinfcostmap}
\end{figure}

Finally, fig.~\ref{fig:luxeinfcostmap} shows a preliminary estimate of the invest cost schedule for the LUXE technical infrastructure. The integrated cost corresponds to 3.5MEUR with a yearly average spending of 1MEUR.  The timeline shown is based on the list of items and cost from the technical infrastructure note tab.~\ref{TC:Annex:Resources_WP61} to \ref{TC:Annex:Resources_WP64}. The cost model is made such that one separate core invest and material cost (in MEUR) and person power (in FTE) that is assumed to come from local resources (i.e. DESY groups, M or FH). The core invest estimates are based on (preliminary) quotes from vendors or on experience from experts at DESY. The estimates of the personnel resources needed come from experts. Overheads, escalation or contingency are not included.

==> chapters3/8orams.tex <==
%Discussion of challenges and approaches related to these five aspects for the system. 
%\subsection{Operability}
%The laser will be operated inside a clean room with power banks for pump lasers situated in the nearby service room. The day to day operation will be carried out by laser experts following all safety regulations.

%\subsection{Reliability}
%The Jeti40 lasers or newly installed TW laser are very reliable in operation.  
%\subsection{Availability}
%The laser will be available for running in both the phases- 0 and 1.
%\subsection{Maintainability}
%Maintenance of the laser parts such as pump lasers, optics are essential after a long run. Most of the time, replacement parts will be arranged in advance to enable a quick change. The check of safety aspects will be also maintained at regular interval as described per rule.


The laser system requires staffing at the level of two scientists (of which one can be a PhD student) and half a technician position for continuous operation. Maintenance will be performed in a accordance with well tested procedures known from the comparable systems being operated. Parts and Maintenance are assured via the optics industry and the major laser component suppliers.

\subsection{Operability}
The laser can operate non-stop over many hours with periodic realignment required if certain parameters drift too far. The laser will  go through a maintenance cycle of a daily alignment and systems performance check. Automated alignment systems will stabilise operations and warn operators of maintenance and operator requirements.  Establishment of unattended overnight running will require a ramp-up phase to gain experience with  the performance of automated alignment systems and malfunction protection devices.

\subsection{Reliability}
Experience of JETI200 operation is that unscheduled downtime is rare during the first two years of operation (once routine has been established) with unscheduled downtime increasing thereafter. Depending on budgetary constraints maintaining backup components and backup pump lasers to allow for fast turnaround parts replacement will be considered. The additional cost for mirrors, crystals and pump lasers is estimated to be of the order of 700 k€. Unscheduled downtime is currently at an average of 1 day/month. 



\subsection{Availability}
The laser system will be housed in a separate clean room as a controlled area and only authorised personnel will be allowed for the operation and maintenance. The laser beams will be transported through beamline from laser room to the interaction area. Apart from the downtime due to the maintenance work the laser beams are continuously available. In initial phase the laser operators will monitor systems and develop the automated alignment system. During the development of automation, staff working hours will limit laser up-time. As discussed in the note, stable overnight running with automated alignment and shut-off systems will be implemented during the early phase of LUXE. 


\subsection{Maintainability}

The system will use parts widely available in the optics industry and from a range of suppliers. This will ensure maintainability of the system for the duration of LUXE.

Routine maintenance is focused on replacement of pump-laser parts and optical components which degrade over time as well as power electronics in the pump lasers on a longer timescale. 

The major components requiring routine maintenance at certain interval are the pump lasers as they use flash lamps. A flash lamp has a lifespan of  30  to 50 million shots to be taken. At 10 Hz repetition rate and running for 24 hours, this would mean that flashlamps must be replaced several times a year. 
Cooling systems also require routine maintenance (filter, water change) which can take place at the same time as flashlamp maintenance. Such maintenance can be performed within a day.  Longer maintenance will be required once a quarter to do a detailed systems check of all sub-systems including optics cleaning and replacement of optics showing signs of degradation.
Vacuum components such as scroll and turbo pumps installed at the compressor and beamline require routine maintenance which will take place during the longer maintenance shut-downs. We note that maintenance shut-down can be minimised by providing redundancy. However this is not deemed cost-effective.


\subsection{Safety}
The LUXE laser system described  is a class 4 laser system capable of generating ionising radiation in focus.  Here we describe the main safety considerations with specific attention given to the set-up at LUXE. The detailed safety requirements are well understood and have been implemented previously at \euxfel and DESY for very similar systems. For example, the multi-100TW Ti:Sa ReLaX laser system at the HED beamline of \euxfel is directly comparable Ti:Sa in all safety relevant aspects and the implementation of the safety system will mirror those at ReLaX closely.

\subsubsection{Laser operation modes} 
The laser will always be operated at minimum power and intensity required to ensure safety at all times. The following energy/power settings will be available and will be interlocked to appropriate operator modes.

\begin{itemize}
\item Ultra-low Intensity (nanosecond) \\
In this mode the laser uses the self-seeded regenerative amplifier (regen) described in the previous sections (i.e. the seed is blocked by an interlocked shutter). The  pulse duration is determined by the regen roundtrip time (12.5 ns in the case of JETI). This reduces the laser intensity for a given pulse energy E by 
\begin {equation}
 I_{ULI}(E)=I_{fs}(E) \frac{\tau_{Regen}}{\tau_L} <3\times10^{-6}  I_{fs}(E)\,\,.
\end {equation}
For full regen output ($<0.5$ mJ at the IP focus) the peak intensity will be   below $10^{11}$ Wcm$^{-2}$ - far below the level at which ionisation becomes relevant.
\item Low Intensity (nanosecond) \\
The same operating mode allows a maximum energy in excess of 10 mJ with  (exact values depending on Regen roundtrip time of laser) while staying below the ionising threshold for all beam sizes including the IP focus and enables the beam to be safely and easily aligned.
\item Low Intensity (femtosecond)  \\
The laser will be attenuated to intensities below ionisation threshold in the the IP focus. Depending on transport efficiency in the system this corresponds to $\upmu$J level pulses.
\end{itemize}

Higher energy modes at full compression will be available with interlocked enclosures to ensure safe working. Intensities  at which ionising radiation can be present will require area interlocks to prevent access.

The interlock system will be zoned to allow operational modes to be set with lasers present only in certain restricted areas.\\

{\bf Mode 1}: Laser-only operation\\
An interlocked shutter system will be installed prior to the beamline transporting the laser to the IP to allow the laser to be operated independently from the beamline/IP chamber for set-up purposes.
The laser shutter will be in a beam dump enclosure and be made of high damage threshold material (e.g. Alumina ceramic) to allow the laser to be operated at up to full power with the energy being dumped/diffused in the shutter/beamdump assembly.

This mode will have different interlock settings  on intensity depending on whether the laser beam can be accessed by the operator or if the compressed beam is fully enclosed.\\

{\bf Mode 2}: Interaction Point (IP) Mode \\
In IP mode the laser will be allowed to propagate to the IP chamber. The availability of the energy modes will depend on the interlock status (IP area without personnel, IP area with vacuum system closed (no access to high intensity), IP area and chamber accessible).



%We need to also ensure that a safe level of laser energy is reached in the IP chamber. All q-switches of the pump lasers of the amplifiers will be interlocked. Meaning that during the alignment in the interaction area, the main amplification can not take place. The front end energy (about $500 \mu$ J ) will be only available. Such level of energy is required to align for example during the set up of optics inside the IP camber. The focused intensity at the IP will be 2.1016 W/cm2 for a tight focus diameter of $3\mu$ m (FWHM). However, the intensity outside the area of 3mm2 will be already below 10w/cm2 due to the fast diverging beam (beam diameter at 2cm from IP= 0.66cm). 

%{\bf high power alignment} \\

The focus of the laser must be characterised both with the IP diagnostic and with the diagnostic system. Meaningful measurement requires the laser to operate under full power conditions.  To ensure that energy in the pulse does not exceed as in the alignment case, an interlockable $10^{-6}$ attenuator  will be inserted in the path of the laser beam after the last stage of the amplification and before the compressor. This attenuator consists of high quality ($<\lambda/20$) uncoated mirrors mounted in a so called dog-leg geometry. The insertion of this attenuator will be done using a motorised translation stage. This stage can be interlocked with the laser to ensure that attenuator is at in position when the beam is fully amplified.  A pointing monitor in laser bay with switchable attenuation will ensure that the laser is propgating down an identical path both with and without the attenuator present.\\

{\bf High power mode} \\

For operation at full power (data acquisition and full power live diagnostic laser only).  The IP area will be searched and fully locked, so that no one can access it while the laser is operating at full power and/or the electron beam is present. In this mode the  full energy laser pulse can be delivered at the IP and, after initial attenuation in the IP chamber, propagate to the diagnostic suite in the laser clean room.  Interactions of the GeV beam with laser pulse can take place.

\subsubsection{Safety protocols}
%do we need to describe all the details of safety interlocks, emergency switches, entry to the laser room etc?\\
In other labs at DESY \cite{laser28m} and in EuXFEL-HIBEF (which host $> 300$ TW class IV lasers) \cite{hibef} the safety procedures for the alignment and focus check is as discussed above. This is so called``Justierung mode-alignment mode". The main safety interlock is at the attenuator which does not allow high energy in the pulse when the laser is in alignment mode. During the ``Sperrbereich-mode" (shooting mode), the interaction area is fully locked and the attenuator moves out of the beam path allowing full energy in the pulse. Other standard procedures are the announcement of the laser beam being sent to the IP area and when the interaction area is being locked for the high power interaction mode.





==> chapters3/9organisation.tex <==
The related costs, manpower and timelines are discussed in detail. The timeline for laser sub-project are largely independent of the \euxfel shutdown schedule. Preparatory work can be conducted at available lasers (Jena or Tel Aviv) and once the clean-room is ready for installation in the clean room. 

The laser installation schedule intercepts with the \euxfel schedule only for the installation of the IP chamber (which is part of the electron beamline in the \euxfel tunnel XS1) and the laser beamline components in XS1. The latter does not require a long shutdown for installation (discussed in Chapter 12) while the IP chamber interior components are modular and can be pre-aligned and installed at short notice. 

There are two distinct scenarios with regards to the installation of the laser. The first is the locating the laser in level -2 above the \euxfel tunnel (considered in the CDR). This could still  be a viable option, but for reasons detailed in Chapter 12 the currently preferred option is a clean room constructed at ground level. This option is visible in the timelines. We note that changing the location does not have a major impact on the laser installation schedule.

The activities regarding the construction of the laser and beamline are distributed across four collaborating institutes: Deutsches Elektronen Synchrotron (DESY), Friederich-Schiller University Jena and Helmholtz Institute  Jena, The Queen's University of Belfast and Tel Aviv University of Israel. Jena will co-ordinate the implementation of the laser system.

\subsection{Human and financial resources}

Below we detail the resources required for the implementation of the preferred option of integrating a new 350 TW laser system into LUXE.
The activities can be split into 5 major areas of investment:

\begin{itemize}
    \item Laser
    \item Laser automation
    \item Diagnostics
    \item Laser Beamline
    \item Tunnel Diagnostics
    
\end{itemize}

Resources for the vacuum components and beamlines directly associated with the laser (compressor, diagnostics chamber) are included in the laser budget while vacuum pumps for the electron beamline and the integration of the laser diagnostics into the DAQ system are considered within the context of the Technical Coordination and DAQ TDR chapters respectively .

\subsubsection{Financial Resources} 
The net investment cost as per quotations and estimates is listed below and summarised in Table \ref{tab:cost}. We note that these costs are currently subject to inflationary pressures.

\begin{itemize}
    \item \textbf{Laser system }\\
This cost is based on a quotation from Thales  as shown in table \ref{tab:cost}. The estimate comprises oscillator, amplifier and compressor+ chamber. A staged implementation would split the capital costs over the course of the project with with phase-0 delaying the cost of the  \euro1700k amplifier to a later stage in the project. Common components of phase-0 with phase-1 such as beamline and compressor will be built to be compatible with both implementation stages.


A detailed breakdown is shown in Table~\ref{tab:New_laser_system_cost} and Table~\ref{tab:Jeti40_laser_system_cost} in the appendix.

\item \textbf{Laser automation: \euro250k}\\
Automation of key alignment procedures in the laser will allow the stable operation for extended periods without manual intervention. 

\begin{table}[]
    \centering
    \caption{Cost estimates for the laser project (in k\euro). }
    %\begin{tabular}{l|r|l}
    \begin{tabular}{|p{4cm}|p{2cm}|p{6cm}|}
         \hline
         350 TW Laser Amplifier System  & 3685 & quote  \\\hline
         Oscillator  & 160 & quote  \\\hline
         Timing  & 80 & quote  \\\hline
         Compressor  & 250 & quote  \\\hline
         Automation & 250 & based on JETI200 components\\\hline
         Laser  diagnostics & 310 & quote + based on JETI200\\\hline
         Beamline & 400 & quote +  based on experience\\\hline
         Vacuum chamber & 95 & quote + based on experience \\\hline
         Tunnel diagnostics & 115 & quote +  based on experience\\\hline

         
        \textbf{Total sum} & \textbf{5345} & Total expenditure
         \\\hline
    \end{tabular}
    \label{tab:cost}
\end{table}

\item \textbf{Laser diagnostics: \euro310k }\\
The costings for laser area diagnostics includes the purchase of all the laser characterisation devices, optics, cameras, mounts, vacuum chamber for the diagnostics and required vacuum pump. Detailed cost breakdown by item  is given in Appendix in  Table~\ref{tab:laser_area_diag_cost}. 
 
\item \textbf{Transport beamline cost: \euro400k}\\
The cost of the laser transport line includes cost of mirror mounts, mirrors and other items required for steering the optics and monitoring.  A detailed cost breakdown is given in the appendix in  Table~\ref{tab:laser_beamline_cost}.

\item \textbf{IP chamber: \euro95k}\\
The IP chamber cost includes the actual IP chamber and the optical table beneath the IP chamber. As the IP chamber is integrated in the LUXE particle beam line cost relating to vacuum pumps, gate valves and control system are included in infrastructure section.

\item \textbf{Tunnel diagnostics:\euro115}\\
The tunnel diagnostics consist of an imaging system for the IP and the optomechnical components for the diagnostics and timing diagnostic. 
\end{itemize}

A detailed budget breakdown can be found in the appendix.

\subsubsection{Human Resources} 

During the life time of the project 2 physicists and 0.5 technicians are required on a permanent basis for the operation of the laser and diagnostics. During the early phase of the project they are responsible for planning, purchasing and development. In particular the tunnel and laser diagnostics can be fully implemented and tested with final installation as soon as the infrastructure at Osdorfer Born is ready.
 They will coordinate with the laser manufacturer during manufacture  and supervise the acceptance procedures and installation.

Additional effort is required during installation to implement laser safety interlock system and integrate it into Osdorfer Born. Support for installation and commissioning of services (electrical/water) and vacuum systems by the respective  technical groups at DESY/XFEL.

\textbf{Additional  personnel for installation}\\
 The disassembly at the factory and installation of the laser will be performed by the laser company. During the installation the LUXE laser team will be present full time and learn the operation of the system.
 
 Additional technical staff is required for the installation of the laser beamline and services. This is estimated at 1.5 FTE (3  technicians for 6 months)
 

%\begin{table}[]
    %\centering
   % \caption{Cost estimates for personnel required during phase 0 and 1.}
    %\begin{tabular}{l|r|l}
  %  \begin{tabular}{|p{4cm}|p{2cm}|p{2cm}|p{1.5cm}|p{2cm}|}
       % \hline
        %Components  & FTE Phase 0 & FTE Phase 1 & Cost (kEur) \\\hline
        % Lasers & 4 & 5  & 720  \\\hline
         
         %Transport Beamline & 3 & - & 240 \\\hline
         
         %Tunnel and laser Diagnostics & 6 & 1 & 440 \\\hline
        % Vacuum chambers & 1 & 1 & - \\\hline
        %\textbf{Total sum} &  &  & 
         %\\\hline
   % \end{tabular}
 %   \label{tab:cost_personnel}
%\end{table}

\subsection{Schedule and milestones}

The schedule for the laser system installation at the LUXE site is shown in the Fig. ~\ref{fig:schedule}. The main constraints on laser readiness are the availability of a laser cleanroom and the delivery of a new laser system (under the preferred scenario). The timelines for these two major constraints are well matched and will take about 2\textonehalf years.

 The preferred  option operationally is to install the complete 350 TW laser system. Installation of a phase-0,  40 TW laser system will result in additional downtime of the order of 6 weeks at a later point and will not allow the full range of parameters at the earliest stage.  
 
 Beamline installation can be performed at any stage. Vacuum components are relatively short lead-time items. Infrastructure work (holes in the walls/floors) is relatively quickly executed and can be fitted into short shut-downs. The beamline can be fully pre-aligned using low power lasers.
 
 Work on diagnostics (both tunnel and laser) can proceed off-line at available facilities and be stored ready for installation once the clean-room/tunnel are available for installation.
 
 The milestones for the installation are as follows:
 
 \begin{itemize}
  \setlength\itemsep{0pt}
     \item {\normalfont \bfseries~M1}	Tender ready
     \item {\normalfont \bfseries~M2}	Laser contract placed
     \item {\normalfont \bfseries~M3} Factory Acceptance Test complete
     \item {\normalfont \bfseries~M4} Laser installation complete
     \item {\normalfont \bfseries~M5} Synchronisation complete
     \item {\normalfont \bfseries~M6} Diagnostics concept finalised
     \item {\normalfont \bfseries~M7} Diagnostics installed
     \item {\normalfont \bfseries~M8}	Beamline defined 
     \item {\normalfont \bfseries~M9}	Target beamline complete
     \item {\normalfont \bfseries~M10} Automation concept complete
     \item {\normalfont \bfseries~M11} Stable operation for data runs
 \end{itemize}

 
\begin{figure}[htbp]
    \centering
    \includegraphics[width=01.0\textwidth]{fig/schedule.pdf}
    \caption{Schedule for the laser installation at the LUXE site.}
    \label{fig:schedule}
\end{figure}
%As we have not decided yet with the laser system option (expected by March 2022), we consider new laser system as option A and Jeti40 system as  a backup. The schedule for laser installation also depends on the release of the fund from DESY (most likely by mid June 2022) and procurement time. Assuming 18 months lead time for the procurement of the brand new laser system (might change with pandemic situation?), we aim the installation and commissioning to be finished by July 2024. 

%It is worth to mention here that if the set up in interaction area is ready by Q1 of 2024, the commissioning of detectors (particle/photon) can take just with the electron beam for the optimisation purpose.


%The installation of the 40TW laser system is dependent of availability of the clean room. As mentioned above, the release of the fund will start at mid of 2022, the clean room is expected to be ready by middle of 2023. Due to high radiation dose in the clean room area (due to e-beam operation of XFEL), it is preferred to install also the Jeti40 during the XFEL long shutdown. 
%Prior to that Jeti40 laser first has to be transported from Jena to Osdorfer Born. The system is continuously developed over the time, hence its architecture (all optical arrangements) has to be exactly reproduced.This will be done in consultation with the laser expert already operating Jeti40. 
%The major milestones en route to LUXE, we would like to mark are the following:\\

%\textbf{For the  laser system}
%\begin{itemize}
%    \item preparation of disassembly of all components (2022?). This means a self made manual for each and every single item related with the laser will be prepared. All the precautionary details will  be noted down and has to be followed while assembly the laser and any item.
%    \item As the laser system will be used for diagnostic development, disassembly will take place at the end (Q3-2023)
%    \item transport at the end of 2023?
%    \item start of the assembly Q1-2024. This includes synchronisation of oscillator and integration also with control software environment, eg. DOOCS/JDDD? 
%    \item Final optimisation and commissioning Q2-2024
%\end{itemize}

%\textbf{For the  laser area diagnostics}\\
%The preparations of setting up all the relevant diagnostics for the LUXE is going on Jeti200/Jeti40 laser systems. The major milestones to achieve are:
%\begin{itemize}
%    \item finish set up and optimisation of all the diagnostics on individual breadboard? untill Q3 2023?
%    \item at the sametime test of TLU-DAQ integration?
%    \item transport to LUXE- end of 2023
%    \item installation at diagnostic table with alignment laser Q1-2 2024. The commissioning with main beam depends on the  laser installation
%    \item commissioning?
%\end{itemize}

%\textbf{For the  transport beamline}\\
%\begin{itemize}
%   \item finalise the the transport line design Q1-2 2023?
%   \item procurement of all hardware parts until 2023?
%   \item installation and integration with IP chamber Q1-2 2024?
%\end{itemize}  

%\textbf{For the IP chamber and target area diagnostics}\\
%\begin{itemize}  
%   \item Most of this diagnostics depends on the final installation of the IP chamber. Once the mechanical installation of IP chamber is finished and integration with other interfaces is completed, the diagnostics can be placed inside it. 
%   \item the optical layout and related hardware with each diagnostics will be already finalised
%    \item what about timing tool
%\end{itemize}
%The commissioning of the laser including diagnostics is planned during Q4-2023 and Q1-2 2024. Optical setup such as for diagnostics which could be pre-aligned outside the laser area will be done to avoid long working time inside the laser area.

%As the probability to purchase a new commercial 40TW laser system already for Phase 0 is growing, the impact of this exercise is also shown in the schedule (see Fig. ~\ref{fig:schedule}. In this case the installation and commissioning can take place during Q3-4 of 2023. Furthermore, the commissioning of diagnostics can take place during Q1 of 2024. 
%\RP{these numbers are just a starter as i am not sure about all the numbers. We need to give each and every details with good confidence!!}

\subsection{Risk management}
The main risks are discussed and their impact is quantified in terms of cost and schedule with respective probabilities and mitigation strategies:

There are two dimensions, the impact and the probability. We separate the impact on the cost and the schedule and use the following terms for impact risks:
\begin{itemize}
    \item Insignificant: Risk is easily mitigated by day to day process. 
    \item Minor: Delays up to 10\% of schedule. Cost increase up to 10\% of budget. 
    \item Moderate: Delays up to 30\% of schedule. Cost increase up to 30\% of budget. 
    \item Major: Delays up to 50\% of schedule. Cost increase up to 50\% of budget. 
    \item Catastrophic: project abandoned
\end{itemize}


For the budget, the denominator used is the budget of that area, i.e. if it is in the phase-0 laser area it is relative to the total phase-0 laser costs. In any case for the cost also the absolute numbers are given, so we can easily renormalize if the total cost changes.

For the schedule, the fraction is taken relative to 24 months, assuming a start in January 2022 and a readiness of January 2024. 

The probability of a risk to be realized is quantified as, rare: ($<3$\%), unlikely (3-10\%), moderate (10-50\%), likely (50-90\%) or certain ($>90\%$). 

Table˜\ref{tab:risks} shows a template for a summary of the risks.
\begin{table}[]
    \centering
    \caption{Risk description, potential impact on cost and schedule, probability to occur and strategy on how to mitigate the risk.}
\begin{tabular}{p{0.2\linewidth}|p{0.1\linewidth}|p{0.13\linewidth}|p{0.13\linewidth}|p{0.3\linewidth}}
         Description & Cost & Schedule & Probability & Strategy\\\hline
         & & & & \\\hline
         Mechanical Jitter Causes Overlap Problems & Medium 30 \% & Moderate (6~Months) & Medium (w/o tests) & Beamline Design and tests prior to installation   \\\hline
         Maintenance downtime & 10\% of laser cost pa & Lost beam weeks & High
& Schedule maintenance,
System monitoring Preemptive maintenance/ new laser rather JETI 40 \\\hline

Radiation degradation of tunnel diagnostics &
Low (replacement)  & Loss of beamtime & High & Choose components with known rad hardness, shield, spares readily available \\\hline

Laser automation not to plan & Moderate 20\%  & Medium Continuous loss of time & Medium & Start design now, Apply  proven automation strategy \\\hline

Low Damage threshold optics - shoot with lower energy & 30 \% & 10 \% & Low & test optics before installation \\\hline


Insufficient Diagnostic precision - lower data precision & Medium 30\%  & Low 10 \% & Low & test optics before installation \\\hline

Synchronisation jitter too high - intensity fluctuations in the data & Low & Medium & Low (based on HIBEF experience) & Active drift stabilisation may be required or changed IP geometry \\
\hline
\hline
\end{tabular}
\label{tab:risks}
\end{table}


\subsection{Responsibilities}
%Discuss which institute takes responsibility for what aspect.
The responsible institutions are Jena, DESY and Tel Aviv. Leadership and responsibility of the overall project is with Jena, and also of the Laser and Diagnostic sub-project. Infrastructure related planning is delegated to DESY and the vacuum chamber design is delegated to Tel Aviv.

\subsection{Laser Safety Considerations}
The LUXE laser system described  is a class 4 laser system capable of generating ionising radiation in focus.  Here we describe the main safety considerations with specific attention given to the set-up at LUXE. The detailed safety requirements are well understood and have been implemented previously at \euxfel and DESY for very similar systems. For example, the multi-100 TW Ti:Sa ReLaX laser system at the HED beamline of \euxfel is directly comparable Ti:Sa in all safety relevant aspects and the implementation of the safety system will mirror those at ReLaX closely.

\subsubsection{Laser operation modes} 
The laser will always be operated at minimum power and intensity required to ensure safety at all times. The following energy/power settings will be available and will be interlocked to appropriate operator modes.

\begin{itemize}
\item Ultra-low Intensity (nanosecond) \\
In this mode the laser uses the self-seeded regenerative amplifier (regen) described in the previous sections (i.e. the seed is blocked by an interlocked shutter). The  pulse duration is determined by the regen roundtrip time (12.5 ns in the case of JETI). This reduces the laser intensity for a given pulse energy E by 
\begin {equation}
 I_{ULI}(E)=I_{fs}(E) \frac{\tau_{Regen}}{\tau_L} <3\times10^{-6}  I_{fs}(E)\,\,.
\end {equation}
For full regen output ($<0.5$ mJ at the IP focus) the peak intensity will be   below $10^{11}$ Wcm$^{-2}$ - far below the level at which ionisation becomes relevant.
\item Low Intensity (nanosecond) \\
The same operating mode allows a maximum energy in excess of 10 mJ with  (exact values depending on Regen roundtrip time of laser) while staying below the ionising threshold for all beam sizes including the IP focus and enables the beam to be safely and easily aligned.
\item Low Intensity (femtosecond)  \\
The laser will be attenuated to intensities below ionisation threshold in the the IP focus. Depending on transport efficiency in the system this corresponds to $\mu$J level pulses.
\end{itemize}

Higher energy modes at full compression will be available with interlocked enclosures to ensure safe working. Intensities  at which ionising radiation can be present will require area interlocks to prevent access.

The interlock system will be zoned to allow operational modes to be set with lasers present only in certain restricted areas.

{\normalfont \bfseries Mode 1}: Laser-only operation\\
An interlocked shutter system will be installed prior to the beamline transporting the laser to the IP to allow the laser to be operated independently from the beamline/IP chamber for set-up purposes.
The laser shutter will be in a beam dump enclosure and be made of high damage threshold material (e.g. Alumina ceramic) to allow the laser to be operated at up to full power with the energy being dumped/diffused in the shutter/beamdump assembly.

This mode will have different interlock settings  on intensity depending on whether the laser beam can be accessed by the operator or if the compressed beam is fully enclosed.\\

{\normalfont \bfseries Mode 2}: Interaction Point (IP) Mode \\
In IP mode the laser will be allowed to propagate to the IP chamber. The availability of the energy modes will depend on the interlock status (IP area without personnel, IP area with vacuum system closed (no access to high intensity), IP area and chamber accessible).



%We need to also ensure that a safe level of laser energy is reached in the IP chamber. All q-switches of the pump lasers of the amplifiers will be interlocked. Meaning that during the alignment in the interaction area, the main amplification can not take place. The front end energy (about $500 \mu$ J ) will be only available. Such level of energy is required to align for example during the set up of optics inside the IP camber. The focused intensity at the IP will be 2.1016 W/cm2 for a tight focus diameter of $3\mu$ m (FWHM). However, the intensity outside the area of 3mm2 will be already below 10w/cm2 due to the fast diverging beam (beam diameter at 2cm from IP= 0.66cm). 

%{\normalfont \bfserieshigh power alignment} \\

The focus of the laser must be characterised both with the IP diagnostic and with the diagnostic system. Meaningful measurement requires the laser to operate under full power conditions.  To ensure that the energy in the pulse does not exceed the one in the alignment case, an interlockable $10^{-6}$ attenuator  will be inserted in the path of the laser beam after the last stage of the amplification and before the compressor. This attenuator consists of high quality ($<\lambda/20$) uncoated mirrors mounted in a so called dog-leg geometry. The insertion of this attenuator will be done using a motorised translation stage. This stage can be interlocked with the laser to ensure that attenuator is at in position when the beam is fully amplified.  A pointing monitor in laser bay with switchable attenuation will ensure that the laser is propagating down an identical path both with and without the attenuator present.\\

{\normalfont \bfseries High power mode} \\

For operation at full power (data acquisition and full power live diagnostic laser only).  The IP area will be searched and fully locked, so that no one can access it while the laser is operating at full power and/or the electron beam is present. In this mode the  full energy laser pulse can be delivered at the IP and, after initial attenuation in the IP chamber, propagate to the diagnostic suite in the laser clean room.  Interactions of the GeV beam with the laser pulse can take place.

\subsubsection{Safety protocols}
%do we need to describe all the details of safety interlocks, emergency switches, entry to the laser room etc?\\
In other labs at DESY \cite{laser28m} and in EU.\\EuXFEL-HIBEF (which host $> 300$ TW class IV lasers) \cite{hibef} the safety procedures for the alignment and focus check is as discussed above. This is so called``Justierung mode-alignment mode". The main safety interlock is at the attenuator which does not allow high energy in the pulse when the laser is in alignment mode. During the ``Sperrbereich-mode" (shooting mode), the interaction area is fully locked and the attenuator moves out of the beam path allowing full energy in the pulse. Other standard procedures are the announcement of the laser beam being sent to the IP area and when the interaction area is being locked for the high power interaction mode.


==> chapters3/9organisation_TDR.tex <==
The related costs, manpower and timelines are discussed in detail. The timeline for laser sub-project are largely independent of the \euxfel shutdown schedule. Preparatory work can be conducted at available lasers (Jena or Tel Aviv) and once the clean-room is ready for installation in the clean room. 

The laser installation schedule intercepts with the \euxfel schedule only for the installation of the IP chamber (which is part of the electron beamline in the \euxfel tunnel XS1) and the laser beamline components in XS1. The latter does not require a long shutdown for installation (discussed in Chapter 12) while the IP chamber interior components are modular and can be pre-aligned and installed at short notice. 

There are two distinct scenarios with regards to the installation of the laser. The first is the locating the laser in level -2 above the \euxfel tunnel (considered in the CDR). This could still  be a viable option, but for reasons detailed in Chapter 12 the currently preferred option is a clean room constructed at ground level. This option is visible in the timelines. We note that changing the location does not have a major impact on the laser installation schedule.

The activities regarding the construction of the laser and beamline are distributed across four collaborating institutes: Deutsches Elektronen Synchrotron (DESY), Friederich-Schiller University Jena and Helmholtz Institute  Jena, The Queen's University of Belfast and Tel Aviv University of Israel. Jena will co-ordinate the implementation of the laser system.

\subsection{Human and financial resources}

Below we detail the resources required for the implementation of the preferred option of integrating a new 350 TW laser system into LUXE.
The activities can be split into 5 major areas of investment:

\begin{itemize}
    \item Laser
    \item Laser automation
    \item Diagnostics
    \item Laser Beamline
    \item Tunnel Diagnostics
    
\end{itemize}

Resources for the vacuum components and beamlines directly associated with the laser (compressor, diagnostics chamber) are included in the laser budget while vacuum pumps for the electron beamline and the integration of the laser diagnostics into the DAQ system are considered within the context of the Technical Coordination and DAQ TDR chapters respectively .

\subsubsection{Financial Resources} 
The net investment cost as per quotations and estimates is listed below and summarised in Table \ref{tab:cost}. We note that these costs are currently subject to inflationary pressures.

\begin{itemize}
    \item \textbf{Laser system }\\
This cost is based on a quotation from Thales  as shown in table \ref{tab:cost}. The estimate comprises oscillator, amplifier and compressor+ chamber. A staged implementation would split the capital costs over the course of the project with with phase-0 delaying the cost of the  \euro1700k amplifier to a later stage in the project. Common components of phase-0 with phase-1 such as beamline and compressor will be built to be compatible with both implementation stages.


A detailed breakdown is shown in Table~\ref{tab:New_laser_system_cost} and Table~\ref{tab:Jeti40_laser_system_cost} in the appendix.

\item \textbf{Laser automation: \euro250k}\\
Automation of key alignment procedures in the laser will allow the stable operation for extended periods without manual intervention. 

\begin{table}[]
    \centering
    \caption{Cost estimates for the laser project (in k\euro). }
    %\begin{tabular}{l|r|l}
    \begin{tabular}{|p{4cm}|p{2cm}|p{6cm}|}
         \hline
         350 TW Laser Amplifier System  & 3685 & quote  \\\hline
         Oscillator  & 160 & quote  \\\hline
         Timing  & 80 & quote  \\\hline
         Compressor  & 250 & quote  \\\hline
         Automation & 250 & based on JETI200 components\\\hline
         Laser  diagnostics & 310 & quote + based on JETI200\\\hline
         Beamline & 400 & quote +  based on experience\\\hline
         Vacuum chamber & 95 & quote + based on experience \\\hline
         Tunnel diagnostics & 115 & quote +  based on experience\\\hline

         
        \textbf{Total sum} & \textbf{5345} & Total expenditure
         \\\hline
    \end{tabular}
    \label{tab:cost}
\end{table}

\item \textbf{Laser diagnostics: \euro310k }\\
The costings for laser area diagnostics includes the purchase of all the laser characterisation devices, optics, cameras, mounts, vacuum chamber for the diagnostics and required vacuum pump. Detailed cost breakdown by item  is given in Appendix in  Table~\ref{tab:laser_area_diag_cost}. 
 
\item \textbf{Transport beamline cost: \euro400k}\\
The cost of the laser transport line includes cost of mirror mounts, mirrors and other items required for steering the optics and monitoring.  A detailed cost breakdown is given in the appendix in  Table~\ref{tab:laser_beamline_cost}.

\item \textbf{IP chamber: \euro95k}\\
The IP chamber cost includes the actual IP chamber and the optical table beneath the IP chamber. As the IP chamber is integrated in the LUXE particle beam line cost relating to vacuum pumps, gate valves and control system are included in infrastructure section.

\item \textbf{Tunnel diagnostics:\euro115}\\
The tunnel diagnostics consist of an imaging system for the IP and the optomechnical components for the diagnostics and timing diagnostic. 
\end{itemize}

A detailed budget breakdown can be found in the appendix.

\subsubsection{Human Resources} 

During the life time of the project 2 physicists and 0.5 technicians are required on a permanent basis for the operation of the laser and diagnostics. During the early phase of the project they are responsible for planning, purchasing and development. In particular the tunnel and laser diagnostics can be fully implemented and tested with final installation as soon as the infrastructure at Osdorfer Born is ready.
 They will coordinate with the laser manufacturer during manufacture  and supervise the acceptance procedures and installation.

Additional effort is required during installation to implement laser safety interlock system and integrate it into Osdorfer Born. Support for installation and commissioning of services (electrical/water) and vacuum systems by the respective  technical groups at DESY/XFEL.

\textbf{Additional  personnel for installation}\\
 The disassembly at the factory and installation of the laser will be performed by the laser company. During the installation the LUXE laser team will be present full time and learn the operation of the system.
 
 Additional technical staff is required for the installation of the laser beamline and services. This is estimated at 1.5 FTE (3  technicians for 6 months)
 

%\begin{table}[]
    %\centering
   % \caption{Cost estimates for personnel required during phase 0 and 1.}
    %\begin{tabular}{l|r|l}
  %  \begin{tabular}{|p{4cm}|p{2cm}|p{2cm}|p{1.5cm}|p{2cm}|}
       % \hline
        %Components  & FTE Phase 0 & FTE Phase 1 & Cost (kEur) \\\hline
        % Lasers & 4 & 5  & 720  \\\hline
         
         %Transport Beamline & 3 & - & 240 \\\hline
         
         %Tunnel and laser Diagnostics & 6 & 1 & 440 \\\hline
        % Vacuum chambers & 1 & 1 & - \\\hline
        %\textbf{Total sum} &  &  & 
         %\\\hline
   % \end{tabular}
 %   \label{tab:cost_personnel}
%\end{table}

\subsection{Schedule and milestones}

The schedule for the laser system installation at the LUXE site is shown in the Fig. ~\ref{fig:schedule}. The main constraints on laser readiness are the availability of a laser cleanroom and the delivery of a new laser system (under the preferred scenario). The timelines for these two major constraints are well matched and will take about 2\textonehalf years.

 The preferred  option operationally is to install the complete 350 TW laser system. Installation of a phase-0,  40 TW laser system will result in additional downtime of the order of 6 weeks at a later point and will not allow the full range of parameters at the earliest stage.  
 
 Beamline installation can be performed at any stage. Vacuum components are relatively short lead-time items. Infrastructure work (holes in the walls/floors) is relatively quickly executed and can be fitted into short shut-downs. The beamline can be fully pre-aligned using low power lasers.
 
 Work on diagnostics (both tunnel and laser) can proceed off-line at available facilities and be stored ready for installation once the clean-room/tunnel are available for installation.
 
 The milestones for the installation are as follows:
 
 \begin{itemize}
  \setlength\itemsep{0pt}
     \item {\normalfont \bfseries~M1}	Tender ready
     \item {\normalfont \bfseries~M2}	Laser contract placed
     \item {\normalfont \bfseries~M3} Factory Acceptance Test complete
     \item {\normalfont \bfseries~M4} Laser installation complete
     \item {\normalfont \bfseries~M5} Synchronisation complete
     \item {\normalfont \bfseries~M6} Diagnostics concept finalised
     \item {\normalfont \bfseries~M7} Diagnostics installed
     \item {\normalfont \bfseries~M8}	Beamline defined 
     \item {\normalfont \bfseries~M9}	Target beamline complete
     \item {\normalfont \bfseries~M10} Automation concept complete
     \item {\normalfont \bfseries~M11} Stable operation for data runs
 \end{itemize}

 
\begin{figure}[htbp]
    \centering
    \includegraphics[width=01.0\textwidth]{fig/schedule.pdf}
    \caption{Schedule for the laser installation at the LUXE site.}
    \label{fig:schedule}
\end{figure}
%As we have not decided yet with the laser system option (expected by March 2022), we consider new laser system as option A and Jeti40 system as  a backup. The schedule for laser installation also depends on the release of the fund from DESY (most likely by mid June 2022) and procurement time. Assuming 18 months lead time for the procurement of the brand new laser system (might change with pandemic situation?), we aim the installation and commissioning to be finished by July 2024. 

%It is worth to mention here that if the set up in interaction area is ready by Q1 of 2024, the commissioning of detectors (particle/photon) can take just with the electron beam for the optimisation purpose.


%The installation of the 40TW laser system is dependent of availability of the clean room. As mentioned above, the release of the fund will start at mid of 2022, the clean room is expected to be ready by middle of 2023. Due to high radiation dose in the clean room area (due to e-beam operation of XFEL), it is preferred to install also the Jeti40 during the XFEL long shutdown. 
%Prior to that Jeti40 laser first has to be transported from Jena to Osdorfer Born. The system is continuously developed over the time, hence its architecture (all optical arrangements) has to be exactly reproduced.This will be done in consultation with the laser expert already operating Jeti40. 
%The major milestones en route to LUXE, we would like to mark are the following:\\

%\textbf{For the  laser system}
%\begin{itemize}
%    \item preparation of disassembly of all components (2022?). This means a self made manual for each and every single item related with the laser will be prepared. All the precautionary details will  be noted down and has to be followed while assembly the laser and any item.
%    \item As the laser system will be used for diagnostic development, disassembly will take place at the end (Q3-2023)
%    \item transport at the end of 2023?
%    \item start of the assembly Q1-2024. This includes synchronisation of oscillator and integration also with control software environment, eg. DOOCS/JDDD? 
%    \item Final optimisation and commissioning Q2-2024
%\end{itemize}

%\textbf{For the  laser area diagnostics}\\
%The preparations of setting up all the relevant diagnostics for the LUXE is going on Jeti200/Jeti40 laser systems. The major milestones to achieve are:
%\begin{itemize}
%    \item finish set up and optimisation of all the diagnostics on individual breadboard? untill Q3 2023?
%    \item at the sametime test of TLU-DAQ integration?
%    \item transport to LUXE- end of 2023
%    \item installation at diagnostic table with alignment laser Q1-2 2024. The commissioning with main beam depends on the  laser installation
%    \item commissioning?
%\end{itemize}

%\textbf{For the  transport beamline}\\
%\begin{itemize}
%   \item finalise the the transport line design Q1-2 2023?
%   \item procurement of all hardware parts until 2023?
%   \item installation and integration with IP chamber Q1-2 2024?
%\end{itemize}  

%\textbf{For the IP chamber and target area diagnostics}\\
%\begin{itemize}  
%   \item Most of this diagnostics depends on the final installation of the IP chamber. Once the mechanical installation of IP chamber is finished and integration with other interfaces is completed, the diagnostics can be placed inside it. 
%   \item the optical layout and related hardware with each diagnostics will be already finalised
%    \item what about timing tool
%\end{itemize}
%The commissioning of the laser including diagnostics is planned during Q4-2023 and Q1-2 2024. Optical setup such as for diagnostics which could be pre-aligned outside the laser area will be done to avoid long working time inside the laser area.

%As the probability to purchase a new commercial 40TW laser system already for Phase 0 is growing, the impact of this exercise is also shown in the schedule (see Fig. ~\ref{fig:schedule}. In this case the installation and commissioning can take place during Q3-4 of 2023. Furthermore, the commissioning of diagnostics can take place during Q1 of 2024. 
%\RP{these numbers are just a starter as i am not sure about all the numbers. We need to give each and every details with good confidence!!}

\subsection{Risk management}
The main risks are discussed and their impact is quantified in terms of cost and schedule with respective probabilities and mitigation strategies:

There are two dimensions, the impact and the probability. We separate the impact on the cost and the schedule and use the following terms for impact risks:
\begin{itemize}
    \item Insignificant: Risk is easily mitigated by day to day process. 
    \item Minor: Delays up to 10\% of schedule. Cost increase up to 10\% of budget. 
    \item Moderate: Delays up to 30\% of schedule. Cost increase up to 30\% of budget. 
    \item Major: Delays up to 50\% of schedule. Cost increase up to 50\% of budget. 
    \item Catastrophic: project abandoned
\end{itemize}


For the budget, the denominator used is the budget of that area, i.e. if it is in the phase-0 laser area it is relative to the total phase-0 laser costs. In any case for the cost also the absolute numbers are given, so we can easily renormalize if the total cost changes.

For the schedule, the fraction is taken relative to 24 months, assuming a start in January 2022 and a readiness of January 2024. 

The probability of a risk to be realized is quantified as, rare: ($<3$\%), unlikely (3-10\%), moderate (10-50\%), likely (50-90\%) or certain ($>90\%$). 

Table˜\ref{tab:risks} shows a template for a summary of the risks.
\begin{table}[]
    \centering
    \caption{Risk description, potential impact on cost and schedule, probability to occur and strategy on how to mitigate the risk.}
\begin{tabular}{p{0.2\linewidth}|p{0.1\linewidth}|p{0.13\linewidth}|p{0.13\linewidth}|p{0.3\linewidth}}
         Description & Cost & Schedule & Probability & Strategy\\\hline
         & & & & \\\hline
         Mechanical Jitter Causes Overlap Problems & Medium 30 \% & Moderate (6~Months) & Medium (w/o tests) & Beamline Design and tests prior to installation   \\\hline
         Maintenance downtime & 10\% of laser cost pa & Lost beam weeks & High
& Schedule maintenance,
System monitoring Preemptive maintenance/ new laser rather JETI 40 \\\hline

Radiation degradation of tunnel diagnostics &
Low (replacement)  & Loss of beamtime & High & Choose components with known rad hardness, shield, spares readily available \\\hline

Laser automation not to plan & Moderate 20\%  & Medium Continuous loss of time & Medium & Start design now, Apply  proven automation strategy \\\hline

Low Damage threshold optics - shoot with lower energy & 30 \% & 10 \% & Low & test optics before installation \\\hline


Insufficient Diagnostic precision - lower data precision & Medium 30\%  & Low 10 \% & Low & test optics before installation \\\hline

Synchronisation jitter too high - intensity fluctuations in the data & Low & Medium & Low (based on HIBEF experience) & Active drift stabilisation may be required or changed IP geometry \\
\hline
\hline
\end{tabular}
\label{tab:risks}
\end{table}


\subsection{Responsibilities}
%Discuss which institute takes responsibility for what aspect.
The responsible institutions are Jena, DESY and Tel Aviv. Leadership and responsibility of the overall project is with Jena, and also of the Laser and Diagnostic sub-project. Infrastructure related planning is delegated to DESY and the vacuum chamber design is delegated to Tel Aviv.

\subsection{Laser Safety Considerations}
The LUXE laser system described  is a class 4 laser system capable of generating ionising radiation in focus.  Here we describe the main safety considerations with specific attention given to the set-up at LUXE. The detailed safety requirements are well understood and have been implemented previously at \euxfel and DESY for very similar systems. For example, the multi-100 TW Ti:Sa ReLaX laser system at the HED beamline of \euxfel is directly comparable Ti:Sa in all safety relevant aspects and the implementation of the safety system will mirror those at ReLaX closely.

\subsubsection{Laser operation modes} 
The laser will always be operated at minimum power and intensity required to ensure safety at all times. The following energy/power settings will be available and will be interlocked to appropriate operator modes.

\begin{itemize}
\item Ultra-low Intensity (nanosecond) \\
In this mode the laser uses the self-seeded regenerative amplifier (regen) described in the previous sections (i.e. the seed is blocked by an interlocked shutter). The  pulse duration is determined by the regen roundtrip time (12.5 ns in the case of JETI). This reduces the laser intensity for a given pulse energy E by 
\begin {equation}
 I_{ULI}(E)=I_{fs}(E) \frac{\tau_{Regen}}{\tau_L} <3\times10^{-6}  I_{fs}(E)\,\,.
\end {equation}
For full regen output ($<0.5$ mJ at the IP focus) the peak intensity will be   below $10^{11}$ Wcm$^{-2}$ - far below the level at which ionisation becomes relevant.
\item Low Intensity (nanosecond) \\
The same operating mode allows a maximum energy in excess of 10 mJ with  (exact values depending on Regen roundtrip time of laser) while staying below the ionising threshold for all beam sizes including the IP focus and enables the beam to be safely and easily aligned.
\item Low Intensity (femtosecond)  \\
The laser will be attenuated to intensities below ionisation threshold in the the IP focus. Depending on transport efficiency in the system this corresponds to $\mu$J level pulses.
\end{itemize}

Higher energy modes at full compression will be available with interlocked enclosures to ensure safe working. Intensities  at which ionising radiation can be present will require area interlocks to prevent access.

The interlock system will be zoned to allow operational modes to be set with lasers present only in certain restricted areas.

{\normalfont \bfseries Mode 1}: Laser-only operation\\
An interlocked shutter system will be installed prior to the beamline transporting the laser to the IP to allow the laser to be operated independently from the beamline/IP chamber for set-up purposes.
The laser shutter will be in a beam dump enclosure and be made of high damage threshold material (e.g. Alumina ceramic) to allow the laser to be operated at up to full power with the energy being dumped/diffused in the shutter/beamdump assembly.

This mode will have different interlock settings  on intensity depending on whether the laser beam can be accessed by the operator or if the compressed beam is fully enclosed.\\

{\normalfont \bfseries Mode 2}: Interaction Point (IP) Mode \\
In IP mode the laser will be allowed to propagate to the IP chamber. The availability of the energy modes will depend on the interlock status (IP area without personnel, IP area with vacuum system closed (no access to high intensity), IP area and chamber accessible).



%We need to also ensure that a safe level of laser energy is reached in the IP chamber. All q-switches of the pump lasers of the amplifiers will be interlocked. Meaning that during the alignment in the interaction area, the main amplification can not take place. The front end energy (about $500 \mu$ J ) will be only available. Such level of energy is required to align for example during the set up of optics inside the IP camber. The focused intensity at the IP will be 2.1016 W/cm2 for a tight focus diameter of $3\mu$ m (FWHM). However, the intensity outside the area of 3mm2 will be already below 10w/cm2 due to the fast diverging beam (beam diameter at 2cm from IP= 0.66cm). 

%{\normalfont \bfserieshigh power alignment} \\

The focus of the laser must be characterised both with the IP diagnostic and with the diagnostic system. Meaningful measurement requires the laser to operate under full power conditions.  To ensure that the energy in the pulse does not exceed the one in the alignment case, an interlockable $10^{-6}$ attenuator  will be inserted in the path of the laser beam after the last stage of the amplification and before the compressor. This attenuator consists of high quality ($<\lambda/20$) uncoated mirrors mounted in a so called dog-leg geometry. The insertion of this attenuator will be done using a motorised translation stage. This stage can be interlocked with the laser to ensure that attenuator is at in position when the beam is fully amplified.  A pointing monitor in laser bay with switchable attenuation will ensure that the laser is propagating down an identical path both with and without the attenuator present.\\

{\normalfont \bfseries High power mode} \\

For operation at full power (data acquisition and full power live diagnostic laser only).  The IP area will be searched and fully locked, so that no one can access it while the laser is operating at full power and/or the electron beam is present. In this mode the  full energy laser pulse can be delivered at the IP and, after initial attenuation in the IP chamber, propagate to the diagnostic suite in the laser clean room.  Interactions of the GeV beam with the laser pulse can take place.

\subsubsection{Safety protocols}
%do we need to describe all the details of safety interlocks, emergency switches, entry to the laser room etc?\\
In other labs at DESY \cite{laser28m} and in EuXFEL-HIBEF (which host $> 300$ TW class IV lasers) \cite{hibef} the safety procedures for the alignment and focus check is as discussed above. This is so called``Justierung mode-alignment mode". The main safety interlock is at the attenuator which does not allow high energy in the pulse when the laser is in alignment mode. During the ``Sperrbereich-mode" (shooting mode), the interaction area is fully locked and the attenuator moves out of the beam path allowing full energy in the pulse. Other standard procedures are the announcement of the laser beam being sent to the IP area and when the interaction area is being locked for the high power interaction mode.


\subsection{Budget Summary}
The costs listed in the previous section are given with more granularity.  Table   ~\ref{tab:New_laser_system_cost} breaks down the individual laser components and upgrade cost from a phase-0 to phase-1 system. Here phase-0 is conceived to have common components at phase-1 specification, with the upgrade consisting of additional amplification and pump lasers. The costs arising in the other areas of this TDR are shown in tables  ~\ref{tab:laser_area_diag_cost}  for the laser area diagnostics,  ~\ref{tab:laser_beamline_cost} for the transport beamline and ~\ref{tab:TA_diagnsotics_cost} for the target area diagnostics. The costing for the hardware part is presented in Infrastructure note \cite{LUXETDR-Infra}. Finally we show for comparison the phase-0 option with the JETI 40 laser in table ~\ref{tab:Jeti40_laser_system_cost}. The investment savings over the project lifetime are clearly limited and very small compared to the total cost of LUXE. On the downside there is the high risk of additional unscheduled maintenance downtime with the possibility that some of the pump lasers might need full replacement during the running period of LUXE. 

\begin{table}[]
   \centering
   \caption{Detailed cost estimates for the new laser system only.}
    %\begin{tabular}{l|r|l}
    \begin{tabular}{|p{4.5cm}|p{1.5cm}|p{4.5cm}|}
       \hline
         & Cost (kEur) & Comment\\\hline
        Laser system phase-0  & 1650 & quote from manufacturer\\ \hline
       Compressor and chamber & 250 & {laser manufacturer quote}\\\hline
         
        Timing system (with EuXFEL master clock)  & 80 & estimates based on input\\\hline
         
         Automation cost & 250 & {estimates based on  quotes and experience}\\\hline
        Oscillator & 160 & {based on  quotes}\\\hline
        Attenuation, shot and  energy control & 195 & {laser manufacturer quote}\\\hline
        Adaptive Optic & 140 & {based on  quotes}\\\hline
       
       \textbf{Phase-0} & \textbf{2725} & \\\hline \hline
       Upgrade to 350 TW & 1700 & {laser manufacturer quote}\\\hline
        
       \textbf{Phase-1}  & \textbf{4425} & \\\hline
        350 TW Laser system for Phase 1  & 3050 & quote from Thales\\\hline
        \textbf{Total sum for phase 0 and 1} & \textbf{3825} & 
        \\\hline
    \end{tabular}
    \label{tab:New_laser_system_cost}
\end{table}


\begin{table}[]
   \centering
    \caption{Laser area diagnostics costing.}
    %\begin{tabular}{l|r|l}
    \begin{tabular}{|p{4.5cm}|p{1.5cm}|p{4.5cm}|}
       \hline
       Laser area diagnostics  & Cost (kEur) & Comment\\\hline
        Wizzler & 35 & estimates based on quote \\\hline
        Sequoia & 30 & quote \\\hline
        Insight  & 60 & estimates based on quote\\\hline
        Spot CCD microscope & 7 & quote \\\hline
        Vacuum chamber for the diagnostics & 45 & estimates based on quote\\\hline
         Pump & 13 & {estimates based on  quote}\\\hline
         Optical tables & 15 & quote \\\hline
         Adaptive optics & 25 & estimates based on quote\\\hline
         Small optics and mounts & 25 & {estimates based on  quote}\\\hline
Nonlinear 2D detectors & 25 & estimates based on quote\\\hline
        Off axis parabola & 30 & {estimates based on  quote}\\\hline
        \textbf{Total sum} & \textbf{310} & 
         \\\hline
    \end{tabular}
   \label{tab:laser_area_diag_cost}
\end{table}


\begin{table}[]
    \centering
    \caption{Laser beamline costs. Tubing, pumps and gate valves are costed in the Infrastructure note TDR.}
    %\begin{tabular}{l|r|l}
    \begin{tabular}{|p{4.5cm}|p{1.5cm}|p{4.5cm}|}
       \hline
       Laser Beamline  & Cost (kEur) & Comment\\\hline
         Mirror mounts & 110 & estimates based on quote \\\hline
         Optics & 200 & quote \\\hline
         Crosses  & 40 & estimates based on input\\\hline
        Mounting breadboards & 50 & quote \\\hline
        \textbf{Total sum} & \textbf{400} & 
         \\\hline
    \end{tabular}
    \label{tab:laser_beamline_cost}
\end{table}



\begin{table}[]
  \centering
   \caption{Detailed cost estimates for the vacuum chambers.}
   \begin{tabular}{|p{4.5cm}|p{1.5cm}|p{4.5cm}|}
       \hline
       Vacuum chambers  & Cost (kEur) & Comment\\\hline
        IP chamber & 40 & estimates based on quote \\\hline
        ICS and gamma chamber & 15 & quote \\\hline
        
       \textbf{Total sum} & \textbf{55} & 
        \\\hline
   \end{tabular}
   \label{tab:vacuum_chamber_cost}
\end{table}


\begin{table}[]
    \centering
    \caption{Tunnel diagnostic costs.}
    %\begin{tabular}{l|r|l}
    \begin{tabular}{|p{4.5cm}|p{1.5cm}|p{4.5cm}|}
        \hline
        Target area diagnostics  & Cost (kEur) & Comment\\\hline
         Microscope & 8 & estimates based on quote \\\hline
         EO Timing tool & 4 & previous quotes \\\hline
         Beam dump  & 3 & estimates based on input\\\hline
         axis parabolas & 30 & quote \\\hline
        Linear stages & 50 & estimates based on quote\\\hline
        Mounts for parabolas & 20 & {estimates based on  experience}\\\hline
       \textbf{Total sum} & \textbf{115} & 
        \\\hline
    \end{tabular}
    \label{tab:TA_diagnsotics_cost}
\end{table}


\begin{table}[]
    \centering
    \caption{Cost estimates for the JETI 40 option to phase-0 and phase-1.}
   % \begin{tabular}{l|r|l}
   \begin{tabular}{|p{4.5cm}|p{1.5cm}|p{4.5cm}|}
        \hline
        Jeti 40 Laser system Phase 0  & Cost (kEur) & Comment\\\hline
         Optical Tables & 30 & estimates based on quote \\\hline
         Oscillator with synchro lock & 160 & quote \\\hline
         Timing system (with EuXFEL master clock)  & 80 & estimates based on input\\\hline
         Jeti 40 laser & 0 & in-kind contribution \\\hline
         Transport of Jeti 40 to XS1 & 5 & estimates based on experience\\\hline
        New pump laser & 250 & {estimates based on  quotes}\\\hline
        Automation cost & 250 & {estimates based on  quotes and experience}\\\hline
         spare pump laser for front end & 40 & estimates based on  quotes\\\hline
         Additional Staff costs & 160 & estimate\\\hline
       & &  \\\hline
       \textbf{Total phase-0} & \textbf{975} & \\\hline
       Full size adaptive optics & 140 & based on quote\\\hline
        Full size compressor & 250 & laser manufacturer quote\\\hline
        Attenuation, shot and energy control  & 195 & laser manufacturer quote \\\hline
        Energy upgrade & 1700 & laser manufacturer quote \\\hline
        Additional maintenance costs & 300 & estimates\\\hline
        & & \\\hline
        \textbf{Total phase-1} & \textbf{3560} & \\\hline
        
        \textbf{cost to upgrade to 350 TW} & \textbf{3050?} & \textbf{estimates based on  quotes}\\\hline
        350 TW Laser system for Phase 1  & 3050 & quote from Thales\\\hline
        \textbf{Total sum for phase 0 and 1} & \textbf{3825} & 
        \\\hline
   \end{tabular}
    \label{tab:Jeti40_laser_system_cost}
\end{table}


==> chapters4/organisation.tex <==
% Includes organisation of work at institutions, discussion of main technical milestones (e.g. internal or external reviews, test beam campaigns etc.) and interfaces to common services.
% Also discusses which institution contributes how.
The related 
%costs, 
manpower and timelines are discussed in detail.

For the installation timeline of the tracker alone, we consider the following three baseline scenarios:
\begin{enumerate}
    \item during the 2024 shutdown,
    \item during 2025 summer shutdown (2 weeks),
    \item during 2025 winter shutdown (4-6 weeks).
\end{enumerate}
The priority will be to finish the installation in scenario 1.
If it is missed due to technical or financial reasons, then the other scenarios may come into play.

In that respect, the ``bare-bones'' tracker scenario is particularly important to outline, as this is the most likely case fit for scenario This case is therefore detailed independently.


\begin{comment}
The manpower costs are roughly:
\begin{itemize}
    \item PhD student: 24~k\euro/year,
    \item PD: 31-37~k\euro/year,
    \item PCF technician at 15\% FTE: $\sim 15$~k\euro/year,
    \item PCF mechanical eng. at 15\% FTE: $\sim 15$~k\euro/year,
    \item PCF electronics eng. at 10\% FTE: $\sim 20$~k\euro/year,
\end{itemize}
where for the PCF technical personnel 1 FTE is calculated assuming 165 work hours per month on average.

\subsubsection{Travel}
\label{sec:travel}
We assume a one-week trip of one person from Israel to Hamburg is roughly 1~k\euro.
Most of the travel is expected to happen in period A in terms of frequency and the number of people travelling, with a notable peak during installation and commissioning.
In period B, the frequency will be lower and the number of people travelling will also reduce, mostly for operation and maintenance.
The foreseen travel expenses are therefore:
\begin{itemize}
    \item Pre-installation: roughly $\sim 10$~k\euro\ for $\simeq 10$ one-week trips inclusively,
    \item Installation and commissioning: roughly $\sim 20$~k\euro\ for a four-weeks trip of five people,
    % \item Post-installation: roughly $\sim 20$~k\euro/year for a period of four years for $\simeq 5$ one-week trips inclusively per year. \NTH{maybe this is too little - TBC with Beate.}
    \item Post-installation: roughly $\sim 10$~k\euro/year for a period of four years for $\simeq 5$ one-week trips inclusively per year.
\end{itemize}
Altogether, travel expenses for the full duration of the experiment are expected at the level of 40~k\euro.

%\clearpage
%\newpage
\subsubsection{Budget summary}
\label{sec:budgetsummary}
\begin{table}[!ht]
\begin{center}
{\footnotesize
\begin{tabular}{ lclcl }
  \toprule\hline
  Item 							& Unit price 		& Quantity 		& Total price & Uncertainty	\\
  \,   							& [k\euro]     	& \,       		& [k\euro]	 & \,	\\
  \toprule
  Staves							& 13					& 8+8+4			& 260 		& 10\%	\\
  Readout units				& 4					& 8+8+4			& 80 			& 20\% (quote yet unavial.)	\\
  Power boards (w/2 units)	& 2					& 4+4+3			& 22 		& 20\% (quote yet unavial.)		\\
  FELIXs and DAQ PCs			& 25 					& 3 				& 75 		& $<5$\%		\\
  \hline
  Power supply	system		& 57 					& NA 				& 57  & 30\%\\
  Cabling						& 70 					& NA 				& 70 		& 30\%		\\
  Mechanics 					& 50 					& NA 				& 50 		& 30\% (rough quote)		\\
  Cooling 						& 40 					& NA 				& 40 			& 50\% (pending design)	\\
  \hline
  {\bf Total equipment}				&  					&  				& 654 		& 19\%	\\
  \hline
  PD (period A)				& 						&					& 99		& $<5$\%		\\
  PhD (period A)				& 						&					& 72			& $<5$\%	\\
%   PD (period B)				& 						&					& 99			& $<5$\%	\\
%   PhD (period B)				& 						&					& 72		& $<5$\%		\\
  Elx. eng. (period A)		& 						&					& 20			& 20\%	\\
  Mec. eng. (period A)		& 						&					& 15			& 10\%	\\
  Technicians (period A)		& 						&					& 30			& 20\%	\\
  Travel							& 						&					& 40		& 30\%		\\
  \hline
  {\bf Total non-equipment}		& 						&					& 276		& 12\%		\\
  \hline
  {\bf Grand total}					&  					&  				& 930 		& 16\%	\\
\hline\bottomrule
\end{tabular}
}
\end{center}
\caption{Equipment, personnel and travel cost breakdown. For the person-power part, period A represents the phase of design, installation and commissioning while period B represents the phase of steady-state operation, maintenance and analysis. The estimated cost for the RUs and PBs is based on discussion with ALICE colleagues. The uncertainties of the total amounts assume the maximum deviations.}
\label{tab:cost}
\end{table}

\begin{table}[!ht]
\begin{center}
{\footnotesize
\begin{tabular}{ lclcl }
  \toprule\hline
  Item 							& Unit price 		& Quantity 		& Total price & Uncertainty	\\
  \,   							& [k\euro]     	& \,       		& [k\euro]	 & \,	\\
  \toprule
  Staves							& 13					& 4+1			& 65 		& 10\%	\\
  Readout units				& 4					& 4+1			& 20 			& 20\% (quote yet unavial.)	\\
  Power boards (w/2 units)	& 2					& 3+1			& 8 		& 20\% (quote yet unavial.)		\\
  FELIXs and DAQ PCs			& 25 					& 1 				& 25 		& $<5$\%		\\
  \hline
  Power supply	system		& 25 					& NA 				& 25  & 30\%\\
  Cabling						& 20 					& NA 				& 20 		& 30\%		\\
  Mechanics 					& 20 					& NA 				& 20 		& 30\% (rough quote)		\\
  Cooling 						& 20 					& NA 				& 20 			& 50\% (pending design)	\\
  \hline
  {\bf Total equipment}				&  					&  				& 203 		& 19\%	\\
\hline\bottomrule
\end{tabular}
}
\end{center}
\caption{Equipment cost breakdown for the ``bare-bones'' tracker. Some elements, like the PUs and the RUs, may be replaced by other (simpler) modules. In addition, the same considerations (uncertainties, manpower and travel) from Table~\ref{tab:cost} apply also here.}
\label{tab:cost_bare-bones}
\end{table}

\end{comment}

%\subsection{Human and financial resources}
%\subsection{ Human resources}

%\label{sec:resources}

\begin{comment}
The project cost is summarised in Table~\ref{tab:cost}.
This Table includes the costing of the equipment components and also the person power needed to construct, install, commission and operate the tracker.

The components which are common to several subsystems (e.g. anti-vibration tables, base platforms, etc.) are excluded as these are parts of the infrastructure.
The items in Table~\ref{tab:cost} which do not specify the quantities (those marked with ``NA'') are multi-component systems as discussed below.



\subsubsection{Equipment}
\label{sec:equipment}
The staves are manufactured at CERN by colleagues from the ALICE collaboration and are assumed to be of the ``gold category'', which means less than 50 dead pixels per sensor (i.e. 50 dead out of $\sim$500k).

The RUs and PUs were designed by ALICE colleagues, but the manufacturing was done by the industry.
The same procedure is expected to be carried out in LUXE, preferably with the same companies that were involved in the ALICE production.

The power supply system is composed completely of CAEN modules which are the industry standard in HEP:
\begin{itemize}
	\item Mainframe (SY4527) at 12~k\euro,
	\item Booster (A4533) at 2~k\euro,
	\item 2(+1) Reverse bias low voltage (LV) supply cards (A2518) with 8 channels each at 2.5~k\euro/card,
	\item 4(+1) LV power supply card (A2518) with 8 channels each at 2.5~k\euro/card,
	\item 1(+1) Control PC at 3~k\euro/PC.
\end{itemize}
There is no distinction between analog and digital upstream of the PU, so effectively one channel per PU is needed.
The analog, digital and reverse bias output of the PU is bundled before it goes on to the staves.
In the scenario of one PU+RU per stave, one needs a one A2518 channel to supply the 3.3~V to one PU, one channel to supply the -5~V reverse bias to one PU and one channel to supply the +8~V to one RU.
Concerning the control of PUs from RUs, one RU has two I2C ports, each one can control one PU.
The foreseen setup is to have one I2C connector between each RU and the corresponding PU.

Note that the quantities comprise the bare-minimum system, without any spares besides the A2518 cards.
To allow redundancy and backup, two independent power systems, each controlling one detector arm individually, are necessary.
In this case, while the number of LV cards will not change, the mainframe and the control PC and the booster will have to be duplicated.
%, adding 15~k\euro\ for the total.\\
%% bare-bones:
%% 12[SY4527]
%% +2[A4533]
%% +2*2.5[A2518]
%% +2*2.5[A2518]
%% +1*3[PC]
%% = 25-27
%% minimum:
%% 12[SY4527]
%% +2[A4533]
%% +(2+1)*2.5[A2518]
%% +(4+1)*2.5[A2518]
%% +(1+1)*3[PC]
%% = 40
%% with redundancy:
%% 12[SY4527]*2
%% +2*2
%% +(2+1)*2.5
%% +(4+1)*2.5
%% +(3+1)*3
%% = 57

The driving component for the cabling is the TwinAx cost, at about 0.85~k\euro\ per 5~m of cable including the connectors.
Two such cables are needed per stave and hence the cost is around 41~k\euro\ for these cables alone, assuming the length of 5~m and assuming 8 spares per arm.
%(i.e. 4 spares beyond the staves spares).
% If instead a length of e.g. 8~m would be needed due to distance constraints, the cost of the TwinAx cables alone would be closer to 66~k\euro.
The 5~m length assumption is reasonable if the readout and power units can be placed at a distance of $<5$~m near the detector, while also being shielded.

Under cabling we also bundle the GBT fibre optics links, LV cables (etc.), which are not priced yet. Hence, the cost is specified higher, at 70~k\euro.

The mechanics component include the tray (only) with its kinematic mounts and the L-shape fixations.
It includes in principle also the costs of the alignment system for the staves themselves and hence the relatively high price tag of 50~k\euro.

For the cooling system, two simple water chillers are enough, but there is a need to design efficient manifolds to distribute the flow to the staves via copper pipes.
The leak-less requirement may impose some additional costs which are not priced yet.
In addition, an array of fans will be needed to cool down the readout units and power boards.
The price tag for this system is at 40~k\euro.

A summary of the costings for the equipment discussed above is given in Table~\ref{tab:cost}.

The ``bare-bones'' tracker would be made of four staves, so one quarter of the full tracker.
The rest of the equipment and hence also the costing cannot be simply scaled down by four.
The detailed costing for the ``bare-bones'' scenario is given in Table~\ref{tab:cost_bare-bones}.
Nevertheless, the costing for this scenario can be further minimised with different, simplified readout and power modules replacing the RUs and the PUs.

\end{comment}

\subsection{Manpower}
\label{sec:manpower}
The manpower requirements follow a two-step logic: (i) design (including simulation), installation and commissioning in ``period A'', and (ii) operation, maintenance and analysis during ``period B''.

In period A, generally one postdoctoral research fellow (PD), one PhD student, one technician, one mechanics engineer/designer and one electronics engineer are required (besides the WIS PI and staff-scientist).
The technicians and engineers of this team are based on WIS personnel of the faculty of physics ``core facilities'' (PCF) department.
This technical team is highly experienced and can be hired on a day-by-day basis.
This arrangement allows maximum flexibility with respect to the schedule compared to the alternative, which essentially involves hiring of equivalent manpower.

Before installation at the experiment, this team is not needed at 100\% FTE, except for the PD.
The design and simulation, including the mechanics is already underway with one PD at 100\% FTE and one mechanics engineer at $\sim 5-10\%$ FTE.

As initial modules (one stave, FELIX, ...) will arrive at WIS, an involvement of an electronics engineer at $\sim 5-10\%$ FTE and a technician at $\sim 5-10\%$ FTE is foreseen (PCF personnel).
This equipment is expected before the end of 2021 independent of LUXE's timeline or budgeting and based on private WIS budget.
This will allow to gain experience with the end-point detector elements and to progress on many fronts (mechanics, cooling, FELIX, readout, software, etc.) even before the bulk budget will arrive.

Once the quantities of detector modules purchased for LUXE will start to arrive at WIS, the work will gain speed with increased involvement of the PCF personnel.
A PhD student is required to be recruited early enough before that point in order to participate effectively in the construction.
Particularly, the reception, testing and assembly of the tracker modules will be done at this step.
The assembled equipment will be shipped to DESY, tested on-surface and installed in the experimental hall by the personnel described above.

As discussed in Section~\ref{sec:install}, the installation itself in period A, a team of at least 5-6 FTEs will be needed.
The team will consist of one WIS PI, one WIS scientist (or a postdoc), one postdoc/student, 1-2 WIS technicians and potentially one WIS electronics expert.
The installation will take at least 2-4 straight weeks, with $\sim$one week on surface and $\sim 2-3$ weeks in the experiment hall.
During that time the team will be fully dedicated to the installation.
With this team in mind, the installation can fit the timeframe of any of the three scenarios outlined at the beginning of this Section.
It would be particularly comfortable in the first scenario, but it can also be fitted in the second or third (shorter) scenarios, given the extra time that will be used to make as much progress as possible at WIS and on-surface at DESY.


In period B, at least one PD and one PhD student are required.
This is expected over a period of three years at least.
It is assumed that minimum technical intervention will be needed at this step.
Hence, the technical team is not needed for extended periods, while in special cases where short technical interventions are needed, these could be covered based on the same WIS technical personnel.
The tasks to be covered in period B by student(s) and postdoc(s) will include software development, data-quality monitoring, on-call expert shifts, etc.
%The PD and PhD components in period B are not included in Table~\ref{tab:cost}.



\subsection{Risk management}
\label{sec:risks}
The main risks are discussed and their impact is quantified in terms of cost and schedule with respective probabilities and  mitigation strategies:
\begin{itemize}
    \item Insignificant: Risk is mitigated by day to day process,
    \item Minor: delays up to 10\% of the schedule and the cost increases by up to 10\% of the budget,
    \item Moderate: delays up to 30\% of the schedule and the cost increases by up to 30\% of the budget,
    \item Major: delays up to 50\% of the schedule and the cost increases by up to 50\% of the budget,
    \item Catastrophic: project abandoned,
\end{itemize}
where the fractions for the budget are taken relative to the overall tracker-project budget alone.
The fractions for the schedule are taken relative to 24 months, assuming a start in January 2022 and readiness on January 2024.
The probability of a risk to be realized is quantified as: rare ($<3$\%), unlikely (3-10\%), moderate (10-50\%), likely (50-90\%) or certain ($>90\%$).

This analysis is done for the \underline{full tracker} scenario.
Similar tough reduced conclusions may be also applied to the ``bare-bones'' tracker scenario.

Table~\ref{tab:risks} shows a summary of the risks analysis.
\begin{table}[!h]
\centering
\begin{tabular}{p{0.22\linewidth}|p{0.05\linewidth}|p{0.1\linewidth}|p{0.12\linewidth}|p{0.37\linewidth}}
Description & Cost & Schedule & Prob. & Mitigation strategy\\
\toprule
%%%%%%%%%%%%%%%%%%%%%%%%%
Problems in the detector design (mostly sensors, readout and DAQ) & 30\% & 30\% & Moderate & Testing of initial modules will start in 2022 with a milestone set for full chain test around Aug 2022 with three months of contingency before modules must be ordered.\\\hline
%%%%%%%%%%%%%%%%%%%%%%%%%
Budget not identified by Oct 2022 & 50\% & 50\% & Likely &Push installation to winter 2025.\\\hline
%%%%%%%%%%%%%%%%%%%%%%%%%
Stave production is delayed & 10\% & 10\% & Unlikely & Contingency of 2 months is taken on top of the most conservative estimate from ALICE. Can also compensate later by descoping testing and assembly steps at WIS.\\\hline
%%%%%%%%%%%%%%%%%%%%%%%%%
CAEN, RU and/or PU production is delayed & 20\% & 10\% & Unlikely & Contingency of 2 months is taken. Can also compensate later by descoping testing and assembly steps at WIS.\\\hline
%%%%%%%%%%%%%%%%%%%%%%%%%
WIS integration is delayed & 10\% & 10\% & Moderate & Contingency is allocated. Reception tests can be descoped to the bare minimum while prioritising connectivity tests and assembly procedures only.\\\hline
%%%%%%%%%%%%%%%%%%%%%%%%%
Leak-less cooling concept underestimated & 20\% & 10\% & Moderate & Contingency is allocated. Start design early in 2022 with WIS experts and in consultation with ALICE engineers. If too expensive and/or complicated work with normal flow (no under-pressure) and take the risk of small (vertical) leaks.\\\hline
%%%%%%%%%%%%%%%%%%%%%%%%%
Radiation in the position of the power system and/or readout backend is too high (from simulation) & 20\% & 30\% & Moderate & Scrutinise design based on detailed dose simulation with proper shielding. If necessary, upgrade the power supply system to the hostile-compatible version (with higher cost and complexity) and increase the shielding.\\
\bottomrule
\end{tabular}
\caption{Risk description, potential impact on cost and schedule, probability to occur and strategy on how to mitigate the risk. The different risks are tied to the steps outlined in Fig.~\ref{fig:schedule}.}
\label{tab:risks}
\end{table}





\subsection{Responsibilities}
\label{sec:responsibilities}
When writing up this document, the responsible institution is only WIS.
The PI of the WIS group devotes $>50\%$ of the time to the LUXE project and particularly to the development of the tracker. 
The facilities and equipment at the WIS lab are also adapted to this purpose.
On top of that, the availability of the faculty's PCF department technical personnel on demand is invaluable.
The mechanical design of different elements in LUXE (not only the tracker) is already benefiting from the expertise of the PCF instrument design team.
Moreover, the expertise of the PCF electronics and DAQ team will be particularly important for the FELIX adaptations (FELIX was developed by WIS experts and is still being worked on for ATLAS phase-1 and phase-2 upgrade campaigns).



==> chapters5/organisation.tex <==


\subsection{Human and financial resources}
%Estimate of human and financial resources required. For the financial resources the sources (e.g. company quotes, experience from previous work...) and uncertainties should be provided. For the human resources it should be clarified what type of people are needed.

ECAL-E and ECAL-P will be built in a joint effort of the AGH-University of Technology (AGH-UST) Cracow, Instituto de Fisica Corpuscular (IFIC),
the Kyushu University (KU), the Laboratoire de Physique des 2 Infinis Irène Joliot-Curie, (IJC) Paris, the 
Laboratoire Leprince-Ringuet (LLR) Paris, the
Institute of Space Science (ISS) Bucharest, the Tel Aviv University (TAU) and the University of Warsaw (UW). These institutes will provide the human and financial resources needed for the design, production, test, commissioning and operation of ECAL-P.
The group of AGH-UST comprises 5 experienced researchers, specialised in ASIC design, 1 technician and several students.
At IFIC, one experienced researcher and one Ph.D. student will perform the gluing.
From the Kyushu University one researcher specialised on sensors will join. The 
Laboratoire -Ringuet Paris will contribute with mechanics, sensor assembly and electronics of ECAL-E with 2 researchers.
From the ISS group, 3 physicists experienced in software and data handling are included. 
The TAU group comprises 3 experienced physicists, 1 part-time technician (full time technician will be hired in the near future), one postdoc, and several graduate students.  The University of Warsaw participates with 2 experienced researchers, one student (postdoc candidate) and engineering support to design and build the mechanical frame of ECAL-P. 

The cost estimates for the production of ECAL-E and ECAL-P are given in Tables~\ref{tab:cost_ECAL-E} and ~\ref{tab:cost_ECAL-P}.
\begin{table}[h]
    \centering
    \caption{Cost estimates for the various components of ECAL-E. The comment in parentheses gives the source of the price. The meaning of the quality factor is given in the appendix.}
        \begin{tabular}{|l|r|l|c|l|}
         \hline
        Component  & Cost         & responsible lab               & Quality     & Status\\
                   &  (kEur)      & (origin of estimates)        & factor      &        \\
         \hline
         Mechanics &    10        &  IJC (previous projects)  &   1         & design\\
         Sensors   &    120       &  KU, LLR, IFIC, IJC       &   1         & Prototyping\\
                   &              &  (offer by the vendor)        &             &            \\
         FE ASICs  &    165      &    IJC, LLR                    &       2    & design ready  \\
                   &              &    (recent submissions)        &            &        \\
         PCBs      &    30        &    LLR, IJC                    &    1       &   \\
                   &              &    (previous production)       &            & \\
         DAQ       &    10        &   IJC                          &      1     & \\
         Power supplies &  20     &   IJC (current offers)         &    1  & \\
         Tooling and gluing   & 25 &  IFIC , IJC                   &     1       & \\
         Tungsten   &    30       &   LLR (offer by the vendor)   &     1       & \\ 
         Auxiliary  &    20       & IJC, LLR (experience from              &     1        & \\
         components &             & previous projects)            &              & \\ 
         \hline
         Total sum  &  430  &   & &
         \\  \hline
    \end{tabular}
    \label{tab:cost_ECAL-E}
\end{table}
\begin{table}[h]
    \centering
    \caption{Cost estimates for the various components of ECAL-P. The comment in parentheses gives the source of the price. The meaning of the quality factor is given in the appendix.}
        \begin{tabular}{|l|r|l|c|l|}
         \hline
        Component  & Cost         & responsible lab               & Quality     & Status\\
                   &  (kEur)      & (origin of estimates)        & factor      &        \\
         \hline
         Mechanics &    40        &  UW (previous projects)        &   1         & design\\
         Sensors   &   100        &  TAU                           &   1         & Prototyping\\
                   &              &  (offer by the vendor)         &             &            \\
         FE ASICs  &    165       &   AGH-UST                      &       2    & Redesign  \\
                   &              &    (recent submissions)        &            &        \\
         PCBs      &    22        &    AGH-UST, TAU                &    1       &   \\
                   &              &    (previous production)       &            & \\
         DAQ       &    27        &   TAU (FCAL experience)        &      1     & \\
         Power supplies &  20     &   AGH-UST, TAU (current offers)&    1       & \\
         Tooling and gluing & 30  &   IFIC, TAU                    &     1       & \\
         Tungsten   &    30       &   TAU (offer by the vendor)    &     1       & \\ 
         Auxiliary  &  30         &   AGH-UST, TAU (experience from              &     1        & \\
         components &             & previous projects)            &              & \\ 
         \hline
         Total sum  &  464  &   & &
         \\  \hline
    \end{tabular}
    \label{tab:cost_ECAL-P}
\end{table}
 The major cost drivers are the sensors and the FE ASICs. TAU will cover the sensor costs for ECAL-P; received support from the PAZY Foundation (Israel Atomic Energy Commission) and will apply for support from the Israel Science Foundation. For the sensor costs of ECAL-E, the labs in the table above will make a joint application to their funding agencies.  
 Compared to the CDR, the estimated price of FE ASICs has increased by about 25\% mainly due to expected increased production costs. 
 To cover the costs of the FE ASICs of ECAL-P the AGH-UST group has successfully applied for a grant from the Polish National Science Centre.
 
 To cover the costs for the mechanics, the UW will apply for support from the national funding agency. Costs for tungsten plates of precise thickness and flatness will be shared between LLR and TAU. The DAQ will be partly funded from the AGH-UST application. IJC and LLR will apply for additional funding. PCBs, power supplies, tooling and auxiliary components will be shared between AGH-UST,  TAU and IJC. IFIC will apply for funding to cover the costs for contact gluing, including the necessary tools. 
 
 In addition, TAU together with the DESY and Freiburg University groups and other participants from Israel and Germany recently applied to the German-Israeli Project Cooperation (DIP) in the 2022 call. If successful, some funds will be dedicated to the shortfalls in the ECAL-P funding, if necessary.
 
 The ECAL-E collaborators in LUXE are also involved in the CALICE SiW calorimeter prototype effort. At the moment it can be assumed that the funding in the next two to three years will be continued at the current level in the frame of the base funding for CALICE and Linear Collider activities. The person-power situation is such that there are at the moment around ten senior researchers and engineers, one postdoc, four PhD students and one master student, and the expectation is that the same level of manpower will remain available for the next two or three years. A positive development towards a Higgs factory as well as the creation of the French-German lab DMLAB, may lead to an improvement of the situation.  
 Currently available is the CALICE prototype ECAL, covering a fiducial area of $18\times 18 \units {cm^2}$, fully equipped with sensors, FE electronics and DAQ. The installation of this ECAL in LUXE would need only a small amount of additional funding. For a full coverage of ECAL-E, a second and a third stack of the same size has to be added, for which additional 430 kEuro are needed.

\subsection{Schedule and milestones}
%Describe here the schedule and the milestones. Normally we will try to be ready for installation by January 2024. There will be risks to that which we can treat as risks and the mitigation is to install later. 

The schedules for the construction of ECAL-E and ECAL-P are shown in Fig.~\ref{fig:ECAL_E_timeline}
and Fig.~\ref{fig:ECAL_P_timeline}.



\begin{figure}[htbp]
 \begin{center}
% \hspace*{-1.5cm}
  \includegraphics[width=\textwidth]{ECAL_pictures/ECAL_E_Sept_2022.png}
 % \vspace*{-10.5cm}
    \caption{The time schedule for the construction, test and commissioning of 
    the ECAL-E.} 
    \label{fig:ECAL_E_timeline}
    \end{center}
\end{figure}
\begin{figure}[htbp]
 \begin{center}
 \hspace*{-1.5cm}
  \includegraphics[width=\textwidth]{ECAL_pictures/ECAL_P_Aug_2022.pdf}
  \vspace*{-10.5cm}
    \caption{The time schedule for the construction, test and commissioning of the ECAL-P.} 
    \label{fig:ECAL_P_timeline}
    \end{center}
\end{figure}

%
% The major milestones ahead are the following:
%\begin{enumerate}
%    \item{Tungsten plate quality check - July 2022.}
%    \item  {Sensor performance measurements in test-beam in November 2021 and September 2022, followed by technology choice in February 2023.}
%    \item { Completion of the ASIC production in June 2023.}
%   \item { Completion of the sensor production in October 2023.}
%    \item { Completion of the sensor plane instrumentation in March 2024.}
%    \item { Completion of ECAL-P assembly in April 2024.}
%   \item { Beam-tests of fully assembled ECAL-P at DESY in May 2024.}
%    \item { Readiness for commissioning by July 2024.}
%\end{enumerate}


\subsection{Risk management}

Two major elements may impact the time-line and the costs of ECAL-P construction. One pertains to the sensors, the other to the readout delivery. 

 The impact on the costs and the timeline of the ECAL-P is negligible as the sensors prices are based on current offers by Hamamatsu. The funding is not yet fully guaranteed for TAU. The labs of ECAL-E are still in the stage of the preparation of applications for funding for the sensors of the second and third tower. A better assessment will be known by December 2022. The expectation is that if the LUXE project goes ahead, shortfalls in funding if any, will be covered potentially by request of extra support from TAU research funds if not from DIP. 

 For the ASIC production, time delays of the order of 6 months may be expected. Another factor is an increase in pricing which may be of the order of 25\% (included in the price estimate). As a mitigating action, for ECAL-P the existing FLAME boards will be used for testing purposes. According to the present schedule, that would give an extra 9 months for completing the production and testing of the FLAXE readout boards. For the ASICs of the second and third tower of ECAL-E funding applications will be prepared.
 
 Since March 2022, the ECAL-P team developed a strategy to mitigate the effects of the present political crisis, since deliveries from Russian collaborators are unlikely. New partner (UW, IFIC) took over the responsibility for the mechanics
 and sensor plane assembly. In IFIC a funding application is pending, and UW applies for funding.  
ECAL-E can in case of major delays in ASIC production only partially assembled.
In the worst case scenario, where the lack of funding would prevent the delivery of ECAL-P on time for the \phaseone data taking, the ECAL-E with at least one tower will be used on the positron side, leaving the electron side uninstrumented for the \glaser runs. .

An attempt to summarise the risks is presented in Table~\ref{tab:risks}.


%Table~\ref{tab:risks} shows a template for a summary of the risks.
\begin{table}[h]
    \centering
    \caption{Risk description, potential impact on cost and schedule, probability to occur and strategy on how to mitigate the risk.}
\begin{tabular}{|p{0.2\linewidth}|p{0.1\linewidth}|p{0.1\linewidth}|p{0.1\linewidth}|p{0.3\linewidth}|}
        \hline
         Description & Cost & Schedule & Prob. & Strategy\\\hline
 FEB chip production      & $\pm 10\%$ & 25\% to 35\% & 30\% & Adapt existing FLAME readout\\
         \hline
         \end{tabular}
         \label{tab:risks}
\end{table}


\subsection{Responsibilities}
Each institute or university will be responsible for a component of ECAL-E and ECAL-P, as shown in Table  
~\ref{tab:responsibilities}.
\begin{table}[h]
    \centering
    \caption{The participating institutes and their main responsibilities in the ECAL-E and ECAL-P construction.}
    \begin{tabular}{|l|l|}
    \hline
        Institute/University  & contribution to ECAL-E \\ \hline
         IFIC    &  contacts of sensors pads with readout traces using conductive glue, sensors  \\
         IJC    &  sensors, readout, DAQ, PCB \\
         KU     &  sensors, contact to Hamamatsu  \\      
         LLR    &  sensors, PCB, assembly, tools, precise tungsten plates  \\
       \hline
       \hline
        Institute/University  & contribution to ECAL-P \\ \hline
         AGH-UST    &  FE-ASICs development and production, DAQ \\
         IFIC    &  contacts of sensors pads with readout traces using conductive glue, sensors  \\
         ISS    &  slow control, software, computing infrastructure \\
         TAU    &  sensors, assembly of detector planes, DAQ \\
         UW     &  design and prototyping of the mechanical frame\\
       \hline
    \end{tabular}
    \label{tab:responsibilities}
\end{table}
A prototype of ECAL-E (CALICE Prototype) has been operated in test-beams at DESY and CERN. The Data analysis is ongoing, and results on the performance are expected within a few months. With relatively small modifications this prototype will be the first tower of ECAL-E. The additional towers will need
further system tests.
To study the performance of sensors and ECAL-P towers, and finally a full system test and calibration, measurements will be done in the test-beam. These campaigns will be organised and funded as a joint effort.

The installation and commissioning of ECAL-E and ECAL-P will again be done in a joint effort, as described in the resource loaded schedule for ECAL-P as example, in appendix A. 




==> chapters6/allnotes.tex <==
%\section{All notes}
%This is the list of all notes and the lead editors:
%\begin{itemize}
%    \item Technical infrastructure and beam instrumentation at LUXE: Louis Helary and Stewart Boogert 
%    \item Laser, interaction chambers and timing system: Matt Zepf et al.
%    \item Laser diagnostics: Matt Zepf et al.
%    \item Common aspects (Simulation, Data Acquisition, Data Quality and Computing): Matthew, Sasha, Federico et al.
%    \item Pixel tracker: Noam Tal Hod
%    \item EM calorimeter: Halina Abramowicz and Wolfgang Lohmann
%    \item Scintillation screens: Matthew Wing and John Hallford 
%    \item Cherenkov detectors: Ruth Jacobs 
%    \item Gamma Profiler: Marco Bruschi 
%    \item Gamma Spectrometer: Gianluca Sarri
%    \item Backscattering calorimeter: Maryna Borysova 
%    \item physics performance: Beate Heinemann
%\end{itemize}
%.... (to be finalized)

==> chapters6/organisation.tex <==
\subsection{Human and Financial Resources}
In Table \ref{tab:scint_costing} is a costing of the screen and camera system(s). Not taken into account is the engineering work required for installation or construction of optical tables - as these are at least shared with the \cer device. These costs are taken to be accounted for within the technical infrastructure estimate (see chapter~\ref{chapt12}). Mounts specific to the screen and cameras, essentially the frame to hold the screen and the mounts for cameras/lenses, \textit{are} costed.  

\begin{table}[h]
\caption{Estimates for costs relating to the scintillation screen. The screen and camera and accessories are increased in number for back-ups and are costed here (2 back-ups for each camera position). The equipment costs are for each instance, and so the cost is also given doubled to include implementation in both regions. Percentage values for labour represents the expected fraction of full-time work expected multiplied by the total cost of the position for this detector at LUXE. }
\label{tab:scint_costing}
\begin{center}
\begin{tabular}{ lclc }
  \hline\hline
  Item 							& Unit price (\EUR{}) 		& Quantity 		& Total price (\EUR{})	\\
  \hline
  Equipment needed\\ for each site: \\
  \hline
  GadOx screen			& 1000			& 2			& 2000 \\
  4K camera     		& 1400			& 3			& 4200 \\
  2K camera             & 400           & 6         & 2400 \\
  $f$=50\,mm lens      	& 250			& 4		    & 1000 \\
  $f$=75\,mm lens       & 600           & 2         & 1200 \\
  Optical Filter                & 725           & 6         & 4350 \\
  Neutral Density Filter & 50 & 2 & 100 \\
  Scintillator Frame    & 1000          & 2         & 2000 \\
  Camera Mounts \& Shielding & 2000     & 2         & 4000 \\
  \hline
  Total equipment, one site				&  					&  				& 21250 \\
  \hline
 \multicolumn{4}{l}{Equipment sharable between both sites/exclusive to one site:} \\
  \hline
  Additional Computing/cabling & 1000 & 1 & 1000 \\
  Calibration Lamp & 1000 & 1 & 1000 \\
  Optical Target(s) & 500 & 1 & 500 \\
  Ceiling Mount Apparatus & 5000 & 1 & 5000 \\
  \hline
   Total equipment both sites	&  					&  				& 49900 \\
  \hline
  25\% PostDoc (3 years)				& 						&					& 75000	\\
  PhD student (3 years)			& 						&					& 75000	\\
  25\% PhD student (5 years) 	& 						&					& 31250	\\
  \hline
  Total non-equipment		& 						&					& 181250 \\
  %\hline
  %Total					&  					&  				& 207400 \\
\hline\hline
\end{tabular}
\end{center}
\end{table}

\subsection{Schedule and Milestones}

Unlike the custom-built detectors common to high-energy physics, these ``off-the-shelf" components leave  comparatively few formal milestones to complete in the construction of the detector. These are listed below: 

\begin{itemize}
    \item Convergence upon a design for the scintillation screen and camera system (2021, completed). 
    \item Prototype testing and quality control (2022/2023, underway). 
    \item Collection and assembly of all commercially sourced components (2022/2023).
    %\JH{irradiation tests??}
    \item Measurement of a light--charge calibration curve with a high-population electron bunch user beam facility (late 2022/2023).
    \item Integration with Cherenkov detector and DAQ and control system (2023).
    \item Pre-installation preparations (2023/2024).
    \item Final Installation in the \euxfel chamber (2024)
\end{itemize}

This schedule ensures a detector ready for installation 2024. In the case of delays of the rest of the experimental setup, deeper analyses of the system, in particular with regard to the detector's resistance to radiation, can be performed before installation. The current state of the system includes a prototype with at least 2 of each component (camera, lens, filter, screen) and developing data acquisition software. The software for reconstruction is well underway and used in the performance chapter on results from a \geant simulation. 

%Describe here the schedule and the milestones. Normally we will try to be ready for installation by January 2024. There will be risks to that which we can treat as risks and the mitigation is to install later. 

%The level of detail of milestones should be quite high but maybe we should put it partially into an appendix. 

\subsection{Risk Management}



%Plain text that discusses the main risk factors, how/if they impact cost and/or schedule, their probability and how they are mitigated.

%There are two dimensions, the impact and the probability. We separate the impact on the cost and the schedule and use the following terms for impact risks:
%\begin{itemize}
%    \item Insignificant: Risk is easily mitigated by day to day process. 
%    \item Minor: Delays up to 10\% of schedule. Cost increase up to 10\% of budget. 
%    \item Moderate: Delays up to 30\% of schedule. Cost increase up to 30\% of budget. 
%    \item Major: Delays up to 50\% of schedule. Cost increase up to 50\% of budget. 
%    \item Catastrophic: project abandoned
%\end{itemize}
%For the budget, the denominator used is the budget of that area, i.e. if it is in the phase-0 \laser area it is relative to the total phase-0 \laser costs. In any case for the cost also the absolute numbers are given, so we can easily renormalize if the total cost changes.

%For the schedule, the fraction is taken relative to 24 months, assuming a start in January 2022 and a readiness of January 2024. 

%The probability of a risk to be realized is quantified as, rare: ($<3$\%), unlikely (3-10\%), moderate (10-50\%), likely (50-90\%) or certain ($>90\%$). 

Table \ref{tab:risks} shows a summary of the risks.
\begin{table}[]
    \centering
    \caption{Risk description, potential impact on cost and schedule, probability to occur and strategy on how to mitigate the risk. }
\begin{tabular}{p{0.2\linewidth}|p{0.1\linewidth}|p{0.1\linewidth}|p{0.1\linewidth}|p{0.35\linewidth}}
         Description & Cost & Schedule & Prob. & Mitigation Strategy\\\hline
         Radiation Damage to Screen & Minor & Minor & 3--10\% & Replace Screen/Rely on \cer measurements \\ \hline
         Permanent Radiation Damage to Cameras & Minor & Low & 10--20\% & Replace Screen/Rely on \cer measurements/increase shielding \\ \hline 
         Excessive unforeseen background & Moderate & Moderate & 3--10\% & Rely on \cer measurements/Increase shielding  \\
         \hline
         \end{tabular}
         \label{tab:risks}
\end{table}


\subsection{Responsibilities}
University College London takes responsibility for development, testing, measurement-taking and maintenance. Further engineering aspects with respect to installation and the creation of mechanical mounts and supports is handled by DESY engineers and technicians, whether employed already or will be in the future for LUXE.

==> chapters7/allnotes.tex <==
\section{All notes}
This is the list of all notes and the lead editors:
\begin{itemize}
    \item Technical infrastructure and beam instrumentation at LUXE: Louis Helary and Stewart Boogert 
    \item Laser, interaction chambers and timing system: Matt Zepf et al.
    \item Laser diagnostics: Matt Zepf et al.
    \item Common aspects (Simulation, Data Acquisition, Data Quality and Computing): Matthew, Sasha, Federico et al.
    \item Pixel tracker: Noam Tal Hod
    \item EM calorimeter: Halina Abramowicz and Wolfgang Lohmann
    \item Scintillation screens: Matthew Wing and John Halford 
    \item Cherenkov detectors: Ruth Jacobs 
    \item Gamma Profiler: Marco Bruschi 
    \item Gamma Spectrometer: Gianluca Sarri
    \item Backscattering calorimeter: Maryna Borysova 
    \item physics performance: Beate Heinemann
\end{itemize}
.... (to be finalized)

==> chapters7/intro.tex <==
The LUXE experiment is a new experiment in planning at DESY Hamburg and the European X-ray Free-Electron-Laser (EuXFEL). LUXE aims to probe Quantum Electrodynamics (QED) processes in the non-perturbative regime by studying collisions between a high-intensity optical laser and the EuXFELs $16.5\,\GeV$ electron beam, or a secondary beam of GeV photons created from the EuXFEL electron beam e.g.\ via Bremsstrahlung in a target. Among the predicted physics processes in this regime are non-linear Compton Scattering ($e^- + n\gamma_{L} \rightarrow e^- + \gamma_{C}$ ) and Breit-Wheeler pair production ($e^- + n\gamma_{L} \rightarrow e^- + e^+ + e^-$, or $\gamma_S+n\gamma_{L} \rightarrow e^+ + e^-$). Here, $\gamma_{L}$ denotes an optical laser photon, $n$ the number of absorbed laser photons, $\gamma_{C}$ is the Compton-produced photon and $\gamma_S$ is a photon from the secondary GeV photon beam. For more detail, see the executive summary technical note~\cite{LXTNExecSum}.\\

In LUXE, \cer detectors are used for the detection of electrons in locations with a high particle flux, of the order of $10^3-10^8~e^-$. There will be two instances of \cer detector systems in the LUXE setup, one for the detection of Compton-scattered electrons in the electron-laser running mode and one for the monitoring of Bremsstrahlung production in the photon-laser running mode. The two systems will be denoted as the electron detection system (EDS) \cer detector and the initial bremsstrahlung monitor (IBM) \cer detector. In both the IBM and EDS systems, the \cer detector is placed behind a scintillating screen that is read out by a camera system~\cite{luxecdr}.\\

A schematic drawing of the EDS is presented in fig.~\ref{fig:ceds-diagram}. The electron energy spectrum will be determined by measuring the number of electrons as function of their displacement by the dipole magnet. \\

Two complementary technologies (\cer and scintillation screen detectors) are used to enable the possibility of cross-calibration and alignment as well as assessment of systematic uncertainties. The scintillation screen offers a simple (and inexpensive) setup with a high resolution in position. The \cer device, for an appropriate choice of refractive medium, will offer a greater resistance to low-energy non-signal particles, and also will be more robust to the challenges of high particle flux. As a result, the scintillation screen is used mainly to measure the lower-flux (and lower electron energy) parts of the spectrum. The presence of a thin screen with a thickness of $0.5 \units{mm}$ (corresponding to $2.8\%$ of a radiation length) in front of the \cer detector will not affect the spectrum of electrons seen by the latter as the loss of the electron velocity $\beta$ is negligible. 

%The \cer and scintillator detectors are placed behind each other, displaced from the nominal \beamline by about $5 \units{cm}$. The \cer detector is $15 \units{cm}$ wide while the scintillator screen is $50 \units{cm}$ wide. 

\begin{figure}[htb!]
\centering
\includegraphics[width=0.6\textwidth]{fig/Sketch_CerenkovPlusScreen.png}
\caption{ A visualisation of the set-up of the electron detection system. Electrons from the IP, deflected by a dipole magnet, interact first with a thin screen of scintillating material and then the \cer detector. The light profile from the screen is imaged remotely with optical cameras, and light produced in the \cer medium is reflected towards an array of photodetectors.}
\label{fig:ceds-diagram}
\end{figure}


\begin{figure}[htb!]
\centering
\includegraphics[width=0.75\textwidth]{fig/SpectrumCompareXi_TomMC.pdf}
\caption{Simulated Compton electron energy spectrum for different values of the Laser intensity parameter $\xi$. Non-linear effects increase with $\xi$.}
\label{fig:comptonspectra}
\end{figure}

The objective for the EDS \cer detector is to measure the Compton electron energy spectrum, with a particular focus on measuring the position of the first Compton edge as a function of the laser intensity parameter $\xi$. A simulation of Compton spectra for different maximum $\xi$ values using the \ptarmigan generator~\cite{ptarm} can be seen in fig. \ref{fig:comptonspectra}. It is expected that the first Compton edge is shifted to larger energy values with a functional behaviour of

\begin{equation}
\label{eq:edgexi}
 \frac{E_\text{edge}(\xi)}{E_\text{beam}}=1-\frac{2\eta}{2\eta+1+\xi^2}\,,
 %\text{where}\; \eta(16.5\,\text{GeV})\approx 0.192 .    
\end{equation}

 where $\eta=\omega_L\epsilon_e/m_e^2\cdot\beta(1+\cos\theta)$ is the electron energy parameter, with the laser frequency $\omega_L$, electron beam energy $\epsilon_e$, velocity $\beta$ and electron-laser crossing angle $\theta$. For LUXE at an electon beam energy of $16.5\,\text{GeV}$, the energy parameter is $\eta \approx 0.192$. \\

The aim for the IBM is to measure the energy spectrum of electrons after the Bremsstrahlung interaction of the EuXFEL electron beam with the initial target in the LUXE photon-laser collision mode. In this case the electron energy spectrum is used to monitor the energy spectrum of the produced secondary photon beam.\\


The operating principle of the \cer detector is as follows: Charged particles traversing an active medium of refractive index $n$ at a speed faster than the speed of light in this medium emit \cer photons in the optical range according to the \textit{Frank-Tamm-Formula}~\cite{FrankTamm}:

\begin{equation}
    \label{eq:franktamm}
    \frac{d^2N_\gamma}{dz\,d\lambda}=\frac{2\pi\alpha}{\lambda^2}\sin^2\theta_c,
\end{equation}

where $\theta_c$ is the \cer angle, defined as $\cos\theta_c=1/\beta n$, $\lambda$ is the wavelength of the \cer photons, $\beta=v/c$ the speed of the charged particle, $z$ its path length in the active medium and $\alpha$ the fine-structure constant.\\

\begin{figure}
    \centering
    \includegraphics[width=0.6\textwidth]{fig/Sketch_CerenkovStraw.png}
    \caption{Visualisation of the production of \cer radiation and the light path in an air-filled reflective straw tube used as light guide.}
    \label{fig:sketch_straw}
\end{figure}

 Since the electron rate for the \cer detectors reach up to the order of $10^8$ per channel and laser shot, the straw diameter traversed by the incident electrons in the active medium produces a sufficient number of \cer photons for detection. The \cer medium used in the straws is air, which, despite its refractive index being low compared to other gases ($n_{\text{air}}\approx1.0028$) produces a sufficient number of \cer photons for the electron rates in LUXE. Fig.~\ref{fig:sketch_straw} shows a sketch of the light path in the straw light guide. Within the straw the \cer photons are reflected multiple times at the straw walls and are guided into the photo-detector placed at the end of the straw. \\

The following list summarized the modifications of the \cer detector system design with respect to the LUXE CDR \cite{luxecdr}:

\begin{itemize}
    \item \textbf{Channel design:} Vertical Straw tubes instead of metal U-shaped channels (\textit{eases finer segmentation}).
    \item \textbf{Photodetectors:} SiPMs and/or APDs instead of gaseous PMs (\textit{eases finer segmentation, allows to measure larger dynamic range of electron rates}).
    \item \textbf{Active medium:} Air instead of argon (\textit{cost reduction}).
\end{itemize}


==> chapters7/organisation.tex <==

\subsection{Human and financial resources}

The human and financial resources are estimated assuming a schedule relative to the point in time $T_0$, where funding for the LUXE experiment is released, with three years until the experiment is ready for data-taking. No explicit assumptions are made about the time of a long \euxfel shutdown.\\

Tables \ref{tab:cost_IBM} and \ref{tab:cost_EDS} list the cost of electrical and mechanical components of the IBM and EDS \cer detector systems respectively. The total cost of the two systems combined amounts to about $150\,\text{kEUR}$. Most of the hardware cost is expected to be spent during the second year after $T_0$, when equipment and components are ordered and delivered.\\

The person-power needed to complete the design, construction and software/readout design integrated over three years from $T_0$ is the following:

\begin{itemize}
    \item 3 FTE-years Post-doc (1 Postdoc FTE/yr) (detector design, readout software, testbeam campaign, supervision of students)
    \item 4 FTE-years PhD students ($2\times2/3$FTE /yr) (detector design, readout software, testbeam campaign)
    \item 0.6 FTE-years electrical/mechanical engineer (mainly required in year 1 for mechanical design, PCB design, )
    \item 0.3 FTE-years technician (mainly required for year 2 for detector assembly)
\end{itemize}
 
\begin{table}[h!]
    \centering
    \caption{Cost estimates for the IBM \cer system with 2 layers of 50 straw channels.}
    \begin{tabular}{|c|c|c|c|}
        \hline
        \textbf{Component}  & \textbf{Unit Cost (kEur)} & \textbf{Units req.} & \textbf{Total Cost (kEur)}\\\hline
         SiPMs & 0.06 & 50 & 3 \\\hline
         APDs & 0.26 & 50 & 13 \\\hline
         Readout electronics & 6.5 (32 channels) & 2 & 13 \\\hline 
         Straws & 0.005 & 100 & 0.5  \\\hline 
         PD PCB & 5 & 2 & 20 \\\hline 
         LED calibration board, fibers & 0.5 & 2 & 1  \\\hline
         cables, filters, small items & 5 & 1 & 5 \\\hline
         Slow-control and PC & 5 & 1 & 5 \\\hline
         Aluminium box & 0.2 & 1 & 0.2  \\\hline
         Gas system & 4 & 1 & 4 \\\hline\hline
         \textbf{Total} & & & 54.2 \\\hline
    \end{tabular}
    \label{tab:cost_IBM}
\end{table}

\begin{table}[h!]
    \centering
    \caption{Cost estimate for the EDS \cer system with 2 layers of 100 straw channels.}
    \begin{tabular}{|c|c|c|c|}
        \hline
        \textbf{Component}  & \textbf{Unit Cost (kEur)} & \textbf{Units req.} & \textbf{Total Cost (kEur)}\\\hline
         SiPMs & 0.06 & 100 & 6 \\\hline
         APDs & 0.26 & 100 & 26 \\\hline
         Readout electronics & 6.5 (32 channels) & 4 & 26 \\\hline 
         Straws & 0.005 & 200 & 1  \\\hline 
         PD PCB & 10 & 2 & 20 \\\hline 
         LED calibration board, fibers & 0.5 & 2 & 1  \\\hline
         cables, filters, small items & 10 & 1 & 10 \\\hline
         Slow-control and PC & 5 & 1 & 5 \\\hline
         Aluminium box & 0.5 & 1 & 0.5  \\\hline
         Gas system & 4 & 1 & 4 \\\hline\hline
         \textbf{Total} & & & 99.5 \\\hline
    \end{tabular}
    \label{tab:cost_EDS}
\end{table}


\subsection{Schedule and milestones}

Fig.~\ref{fig:cer_planning} shows an overview of the schedule and milestones for the LUXE \cer detector. The schedule for the \cer detectors is estimate until the point where the detector is ready for physics data-taking. It focuses on the EDS detector system, since this is a part of the minimal LUXE setup to take first physics measurements. Fig.~\ref{fig:cer_planning} shows the schedule with respect to $T_0$, the point in time, where the funding for LUXE is secured until three years from that point where the installation and commissioning phase is complete and the system is ready for data-taking. The first year is mainly dedicated to the finalization of the \cer detector design and test beam campaigns with a more advanced prototype with several channels and a more advanced electronics design. The second year is needed to procure the detector components, perform quality checks and to construct the full \cer detector. The first half of the third year is used to characterize the full detector, calibrate the channels and conduct the channel pre-alignment. In the second half of year three, the detector is installed and commissioned in the LUXE experimental area. For a more detailed discussion on the installation see section \ref{sec:instcommcal}.\\

%\begin{landscape}
\begin{figure}[h!]
   \centering  
    \makebox[\linewidth]{
    \includegraphics[width=1.1\textwidth]{fig/CherenkovScheduleMilestones.png}
    }
    \caption{Schedule and milestones for the LUXE \cer detector.}
    \label{fig:cer_planning}
\end{figure}
%\end{landscape}

The milestones associated with the LUIXE \cer system are:

\begin{itemize}
    \item MS 1: Calibration test with an advanced prototype at a high-rate testbeam facility. This milestone concludes the prototyping phase of the \cer detector. By testing the response of an advanced prototype with a representative and scaleable readout system at a high-statistics testbeam dataset, conclusions can be drawn if the detector design fulfils the requirements discussed in section~\ref{sec:requirements} and necessary adaptations to the design can be made if necessary.
    \item MS 2: Strategy and testbench for quality control completed. This step is necessary before orders of a large number of active components can be placed. The quality control testbench will be used to characterize the photodetectors as they arrive from the supplier.
    \item MS 3: The \cer detector design is fully completed, with all aspects of the system defined, such that orders to workshop, electronics components manufacturers etc. can be placed.
    \item MS 4: The \cer detector is fully assembled, basic funcionality tests are performed and the gas-tight box is sealed. This step is necessary to fill and start the characterization of the full detector.
    \item MS 5: The full \cer detector can be operated successfully stand-alone. All channels are pre-calibrated using LED and test beam runs and they fulfil the requirements discussed in section~\ref{sec:requirements}. The pre-alignment of the detector on its mounting structure is completed up to the required precision. The detector is ready for installation in the LUXE experimental area.
    \item MS 5: The detector is installed in the LUXE experimental area. Commissioning without beam is concluded. The detector is ready for beam-based commissioning. For a more detailed discussion of the steps needed during installation and commissioning, see section \ref{sec:instcommcal}.
\end{itemize}


\subsection{Risk management}

The risks to the LUXE \cer detector project associated with the Milestones above are estimated based on the following scale:

\begin{itemize}
    \item Insignificant: Risk is easily mitigated by day to day process. 
    \item Minor: Delays up to 10\% of schedule. Cost increase up to 10\% of budget. 
    \item Moderate: Delays up to 30\% of schedule. Cost increase up to 30\% of budget. 
    \item Major: Delays up to 50\% of schedule. Cost increase up to 50\% of budget. 
    \item Catastrophic: project abandoned
\end{itemize}


The probability of a risk to be realized is quantified as, rare: ($<3$\%), unlikely (3-10\%), moderate (10-50\%), likely (50-90\%) or certain ($>90\%$).\\

Table \ref{tab:risks} lists the risks associated with the milestones foreseen for the LUXE \cer detector system. Since Milestone I (low-rate TB with detector prototype) has been reached at the time of compiling the technical note, the risk assessment starts with Milestone II. Since the design of LUXE on purpose foresees two complementary detector technologies for the EDS and IBM systems (Scintillator screen and \cer detectors) no catastrophic risk to the LUXE experiment could be identified.\\

\begin{table}[htb!]
    \centering
    \caption{Risk description, potential impact on cost and schedule, probability to occur and strategy on how to mitigate the risk.}
\begin{tabular}{p{0.2\linewidth}|p{0.12\linewidth}|p{0.12\linewidth}|p{0.12\linewidth}|p{0.35\linewidth}}
        \hline
        \textbf{Description} & \textbf{Cost} & \textbf{Schedule} & \textbf{Prob.} & \textbf{Strategy}\\\hline
         \multicolumn{5}{c}{\textbf{Milestone 1: Advanced Prototype high-rate test}} \\\hline
         Delay in prototype construction & Insignificant & Moderate & Moderate & assign enough person-power \\\hline
         Suitable TB facility not available & Insignificant & Moderate & Moderate & apply for beam time early, at several places \\\hline
         \multicolumn{5}{c}{\textbf{Milestone 2: Electrical components test bench and routine}} \\\hline
         Delayed past order arrival & Minor & Minor & Moderate & assign enough person power \\\hline
         \multicolumn{5}{c}{\textbf{Milestone 3: Final detector design}} \\\hline
         Suboptimal design noticed late & Moderate & Moderate & Moderate & early engineering review, thorough beam tests with realistic prototype\\\hline
         \multicolumn{5}{c}{\textbf{Milestone 4: Detector construction}} \\\hline
         Delay in order of electrical components & Moderate & Moderate & Moderate & foresee enough time in planning \\\hline
         Electrical components failure & Minor & Minor &  Likely & establish quality control, order feasible amount of spares, exchange-friendly design \\\hline
         \multicolumn{5}{c}{\textbf{Milestone 5: Charge calibration}} \\\hline
         Detector construction delayed & Insignificant & Minor & Moderate & can do in-situ in LUXE experimental area\\\hline
         \multicolumn{5}{c}{\textbf{Milestone 6: Installation and Commissioning}} \\\hline
         Critical component failure unnoticed & Moderate & Minor & Unlikely & frequent functionality tests, exchange-friendly design  \\
         \hline
         \end{tabular}
         \label{tab:risks}
\end{table}


\subsection{Responsibilities}
The responsibility and human resources for the development, construction and installation of the \cer system will be taken by DESY Hamburg. Certain aspects of the construction and installation in the experimental area require access to central DESY services, such as mechanical and electronics workshops, electrical and gas system installations in the experimental area as well as lifting the detector systems into the LUXE area by crane. In addition the use of DESY test beam facilities is foreseen as a part of the detector development and calibration process.\\


==> chapters8/organisation.tex <==
%\section{Project organisation}

We are aiming at starting installation during one of the longer planned shutdown of the EuXFEL operations. In Table~\ref{manpower}, a breakdown of required human resources is given for the different stages of preparation (Years -2 and -1), installation (Year 0), and data acquisition (Years 1,2, and 3). The available funding is shown assuming installation in 2025  and is currently obtained mainly via support of a national research council, the Engineering and Physical Science Research Council (EPSRC) in the UK. 

\begin{table}[t!]
\centering
\begin{tabular}{|l||c|c|c|c|c|c|}
\hline
\textbf{Human resource } & \textbf{Year -2} & \textbf{Year -1} & \textbf{Year 0} & \textbf{Year 1} & \textbf{Year 2} & \textbf{Year 3}  \\
\hline
\hline
PhD FTE & 1 & 1 & 1 & 1 & 1 & 1 \\
\hline
Post-doc FTE  & 1 & 1 & 1 & 1 & 1 & 1 \\
\hline
Senior scientist FTE & 0.2 & 0.2 & 0.2 & 0.2 & 0.2 & 0.2 \\
\hline
\hline
 \multicolumn{7}{|r|}{ \textbf{\centerline{\emph{Funding secured (assuming 2025 as Year 0)}}}} \\
\hline
PhD FTE & 0.5 & 0.5 & 0 & 0 & 0 & 0 \\
\hline
Post-doc FTE  & 0.5 & 0.5 & 0.5 & 0 & 0 & 0 \\
\hline
Senior scientist FTE & 0.1 & 0.1 & 0.1 & 0 & 0 & 0 \\
\hline
\hline
\end{tabular}
\caption{FTE requested for the preparation, installation, and running of the gamma-ray spectrometer in LUXE. Secured funding is shown in the bottom half of the table, assuming installation in 2025.}
\label{manpower}
\end{table}

Several milestones can be identified to reach a final version of the spectrometer to be installed in LUXE. The analysis and deconvolution algorithms have already been finalised and tested both numerically and experimentally at two proof-of-principle experimental campaigns carried out using the Astra-Gemini laser at the Central Laser Facility in the UK and the Apollon laser facility in France (results are currently being prepared for publication). In both cases the spectrometer has been tested using a bright bremsstrahlung source with a variable maximum energy of the order of 1 -- 2\,GeV. Crucially, both campaigns confirmed that the converter foil does not experience noticeable degradation during sustained high-dose irradiations and that single-shot electron and positron spectra can be obtained using commercially available scintillator screens, two critical points for the successful implementation of the spectrometer within LUXE.

The second step of the project will be the design and construction of the dedicated vacuum chamber and the lead collimator, which is expected to be provided by the facility by the end of 2023. The dipole magnet is also expected to be available at DESY.

In summary, the main milestones of the project are:
\begin{itemize}
    \item [1.] \textbf{Algorithms and deconvolution routine}: completed.
    \item [2.] \textbf{First tests at low energy (sub-GeV)}: completed.
    \item [3.] \textbf{Tests at moderate energy (2 GeV)}: completed.
    \item [4.] \textbf{Construction of the first prototype}: to be completed by the end of 2023.
     \item [5.] \textbf{Installation, testing, and calibration}: to be completed during dedicated access.
\end{itemize}

As one can see from the list above, all the preparatory numerical modelling and experimental testing have been successfully completed, placing high confidence in the successful implementation of the detector in LUXE.

An estimate of the overall cost of the detector is given in Table~\ref{cost}. The costs breakdown  does not include the cost of the dipole magnet (expected to be available at DESY) and vacuum chamber (quotes currently been sought from vendors). An estimate of 60 k\euro for the optical elements assumes the use of optical fiber bundles; a lower cost option would consist in using relay imaging with conventional optics. The group at Queen's University Belfast will provide the scintillator screens, CCD cameras, filters, and target mounts, for an overall contribution estimated to be of the order of 66 k\euro. 

\begin{table}[t!]
\centering
\footnotesize
\begin{tabular}{|l|c|c|c|l|}
\hline
\footnotesize{\textbf{Item}} & \textbf{Cost} & \textbf{Notes} & \textbf{Responsible}  \\
\hline
\hline
\footnotesize{10 $\mu$m W foil 25x25 mm} & 0.2 & & QUB\\
\hline
interference filters & 0.8 &  & QUB\\
\hline 
scintillators with mounts & 2 &  & QUB\\
\hline
2-D motorised mount & 3 & motorisation for fine alignment & QUB\\
\hline
collimator & 5 &  & QUB\\
\hline
2 iCCD cameras & 60 &  & QUB\\
\hline
optical elements & 60 & mirrors, lenses and fibre-bundles & DESY \\
\hline
dipole magnet & TBC &  & DESY\\
\hline
vacuum chamber & TBC & & DESY\\
\hline 
\hline
\textbf{TOTAL} & \textbf{131 + TBC} & & \\
\hline
\end{tabular}
\caption{Estimate of the equipment and consumables cost of the detector. All costs are given in k\euro.}
\label{cost}
\end{table}

A risk mitigation strategy has been devised and a summary of the main risks and associated actions is given in Table~\ref{risks}. It must be noted that the advanced stage of analysis and preliminary experimental testing of the detector result in all risks to be low to moderate. 

\begin{table}[b!]
\footnotesize
\centering
\begin{tabular}{|l|c|c|c|l|}
\hline
Issue  & Probability & Impact on cost & Impact on schedule & Mitigation  \\
\hline
\hline
Difficulty in  & Low & Moderate & Low & Explore alternative \\
securing funding& & & & funding streams\\
\hline
Low signal & Low & Low & Low & Increased shielding \\
to noise& & & & and improved analysis\\
& & & & tools\\
\hline
Area unsuited & Low & Moderate & Low & Move iCCD cameras \\
for iCCD cameras& & & & in shielded area\\
& & & & upstairs with\\
& & & & longer optical path\\
\hline
Degradation of & Low & Low & Moderate & Revert to \\
fibre bundles& & & & relay imaging\\
due to radiation& & & & with conventional\\
& & & & optics\\
\hline
Degradation & Low & Moderate & Low & Use GRS  \\
of W target& & & & for dedicated runs\\
& & & & or implement\\
& & & & replacement system\\
\hline
\hline
\end{tabular}
\caption{Identified potential risks and associated mitigation strategy. }
\label{risks}
\end{table}

==> chapters9/organisation.tex <==
\label{sec:gbp:organisation}

This chapter describes the organisation, the planning and the resources needed to build, install and commission the GBP system.

Section~\ref{sec:org_int} introduces the main elements of the organisation of the project, i.e.\ the high level product breakdown structure (PBS), the management structure and the responsibility matrix.  
Then, Section~\ref{sec:org_res} describes the costs of the project, with their basis of estimate, and an evaluation of the human resources needed. Foreseen contributions from the project institutions, in terms of effort  that is expected to be available, are also reported.  Section~\ref{sec:org_sch} discusses the schedule and timeline, including a list of the main milestones.
The risks involved with the project, and the strategies to mitigate them, are dealt with  in Section~\ref{sec:org_risk}. 

\subsection{Organisation}
\label{sec:org_int}

The GBP project will be performed by a group of institutions that commit to developing, designing, constructing and installing all the components, and then to commissioning the system, running it and analysing the data it will produce.  All groups participating in the project are represented in   the GBP institute board (IB) by group representatives. The current set of institutions and groups at the time of writing this report, with their representatives,
is reported in Table~\ref{gbp:instit}.
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htbp]
  \centering
%  \caption{Add caption}
\footnotesize
    \begin{tabular}{l|l|l}
    \multicolumn{1}{c|}{Institution} & \multicolumn{1}{c|}{Group} & \multicolumn{1}{c}{Representative} \\
    \hline
    INFN & Bologna Section & Marco Bruschi \\
    INFN & Padova Section & Mauro Morandin \\
    The Queen's University of Belfast & School of Math. and Phys. & Gianluca Sarri \\
    \hline
    \end{tabular}%
    \caption{Institutions and their representatives in the GBP IB.}
  \label{gbp:instit}%
\end{table}%

The activities within the project are coordinated by a project leader and the project’s PBS is shown in Table~\ref{tab:wbs} with the distribution of responsibility assignments across the participating groups.
\begin{table}
    \centering
    \includegraphics[width=\textwidth]{figures_chapt9/GBP_WBS_v2.0.png}
    \caption{The level-3 GBP PBS.}
    \label{tab:wbs}
\end{table}
There are 9 entries at level-2 with the last three encompassing global deliverables of the project. At the time of writing, managers have been appointed for all the level-2 items. 
The level-2 and level-3 managers form the GBP coordination board.

Dedicated working groups have also been created, led by one or two coordinators each, that comprise experts collaborating on the key aspects of the project and report to the project leader.

The following groups have been setup:
\begin{itemize}
\item Sensors characterisation, tests and qualification process;
\item GBP sensors physics performance;
\item GBP stand-alone and global simulation.
\end{itemize}

In addition, a resource coordinator and a risk manager have been appointed. The resource coordinator maintains a database of required and pledged resources, both financial and human. The risk manager develops and maintains the risk register in coordination with
the level-2 and 3 managers. 

\subsection{Human and financial resources} \label{sec:org_res}

The estimates of the costs are explained in a basis of estimates document and Table~\ref{tab:GBP_costs} reports an overview of the costs at level-2 with the foreseen spending profile.

\begin{table}[htbp]
 \includegraphics[width=\textwidth,keepaspectratio]{figures_chapt9/GBP_costs}
      \caption{Estimated costs and foreseen spending profile.}
  \label{tab:GBP_costs}%
\end{table}%

The amount of resources needed to build, install and maintain the detector was originally evaluated for the years 2022--2025, assuming an installation taking place in 2024. The quantification has been performed for engineers, technicians, students (including PhD) and physicists and possible matching contributions from the various institutions have been assessed.  The  Table~\ref{tab:GBP_Resources} shows the requirements and the plausible amount of resources that institutions could provide, once the LUXE experiment has been approved.  The comparison indicates that the collaborating institutions should have sufficient resources to provide the needed effort. 

\begin{table}
    \centering
    \includegraphics[width=\textwidth,keepaspectratio]{figures_chapt9/GBP_Resource_profile_for_TN_v1.0.png}
    \caption{Estimated amount of resources needed and plausible to build, install and maintain the GBP, 2022--2025.}
    \label{tab:GBP_Resources}
\end{table}

\subsection{Schedule and milestones} \label{sec:org_sch}

A schedule for the construction and the installation of the GBP has been developed and is currently maintained as a ProjcetLibre file.  The GANNT chart illustrating the relationship among the various activities and the milestones appear in the Appendix separately for the construction phase, which is expected to be concluded in Summer 2025 and for the installation activities that are nominally taken to start in the 2025--26 shutdown. 

The main phases and milestones for the construction of the GBP are summarised in  Table~\ref{tab:GBP_milestones}.

\begin{table}[htbp]
  \centering
%  \caption{Add caption}
\footnotesize
    \begin{tabular}{l|l|c}
    \multicolumn{1}{c|}{Phase} & \multicolumn{1}{c|}{Milestone} & \multicolumn{1}{c}{Milestone date} \\
    \hline
    Prototype lab. and beam tests & Prototype validated & 30-6-2023 \\
    GBP construction & GBP ready for installation & 01-06-2025 \\
    GBP installation & GBP installed & 30-01-2026 \\
    \hline
    \end{tabular}%
    \caption{Main construction phases and milestones.}
  \label{tab:GBP_milestones}%
\end{table}%

\subsection{Risk management} \label{sec:org_risk}

Management of the risk is performed through the regular update of a risk register in which risks are classified for their impact: 

\begin{itemize}
    \item Irrelevant: Risk is easily mitigated by day to day process. 
    \item Minor: Delays up to 10\% of schedule. Cost increase up to 10\% of budget. 
    \item Moderate: Delays up to 30\% of schedule. Cost increase up to 30\% of budget. 
    \item Major: Delays up to 50\% of schedule. Cost increase up to 50\% of budget. 
    \item Catastrophic: project abandoned
\end{itemize}

and for the probability of realisation as follows:   rare ($<3$\%), unlikely (3-10\%), moderate (10-50\%), likely (50-90\%) or certain ($>90\%$).

In Table~\ref{tab:GBP_RR} the main risks are reported, together with their mitigation strategy. 

\begin{table}
    \centering
    \includegraphics[width=\textwidth,keepaspectratio]{figures_chapt9/GBP_Risk_Register_V3.0.png}
    \caption{Risk description, mitigation strategy, probability to occur, cost and schedule impact.}
    \label{tab:GBP_RR}
\end{table}


The most critical risk is related to the possibility that the charge collection efficiency (CCE) of the sapphire sensors turns out to be significantly lower than the values extrapolated from previous measurements or that the CCE is not uniform across the sensors. The first possibility was ruled out with the first tests carried out at the INFN LNF in 2022 and described in this document.  Measurements to demonstrate the necessary CCE uniformity will be carried out in 2023.  In the worst case, it will be possible to replace the sapphire sensors with diamond microstrip detectors that have been successfully used as particle detectors in extremely high radiation environments. They represent a solid backup solution, though the costs would be higher, since the diamond wafers are more expensive and we would need to replace them more frequently.  
The realisation of the second risk would cause an increase of the sensors size but without changing the number of the strips and therefore the number of electronics channels, so the impact on the total costs would be minor and it could be compensated by the lower dose absorbed.   Finally the background due to charged tracks can have an impact since the gammas convert with a very low probability inside the sapphire while possible background charged tracks always produce a signal. The countermeasure in this case would be to insert a converter in front of the GBP with the proper thickness to create electron--positron pairs that would overcome the background.  This would cause an increase of the dose absorbed by the sensors with the need of more frequent sensors replacement.

\subsection{Construction and installation schedules}

The construction and installation schedules are shown in fig.~\ref{fig:construction_gannt} and fig.~\ref{fig:installation_gannt}

\begin{figure}    \includegraphics[width=\textwidth,keepaspectratio]{figures_chapt9/GBP_GANNT_charts_v1.0.eps}
    \caption{GBP construction GANNT chart.}
    \label{fig:construction_gannt}
\end{figure}

\begin{sidewaysfigure}    \includegraphics[width=\textwidth,keepaspectratio]{figures_chapt9/GBP_inst_GANNT_v2.0.png}
    \caption{GBP installation GANNT chart.}
    \label{fig:installation_gannt}
\end{sidewaysfigure}


==> figures_chapt5/ECAL_pictures/performance.tex <==
The performance of the ECAL-P was studied with the LUXE \textsc{Geant4} simulation assuming that a sensor plane consists of $320 \units{\mu m}$ thick silicon sensor, sandwiched between two Kapton layers supported by a thin carbon envelop, with the whole structure having a thickness of $830 \units{\mu m}$.
The sensors are subdivided into pads of $5 \times 5 \units{mm^2}$ area.
For the current studies, the energy deposited in each pad is used. Signal sharing between pads and signal digitisation will be implemented in the future, based on the results of beam-tests.

In the following, we discuss the performance of the ECAL-P for single showers, with and without background, and the expected results for high rates of positrons where single showers cannot be identified and the spectrum is reconstructed through an energy-flow type of approach. The latter case is studied without background implementation. For the medium range rates, we are developing a clustering algorithm which should then lead to a performance similar to the one of single showers.


\subsection{Energy and Position Resolution for single positrons}
The performance of the ECAL-P for single positrons was studied by generating samples of positrons in the energy ($E_0$) range between 2 and $15 \units{GeV}$ in steps of $0.5 \units{GeV}$, assuming the positrons originated from the IP. The positrons enter the calorimeter at an angle due to the deflection in the dipole magnet. After calibration, which takes into account the angular dependence of the response, the dependence of the relative resolution $\sigma/E$ as a function of the initial positron energy is shown in Fig.~\ref{fig:ECAL-elaser-resolutions} (left). A fit of the form $\sim 1/\sqrt{E_0}$ leads to
\begin{equation}
    \frac{\sigma_E}{E} = \frac{(20.2 \pm 0.1)\%  }{\sqrt{E_0/\text{GeV}}}\, .
    \label{eq:ECAL-elaser-eresolution}
\end{equation}
\begin{figure}[!htbp]
    \centering
    \includegraphics[width=0.45\textwidth]{ECAL_pictures/simulation/ECAL_elaser_energy_resolution.pdf}
    \includegraphics[width=0.45\textwidth]{ECAL_pictures/simulation/ECAL_position_resolution_10GeV.pdf}
\caption{Left: The relative energy resolution of the ECAL-P as a function of the positron energy $E_0$. Right: The probability distribution function (PDF) of the difference between the reconstructed and the generated entry point of the positron shower along the magnetic deflection ($x$) axis,  for 10\,GeV positrons.}
    \label{fig:ECAL-elaser-resolutions}
\end{figure}
\begin{figure}[!htbp]
    \centering
    \includegraphics[height=0.35\textwidth]{ECAL_pictures/simulation/ECAL_elaser_position_resolution.pdf}
    \includegraphics[height=0.35\textwidth]{ECAL_pictures/simulation/ECAL_elaser_resolutions.pdf}
\caption{Left: Position resolution as a function of positron energy. Right: The relative energy resolution of the ECAL-P as a function of the positron energy $E_0$ from position reconstruction (right $y$-scale) compared to the relative resolution from calorimetry (left $y$-scale).}
    \label{fig:ECAL-elaser-x-resolutions}
\end{figure}

For the position reconstruction, a logarithmic weighting of the energy deposits in the pads is applied, with a threshold optimised to give the best resolution. Along the $y$-axis, not affected by the deflection in the dipole magnet, a resolution of $\sigma_y= 460 \units{\mu m}$ is achieved (not shown). Along the $x$-axis, $\sigma_x= 550 \units{\mu m}$ at $10 \units{GeV}$ is obtained, and a mild dependence on the energy is found. However, while along the $y$-axis no bias in the position reconstruction is observed, this is not the case for the $x$ position. As shown in Fig.~\ref{fig:ECAL-elaser-resolutions} (right), for positrons of $10 \units{GeV}$, a bias of $\delta x \simeq 500  \units{\mu m}$ is generated by the fact that the positrons impact the ECAL-P under a small angle. This is not critical as this bias can be corrected for. An approach based on convoluted neural networks was also applied to the position reconstruction. The position resolution (not shown) was not better than for the logarithmic weighting, however there was no bias in the results.

The alternative method of determining the energy for single positron showers is by making use of the correlation between energy and position of the positron entry point on the face of the ECAL-P. The relative energy resolution is then determined by the position resolution. The position resolution as a function of positron energy is shown in Fig.~\ref{fig:ECAL-elaser-x-resolutions} (left). Also shown in the figure (right) is the resulting $\sigma/E$ compared to the one from calorimetry shown in Fig.~\ref{fig:ECAL-elaser-resolutions}. Not surprisingly, the $\sigma/E$ from position reconstruction is better by factor 10 (high energy) to better than 40  (low energy) in the relevant energy range.


\subsection{Impact of background}
It is important to ensure that this performance can also be achieved in the presence of background, which is particularly sizeable near the beam-line. In this section, first the electromagnetic component of the background is considered. For the hadronic component, a preliminary result is shown in the last figure. In addition, the material of the beam exit window of the interaction chamber will be changed from Kapton to aluminium, being not yet considered in all studies. Hence, further studies 
are underway.

The distribution of the background depositions per \elaser bunch crossing is shown in Fig.~\ref{fig:ECAL-3D-background} (left). Also shown in the figure (right) are the depositions for a single positron of $5 \units{GeV}$.
\begin{figure}[htbp]
\centering
    \includegraphics[width=0.49\textwidth]{ECAL_pictures/simulation/ECAL_fast_BG.pdf}
    \includegraphics[width=0.49\textwidth]{ECAL_pictures/simulation/ECAL_positron_5GeV.pdf}
    \caption{Left: Depositions per bunch-crossing from beam-related electromagnetic background inside the ECAL-P. The beam-pipe is located on the right side. The beam exit window at the interaction chamber is made of Kapton. Right: Depositions from a single positron of $5 \units{GeV}$.}
    \label{fig:ECAL-3D-background}
\end{figure}
The depositions of the single positron are in a small cone around the shower axis. The background is widely spread and its contribution increases towards the beam-pipe.
The effect of this background on the energy deposited in the cone around the shower axis is shown in Fig.~\ref{fig:ecal-singlep-edep-elaser} for several positron energies. The distribution of the energy deposited by positrons of a given energy is compared to the distribution obtained after adding the background to all pads containing the electromagnetic shower.
\begin{figure}[htbp]
\centering
     \includegraphics[width=0.8\textwidth]{ECAL_pictures/simulation/ECAL_elaser_sbOs_hist}
    \caption{Distribution of total energy deposited in the sensor-pads of the ECAL-P for selected energies of positrons (full lines) and for the same positron showers with added electromagnetic background (dashed-lines) in the \elaser setup. The various energies of the positrons listed in the legend are identified by different colours. The beam exit window of the interaction chamber is made of Kapton.}
    \label{fig:ecal-singlep-edep-elaser}
\end{figure}
One clearly observes a shift in the total deposited energy but no significant deterioration in the resolution. As expected, the shift in energy is the more pronounced the closer it gets to the beam-line, i.e. the higher the energy of the positron. 

In recent simulations, the depositions induced by neutrons are added \footnote{Only neutron induced depositions produced within 100 ns after the bunch crossing are considered. Depositions produced later are ignored, since they will not be registered by the read-out electronics.} and the beam exit window of the interaction chamber is made of aluminium, enhancing the electromagnetic background in the order of 10\%. 
In Fig.~\ref{fig:ECAL-sig+bgr} the ratio between the sum of signal and background depositions and the depositions from the signal only is shown as a function of the positron energy $E_0$ both for the \elaser and \glaser setup.  This ratio is between 1.0, at low and 1.6, at high $E_0$.
For a further suppression of the background, the shielding against photons and neutrons will be optimised. The remaining impact of the background depositions  
will finally be corrected for by direct background measurements with electron or photon bunches crossing the detector without interaction with a laser pulse.
\begin{figure}[!hpbt]
\centering
\includegraphics[height=0.45\textwidth]{ECAL_pictures/simulation/ECAL_fullBG_both_setups.pdf}
\caption{
Ratio of the expected energy deposition in a positron shower with electromagnetic and neutron induced background to the one without background as a function of the positron energy $E_0$, for the \elaser and \glaser setup. The beam exit-window at the interaction chamber is made of aluminium.}
\label{fig:ECAL-sig+bgr}
\end{figure}

\subsection{Reconstruction of Positron Number and Spectrum}
When the number of positrons entering the ECAL-P becomes large, the showers start overlapping and it becomes impossible to identify individual clusters. Instead, a method based on energy-flow is proposed~\cite{mykyta_thesis_2020}, whereby each pad contributes a fraction of the number of positrons in a given energy bin. The latter is determined from the crossing of the path connecting the centre of the pad to the IP, according to the dipole magnet field and the geometry, with the face of the ECAL-P, as if the pad was located on the axis of the shower generated by the impinging positron. At the end of this procedure, both the energy spectrum observed in the ECAL-P and the number of positrons (sum over all energy bins) are reconstructed. An overall correction of the order of 2\% has to be applied to the reconstructed number of positrons to obtain the number of generated positrons. The relative spread of the number of reconstructed positrons as a function of the number of incident positrons is shown in Fig.~\ref{fig:mult-pos} (left). For an average positron multiplicity of about 1000 the projection on the vertical axis is shown in Fig.~\ref{fig:mult-pos} (right) . The uncertainty is less than 0.5\%.
\begin{figure}[!htbp]
\centering
\includegraphics[height=0.35\textwidth]{ECAL_pictures/simulation/ECAL_number_reconstruction-coloured.pdf}
\includegraphics[height=0.35\textwidth]{ECAL_pictures/simulation/ECAL_number_reconstruction.pdf}
\caption{Left: The relative spread of the number of reconstructed positrons as a function of the number of incident positrons. Right: Projection of the relative spread onto the vertical axis for an average positron multiplicity of 1000.}
\label{fig:mult-pos}
\end{figure}
The comparison between the generated and reconstructed energy spectra is shown in Fig.~\ref{fig:ECAL-energy-spectrum}.
\begin{figure}[!hptb]
\centering
    \includegraphics[width=0.9\textwidth]{ECAL_pictures/simulation/ECAL_elaser_energy_flow}
    \caption{Comparison between the reconstructed and generated energy spectra of the positrons. The ratio of the two spectra as a function of energy is displayed in the lower panel.}
    \label{fig:ECAL-energy-spectrum}
\end{figure}
A good agreement between the two spectra is found, with the exception of the low-energy and high-energy tails, where leakage of the showers sets in.
The same reconstruction method was applied to multiplicities of the order of $10^5$ (not shown) and still reasonable agreement was found, though the overall correction factor increased to 5\%. However, positron multiplicities of this order very likely cannot be measured by the ECAL-P, as they would lead to distortions in the charge drift due to high charge density in the sensor and to saturation of the front-end (FE) ASICs. This problem is under study in order to determine the highest positron multiplicity that can be handled by the ECAL-P. Changing the bunch charge or the electron beam width allows at very large $\xi$ to reduce the number of positrons such that it matches the dynamic range of ECAL-P.

Studies to implement image recognition with convoluted neural networks for the reconstruction of the energy spectra and multiplicities is under investigation. It turns out that with the first 10 layers of the ECAL-P one can already derive the positron multiplicity and the average energy on an event by event basis. Further studies are underway to reconstruct the full energy spectrum.

The ECAL-E has been introduced only recently into the geometry of LUXE and the study of its performance is underway. However given the similarity between the ECAL-P and ECAL-E in sampling and granularity, similar results are expected.

\begin{comment}
\subsection{Saturation of Charge in the Sensitive Materials}


\SH{Work in Progress}
\vspace{1cm}

\subsection{Impact of background}

\SH{TBD after the shielding of neutron background}
\vspace{1cm}
***can be added also in the previous subsections.
\vspace{1cm}
\end{comment}

==> journal/Makefile <==
# Makefile for creating an ATLAS paper draft using journal classes

TEXLIVE  = 2020
LATEX    = latex
PDFLATEX = pdflatex
BIBTEX   = bibtex
DVIPS    = dvips
DVIPDF   = dvipdf
OPEN     = open

TEXFILES = $(wildcard *.tex)

.PHONY: texlive clean

all: atlas-elsevier atlas-jhep atlas-jinst atlas-revtex

texlive:
	for file in $(TEXFILES); do \
	  if [ $(TEXLIVE) -ge 2013 -a $(TEXLIVE) -lt 2100 ]; then \
	    echo "Changing texlive value in $$file"; \
	    sed -i'.bak' 's/texlive=20[0-9][0-9]/texlive=$(TEXLIVE)/' $$file; \
	  else echo "Invalid value for TEXLIVE: $(TEXLIVE)"; fi; \
	done

atlas-elsevier: atlas-elsevier.pdf
	@echo "Made $<"
	# $(OPEN) $<

atlas-jhep: atlas-jhep.pdf
	@echo "Made $<"
	# $(OPEN) $<

atlas-jinst: atlas-jinst.pdf
	@echo "Made $<"
	# $(OPEN) $<

atlas-revtex: atlas-revtex.pdf
	@echo "Made $<"
	# $(OPEN) $<

run_latex: $(BASENAME).dvi
	$(DVIPDF) -sPAPERSIZE=a4 -dPDFSETTINGS=/prepress $<
	@echo "Made $< and $(basename $<).pdf"

# Standard LaTeX targets
%.pdf: %.tex *.bib
	$(PDFLATEX) $<
	-$(BIBTEX)  $(basename $<)
	$(PDFLATEX) $<
	$(PDFLATEX) $<

%.dvi: $(BASENAME).tex
	$(LATEX)    $<
	$(LATEX)    $<

clean:
	-rm *.dvi *.toc *.aux *.log *.out *.blg *.bbl *.bcf \
	 *.fdb_latexmk *.spl *-revtexNotes.bib *.run.xml *.synctex.gz *~

cleanall: clean
	-rm *.pdf


==> journal/atlas-document-metadata.tex <==
%-------------------------------------------------------------------------------
% This file contains the title, author and abstract.
% It also contains all relevant document numbers used by the different cover pages.
%-------------------------------------------------------------------------------

%% Title
\AtlasTitle{A simple ATLAS paper draft}
%
% Author - this does not work with revtex
% \author{The ATLAS Collaboration}
%
% Date: if not given, uses current date
% \date{\today}

% Draft version:
% Should be 1.0 for the first circulation, and 2.0 for the second circulation.
% If given, adds draft version on front page, a 'DRAFT' box on top of each other page, 
% and line numbers.
% Comment or remove in final version.
\AtlasVersion{1.0}

% ATLAS reference code, to help ATLAS members to locate the paper
\AtlasRefCode{GROUP-2020-XX}

% ATLAS note number. Can be an COM, INT, PUB or CONF note
% \AtlasNote{ATLAS-CONF-2020-XXX}
% \AtlasNote{ATLAS-PUB-2020-XXX}
\AtlasNote{ATLAS-COM-PHYS-2020-XXX}

% Submission journal
\AtlasJournal{Phys.\ Lett.\ B.}

% Abstract - % directly after { is important for correct indentation
\AtlasAbstract{%
	This is a bare bones ATLAS document used to demonstrate how to use journal templates.

	This document is typeset using the \DocumentStyle.
}

%-------------------------------------------------------------------------------
% The following information is needed for the cover page. The commands are only defined
% if you use the coverpage option in atlasdoc or use the atlascover package
%-------------------------------------------------------------------------------

% Explicit list of supporting notes  (leave as null \AtlasCoverSupportingNote{} if you want to skip this option)
\AtlasCoverSupportingNote{A supporting note}{http://cds.cern.ch/record/XXXXXX}
\AtlasCoverSupportingNote{Another supporting note}{http://cds.cern.ch/record/YYYYYY}
%
% OR (the 2nd option is deprecated, especially for CONF and PUB notes)
%
% Supporting material TWiki page  (leave as null \AtlasCoverTwikiURL{} if you want to skip this option)
% \AtlasCoverTwikiURL{https://twiki.cern.ch/twiki/bin/view/Atlas/WebHome}

% Comment deadline
\AtlasCoverCommentsDeadline{DD Month 2020}

% Analysis team members - contact editors should no longer be specified
% as there is a generic email list name for the editors
\AtlasCoverAnalysisTeam{Peter Analyser, Susan Editor1, Jenny Editor2, Alphonse Physicien}

% Editorial Board Members - indicate the Chair by a (chair) after his/her name
\AtlasCoverEdBoardMember{EdBoard~Chair~(chair), EB~Member~1, EB~Member~2, EB~Member~3}

% Editors egroup
\AtlasCoverEgroupEditors{atlas-GROUP-2020-XX-editors@cern.ch}

% EdBoard egroup
\AtlasCoverEgroupEdBoard{atlas-GROUP-2020-XX-editorial-board@cern.ch}

% CERN preprintnumber
\PreprintIdNumber{CERN-EP-2020-XX}


==> template/EXOT/btagging_selection.tex <==
\subsection{Jet flavor tagging selection}

\begin{table}[ht]
  \caption{\btag selection criteria.}%
  \label{tab:object:btag}
  \centering
  % \resizebox{\textwidth}{!}{
  \begin{tabular}{ll}
    \toprule
    Feature & Criterion \\ 
    \midrule
    & EM Topo Jets / Track jets / VR jets \\
    \midrule
    Jet collection  & \texttt{AntiKt4EMTopo/AntiKt2PV0/AntiKtVR30Rmax4Rmin02} \\
    Jet selection   & \(\pT > \SI[parse-numbers=false]{XX}{\GeV}\) \\
    	            	& \(|\eta| < X\) \\				
                    & JVT cut if applicable \\
    \midrule
    Algorithm 		  & \texttt{MV2c10/MV2c10mu/MV2c10rnn/DL1/DL1mu/DL1rnn} \\
    \midrule
    Operating point & Hybrid /  Fixed \\
                    & Eff = 60 / 70 / 77 / 85 \\
    CDI             & \texttt{2017-21-13TeV-MC16-CDI-2017-12-22\_v1} \\
  \bottomrule
  \end{tabular}
  % }
\end{table}%


==> template/EXOT/egamma_selection.tex <==
\subsection{Electron selection}

\begin{table}[ht]
  \caption{Electron selection criteria.}%
  \label{tab:object:electron}
  \centering
  % \resizebox{\textwidth}{!}{
  \begin{tabular}{ll}
    \toprule
    Feature & \multicolumn{1}{c}{Criterion} \\
    \midrule
    Pseudorapidity range & \(|\eta| <\) X\\
    Energy calibration & \texttt{es2017\_R21\_PRE} (ESModel)\\
    Energy & \(E > \SI[parse-numbers=false]{XX}{\GeV}\) \\
    Transverse energy & \(\ET > \SI[parse-numbers=false]{XX}{\GeV}\) \\
    Transverse momentum & \(\pT > \SI[parse-numbers=false]{XX}{\GeV}\) \\
    \midrule
    \multirow{2}{*}{Object quality} & Not from a bad calorimeter cluster (\texttt{BADCLUSELECTRON})\\ %\cline{2-2}
      & Remove clusters from regions with EMEC bad HV (2016 data only) \\
    \midrule
    \multirow{2}{*}{Track to vertex association} & \(|d_{0}^{\text{BL}}(\sigma)| < X\) \\ %\cline{2-2}
    & \(|\Delta z_{0}^{\text{BL}} \sin{\theta}| < \SI[parse-numbers=false]{X}{\mm}\) \\
    \midrule
    Identification & (\texttt{Loose/Medium/Tight}) \\
    Isolation & \texttt{LooseTrackOnly / Loose / Tight / Gradient / \ldots} \\
      \bottomrule
  \end{tabular}
  % }
\end{table}

Notes:
\begin{itemize}
\item Pseudorapidity: when the calorimeter crack is not excluded, the range can be indicated simply as \enquote{\(|\eta| < 2.47\)}, when the crack is excluded: \enquote{\((|\eta| < 1.37) \quad || \quad (1.52 < |\eta| < 2.47)\)}.
\item Usually only one among \enquote{Energy}, \enquote{Transverse energy} and \enquote{Transverse momentum} criteria is applied --- the \SI{30}{\GeV} value is just an example.
  In special cases energy (i.e.\ calorimeter-based measurement) and momentum (i.e.\ tracking-based measurement) criteria can be required in order to constraint different aspects of the reconstruction.
\item Electron ID\@: 3 working points (Loose/Medium/Tight) are evaluated using the Likelihood-based (LH) method, by the
  \href{https://twiki.cern.ch/twiki/bin/view/AtlasProtected/EGammaIdentificationRun2}{ElectronPhotonSelectorTools}.
\item Energy calibration of electrons is implemented in the\\
  \href{https://twiki.cern.ch/twiki/bin/view/AtlasProtected/ElectronPhotonFourMomentumCorrection}{ElectronPhotonFourMomentumCorrection} tool.
\item Scale Factors for efficiencies for electrons are implemented in the\\
  \href{https://twiki.cern.ch/twiki/bin/view/AtlasProtected/XAODElectronEfficiencyCorrectionTool}{ElectronEfficiencyCorrection} tool.
\item Updated configurations for the EGamma CP tools can be found on this \href{https://twiki.cern.ch/twiki/bin/view/AtlasProtected/EGammaRecommendationsR21}{TWiki} page.
\end{itemize}

\newpage

\subsection{Photon selection}

\begin{table}[ht]
  \caption{Photon selection criteria.}%
  \label{tab:object:photon} 
  \centering
  % \resizebox{\textwidth}{!}{
  \begin{tabular}{ll}
    \toprule
    Feature & \multicolumn{1}{c}{Criterion} \\
    \midrule
    Pseudorapidity range & \(|\eta| <\) X\\
    Energy calibration & \texttt{es2017\_R21\_PRE} (ESModel)\\
    Energy & \(E > \SI[parse-numbers=false]{XX}{\GeV}\) \\
    Transverse energy & \(\ET > \SI[parse-numbers=false]{XX}{\GeV}\) \\
    \midrule
    \multirow{2}{*}{Object quality} & Not from a bad calorimeter cluster (\texttt{BADCLUSELECTRON})\\ %\cline{2-2}
      & Remove clusters from regions with EMEC bad HV (2016 data only) \\
    \midrule
    Photon cleaning & \texttt{passOQquality} \\
    Fudging & Applied for Full sim / not for AtlFastII \\
    \midrule
    Identification & (\texttt{Loose/Tight}) \\
    Isolation &  \texttt{FixedCutTightCaloOnly / FixedCutTight / FixedCutLoose} \\
    \bottomrule
  \end{tabular}
  %  }
\end{table}

Notes:
\begin{itemize}
\item Pseudorapidity: please note that the maximum value for \(|\eta|\) for photon candidates (2.37) is smaller than for electron candidates (2.47). 
  If crack excluded: \enquote{\((|\eta| < 1.37) \quad || \quad (1.52 < |\eta| < 2.37)\)}.
\item Usually only one between \enquote{Energy} and \enquote{Transverse energy} criteria is applied --- the \SI{30}{\GeV} value is just an example.
\item Photon cleaning: a new Photon helper is available to apply the photon cleaning cut 
  (from the \texttt{ElectronPhotonSelectorTools}, tag \(\ge\) 00-02-92-21, release \(\ge\) 2.4.30).
\item Photon ID\@: 2 working points (Loose/Tight) are evaluated using a cut-based method, by the
  \href{https://twiki.cern.ch/twiki/bin/view/AtlasProtected/EGammaIdentificationRun2}{ElectronPhotonSelectorTools}.
\item Energy calibration of photons is implemented in the\\
  \href{https://twiki.cern.ch/twiki/bin/view/AtlasProtected/ElectronPhotonFourMomentumCorrection}{ElectronPhotonFourMomentumCorrection} tool.
\item Scale Factors for efficiencies for photons are implemented in the\\
  \href{https://twiki.cern.ch/twiki/bin/view/AtlasProtected/XAODElectronEfficiencyCorrectionTool}{ElectronEfficiencyCorrection} tool.
\item Updated configurations for the EGamma CP tools can be found on this \href{https://twiki.cern.ch/twiki/bin/view/AtlasProtected/EGammaRecommendationsR21}{TWiki} page.
\end{itemize}


==> template/EXOT/event_cleaning.tex <==
\subsection{Event cleaning}
Following the \href{https://twiki.cern.ch/twiki/bin/viewauth/Atlas/DataPreparationCheckListForPhysicsAnalysis}{recommendations of the DataPrep group}, the following event-level requirements are made.

We use the official GRL\@:
 \begin{verbatim} FILL IN HERE \end{verbatim}
 
The following event-level vetos are made to reject bad / corrupt events:
 \begin{itemize}
  \item LAr noise burst and data corruption (\verb|xAOD::EventInfo::LAr|),
  \item Tile corrupted events (\verb|xAOD::EventInfo::Tile|),
  \item events affected by the SCT recovery procedure for single event upsets (\verb|xAOD::EventInfo::SCT|),
  \item incomplete events (\verb|xAOD::EventInfo::Core|).
 \end{itemize}
 
 Debug stream events [have/have not] been included.
 
 Checks [have/have not] been done to remove duplicate events.
 
Events are required to have a primary vertex with at least two associated tracks.
The primary vertex is selected as the one with the largest \(\Sigma \pT^2\),
where the sum is over all tracks with transverse momentum \(\pT > \SI{0.4}{\GeV}\) that are associated with the vertex.
 
 

==> template/EXOT/executive_summary.tex <==
\subsection{Target} 

\(\mathcal{O}\)(1 paragraph)
Is this a new analysis? If not, what are the main improvements expected with respect to the previous version?
What is the target publication date / conference?

\subsection{Context and Motivation} 

Motivate this analysis in 1 paragraph: why is this signature interesting? Which kind of models are you probing?

How is the analysis done is 1 paragraph: what are the main BG processes and how do you estimate them (are they MC- or data-driven,
what is the general idea of the control regions, \ldots), general characteristics of the PL fit (which distribution, binned?, \ldots)

\subsection{Milestones}

 Table giving a factual list of who is working on what and what else they do; the idea is to show how the team can / does progress. 
 Including dates for completion of these milestones will help further demonstrate that you are ready for the collaboration
 review, in the form of an editorial board.

%Example : 
The following table summarizes the tasks to be worked on by analysis team.
This is not a complete analysis outline but only an overview of the further steps to be taken as of the time of writing.
Details are not provided here but in the dedicated sections throughout this note.
Tasks which are based on established techniques and straightforward to achieve are marked green in the table.
Tasks which require new work are marked red.
Concerning the involved people, the responsible student supervisors and analysis coordinators are already mentioned in the list of contributions above,
which shall not be repeated here.
A fair overview of all single tasks including past work and of all relevant team members is only given in the list of contributions above!
It is also worth noting that some of the tasks listed below are being worked on in parallel. 

\begin{table}[ht]
  \caption{Milestones in the analysis.}%
  \label{tab:Miles_Ahead} 
  % \resizebox{\textwidth}{!}{
\begin{tabular}{llll} 
  \toprule
  \textbf{Task} & \textbf{Analyzer} & \textbf{Role} & \textbf{Other responsibilities} \\
  \midrule
  \multicolumn{4}{p{\textwidth}}{\textbf{Describe a first milestone.}} \\
  \midrule
  \textcolor{green}{A straightforward task}       & Name         & PhD student, PostDoc/Prof/\ldots & thesis writing \\
  &&& / teaching \\
  &&& / name some CP work \ldots \\ 
  \textcolor{red}{A more involved task}      &    &    &  \\ 
  \bottomrule
  
  \multicolumn{4}{l}{\textbf{Describe a second milestone}} \\
  \midrule
  First task \ldots      &          &  &  \\ 
  \bottomrule
\end{tabular}
%}
\end{table}




==> template/EXOT/jet_selection.tex <==
\subsection{Small-$R$ jet selection}

If you want to use variables such as \verb|\fcut| you need to add the option
\texttt{jetetmiss} to \texttt{atlaspackage}.

\begin{table}[ht]
  \caption{Jet reconstruction criteria.}%
  \label{tab:object:jet1}
  \centering
  % \resizebox{\textwidth}{!}{
  \begin{tabular}{ll}
  \toprule
  Feature & Criterion \\
  \midrule
  Algorithm & \Antikt  \\
  \(R\)-parameter & 0.4 \\
  Input constituent & EMTopo \\
  Analysis release number & 21.2.10 \\
  %Calibration tag & JetCalibTools-00-04-76 \\
  \texttt{CalibArea} tag & 00-04-81 \\
  Calibration configuration & \texttt{JES\_data2017\_2016\_2015\_Recommendation\_Feb2018\_rel21.config} \\
  Calibration sequence (Data) & \texttt{JetArea\_Residual\_EtaJES\_GSC\_Insitu} \\
  Calibration sequence (MC) & \texttt{JetArea\_Residual\_EtaJES\_GSC} \\
  %Calibration sequence (AFII) & \texttt{JetArea\_Residual\_EtaJES\_GSC} \\
  \midrule
  \multicolumn{2}{c}{Selection requirements} \\
  \midrule
  Observable & Requirement \\
  \midrule
  Jet cleaning & \texttt{LooseBad} \\
  BatMan cleaning & No \\
  \pT & \(> \SI[parse-numbers=false]{XX}{\GeV}\) \\
  \(|\eta|\) & \(< X\) \\
  JVT & (\emph{Update if needed}) \(>0.59\) for \(\pT < \SI{60}{\GeV}\), \(|\eta| < 0.4\)\\
  \bottomrule
  \end{tabular}
  % }
\end{table}


\clearpage
\subsection{Large-$R$ jet selection}

\begin{table}[ht]
  \caption{Large-\(R\) jet reconstruction criteria.}%
  \label{tab:object:jet2}
  \centering
  % \resizebox{\textwidth}{!}{
  \begin{tabular}{ll}
    \toprule
    Feature & Criterion \\ 
    \midrule
    Algorithm & \antikt  \\
    R-parameter & 1.0 \\
    Input constituent & \texttt{LCTopo} \\
    Grooming algorithm & Trimming \\ 
    \fcut & 0.05 \\
    \(R_{\text{trim}}\) & 0.2 \\
    Analysis release number & 21.2.10 \\
    %Calibration tag & JetCalibTools-00-04-76 \\
    \texttt{CalibArea} tag & 00-04-81 \\
    Calibration configuration & \texttt{JES\_MC16recommendation\_FatJet\_JMS\_comb\_19Jan2018.config} \\
    Calibration sequence (Data) & \texttt{EtaJES\_JMS\_Insitu} \\
    Calibration sequence (MC) & \texttt{EtaJES\_JMS} \\
    \bottomrule
    \multicolumn{2}{c}{Selection requirements} \\
    \midrule
    Observable & Requirement \\
    \midrule
    \pT  & \(> \SI[parse-numbers=false]{XX}{\GeV}\) \\
    \(|\eta|\) & \(< X\) \\
    Mass & \(> \SI[parse-numbers=false]{XX}{\GeV}\) \\
    \bottomrule
    \multicolumn{2}{c}{Boosted object tagger} \\
    \midrule
    Object  & Working point \\
    \midrule
    \(W\) / \(Z\) / top & 50\% / 80\% \\
    \(X\rightarrow bb\) & single/double \btag with/without loose/tight mass \\
    \bottomrule
  \end{tabular}
  % }
\end{table}


\subsection{\MET selection}

\begin{table}[ht]
  \caption{\MET reconstruction criteria.}%
  \label{tab:object:met}
  \centering
  \begin{tabular}{ll}
    \toprule
    Parameter & Value \\ 
    \midrule
    Algorithm & Calo-based \\
    Soft term & Track-based (TST) \\ 
    MET operating point & \texttt{Tight} \\
    Analysis release & 21.2.16 \\
    Calibration tag & \texttt{METUtilities-00-02-46} \\
    \bottomrule
    \multicolumn{2}{c}{Selection requirements} \\
    \midrule
    Observable & Requirement \\
    \midrule
    \MET & \(> \SI[parse-numbers=false]{XX}{\GeV}\) \\
    \(\sum{\ET} / \MET\)  & \(< X\) \\
    Object-based \MET significance & \(> X\) \\
    \bottomrule
  \end{tabular}
\end{table}




==> template/EXOT/muon_selection.tex <==
\subsection{Muon selection}

\begin{table}[ht]
  \caption{Muon selection criteria.}%
  \label{tab:object:muon}
  \centering
  % \resizebox{\textwidth}{!}{
  \begin{tabular}[ht]{ll}
    \toprule
    Feature & Criterion \\
    \midrule
    Selection working point & \texttt{Loose/Medium/Tight /High-pT} \\
    Isolation working point & \texttt{LooseTrackOnly/Loose/Tight/Gradient/\ldots}\\
    Momentum calibration & Sagitta correction [used/not used] \\
    \pT Cut & \SI[parse-numbers=false]{X}{\GeV} \\
    \(|\eta|\) cut & \(< X\) \\
    \dzero significance cut & X \\
    \(z_{0}\) cut & \SI[parse-numbers=false]{X}{\mm} \\
    \bottomrule
  \end{tabular}
  % }
\end{table}

The selection criteria are implemented in the \texttt{MuonSelectorTools-XX-XX-XX}\\
with \texttt{MuonMomentumCorrections-XX-XX-XX}, 
isolation in \texttt{IsolationSelection-XX-XX-XX} and \dzero and \(z_{0}\) cuts in \texttt{xAODTracking-XX-XX-XX}.
The muon recommendations can be found in 
\href{https://twiki.cern.ch/twiki/bin/view/AtlasProtected/MCPAnalysisGuidelinesMC16}{MCPAnalysisGuidelinesMC16}.


==> template/EXOT/overlap_removal.tex <==
\subsection{Overlap removal}

The reconstruction of the same energy deposits as multiple objects is resolved using the standard overlap removal tools, \texttt{AssociationUtils}, documented \href{https://gitlab.cern.ch/atlas/athena/blob/21.2/PhysicsAnalysis/AnalysisCommon/AssociationUtils/README.rst}{here}

The (Standard/Heavy-flavor/Boosted/Boosted+Heavy-flavor/lepton-favored) working point is used corresponding to:

\begin{table}[ht]
  % \resizebox{\textwidth}{!}{
  \begin{tabular}{lll}
    \toprule
    Reject & Against & Criteria \\
    \midrule
    Electron & Electron & shared track, \(\pTX[][1] < \pTX[][2]\) \\
    Tau      & Electron & \(\Delta R <\) 0.2 \\
    Tau      & Muon     & \(\Delta R <\) 0.2 \\
    Muon     & Electron & is Calo-Muon and shared ID track \\
    Electron & Muon     & shared ID track \\
    Photon   & Electron & \(\Delta R < 0.4\) \\
    Photon   & Muon     & \(\Delta R < 0.4\) \\
    Jet      & Electron & [\(\Delta R < 0.2\) / Not a \bjet and \(\Delta R <\) 0.2] \\
    Electron & Jet      & [\(\Delta R < 0.4\) / \(\Delta R < \min(0.4, 0.04 + \SI{10}{\GeV}/\pT(e))\)/None] \\
    Jet      & Muon     & [\(\texttt{NumTrack} < 3\) and (ghost-associated or \(\Delta R < 0.2\)) / \\
                       && not a \bjet and \(\texttt{NumTrack} < 3\) and (ghost-associated or \(\Delta R < 0.2\))] \\
    Muon     & Jet      & [\(\Delta R < 0.4\) / \(\Delta R < \min(0.4, 0.04 + \SI{10}{\GeV}/\pT(\mu))\)/None] \\
    Jet      & Tau      & \(\Delta R < 0.2\) \\
    Photon   & Jet      & \(\Delta R < 0.4\) \\
    Fat-jet  & Electron & \(\Delta R < 1.0\) \\
    Jet      & Fat-jet  & \(\Delta R < 1.0\) \\
    \bottomrule
  \end{tabular}
  % }
\end{table}

\(\Delta R\) is calculated using rapidity by default.




==> template/EXOT/systematics.tex <==
Systematic uncertainties arise from the reconstruction of the various physics objects and 
from theoretical and/or modelling uncertainties affecting the predictions for both the backgrounds and signals. 
These uncertainties manifest themselves as uncertainties both in the overall yield and 
shape of the final observable.

\subsection{Experimental}

A summary of the experimental systematic uncertainties taken into account in this analysis is given in
Table~\ref{tab:syst_summary_sources}, along with the shorthand name of the uncertainty used throughout 
the analysis. 

\textit{Include also subsections for each of the individual descriptions of the uncertainty groups and the
source where they come from.  If the recommendation is not available at this time, state that in the section.}

\begin{table}[h]
	\centering
	\scriptsize
	\begin{center}
		\begin{tabular}{ll}
			\toprule \midrule
			Systematic uncertainty        & Short description                                                                          \\ \midrule
			\multicolumn{2}{c}{\textbf{Event}}  \\ \midrule
			Luminosity  & uncertainty on the total integrated luminosity  \\ \midrule
			\multicolumn{2}{c}{\textbf{Electrons}}  \\ \midrule
			EL\_EFF\_Trigger\_TOTAL\_1NPCOR\_PLUS\_UNCOR   & trigger efficiency uncertainty    \\
			EL\_EFF\_Reco\_TOTAL\_1NPCOR\_PLUS\_UNCOR    & reconstruction efficiency uncertainty          \\ 
			EL\_EFF\_ID\_TOTAL\_1NPCOR\_PLUS\_UNCOR    & ID efficiency uncertainty               \\ 
			EL\_EFF\_Iso\_TOTAL\_1NPCOR\_PLUS\_UNCOR    & isolation efficiency uncertainty       \\
			EG\_SCALE\_ALL & energy scale uncertainty  \\ 
			EG\_RESOLUTION\_ALL & energy resolution uncertainty  \\ \midrule
			\multicolumn{2}{c}{\textbf{Muons}}  \\ \midrule
			mu20\_iloose\_L1MU15\_OR\_HLT\_mu40\_MUON\_EFF\_Trig   & \multirow{ 2}{*}{trigger efficiency uncertainties (2 muon selection)}       \\ 
			mu24\_ivarmed\_OR\_HLT\_mu40\_MU\_EFF\_TrigStat        &         \\ 
			mu24\_ivarmed\_OR\_HLT\_mu50\_MU\_EFF\_TrigStat        &         \\ 
			mu26\_ivarmed\_OR\_HLT\_mu50\_MU\_EFF\_TrigStat        &         \\ 
			MUON\_EFF\_RECO\_STAT        & \multirow{ 2}{*}{reconstruction uncertainty for \pt > 15 GeV}        \\ % todo: guess that includes the ID uncertainty? PR.
			MUON\_EFF\_RECO\_SYS        &        \\ 
			MUON\_EFF\_RECO\_STAT\_LOWPT        & \multirow{ 2}{*}{reconstruction and ID efficiency uncertainty for \pt < 15 GeV}        \\ 
			MUON\_EFF\_RECO\_SYS \_LOWPT       &        \\ 
			MUON\_ISO\_STAT        & \multirow{ 2}{*}{isolation efficiency uncertainty}        \\ 
			MUON\_ISO\_SYS        &        \\ 
			MUON\_TTVA\_STAT        & \multirow{ 2}{*}{track-to-vertex association efficiency uncertainty}        \\ 
			MUON\_TTVA\_SYS        &        \\ 
			MUONS\_SCALE        & energy scale uncertainty                                                           \\ 
			MUONS\_SAGITTA\_RHO        & variations in the scale of the momentum (charge dependent)                  \\ 
			MUONS\_SAGITTA\_RESBIAS        & variations in the scale of the momentum (charge dependent)              \\ 
			MUONS\_ID        & energy resolution uncertainty from inner detector                              \\ 
			MUONS\_MS & energy resolution uncertainty from muon system  \\ \midrule
			\multicolumn{2}{c}{\textbf{Small-R Jets}}  \\ \midrule
			JET\_GroupedNP  & energy scale uncertainty split into 3 components              \\ 
			JET\_SR1\_JET\_EtaIntercalibration\_NonClosure & non-closure in the jet response at $2.4<|\eta|<2.5$   \\
			JET\_SR1\_JER\_SINGLE\_NP  & energy resolution uncertainty  \\
			JvtEfficiency & JVT efficiency uncertainty  \\
			%
			%
			% todo: decide on b-tagging EV prescription. So far we only have the simplest prescription, but we should switch.
			%
			%
			FT\_EFF\_EIGEN\_B & $b$-tagging efficiency uncertainties ("BTAG\_MEDIUM):   \\
			FT\_EFF\_EIGEN\_C & \\ % \multirow{2}{*}{3 components for $b$-jets, 4 for $c$-jets and 5 for light jets} \\
			FT\_EFF\_EIGEN\_L &   \\ 
			FT\_EFF\_EIGEN\_extrapolation &  $b$-tagging efficiency uncertainty on the extrapolation on high \pt-jets  \\ 
			FT\_EFF\_EIGEN\_extrapolation\_from\_charm & $b$-tagging efficiency uncertainty on $\tau$-jets   \\ \midrule
			\multicolumn{2}{c}{\textbf{Large-R Jets}}  \\ \midrule
			%
			%
			%
			FATJET\_JMR   & mass resolution uncertainty                                                                 \\ 
			FATJET\_JER    & energy resolution uncertainty                                                               \\ 
			JET\_Comb\_Baseline\_Kin &  \multirow{4}{*}{energy scale uncertainties (\pt and mass scales fully correlated)}  \\
			JET\_Comb\_Modelling\_Kin &  \\
			JET\_Comb\_TotalStat\_Kin &  \\
			JET\_Comb\_Tracking\_Kin   &  \\ 
			\midrule % TODO: which uncertainties do we need for large-R jets?
			% calo mass 
			%JET\_Medium\_JET\_Rtrk\_Baseline\_Kin &  \multirow{4}{*}{energy scale uncertainties (\pt and mass scales fully correlated)}  \\
			%JET\_Medium\_JET\_Rtrk\_Modelling\_Kin &  \\
			%JET\_Medium\_JET\_Rtrk\_TotalStat\_Kin &  \\
			%JET\_Medium\_JET\_Rtrk\_Tracking\_Kin   &  \\ \midrule
			%
			%
			% todo: decide on b-tagging EV prescription also for track jets. So far we only have the simplest prescription, but we should switch.
			%
			%
			\multicolumn{2}{c}{\textbf{Track-Jets}}  \\ \midrule
			FT\_EFF\_EIGEN\_B & $b$-tagging efficiency uncertainties ("BTAG\_MEDIUM):   \\
			FT\_EFF\_EIGEN\_C & \\ % \multirow{2}{*}{3 components for $b$-jets, 4 for $c$-jets and 5 for light jets} \\
			FT\_EFF\_EIGEN\_L &   \\ 
			FT\_EFF\_EIGEN\_extrapolation &  $b$-tagging efficiency uncertainty on the extrapolation on high \pt-jets  \\ 
			FT\_EFF\_EIGEN\_extrapolation\_from\_charm & $b$-tagging efficiency uncertainty on $\tau$-jets   \\ \midrule
			\multicolumn{2}{c}{\textbf{\MET-Trigger and \MET-Terms}}  \\ \midrule
			METTrigStat    & \multirow{2}{*}{trigger efficiency uncertainty} -  \\
			METTrigSyst &    \\
			MET\_SoftTrk\_ResoPerp           & track-based soft term related to transversal resolution uncertainty                  \\ 
			MET\_SoftTrk\_ResoPara           & track-based soft term related to longitudinal resolution uncertainty                  \\ 
			MET\_SoftTrk\_Scale                  & track-based soft term related to longitudinal scale uncertainty                          \\ 
			MET\_JetTrk\_Scale                   & track MET scale uncertainty due to tracks in jets                                            \\ \midrule
			PRW\_DATASF         & uncertainty on data SF used for the computation of pileup reweighting      \\
			
			\bottomrule
		\end{tabular}
	\end{center}
	\caption{ Qualitative summary of the experimental systematic uncertainties considered in this analysis.}
	\label{tab:syst_summary_sources}
\end{table}


\subsection{Theory/Modelling}

\textit{Modelling uncertainties can be analysis specific in the case of the background.  However, you should 
have a clear idea for your analysis how you will estimate these uncertainties.  If you are doing 
an MC-based background estimation, describe the sources of these uncertainties and the comparisons that
you will make.  If you are doing a data driven estimation, describe the sources.}

\textit{For signal yield uncertainties, these uncertainties are evaluated in a standard way and should 
include PDF variations and renormalization/factorization scale variations.  There is more information
provided on the PMG TWiki pages for this.}


\clearpage


==> template/EXOT/tau_selection.tex <==
\subsection{Tau selection}

\begin{table}[ht]
  \caption{Tau selection criteria.}%
  \label{tab:object:tau}
  \centering
  % \resizebox{\textwidth}{!}{
  \begin{tabular}{ll}
  \toprule
  Feature & Criterion \\
  \midrule
  Pseudorapidity range & \(|\eta| < X\) \\
  Track selection & 1 or 3 tracks \\\
  Charge & \(|Q| = 1\) \\
  Tau energy scale & \texttt{MVA TES}\\
  Transverse momentum & \(\pT > \SI[parse-numbers=false]{XX}{\GeV}\) \\
  Jet rejection & BDT-based (\texttt{Loose/Medium/Tight}) \\
  Electron rejection & BDT-based\\
  Muon rejection & Via overlap removal in \(\Delta R < 0.2\) and \(\pT > \SI{2}{\GeV}\).
    Muons must not be Calo-tagged\\
  \bottomrule
  \end{tabular}
  % }
\end{table}

If the crack is excluded: \((|\eta| < 1.37) || (1.52 < |\eta| < 2.5)\)

The selection criteria are all implemented in the \texttt{TauSelectionTool} as part of the \texttt{TauAnalysisTools}.
Documentation can be found in the \href{https://gitlab.cern.ch/atlas/athena/blob/21.2/PhysicsAnalysis/TauID/TauAnalysisTools/doc/README-TauSelectionTool.rst}{README-TauSelectionTool.rst}.


==> template/EXOT/tracks_selection.tex <==
\subsection{Track selection}

If you use tracks as particular objects on which you cut in your analysis.

\begin{table}[ht]
  \caption{\texttt{TrackParticle} object selection criteria.}%
  \label{tab:object:track}
  \centering
  % \resizebox{\textwidth}{!}{
  \begin{tabular}{ll}
    \toprule
    Tracking algorithm								    & Primary / Large Radius Tracking / Custom \\
    Track quality selection (official)    & \texttt{Loose/Tight} \\
    \pT                                   & \(> \SI[parse-numbers=false]{XX}{\GeV}\) \\
    \(|\eta|\)                            & \(< X\) \\
    Track-vertex association criteria     & \texttt{Loose/Tight} \\
    Track-to-tet association method       & Ghost Matched / \(\Delta R\) \\
    \bottomrule
  \end{tabular}
  % }
\end{table}


==> template/MC_snippets/BJ.tex <==
% !TEX root = MC_snippets.tex

\chapter{Single-boson processes}
%\label{sec:VJ}

In the following paragraphs, the set-up of the current ATLAS single-boson baseline samples is described.
Details of the full process configuration are given in the PUB note~\cite{ATL-PHYS-PUB-2017-006}. In the case of \SHERPA samples,
a minimal description of built-in systematic uncertainties is also given.

%In addition, \SHERPA[2.1.1] is still used for cross checks and in the evaluation of theoretical uncertainties.
%Samples using this version have been generated with the \CT[10nlo] set of PDFs~\cite{Lai:2010vv}, in conjunction
%with the dedicated set of tuned parton-shower parameters developed by the \SHERPA authors for this generator version.

\section[Sherpa MEPS@NLO]{\SHERPA (\MEPSatNLO)}
%\label{sec:vjets-sherpa}

\subsection{QCD \(V+\)jets}
%\label{sec:vjets-sherpa-vjets}

\subsection*{Samples}
%\label{sec:vjets-sherpa-samples}

The descriptions below correspond to the samples in \cref{tab:vjets-sherpa}.

\begin{table}[!htbp]
  \caption{\(V\)+jets samples with \SHERPA.}%
  \label{tab:vjets-sherpa}
  \centering
  \begin{tabular}{l l}
    \toprule
    DSID range & Description \\
    \midrule
    364100--364113    & \(Z\to\mu\mu\)   \\
    364198--364203    & \(Z\to \mu\mu\) (\(\SI{10}{\GeV} < m_{\ell\ell} < \SI{40}{\GeV}\)) \\
    364359, 364362, 364281  &  \(Z\to\mu\mu\) (very low mass)   \\
    364114--364127    & \(Z\to ee\)    \\
    364204--364209    & \(Z\to ee\) (\(\SI{10}{\GeV} < m_{\ell\ell} < \SI{40}{\GeV}\)) \\
    364358, 364361, 364282 & \(Z\to ee\) (very low mass) \\
    364128--364141    & \(Z\to \tau\tau\)    \\
    364210--364215    & \(Z\to \tau\tau\) (\(\SI{10}{\GeV} < m_{\ell\ell} < \SI{40}{\GeV}\)) \\
    364282, 364360, 364363 &  \(Z\to \tau\tau\) \\
    364142--364155    & \(Z\to \nu\nu\)   \\
    364156--364169    & \(W\to \mu\nu\)   \\
    364170--364183    & \(W\to e\nu\)    \\
    364184--364197    & \(W\to \tau\nu\)  \\
    364216--364229    & \(Z\to\ell\ell,W\to\ell\nu\) (high \pT)\\
    \bottomrule
  \end{tabular}
\end{table}

\paragraph{Short description:}

The production of \(V+\)jets was simulated with the
\SHERPA[2.2.1]~\cite{Bothmann:2019yzt}
generator using next-to-leading-order (NLO) matrix elements (ME) for up to two partons, and leading-order (LO) matrix elements
for up to four partons calculated with the Comix~\cite{Gleisberg:2008fv}
and \OPENLOOPS~\cite{Buccioni:2019sur,Cascioli:2011va,Denner:2016kdg} libraries. They
were matched with the \SHERPA parton shower~\cite{Schumann:2007mg} using the \MEPSatNLO
prescription~\cite{Hoeche:2011fd,Hoeche:2012yf,Catani:2001cc,Hoeche:2009rj}
using the set of tuned parameters developed by the \SHERPA authors.
The \NNPDF[3.0nnlo] set of PDFs~\cite{Ball:2014uwa} was used and the samples
were normalised to a next-to-next-to-leading-order (NNLO)
prediction~\cite{Anastasiou:2003ds}.


\paragraph{Long description:}

The production of \(V+\)jets was simulated with the \SHERPA[2.2.1]~\cite{Bothmann:2019yzt}
generator. In this set-up, NLO-accurate matrix elements for up to two partons, and LO-accurate matrix elements for up
to four partons were calculated with the Comix~\cite{Gleisberg:2008fv} and
\OPENLOOPS~\cite{Buccioni:2019sur,Cascioli:2011va,Denner:2016kdg} libraries.
The default \SHERPA parton shower~\cite{Schumann:2007mg} based on
Catani--Seymour dipole factorisation and the cluster hadronisation model~\cite{Winter:2003tt}
were used. They employed the dedicated set of tuned parameters developed by the
\SHERPA authors and the \NNPDF[3.0nnlo] PDF set~\cite{Ball:2014uwa}.

The NLO matrix elements for a given jet multiplicity were matched to the parton
shower (PS) using a colour-exact variant of the MC@NLO
algorithm~\cite{Hoeche:2011fd}. Different jet multiplicities were then merged
into an inclusive sample using an improved CKKW matching
procedure~\cite{Catani:2001cc,Hoeche:2009rj} which was extended to NLO
accuracy using the \MEPSatNLO prescription~\cite{Hoeche:2012yf}. The merging threshold
was set to \SI{20}{\GeV}.

\input{sherpa_scale_pdf.tex}

The \(V\)+jets samples were normalised to a next-to-next-to-leading-order (NNLO)
prediction~\cite{Anastasiou:2003ds}.


\subsection{Electroweak \(Vjj\) (VBF)}
%\label{sec:vjets-sherpa-vjj}

The descriptions below correspond to the samples in
\cref{tab:ewkvjets-sherpa}.  Samples include the VBF and \(V\)-strahlung diagrams, but
they do not include semileptonic \(VV\) diagrams and do not overlap with QCD \(V+\)jets samples.

\begin{table}[!htbp]
  \caption{Electroweak \(Vjj\) samples with \SHERPA.}%
  \label{tab:ewkvjets-sherpa}
  \centering
  \begin{tabular}{l l}
    \toprule
    DSID range & Description \\
    \midrule
    308092--308096 & EWK \(Vjj\) \\
    \bottomrule
  \end{tabular}
\end{table}

\paragraph{Description:}

Electroweak production of \(\ell\ell jj\), \(\ell\nu jj\) and \(\nu\nu jj\) final states
was simulated with \SHERPA[2.2.1]~\cite{Bothmann:2019yzt} using
leading-order (LO) matrix elements with up to two additional parton emissions.
The matrix elements were merged with the \SHERPA parton
shower~\cite{Schumann:2007mg} following the \MEPSatLO
prescription~\cite{Catani:2001cc} and using the set of tuned
parameters developed by the \SHERPA authors.  The \NNPDF[3.0nnlo] set of
PDFs~\cite{Ball:2014uwa} was employed. The samples were produced
using the VBF approximation, which avoids overlap  with semileptonic
diboson topologies by requiring a \(t\)-channel colour-singlet exchange.

%These samples are generated in the \(G_\mu\) scheme using, ensuring an
%optimal description of pure electroweak interactions at the
%electroweak scale.


\section[MadGraph5 (CKKW-L)]{\MADGRAPH (CKKW-L)}
%\label{sec:vjets-mg5py8_ckkwl}

\subsection*{Samples}
%\label{sec:vjets-mg5py8_ckkwl-samples}

The descriptions below correspond to the samples in
\cref{tab:vjets-mg5py8_ckkwl}. The set-ups of \(N_\text{parton}\)- and
\HT-sliced samples differ slightly between the two slicing schemes
with regard to the matrix element PDF, the jet-clustering radius parameter
and the scale used in the evaluation of  \alphas to determine the weight of
each splitting. The short description merges the two set-ups and requires
the paper editors to select the appropriate PDF set (or gracefully describe
both); the long description is left unmerged.

\begin{table}[!htbp]
  \caption{\(V\)+jets samples with \MGPY[8] using CKKW-L merging.}%
  \label{tab:vjets-mg5py8_ckkwl}
  \centering
  \begin{tabular}{l l}
    \toprule
    DSID range & Description \\
    \midrule
    363123--363146 & \HT-sliced \(Z\to\mu\mu\)   \\
    363147--363170 & \HT-sliced \(Z\to ee\)     \\
    361510--361514 & \(N_\text{parton}\)-sliced \(Z\to\tau\tau\) \\
    361515--361519 & \(N_\text{parton}\)-sliced \(Z\to\nu\nu\)   \\
    363624--363647 & \HT-sliced \(W\to \mu\nu\)   \\
    363600--363623 & \HT-sliced \(W\to e\nu\)    \\
    363648--363671 & \HT-sliced \(W\to\tau\nu\)  \\
    \bottomrule
  \end{tabular}
\end{table}

\paragraph{Short description for \HT-sliced and \(N_\text{parton}\)-sliced \(V\)+jets:}

QCD \(V\)+jets production was simulated with \MGNLO[2.2.2]~\cite{Alwall:2014hca},
using LO-accurate matrix elements (ME) with up to four final-state partons.
The ME calculation employed the \NNPDF[3.0nlo] set of PDFs~\cite{Ball:2014uwa}
(\HT-sliced) / \NNPDF[2.3lo] set of PDFs~\cite{Ball:2012cx} (\(N_\text{parton}\)-sliced).
Events were interfaced to \PYTHIA[8.186]~\cite{Sjostrand:2007gs} for the modelling
of the parton shower, hadronisation, and  underlying event. The overlap between
matrix element and parton shower emissions was removed using the CKKW-L
merging procedure~\cite{Lonnblad:2001iq,Lonnblad:2011xx}. The A14
tune~\cite{ATL-PHYS-PUB-2014-021} of \PYTHIA[8] was used with the
\NNPDF[2.3lo] PDF set~\cite{Ball:2012cx}.
The decays of bottom and charm
hadrons were performed by \EVTGEN[1.2.0]~\cite{Lange:2001uf}.
The \(V\)+jets samples were normalised to a next-to-next-to-leading-order (NNLO)
prediction~\cite{Anastasiou:2003ds}.


\paragraph{\HT-sliced long description:}

QCD \(V\)+jets production was simulated with LO-accurate matrix elements (ME)
for up to four partons with \MGNLO[2.2.2]~\cite{Alwall:2014hca}. The ME calculation was interfaced with
\PYTHIA[8.186]~\cite{Sjostrand:2007gs} for the modelling of the parton
shower, hadronisation, and underlying event. To remove overlap between the matrix
element and the parton shower the CKKW-L merging
procedure~\cite{Lonnblad:2001iq,Lonnblad:2011xx} was applied with a
merging scale of \SI{30}{\GeV} and a jet-clustering radius parameter of
\(0.2\). In order to better model the region of large jet \pT, the
strong coupling constant \alphas was evaluated at the scale of each splitting to
determine the weight. The matrix element calculation was performed with
the \NNPDF[3.0nlo] PDF set~\cite{Ball:2014uwa} with \(\alphas= 0.118\). The calculation was done
in the five-flavour number scheme with massless \(b\)- and
\(c\)-quarks. Quark masses were reinstated in the \PYTHIA[8] parton shower.
The renormalisation and factorisation scales were set to the \MADGRAPH default
values, based on a clustering of the event. The A14
tune~\cite{ATL-PHYS-PUB-2014-021} of \PYTHIA[8] was used with the
\NNPDF[2.3lo] PDF set~\cite{Ball:2012cx} with \(\alphas=0.13\).
The decays of bottom and charm hadrons were performed by \EVTGEN[1.2.0]~\cite{Lange:2001uf}.


\paragraph{\(N_\text{parton}\)-sliced long description:}

QCD \(V\)+jets production was simulated with LO-accurate matrix elements (ME) for up to four partons with
\MGNLO[2.2.2]~\cite{Alwall:2014hca}. The ME calculation was interfaced
with \PYTHIA[8.186]~\cite{Sjostrand:2007gs} for the modelling of the parton
shower and underlying event. To remove overlap between the matrix
element and the parton shower the CKKW-L merging
procedure~\cite{Lonnblad:2001iq,Lonnblad:2011xx} was applied with a
merging scale of \SI{30}{\GeV} and a jet-clustering radius parameter of
\(0.4\). In order to better model the region of large jet \pT, the
strong coupling constant \alphas was evaluated at the scale of each splitting to
determine the weight. The matrix element calculation was performed with
the \NNPDF[2.3lo] PDF set~\cite{Ball:2012cx} with \(\alphas= 0.13\). The calculation was done
in the five-flavour number scheme with massless \(b\)- and
\(c\)-quarks. Quark masses were reinstated in the \PYTHIA[8] parton shower.
The renormalisation and factorisation scales were set to the \MADGRAPH default
values, based on a clustering of the event. The A14 tune~\cite{ATL-PHYS-PUB-2014-021}
of \PYTHIA[8] was used with the \NNPDF[2.3lo] PDF set~\cite{Ball:2012cx} with \(\alphas=0.13\).
The decays of bottom and charm hadrons were performed by \EVTGEN[1.2.0]~\cite{Lange:2001uf}.

% No usable aMC@NLO \FXFX samples exist in ATLAS central production, therefore
% the description is commented out to avoid confusion

%% \section{\MGNLO (\FXFX)}
%% \label{sec:vjets-mg5-fxfx}

%% \begin{table}[!htbp]
%% \caption{Samples with \MGNLOPYTHIA[8] using CKKW-L merging.}%
%% \label{tab:mg5-fxfx}
%% \centering
%% \begin{tabular}{l l}
%% \toprule
%% DSID range & Description \\
%% \midrule
%% 999999-888888 & V+jets HT-sliced\\
%% \bottomrule
%% \end{tabular}
%% \end{center}
%% \end{table}

%% Samples have also been generated using the \MGNLO program to
%% generate matrix elements for \(V\) + 0, 1 and 2 partons at NLO accuracy.
%% The showering and subsequent hadronisation has been performed using \PYTHIA[8.210] with the A14 tune, using the \NNPDF[2.3lo]
%% PDF set with \(\alphas = 0.13\).
%% The different jet multiplicities are merged using the
%% \FXFX prescription~\cite{Frederix:2012ps} implemented in the \MGNLO program
%% (version 2.3.3 is used here).

%% \MGNLO performs a 5FNS calculation with massless \(b\)- and \(c\)-quarks in the matrix element, and massive quarks in the
%% \PYTHIA shower.
%% The PDF input set in use for event generation is \NNPDF[2.3nlo] PDF set with \(\alphas = 0.119\)
%% and the samples have been generated with additional weights for the PDF replicas as well as scale variations of
%% the renormalisation and the factorisation scales~\cite{Frederix:2011ss}.

%% The impact of various merging scales (\muQ) has been studied,
%% analysing three different values: \SI{20}{\GeV} (down variation), \SI{25}{\GeV} (nominal value) and \SI{50}{\GeV} (up variation).
%% At the event-generation level, the minimum jet transverse momentum, \(\pT^j\) is required to be at least
%% \SI{8}{\GeV} with no restriction on the absolute value of the jet pseudorapidity (jet \(|\eta|\)).
%% %The cut on the \(\pT^j\) should be at least half the value used for the merging scale,
%% %in order to not introduce any bias in the MC generation.
%% The samples have been generated using LHAPDF-6.1.5~\cite{Butterworth:2014efa} and FastJet-3.1.0~\cite{Cacciari:2006sm}.


\section[Inclusive Powheg \(V\)]{Inclusive \POWHEG \(V\)}
%\label{sec:v-powheg}

The descriptions below correspond to the samples in \cref{tab:v-powheg}.

\begin{table}[!htbp]
  \caption{Inclusive \(V\) samples with \POWHEG.}%
  \label{tab:v-powheg}
  \centering
  \begin{tabular}{l l}
    \toprule
    DSID range & Description \\
    \midrule
    361100--361108    & \(W^+,W^-,Z/\gamma^\ast\) with \(e,\mu,\tau\) decays\\
    301000--301178, 344722    & high-mass slices: \(W^+,W^-,Z\) with \(e,\mu,\tau\) decays \\
    361664--361669 & \(Z/\gamma^\ast\) low-mass slices (\(m=6\)--10--60\,\si{\GeV})\\
    426335--426336 & \(Z/\gamma^\ast\) high-\(\pTX[][\ell\ell] > \SI{150}{\GeV}\) slices \\
    \bottomrule
  \end{tabular}
\end{table}

\paragraph{Description:}

The \POWHEGBOX[v1] MC generator~\cite{Nason:2004rx,Frixione:2007vw,Alioli:2010xd,Alioli:2008gx}
was used for the simulation at NLO accuracy of the hard-scattering processes of \(W\)
and \(Z\) boson production and decay in the electron, muon, and \(\tau\)-lepton
channels. It was interfaced to \PYTHIA[8.186]~\cite{Sjostrand:2007gs}
for the modelling of the parton shower, hadronisation, and underlying
event, with parameters set according to the \AZNLO
tune~\cite{STDM-2012-23}. The \CT[10nlo] PDF set~\cite{Lai:2010vv} was used
for the hard-scattering processes, whereas the \CTEQ[6L1] PDF
set~\cite{Pumplin:2002vw} was used for the parton shower. The effect of
QED final-state radiation was simulated with \PHOTOSpp[3.52]~\cite{Golonka:2005pn,Davidson:2010ew}.
The \EVTGEN[1.2.0] program~\cite{Lange:2001uf} was used to decay bottom and charm hadrons.

% No usable \POWHEG \MINLO samples exist in ATLAS central production, therefore
% the description is commented out to avoid confusion

%% \section{\POWHEG \MINLO}
%% \label{sec:vjets-minlo}

%% Predictions from \POWHEG \MINLO~\cite{Alioli:2010xd,Hamilton:2012np,Hamilton:2012rf}
%% interfaced to \PYTHIA[8.210]~\cite{Sjostrand:2007gs} with the
%% AZNLO tune~\cite{STDM-2012-23} are obtained to produce
%% \(V\)+jets events, and will be referred to in the remainder of the note
%% as \POWHEG \MINLO+\PYTHIA[8]. The \EVTGEN[1.2.0] program~\cite{Lange:2001uf}
%% is used as an afterburner to better simulate the decays of bottom and charm hadrons.
%% The \PHOTOSpp[3.61] program~\cite{Golonka:2005pn,Davidson:2010ew} is interfaced to \PYTHIA to accurately
%% describe the QED final state radiation, and the emission of lepton pairs is activated in this setup.
%% The PDF set used in \POWHEG is \CT[14nnlo]~\cite{Dulat:2015mca} whereas the PDF set used in the parton shower
%% is the \CTEQ[6L1]~\cite{Pumplin:2002vw} leading order set.

%% \POWHEG \MINLO is an improvement of the CKKW matching procedure to reach NLO accuracy for
%% boson production in association one jet, and smoothly
%% merges to NLO single boson production at low boson \pT, using no external merging scale.
%% NLO contributions from the CKKW Sudakov form factors are subtracted to the virtual corrections provided by \POWHEGBOX.
%% Thanks to the optimal scale and to the Sudakov form factors, the
%% \POWHEG \MINLO samples do not need any Born suppression cut, and their cross-sections are well-behaved at small boson \pT,
%% contrary to fixed order predictions that diverge in this kinematic phase space.


==> template/MC_snippets/GJ.tex <==
\chapter{Photon processes}
%\label{sec:GJ}

The following paragraphs describe the set-up of the current ATLAS \(\gamma\)+jets and \(\gamma\gamma\)+jets baseline samples.

\section[Sherpa (MEPS@NLO)]{\SHERPA (\MEPSatNLO)}
%\label{sec:gammajets-sherpa-nlo}

\subsection*{Samples}
%\label{sec:gammajets-sherpa-nlo-samples}

The descriptions below correspond to the samples in \cref{tab:gammajets-sherpa-nlo}.

\begin{table}[!htbp]
  \caption{\(\gamma\)+jets and \(\gamma\gamma\)+jets samples with \SHERPA NLO\@.}%
  \label{tab:gammajets-sherpa-nlo}
  \centering
  \begin{tabular}{l l}
    \toprule
    DSID range & Description \\
    \midrule
    364541--364547 & single photon \\
    364350--364354 & diphoton  \\
    \bottomrule
  \end{tabular}
\end{table}


%same description as in~\cref{sec:vjets-sherpa-vjets}
\subsection{\(\gamma\)+jets}
%\label{sec:gammajets-sherpa-nlo-singlephoton}

\paragraph{Short description:}

Prompt single-photon production was simulated with the
\SHERPA[2.2]~\cite{Bothmann:2019yzt} generator. In this set-up, NLO-accurate
matrix elements for up to two partons, and LO-accurate matrix elements for up
to four partons were calculated with the Comix~\cite{Gleisberg:2008fv} and
\OPENLOOPS~\cite{Buccioni:2019sur,Cascioli:2011va,Denner:2016kdg} libraries. They were matched
with the \SHERPA parton shower~\cite{Schumann:2007mg} using the \MEPSatNLO
prescription~\cite{Hoeche:2011fd,Hoeche:2012yf,Catani:2001cc,Hoeche:2009rj}
with a dynamic merging cut~\cite{Siegert:2016bre} of \SI{20}{\GeV}.
Photons were required to be isolated according to
a smooth-cone isolation criterion~\cite{Frixione:1998jh}. Samples were generated using the
\NNPDF[3.0nnlo] PDF set~\cite{Ball:2014uwa}, along with the dedicated set of
tuned parton-shower parameters developed by the \SHERPA authors.


\paragraph{Long description:}

Prompt single-photon production was simulated with the
\SHERPA[2.2]~\cite{Bothmann:2019yzt} parton shower Monte Carlo
generator. In this set-up, NLO-accurate
matrix elements for up to two partons, and LO-accurate matrix elements for up
to four partons were calculated with the Comix~\cite{Gleisberg:2008fv} and
\OPENLOOPS~\cite{Buccioni:2019sur,Cascioli:2011va,Denner:2016kdg} libraries.
The default \SHERPA parton shower~\cite{Schumann:2007mg} based on
Catani--Seymour dipole factorisation and the cluster hadronisation model~\cite{Winter:2003tt}
were used. They employed the dedicated set of tuned parameters developed by the
\SHERPA authors for this generator version and the \NNPDF[3.0nnlo] PDF
set~\cite{Ball:2014uwa}.

The NLO matrix elements for a given jet multiplicity were matched to the parton
shower using a colour-exact variant of the MC@NLO
algorithm~\cite{Hoeche:2011fd}. Different jet multiplicities were then merged
into an inclusive sample using an improved CKKW matching
procedure~\cite{Catani:2001cc,Hoeche:2009rj} which was extended to NLO
accuracy using the \MEPSatNLO prescription~\cite{Hoeche:2012yf}.
The merging cut was set dynamically at a scale of \SI{20}{\GeV}
according to the prescription in Ref.~\cite{Siegert:2016bre}.

The renormalisation and factorisation scales for the photon-plus-jet core
process were set to the transverse energy of the photon, \(E_\text{T}^\gamma\).
The strong coupling constant was set to \(\alphas (m_Z)= 0.118\) and the QED coupling
constant was evaluated in the Thomson limit. Photons from the matrix elements were required
to be central, by being within the rapidity range \(|y_{\gamma}|<2.7\), and isolated according to a
smooth-cone isolation criterion~\cite{Frixione:1998jh} with \(\delta_0=0.1\), \(\epsilon_{\gamma}=0.1\) and \(n=2\).

The effects of QCD scale uncertainties were evaluated~\cite{Bothmann:2016nao} using
seven-point variations of the factorisation and renormalisation scales in the matrix elements.
The scales were varied independently by factors of \(0.5\) and \(2\), avoiding variations in opposite directions.

PDF uncertainties for the nominal PDF set were
evaluated using the 100 variation replicas, as well as \(\pm 0.001\) shifts
of \alphas. Additionally, the results were cross-checked using the central values of the
\CT[14nnlo]~\cite{Dulat:2015mca} and \MMHT[nnlo]~\cite{Harland-Lang:2014zoa}
PDF sets.

%\textcolor{red}{ Several Monte Carlo slices were generated to ensure good statistics over the whole phase space. In each of them, the photon was required to fall within a \(E_{T}^{\gamma}\) range that depends on the slice avoiding any double-counting when the different slices are combined.}


\subsection[yy+jets]{ \(\gamma\gamma\)+jets}
%\label{sec:gammajets-sherpa-nlo-diphoton}

\paragraph{Short description:}

Prompt diphoton production was simulated with the
\SHERPA[2.2]~\cite{Bothmann:2019yzt} generator. In this set-up, NLO-accurate
matrix elements for up to one parton, and LO-accurate matrix elements for up
to three partons were calculated with the Comix~\cite{Gleisberg:2008fv} and
\OPENLOOPS~\cite{Buccioni:2019sur,Cascioli:2011va,Denner:2016kdg} libraries. They were matched
with the \SHERPA parton shower~\cite{Schumann:2007mg} using the \MEPSatNLO
prescription~\cite{Hoeche:2011fd,Hoeche:2012yf,Catani:2001cc,Hoeche:2009rj}
with a dynamic merging cut~\cite{Siegert:2016bre} of \SI{10}{\GeV}.
Photons were required to be isolated according to a smooth-cone isolation
criterion~\cite{Frixione:1998jh}. Samples were generated using the
\NNPDF[3.0nnlo] PDF set~\cite{Ball:2014uwa}, along with the dedicated set of tuned
parton-shower parameters developed by the \SHERPA authors.


\paragraph{Long description:}

Prompt diphoton production was simulated with the
\SHERPA[2.2]~\cite{Bothmann:2019yzt} parton shower Monte Carlo
generator. In this set-up, NLO and LO-accurate
matrix elements were calculated with the Comix~\cite{Gleisberg:2008fv} and
\OPENLOOPS~\cite{Buccioni:2019sur,Cascioli:2011va,Denner:2016kdg} libraries.
The default \SHERPA parton shower~\cite{Schumann:2007mg} based on
Catani--Seymour dipole factorisation and the cluster hadronisation model~\cite{Winter:2003tt}
were used. They employed the dedicated set of tuned parameters developed by the
\SHERPA authors for this generator version and the \NNPDF[3.0nnlo]
PDF set~\cite{Ball:2014uwa}.

The NLO matrix elements for a given jet multiplicity were matched to the parton
shower using a colour-exact variant of the MC@NLO algorithm~\cite{Hoeche:2011fd}.
Different jet multiplicities were then merged
into an inclusive sample using an improved CKKW matching
procedure~\cite{Catani:2001cc,Hoeche:2009rj} which was extended to NLO
accuracy using the \MEPSatNLO prescription~\cite{Hoeche:2012yf}.
The merging cut was set dynamically to a scale of \SI{20}{\GeV},
according to the prescription in Ref.~\cite{Siegert:2016bre}.

The renormalisation and factorisation scales for the diphoton core process
were set to the invariant mass of the photon pair, \(m_{\gamma\gamma}\).
The strong coupling constant was set to \(\alphas (m_Z)= 0.118\) and the QED coupling
constant was evaluated in the Thomson limit. Photons from the matrix elements were required to be central,
by being within the rapidity range \(|y_{\gamma}|<2.7\), and isolated according to a smooth-cone isolation
criterion~\cite{Frixione:1998jh} with \(\delta_0=0.1\), \(\epsilon_{\gamma}=0.1\) and \(n=2\).
Additionally, the photons were required to be separated by \(\Delta R(\gamma_1,\gamma_2) > 0.2\).


The effects of QCD scale uncertainties were evaluated~\cite{Bothmann:2016nao} using
seven-point variations of the factorisation and renormalisation scales in the matrix elements.
The scales were varied independently by factors of \(0.5\) and \(2\), avoiding variations in opposite directions.

PDF uncertainties for the nominal PDF set were
evaluated using the 100 variation replicas, as well as \(\pm 0.001\) shifts
of \alphas. Additionally, the results were cross-checked using the central values of the
\CT[14nnlo]~\cite{Dulat:2015mca} and \MMHT[nnlo]~\cite{Harland-Lang:2014zoa}
PDF sets.
%\textcolor{red}{ Several Monte Carlo slices were generated to ensure good statistics over the whole phase space. In each of them, the photon pair was required to fall within a \(m_{\gamma\gamma}\) range that depends on the slice avoiding any double-counting when the different slices are combined.}


\section[Sherpa (MEPS@NLO)]{\SHERPA (\MEPSatNLO)}
%\label{sec:gammajets-sherpa-lo}

\subsection*{Samples}
%\label{sec:gammajets-sherpa-lo-samples}

The descriptions below correspond to the samples in \cref{tab:gammajets-sherpa-lo}.

\begin{table}[!htbp]
  \caption{\(\gamma\)+jets and  \(\gamma\gamma\)+jets samples with \SHERPA LO\@.}%
  \label{tab:gammajets-sherpa-lo}
  \centering
  \begin{tabular}{l l}
    \toprule
    DSID range & Description \\
    \midrule
    361039--361062 & single photon \\
    303727--303742 & diphoton \\
    \bottomrule
  \end{tabular}
\end{table}


\subsection[y+jets]{\(\gamma\)+jets}
%\label{sec:gammajets-sherpa-lo-singlephoton}

\paragraph{Description:}

Prompt single-photon production was simulated using the \SHERPA[2.1]~\cite{Bothmann:2019yzt}
generator. The tree-level matrix elements, generated for up to three
additional partons, were merged with the initial- and final-state parton showers using the
\MEPSatLO prescription~\cite{Hoeche:2009rj}. The \CT[10nlo] set of PDFs~\cite{Lai:2010vv} was
used to parameterise the proton structure in conjunction with the dedicated set of tuned
parton-shower parameters developed by the \SHERPA authors for this generator version. A
modified version of the cluster model~\cite{Winter:2003tt} was used
for the description of the fragmentation into hadrons. Photons from the matrix elements were
required to be isolated according to a smooth-cone hadronic isolation criterion~\cite{Frixione:1998jh}
with \(\delta_0=0.3\), \(\epsilon_{\gamma}=0.025\) and \(n=2\).


\subsection[yy+jets]{ \(\gamma\gamma\)+jets}
%\label{sec:gammajets-sherpa-lo-diphoton}

\paragraph{Description:}

Prompt diphoton production was simulated using the \SHERPA[2.1]~\cite{Bothmann:2019yzt}
generator. The tree-level matrix elements, generated for up to two
additional partons, were merged with the initial- and final-state parton showers using the
\MEPSatLO prescription~\cite{Hoeche:2009rj}. The \CT[10nlo] set of PDFs~\cite{Lai:2010vv} was
used to parameterise the proton structure in conjunction with the dedicated set of tuned
parton-shower parameters developed by the \SHERPA authors for this generator version. A
modified version of the cluster model~\cite{Winter:2003tt} was used
for the description of the fragmentation into hadrons. Photons from the matrix elements were
required to be isolated according to a smooth-cone hadronic isolation criterion~\cite{Frixione:1998jh}
with \(\delta_0=0.3\), \(\epsilon_{\gamma}=0.025\) and \(n=2\). Additionally, the photons were
required to be separated by \(\Delta R(\gamma_1,\gamma_2) > 0.2\).


\section[Pythia (LO)]{\PYTHIA (LO)}
%\label{sec:gammajets-pythia-lo}

The descriptions below correspond to the samples in \cref{tab:gammajets-pythia-lo}.

\begin{table}[!htbp]
  \caption{\(\gamma\)+jets and  \(\gamma\gamma\)+jets samples with \PYTHIA.}%
  \label{tab:gammajets-pythia-lo}
  \centering
  \begin{tabular}{l l}
    \toprule
    DSID range & Description \\
    \midrule
    423099--423112 & single photon \\
    344008, 302520--34, 364423 & diphoton \\
    \bottomrule
  \end{tabular}
\end{table}


\subsection[y+jets]{\(\gamma\)+jets}
%\label{sec:gammajets-pythia-lo-singlephoton}

\paragraph{Description:}

Prompt single-photon production was simulated using the \PYTHIA[8.186]~\cite{Sjostrand:2007gs} generator.
Events were generated using tree-level matrix elements for photon-plus-jet final
states as well as LO QCD dijet events, with the inclusion of initial-
and final-state parton showers. The fragmentation component was
modelled by final-state QED radiation arising from calculations of all
\(2\rightarrow 2\) QCD processes. The \NNPDF[2.3lo]~\cite{Ball:2012cx} PDF
set was used in the matrix element calculation, the parton shower, and
the simulation of the multi-parton interactions. The samples
include a simulation of the underlying event with parameters set
according to the A14 tune~\cite{ATL-PHYS-PUB-2014-021}. The Lund
string model~\cite{Andersson:1983ia,Sjostrand:1984ic} was used for the
description of the fragmentation into hadrons.


\subsection[yy+jets]{ \(\gamma\gamma\)+jets}
%\label{sec:gammajets-pythia-lo-diphoton}

\paragraph{Description:}

Prompt diphoton production was simulated using the
\PYTHIA[8.186]~\cite{Sjostrand:2007gs} generator. Events were
generated using tree-level matrix elements for diphoton final states,
with the inclusion of initial- and final-state parton showers.  The
fragmentation component was modelled by final-state QED radiation
arising from calculations of photon-plus-jet processes in dedicated
samples. The \NNPDF[2.3lo]~\cite{Ball:2012cx} PDF set was used in the
matrix element calculation, the parton shower, and in the simulation of the
multi-parton interactions. The samples include a simulation of the
underlying event with parameters set according to the A14
tune~\cite{ATL-PHYS-PUB-2014-021}. The Lund string
model~\cite{Andersson:1983ia,Sjostrand:1984ic} was used for the
description of the fragmentation into hadrons.


==> template/MC_snippets/Higgs.tex <==
% !TEX root = MC_snippets.tex

\chapter{Higgs boson processes}
%\label{sec:higgs}

In this chapter, the set-up of the current ATLAS samples for Higgs boson production in gluon--gluon fusion,
vector-boson fusion and Higgs-strahlung processes is described.

\section{\(H\) via gluon--gluon fusion}
%\label{sec:higgs-ggH}

\subsection*{\texorpdfstring{\POWPY[8]}{Powheg+Pythia8} samples}
%\label{sec:higgs-ggH-samples}

%HGam: https://twiki.cern.ch/twiki/bin/view/Sandbox/RuggeroTurraSandbox
%ZZ: https://twiki.cern.ch/twiki/bin/view/AtlasProtected/HZZllllRun2MCSamplesMC16#mc16
%WW: https://twiki.cern.ch/twiki/bin/view/AtlasProtected/HWWMC
%Hlep:https://twiki.cern.ch/twiki/bin/view/AtlasProtected/HSG4MCrequests2015
%Hbb: https://twiki.cern.ch/twiki/bin/view/AtlasProtected/HbbMC

The descriptions below correspond to the samples in \cref{tab:higgs-ggH-samples}.

\begin{table}[!htbp]
  \caption{\POWHEG Higgs gluon--gluon fusion samples with \POWPY[8] for different Higgs boson decay channels.}%
  \label{tab:higgs-ggH-samples}
  \centering
  \begin{tabular}{ l | l | l}
    \toprule
    DSID   & Decay channel & Additional comment \\
    \midrule
    343981 & \(H\to\gamma\gamma\)&   \\
    345316 & \(H\to Z\gamma\) & \\
    345060 & \(H\to ZZ^{*} \to 4\ell \) & \(\ell=e,\mu,\tau\)   \\
    345324 & \(H\to WW^{*} \to 2\ell2\nu \) &  \(\pTX[][\ell1] > \SI{15}{\GeV}\) and \(\pTX[][\ell2] > \SI{5}{\GeV}\) \\
    308284 & \(H\to ZZ^{*}\to 4\nu\) & \(\MET > \SI{75}{\GeV}\)\\
    345342 & \(H\to b \bar{b}\) & \\
    345097 & \(H\to\mu\mu\)      &     \\
    345120 & \(H\to\tau\tau\to \ell^{+}\ell^{-}\) & \(\pTX[][\ell1] > \SI{13}{\GeV}\) and \(\pTX[][\ell2] > \SI{7}{\GeV}\) \\
    345121 & \(H\to\tau\tau\to h^{+}\ell^{-}\)    & \(\pTX[][\ell]  > \SI{15}{\GeV}\) and \(\pTX[][h]     > \SI{20}{\GeV}\) \\
    345122 & \(H\to\tau\tau\to \ell^{+}h^{-}\)    & \(\pTX[][\ell]  > \SI{15}{\GeV}\) and \(\pTX[][h]     > \SI{20}{\GeV}\) \\
    345123 & \(H\to\tau\tau\to h^{+}h^{-}\)       & \(\pTX[][h1]    > \SI{30}{\GeV}\) and \(\pTX[][h2]    > \SI{20}{\GeV}\) \\
    345124 & \(H\to\tau\tau\to \mu\tau\)          & \\ %\(\pTX[][h1] > \SI{30}{\GeV}\) and \(\pTX[][h2]    > \SI{20}{\GeV}\)
    345125 & \(H\to\tau\tau\to e \tau\)           & \\ %\(\pTX[][h1] > \SI{30}{\GeV}\) and \(\pTX[][h2]    > \SI{20}{\GeV}\)
    \bottomrule
  \end{tabular}
\end{table}

\paragraph{Short description:}

Higgs boson production via gluon--gluon fusion was simulated at next-to-next-to-leading-order (NNLO) accuracy in
QCD using \POWHEGBOX[v2]~\cite{Hamilton:2013fea,Hamilton:2015nsa,Alioli:2010xd,Nason:2004rx,Frixione:2007vw}.
The simulation achieved NNLO accuracy for arbitrary inclusive \(gg\to H\) observables by reweighting the Higgs boson
rapidity spectrum in \textsc{Hj}-\MINLO~\cite{Hamilton:2012np,Campbell:2012am,Hamilton:2012rf} to that of HNNLO~\cite{Catani:2007vq}.
%The transverse momentum spectrum of the Higgs boson obtained with this sample was found to be compatible with the fixed-order HNNLO calculation and the Hres2.3 calculation~\cite{Bozzi:2005wk,deFlorian:2011xf} performing resummation at next-to-next-to- leading-logarithm accuracy matched to a NNLO fixed-order calculation (NNLL+NNLO).
The \PDFforLHC[15nnlo] PDF set~\cite{Butterworth:2015oua} and the \AZNLO tune~\cite{STDM-2012-23}
of \PYTHIA[8]~\cite{Sjostrand:2014zea} were used.

The gluon--gluon fusion prediction from the Monte Carlo samples was normalised to the
next-to-next-to-next-to-leading-order cross-section in QCD plus electroweak corrections
at next-to-leading order
(NLO)~\cite{deFlorian:2016spz,Anastasiou:2016cez,Anastasiou:2015ema,Dulat:2018rbf,Harlander:2009mq,Harlander:2009bw,Harlander:2009my,Pak:2009dg,Actis:2008ug,Actis:2008ts,Bonetti:2018ukf,Bonetti:2018ukf}. The decays of bottom and charm hadrons
were performed by \EVTGEN~\cite{Lange:2001uf}.
The normalisation of all Higgs boson
samples accounts for the decay branching ratio calculated with HDECAY~\cite{Djouadi:1997yw,Spira:1997dg,Djouadi:2006bz}
and \PROPHECY~\cite{Bredenstein:2006ha,Bredenstein:2006rh,Bredenstein:2006nk}.


\paragraph{Long description:}

Higgs boson production via gluon--gluon fusion was simulated at next-to-next-to-leading-order (NNLO) accuracy in QCD using
\POWHEGBOX[v2]~\cite{Hamilton:2013fea,Hamilton:2015nsa,Alioli:2010xd,Nason:2004rx,Frixione:2007vw}. The simulation achieved NNLO
accuracy for arbitrary inclusive \(gg\to H\) observables by reweighting the Higgs boson rapidity spectrum
in \textsc{Hj}-\MINLO~\cite{Hamilton:2012np,Campbell:2012am,Hamilton:2012rf} to that of HNNLO~\cite{Catani:2007vq}. The transverse momentum
spectrum of the Higgs boson obtained with this sample was found to be compatible with the fixed-order HNNLO calculation and the
\HRES[2.3] calculation~\cite{Bozzi:2005wk,deFlorian:2011xf} performing resummation at next-to-next-to-leading-logarithm accuracy
matched to a NNLO fixed-order calculation (NNLL+NNLO).
Top- and bottom-quark mass effects were included up to next-to-leading order (NLO).

The renormalisation and factorisation scales were set to half of the Higgs boson mass and the \PDFforLHC[15nnlo] PDF
set~\cite{Butterworth:2015oua} was used. The matrix elements were matched to the parton shower of \PYTHIA[8]~\cite{Sjostrand:2014zea}
which uses the AZNLO tune~\cite{STDM-2012-23}. The decays of bottom and charm hadrons
were performed by \EVTGEN~\cite{Lange:2001uf}.

The QCD scale uncertainties were obtained using nine-point scale variations of the NLO renormalisation and factorisation scales and applying the NNLO reweighting to those variations, including up and down variations of \(\muR=\muF\) around the central value for the NNLO part, yielding a total of 27 scale variations.
PDF and \alphas uncertainties were estimated using the \PDFforLHC[15nlo] set of eigenvectors.
The envelope of the resulting 27 scale variations was taken to estimate the QCD scale uncertainty.
Uncertainties were also provided for switching off bottom- and top-quark mass effects.
%From YR4

The prediction from the Monte Carlo samples was normalised to the next-to-next-to-next-to-leading-order
cross-section in QCD in the infinite top-quark mass
limit~\cite{deFlorian:2016spz,Anastasiou:2016cez,Anastasiou:2015ema,Dulat:2018rbf,Aglietti:2004nj} and including exact
corrections for all finite quark-mass effects at NLO in QCD as well as NLO electroweak
effects~\cite{Actis:2008ug,Bonetti:2018ukf}. Additionally, corrections to the inverse of the top-quark mass were taken
into account at NNLO~\cite{Harlander:2009mq,Harlander:2009bw,Harlander:2009my,Pak:2009dg}.
The normalisation of all Higgs boson samples accounts for the decay branching ratio calculated with
HDECAY~\cite{Djouadi:1997yw,Spira:1997dg,Djouadi:2006bz}
and \PROPHECY~\cite{Bredenstein:2006ha,Bredenstein:2006rh,Bredenstein:2006nk}.


\section{\(H\) via vector-boson fusion}
%\label{sec:higgs-VBF}

\subsection*{\texorpdfstring{\POWPY[8]}{Powheg+Pythia8} samples}
%\label{sec:higgs-VBF-samples}

The descriptions below correspond to the samples in \cref{tab:higgs-VBF-samples}.

\begin{table}[!htbp]
  \caption{\POWPY[8] Higgs vector-boson fusion samples for different Higgs boson decay channels.}%
  \label{tab:higgs-VBF-samples}
  \centering
  \begin{tabular}{ l l l}
    \toprule
    DSID   & Decay channel & Additional comment \\
    \midrule
    346317 & \(H\to\) all  & \\
    346214 & \(H\to\gamma\gamma\)& \\
    345833 & \(H\to Z\gamma\) & \(Z\to \ell^{+}\ell^{-}\) \\
    345834 & \(H\to \gamma\gamma^{*}\) & \(\gamma^{*}\to \ell^{+}\ell^{-}\) \\
    346228 & \(H\to ZZ^{*} \to 4\ell \) & \(\ell=e,\mu\) \\
    450576 & \(H\to ZZ^{*} \to 2\ell2b \) &  \\
    345948 & \(H\to WW^{*} \to 2\ell2\nu \) &  \(\pTX[][\ell1] > \SI{15}{\GeV}\) and \(\pTX[][\ell2] > \SI{5}{\GeV}\) \\
    346600 & \(H\to ZZ^{*}\to 4\nu\) & \(\MET > \SI{75}{\GeV}\) \\
    345949 & \(H\to b \bar{b}\) & \\
    % & \(H\to\mu\mu\)      &     \\
    346190& \(H\to\tau\tau\to \ell^{+}\ell^{-}\) & \(\pTX[][\ell1] > \SI{13}{\GeV}\) and \(\pTX[][\ell2] > \SI{7}{\GeV}\) \\
    346191 & \(H\to\tau\tau\to h^{+}\ell^{-}\)   & \(\pTX[][\ell]  > \SI{15}{\GeV}\) and \(\pTX[][h]     > \SI{20}{\GeV}\) \\
    346192 & \(H\to\tau\tau\to \ell^{+}h^{-}\)   & \(\pTX[][\ell]  > \SI{15}{\GeV}\) and \(\pTX[][h]     > \SI{20}{\GeV}\) \\
    346193 & \(H\to\tau\tau\to h^{+}h^{-}\)      & \(\pTX[][h1]    > \SI{30}{\GeV}\) and \(\pTX[][h2]    > \SI{20}{\GeV}\) \\
    346194 & \(H\to\tau\tau\to e\tau\)           & \\%\(\pTX[][l1] > \SI{10}{\GeV}\) and \(\pTX[][h1]    > \SI{20}{\GeV}\) \\
    346195 & \(H\to\tau\tau\to \mu\tau\)         & \\%\(\pTX[][l1] > \SI{10}{\GeV}\) and \(\pTX[][h1]    > \SI{20}{\GeV}\) \\
    \bottomrule
  \end{tabular}
\end{table}

\paragraph{Short description:}

Higgs boson production via vector-boson fusion was simulated with
\POWHEGBOX[v2]~\cite{Nason:2009ai,Alioli:2010xd,Nason:2004rx,Frixione:2007vw}
and interfaced with \PYTHIA[8]~\cite{Sjostrand:2014zea} for parton shower and non-perturbative effects,
with parameters set according to the \AZNLO tune~\cite{STDM-2012-23}.
The \POWHEGBOX prediction is accurate to next-to-leading order (NLO) and uses
the \PDFforLHC[15nlo] PDF set~\cite{Butterworth:2015oua}.
%It was tuned to match calculations with effects due to finite heavy-quark masses
%and soft-gluon resummation up to NNLL.
It was normalised to an approximate-NNLO QCD cross-section
with NLO electroweak corrections~\cite{Ciccolini:2007jr,Ciccolini:2007ec,Bolzoni:2010xr}.
The decays of bottom and charm hadrons were performed by \EVTGEN~\cite{Lange:2001uf}.
The normalisation of all Higgs boson samples accounts for the decay branching ratio calculated
with \textsc{HDECAY}~\cite{Djouadi:1997yw,Spira:1997dg,Djouadi:2006bz}
and \PROPHECY~\cite{Bredenstein:2006ha,Bredenstein:2006rh,Bredenstein:2006nk}.


\paragraph{Long description:}

Higgs boson production via vector-boson fusion was simulated with
\POWHEGBOX[v2]~\cite{Nason:2009ai,Alioli:2010xd,Nason:2004rx,Frixione:2007vw}. A factorised approximation, where cross-talk between the
fermion lines is neglected, was used. The implementation is based on the respective NLO QCD calculations for genuine \(W/Z\) vector-boson
fusion topologies (VBF approximation). Quark--antiquark annihilation and interference contributions
between \(t\)- and \(u\)-channel contributions were disregarded.
%External fermion masses are neglected throughout.  For the choice of renormalisation and factorisation scales, various options are available.  For this report, fixed scales,μF=μR=MW, are used, and contributions from external bottom and top quarks are entirely disregarded.

The renormalisation and factorisation scales were set to the \(W\) boson mass and the \PDFforLHC[15nlo] PDF set~\cite{Butterworth:2015oua}
was used. The matrix elements were matched to the parton shower of \PYTHIA[8]~\cite{Sjostrand:2014zea} which uses the \AZNLO
tune~\cite{STDM-2012-23}. A dipole-recoil strategy was used for the parton shower.The decays of bottom and charm hadrons
were performed by \EVTGEN~\cite{Lange:2001uf}.%, which provides a better agreement than other recoil schemes with the NNLO predictions of proVBFH (not included in the HiggsReference twiki). % cite https://arxiv.org/pdf/1710.00391.pdf ?,

%The samples include weight variations evaluated on-the-fly for the estimation of QCD scale, PDF- and \alphas-induced uncertainties.
The QCD scales \muR and \muF were varied independently by factors of 0.5 and 2.0, both in the matrix element
and in the parton shower.

The prediction from the \POWHEGBOX sample was normalised to the next-to-next-to-leading-order cross-section in QCD
using the VBF approximation~\cite{Ciccolini:2007jr,Ciccolini:2007ec,Bolzoni:2010xr}. Relative
next-to-leading-order electroweak corrections were also taken into account for the \(t\)- and \(u\)-channel contribution
considered in the VBF approximation. The normalisation of all Higgs boson samples accounts for the decay branching
ratio calculated with \textsc{HDECAY}~\cite{Djouadi:1997yw,Spira:1997dg,Djouadi:2006bz} and
\PROPHECY~\cite{Bredenstein:2006ha,Bredenstein:2006rh,Bredenstein:2006nk}.


\section{\(VH\)}
%\label{sec:higgs-VH}

This section describes the generation details of nominal samples for Higgs-strahlung production.

\subsection*{\texorpdfstring{\POWPY[8]}{Powheg+Pythia8} samples}
%\label{sec:higgs-VH-samples}

The descriptions below correspond to the samples in \crefrange{tab:higgs-ZH-samples}{tab:higgs-ggZH-samples}.

\begin{table}[!htbp]
  \caption{\POWPY[8] samples of Higgs boson production in association with a \(Z\) boson for different Higgs boson decay channels.}%
  \label{tab:higgs-ZH-samples}
  \centering
  \begin{tabular}{ l l l}
    \toprule
    DSID   & Decay channel & Additional comment \\
    \midrule
    345038 & \(H \to ZZ^{*} \to 4\ell\) & \(Z\to\) all\\
    345319 & \(H \to \gamma\gamma\) & \(Z\to\) all\\
    345322 & \(H \to Z\gamma\) & \(Z\to\) all\\
    345103 & \(H \to\mu\mu\) & \(Z\to\) all\\
    345217 & \(H \to\tau\tau\)& \(Z\to\) all\\
    345218 & \(H \to e\tau\) &\(Z\to\) all\\
    345219 & \(H \to \mu\tau\)&\(Z\to\) all\\
    345445 & \(H \to WW^{*} \to 2\ell2\nu \) & \(Z\to\) all \\
    345876 & \(H\ to ee\) &\(Z\to\) all \\
    345965 & \(H \to \gamma\gamma^{*}\) & \(\gamma^{*}\to \ell^{+}\ell^{-}\); \(Z\to\) all\\
    346310 & \(H \to\) all&\(Z\to\) all\\
    346607 & \(H \to ZZ^{*} \to 4\nu \) &\(Z\to \ell^{+}\ell^{-}\) \\
    345055 & \(H \to b\bar{b}\)              & \pTX[][Z] enhancement; \(Z\to \ell^{+}\ell^{-}\)\\
    345111 & \(H \to c\bar{c}\)              & \pTX[][Z] enhancement; \(Z\to \ell^{+}\ell^{-}\)\\
    345337 & \(H \to WW^{*} \to 2\ell2\nu \) & \pTX[][Z] enhancement; \(Z\to \ell^{+}\ell^{-}\)\\
    346326 & \(H \to\tau\tau\)               & \pTX[][Z] enhancement; \(Z\to \ell^{+}\ell^{-}\)\\
    346693 & \(H \to ZZ^{*} \to 4\nu \)      & \pTX[][Z] enhancement; \(Z\to \ell^{+}\ell^{-}\)\\
    345056 & \(H \to b\bar{b}\)              & \pTX[][Z] enhancement; \(Z\to \nu\bar{\nu}\)\\
    345112 & \(H \to c\bar{c}\)              & \pTX[][Z] enhancement; \(Z\to \nu\bar{\nu}\)\\
    345445 & \(H \to WW^{*} \to 2\ell2\nu\)  & \pTX[][Z] enhancement; \(Z\to \nu\bar{\nu}\)\\
    \bottomrule
  \end{tabular}
\end{table}

\begin{table}[!htbp]
  \caption{\POWPY[8] samples of Higgs boson production in association with a \(W^{+}\) boson for different Higgs boson decay channels.}
  \label{tab:higgs-WpH-samples}
  \centering
  \begin{tabular}{l l l}
    \toprule
    DSID   & Decay channel & Additional comment \\
    \midrule
    345039 & \(H \to ZZ^{*} \to 4\ell\) & \(W^{+}\to\) all\\
    345318 & \(H \to \gamma\gamma\) & \(W^{+}\to\) all\\
    345104 & \(H \to \mu\mu\) &  \(W^{+}\to\) all\\
    345212 & \(H \to \tau\tau\) &  \(W^{+}\to\) all\\
    345214 & \(H \to e \tau \) & \(W^{+}\to\) all\\
    345216 & \(H \to \mu \tau \) & \(W^{+}\to\) all\\
    345321 & \(H \to Z\gamma\) & \(W^{+}\to\) all\\
    345325 & \(H \to WW^{*} \to 2\ell2\nu \) & \(W^{+} \to q\bar{q}\) \\
    345877 & \(H \to e^{+}e^{-}\) & \(W^{+}\to\) all\\
    345964 & \(H \to \gamma\gamma^{*}\) & \(\gamma^{*}\to \ell^{+}\ell^{-}\); \(W^{+}\to\) all\\
    346311 & \(H \to\) all & \(W^{+}\to\) all\\
    346605 & \(H \to ZZ^{*} \to 4\nu \) & \(W^{+}\to\) all\\
    346699 & \(H \to 4\ell\) & interfaced to PROPHECY4F \\
    346705 & \(H \to 4\ell\) & interfaced to Hto4l \\
    345054 & \(H \to b\bar{b}\)                   & \pTX[][W] enhancement; \(W^{+}\to \ell^{+}\nu\) \\
    345110 & \(H \to c\bar{c}\)                   & \pTX[][W] enhancement; \(W^{+}\to \ell^{+}\nu\) \\
    345327 & \(H \to WW^{*} \to 2\ell2\nu\)       & \pTX[][W] enhancement; \(W^{+}\to \ell^{+}\nu\) \\
    346561 & \(H \to WW^{*} \to q\bar{q}\ell\nu\) & \pTX[][W] enhancement; \(W^{+}\to \ell^{+}\nu\) \\
    346325 & \(H \to \tau\tau\)                   & \pTX[][W] enhancement; \(W^{+}\to \ell^{+}\nu\) \\
    346729 & \(H \to ZZ^{*} \to 4\nu\)            & \pTX[][W] enhancement; \(W^{+}\to \ell^{+}\nu\) \\
    \bottomrule
  \end{tabular}
\end{table}

\begin{table}[!htbp]
  \caption{\POWPY[8] samples of Higgs boson production in association with a \(W^{-}\) boson for different Higgs boson decay channels.}
  \label{tab:higgs-WmH-samples}
  \centering
  \begin{tabular}{l l l}
    \toprule
    DSID   & Decay channel & Additional comment \\
    \midrule
    345040 & \(H \to ZZ^{*} \to 4\ell\) & \(W^{-}\to\) all\\
    345317 & \(H \to \gamma\gamma\) & \(W^{-}\to\) all\\
    345105 & \(H \to \mu\mu\) &  \(W^{-}\to\) all\\
    345211 & \(H \to \tau\tau\) &  \(W^{-}\to\) all\\
    345213 & \(H \to e \tau \) & \(W^{-}\to\) all\\
    345215 & \(H \to \mu \tau \) & \(W^{-}\to\) all\\
    345320 & \(H \to Z\gamma\) & \(W^{-}\to\) all\\
    345333 & \(H \to WW^{*} \to 2\ell2\nu \) & \(W^{-} \to q\bar{q}\) \\
    345878 & \(H \to e^{+}e^{-}\) & \(W^{-}\to\) all\\
    345963 & \(H \to \gamma\gamma^{*}\) & \(\gamma^{*}\to \ell^{+}\ell^{-}\); \(W^{-}\to\) all\\
    346312 & \(H \to\) all & \(W^{-}\to\) all\\
    346606 & \(H \to ZZ^{*} \to 4\nu \) & \(W^{-}\to\) all\\
    346700 & \(H \to 4\ell\) & interfaced to PROPHECY4F \\
    346706 & \(H \to 4\ell\) & interfaced to Hto4l \\
    345053 & \(H \to b\bar{b}\)                   & \pTX[][W] enhancement; \(W^{-}\to \ell^{-}\bar{\nu}\) \\
    345109 & \(H \to c\bar{c}\)                   & \pTX[][W] enhancement; \(W^{-}\to \ell^{-}\bar{\nu}\)  \\
    345326 & \(H \to WW^{*} \to 2\ell2\nu\)       & \pTX[][W] enhancement; \(W^{-}\to \ell^{-}\bar{\nu}\) \\
    346560 & \(H \to WW^{*} \to q\bar{q}\ell\nu\) & \pTX[][W] enhancement; \(W^{-}\to \ell^{-}\bar{\nu}\) \\
    346324 & \(H \to \tau\tau\)                   & \pTX[][W] enhancement; \(W^{-}\to \ell^{-}\bar{\nu}\) \\
    346730 & \(H \to ZZ^{*} \to 4\nu\)            & \pTX[][W] enhancement; \(W^{-}\to \ell^{-}\bar{\nu}\) \\
    \bottomrule
  \end{tabular}
\end{table}

\begin{table}[!htbp]
  \caption{\POWPY[8] samples of loop-induced Higgs boson production in association with a \(Z\) boson for different
  Higgs boson decay channels.}%
  \label{tab:higgs-ggZH-samples}
  \centering
  \begin{tabular}{ l | l | l}
    \toprule
    DSID   & Decay channel & Additional comment \\
    \midrule
    345061 & \(H \to \gamma\gamma\) & \(Z\to\) all \\
    345066 & \(H \to ZZ^{*} \to 4\ell\) & \(Z\to\) all \\
    345098 & \(H \to \mu\mu\) & \(Z\to\) all \\
    345596 & \(H \to ZZ^{*} \to 4\nu\) & \(Z\to\) all \\
    346524 & \(H \to WW^{*} \to 2\ell2\nu \) & \(Z\to\) all \\
    346697 & \(H \to ZZ^{*} \to 4\nu\) & interfaced to PROPHECY4F \\
    346703 & \(H \to ZZ^{*} \to 4\nu\) & interfaced to Hto4l \\
    345057 & \(H \to b\bar{b}\) &  \(Z\to \ell^{+}\ell^{-}\)\\
    345113 & \(H \to c\bar{c}\) & \(Z\to \ell^{+}\ell^{-}\)\\
    345446 & \(H \to WW^{*} \to 2\ell2\nu\) &  \(Z\to \ell^{+}\ell^{-}\)\\
    346329 & \(H \to \tau\tau\) &  \(Z\to \ell^{+}\ell^{-}\)\\
    346694 & \(H \to ZZ^{*} \to 4\nu\) &  \(Z\to \ell^{+}\ell^{-}\)\\
    345058 & \(H \to b\bar{b}\) & \(Z\to \nu\bar{\nu}\)\\
    345114 & \(H \to c\bar{c}\) & \(Z\to \nu\bar{\nu}\)\\
    \bottomrule
  \end{tabular}
\end{table}

\paragraph{Short description:}

Higgs boson production in association with a vector boson was simulated using
\POWHEGBOX[v2]~\cite{Nason:2009ai,Alioli:2010xd,Nason:2004rx,Frixione:2007vw} and interfaced with \PYTHIA[8]~\cite{Sjostrand:2014zea} for
parton shower and non-perturbative effects. The \POWHEGBOX prediction is accurate to next-to-leading order for \(VH\) boson plus one-jet production.
The loop-induced \(gg\to ZH\) process was generated separately at leading order. The \PDFforLHC[15nlo] PDF
set~\cite{Butterworth:2015oua} and the \AZNLO tune~\cite{STDM-2012-23} of \PYTHIA[8]~\cite{Sjostrand:2014zea} were used. The decays of bottom and charm hadrons
were performed by \EVTGEN~\cite{Lange:2001uf}. The Monte Carlo
prediction was normalised to cross-sections calculated at NNLO in QCD with NLO electroweak corrections for \(q\bar{q}/qg \to VH\) and at NLO
and next-to-leading-logarithm accuracy in QCD for
\(gg \to ZH\)~\cite{Ciccolini:2003jy,Brein:2003wg,Brein:2011vx,Altenkamp:2012sx,Denner:2014cla,Brein:2012ne,Harlander:2014wda}.
The normalisation of all Higgs boson samples accounts for the decay branching ratio calculated with
HDECAY~\cite{Djouadi:1997yw,Spira:1997dg,Djouadi:2006bz} and \PROPHECY~\cite{Bredenstein:2006ha,Bredenstein:2006rh,Bredenstein:2006nk}.


\paragraph{Long description:}

Higgs boson production in association with a vector boson was simulated using
\POWHEGBOX[v2]~\cite{Nason:2009ai,Alioli:2010xd,Nason:2004rx,Frixione:2007vw}. The computation was carried out using the
\MINLO~\cite{Luisoni:2013cuh} prescription, which achieves NLO accuracy for the \(VH\) and \(VH\) boson plus one-jet production
inclusive distributions and dictates the choice of renormalisation and factorisation scales. Virtual amplitudes were constructed
through the interface to the \GOSAM package~\cite{Cullen:2011ac}. The loop-induced \(gg\to ZH\) process was generated separately at
leading order with \POWHEGBOX. In all cases, the \PDFforLHC[15nlo] PDF set~\cite{Butterworth:2015oua} was used.

The matrix elements were matched to the parton shower of \PYTHIA[8]~\cite{Sjostrand:2014zea} which uses the \AZNLO
tune~\cite{STDM-2012-23}. The decays of bottom and charm hadrons were performed by \EVTGEN~\cite{Lange:2001uf}.
%The samples include weight variations evaluated on-the-fly for the estimation of QCD scale, PDF- and \alphas-induced uncertainties.
The QCD scales \muR and \muF were varied independently by factors of 0.5 and 2.0 to account for their uncertainties.

The predictions from \POWHEGBOX were normalised to the best available theoretical prediction. The  \(q\bar{q}/qg \to VH\) cross-sections
were calculated at NNLO in QCD with NLO electroweak corrections and the \(gg \to ZH\) cross-sections were calculated at NLO and
next-to-leading-logarithm accuracy~\cite{Ciccolini:2003jy,Brein:2003wg,Brein:2011vx,Altenkamp:2012sx,Denner:2014cla,Brein:2012ne,Harlander:2014wda}.
The normalisation of the \(q\bar{q}\to ZH\) samples was extracted from the subtraction of the latter from the former.
Differential NLO EW corrections were available from the \textsc{HAWK} program~\cite{Denner:2014cla} to be applied to
\(q\bar{q}\)-initiated \(VH\) production as a function of the vector boson's transverse momentum.
The normalisation of all Higgs boson samples accounts for the decay branching ratio calculated with
\textsc{HDECAY}~\cite{Djouadi:1997yw,Spira:1997dg,Djouadi:2006bz} and
\PROPHECY~\cite{Bredenstein:2006ha,Bredenstein:2006rh,Bredenstein:2006nk}.


==> template/MC_snippets/MB.tex <==
% !TEX root = MC_snippets.tex

\chapter{Multiboson processes}
%\label{sec:MB}

In the following paragraphs, the set-ups of the current ATLAS multiboson baseline samples are described.
Details of the full process configuration are given in the PUB note~\cite{ATL-PHYS-PUB-2017-005}.


\section[Inclusive Powheg]{Inclusive \POWHEG}
%\label{sec:MB-powheg}

The descriptions below correspond to the samples in \cref{tab:MB-powheg}.

\begin{table}[htbp]
  \caption{Inclusive \(VV\) samples with \POWHEG.}%
  \label{tab:MB-powheg}
  \centering
  \begin{tabular}{l l}
    \toprule
    DSID range & Description \\
    \midrule
    361600--361605 & inclusive \(WW(2\ell 2\nu), WZ(3\ell\nu), ZZ(4\ell), ZZ(4\nu), ZZ(2\ell 2\nu)\) (all lepton flavours)\\
    361606--361611 & inclusive \(WW/WZ/ZZ\) semileptonic decays (\(\ell\ell qq\), \(\ell\nu qq\), \(\nu\nu qq\), all lepton flavours)\\
    \bottomrule
  \end{tabular}
\end{table}

\paragraph{Description:}

The \POWHEGBOX[v2]~\cite{Nason:2004rx,Frixione:2007vw,Alioli:2010xd} generator
was used to simulate the \(WW\), \(WZ\) and \(ZZ\)~\cite{Nason:2013ydw} production
processes at NLO accuracy in QCD. The effect of singly resonant
amplitudes and interference effects due to \(Z/\gamma^*\) and
same-flavour lepton combinations in the final state were included, where appropriate.
Interference effects between \(WW\) and \(ZZ\) for same-flavour charged leptons and
neutrinos were ignored.
Events were interfaced to \PYTHIA[8.210]~\cite{Sjostrand:2014zea}
for the modelling of the parton shower, hadronisation, and underlying
event, with parameters set according to the \AZNLO
tune~\cite{STDM-2012-23}. The \CT[10] PDF set~\cite{Lai:2010vv} was used
for the hard-scattering processes, whereas the \CTEQ[6L1] PDF
set~\cite{Pumplin:2002vw} was used for the parton shower. The \EVTGEN[1.2.0]
program~\cite{Lange:2001uf} was used to decay bottom and charm hadrons.

The factorisation and renormalisation scales were set to the invariant mass of
the boson pair. An invariant mass of \(m_{\ell\ell} > \SI{4}{\GeV}\) was required
at matrix-element level for any pair of same-flavour charged leptons.


\section[Sherpa]{\SHERPA}
%\label{sec:MB-sherpa}

\subsection{Fully leptonic, semileptonic and loop-induced \texorpdfstring{\(VV\)}{VV}}
%\label{sec:MB-sherpa-fully}

The descriptions below correspond to the samples in
\cref{tab:MB-sherpa}. They describe the almost
identical set-ups of fully leptonic (including loop-induced \(VV\) production)
and semileptonic \(VV\) decays. For loop-induced processes \(gg\to VV\),
the description below assumes that the `nominal' samples with
Higgs contributions are used. If you are using specialised set-ups that
exclude the Higgs component, the description should be modified appropriately.
(Get in touch with the PMG Weak Boson Processes subgroup if you are unsure.)

\begin{table}[htbp]
  \caption{\(VV\) samples with \SHERPA: fully leptonic, semileptonic,
    loop-induced fully leptonic, loop-induced semileptonic. SFOS stands for
    \enquote{same flavour opposite-charge sign}.}%
  \label{tab:MB-sherpa}
  \centering
  \begin{tabular}{l l}
    \toprule
    DSID range & Description \\
    \midrule
    364250--364255, 363494   & \(4\ell, 3\ell\nu, 2\ell 2\nu, 4\nu\) with \(m_{\ell\ell}\mathrm{(SFOS)} > \SI{4}{\GeV}\), \(\pTX[\ell](1,2) > \SI{5}{\GeV}\)\\
    364288--364290 & fully leptonic low \(m_{\ell\ell}\) and \(\pTX[\ell]\) complement\\
    \midrule
    345705--345727   & loop-induced leptonic\\
    \midrule
    363355-363360, 363489   & semileptonic, on-shell diboson production with factorised decays\\
    \midrule
    364302-364305   & loop-induced semileptonic, using factorised on-shell decays)\\
    \bottomrule
  \end{tabular}
\end{table}

\paragraph{Description:}

Samples of diboson final states (\(VV\)) were simulated with the
\SHERPA[2.2.1] or 2.2.2~\cite{Bothmann:2019yzt} generator depending on the process,
%~\footnote{This is an admixture of 2.2.1 and above versions, so the version should be kept generic to avoid confusions. As an
%alternative, the sentence can be modified indicating that samples are simulated with the \SHERPA[2.2.1] or 2.2.2 depending on the process.}
including off-shell effects and Higgs boson contributions, where appropriate.
Fully leptonic final states and semileptonic final states, where one boson
decays leptonically and the other hadronically, were generated using
matrix elements at NLO accuracy in QCD for up to one additional parton
and at LO accuracy for up to three additional parton
emissions. Samples for the loop-induced processes \(gg \to VV\) were
generated using LO-accurate matrix elements for up to one
additional parton emission for both the cases of fully leptonic and
semileptonic final states. The matrix element calculations were matched
and merged with the \SHERPA parton shower based on Catani--Seymour
dipole factorisation~\cite{Gleisberg:2008fv,Schumann:2007mg} using the MEPS@NLO
prescription~\cite{Hoeche:2011fd,Hoeche:2012yf,Catani:2001cc,Hoeche:2009rj}.
The virtual QCD corrections were provided by the
\OPENLOOPS library~\cite{Buccioni:2019sur,Cascioli:2011va,Denner:2016kdg}. The
\NNPDF[3.0nnlo] set of PDFs was used~\cite{Ball:2014uwa}, along with the
dedicated set of tuned parton-shower parameters developed by the
\SHERPA authors.


\paragraph{Additional description:}

The ME+PS matching~\cite{Hoeche:2011fd} was employed for different jet
multiplicities which were then merged into an inclusive sample using an
improved CKKW matching procedure~\cite{Catani:2001cc,Hoeche:2009rj}
which is extended to NLO accuracy using the MEPS@NLO
prescription~\cite{Hoeche:2012yf}. The virtual QCD corrections for
matrix elements at NLO accuracy were provided by the
\OPENLOOPS library~\cite{Buccioni:2019sur,Cascioli:2011va,Denner:2016kdg}. The
calculation was performed in the \(G_\mu\) scheme, ensuring an
optimal description of pure electroweak interactions at the
electroweak scale.

\input{sherpa_scale_pdf.tex}


\subsection[Electroweak VVjj]{Electroweak \(VVjj\)}
%\label{sec:MB-sherpa-vvjj}

The descriptions below correspond to the samples in
\cref{tab:MB-sherpa-vvjj}.

\begin{table}[htbp]
  \caption{Electroweak \(VVjj\) samples with \SHERPA.}%
  \label{tab:MB-sherpa-vvjj}
  \centering
  \begin{tabular}{l l}
    \toprule
    DSID range & Description \\
    \midrule
    364283--364284   & \(\ell\ell\ell\ell jj\), \(\ell\ell\ell\nu jj\)\\
    364285   &  \(\ell\ell\nu\nu jj\) opposite-sign\\
    364287   &  \(\ell\ell\nu\nu jj\) same-sign\\
    366086--366089   &  \(\ell\ell\ell\ell jj\), \(\ell\ell\ell\nu jj\), \(\ell\ell\nu\nu jj\), with the triboson contributions removed\\
    \bottomrule
  \end{tabular}
\end{table}

\paragraph{Description:}

Electroweak production of a diboson in association with two jets
(\(VVjj\)) was simulated with the \SHERPA[2.2.2]~\cite{Bothmann:2019yzt}
generator. The LO-accurate matrix elements were matched to a parton
shower based on Catani--Seymour dipole factorisation~\cite{Gleisberg:2008fv,Schumann:2007mg} using the MEPS@LO
prescription~\cite{Hoeche:2011fd,Hoeche:2012yf,Catani:2001cc,Hoeche:2009rj}.
Samples were generated using the \NNPDF[3.0nnlo] PDF set~\cite{Ball:2014uwa},
along with the dedicated set of tuned parton-shower parameters
developed by the \SHERPA authors.

\paragraph{Additional description:} The calculation was performed in the
\(G_\mu\) scheme, ensuring an optimal description of pure
electroweak interactions at the electroweak scale.

\input{sherpa_scale_pdf.tex}


\subsection[Vgamma (NLO, biased)]{\(V\gamma\) (NLO, biased)}
%\label{sec:MB-sherpa-vgamma-nlo-biased}

The descriptions below correspond to the samples in
\cref{tab:MB-sherpa-vynlo-ew}.

\begin{table}[htbp]
  \caption{NLO \(V\gamma\) samples with \SHERPA.}%
  \label{tab:MB-sherpa-vynlo-ew}
  \centering
  \begin{tabular}{l l}
    \toprule
    DSID range & Description \\
    \midrule
    700011--700017 & biased in \(\log_{10}(\max[\pT(V), \pT(\gamma)])\)\\
    \bottomrule
  \end{tabular}
\end{table}

\paragraph{Description:}

The production of \(V\gamma\) final states was simulated with the
\SHERPA[2.2.8]~\cite{Bothmann:2019yzt} generator.  Matrix elements at
NLO QCD accuracy for up to one additional parton and LO accuracy for
up to three additional parton emissions were matched and merged with
the \SHERPA parton shower based on Catani--Seymour
dipole factorisation~\cite{Gleisberg:2008fv,Schumann:2007mg} using the MEPS@NLO
prescription~\cite{Hoeche:2011fd,Hoeche:2012yf,Catani:2001cc,Hoeche:2009rj}.
The virtual QCD corrections for matrix elements at NLO accuracy were provided by
the \OPENLOOPS[2] library~\cite{Buccioni:2019sur,Cascioli:2011va,Buccioni:2017yxi,Denner:2016kdg}.
Samples were generated using the \NNPDF[3.0nnlo] PDF set~\cite{Ball:2014uwa}, along with
the dedicated set of tuned parton-shower parameters developed by the \SHERPA authors.


\paragraph{Additional description:}

The ME+PS matching~\cite{Hoeche:2011fd} was employed for different jet
multiplicities which were then merged into an inclusive sample
using an improved CKKW matching
procedure~\cite{Catani:2001cc,Hoeche:2009rj} which was extended to NLO
accuracy using the MEPS@NLO prescription~\cite{Hoeche:2012yf}.
The virtual QCD corrections for matrix elements at NLO accuracy were provided by
the \OPENLOOPS[2] library~\cite{Buccioni:2019sur,Cascioli:2011va,Buccioni:2017yxi,Denner:2016kdg}.
Multijet merging at NLO accuracy in the electroweak coupling was based on
the \NLOEWvirt approach~\cite{Kallweit:2014xda,Kallweit:2015dum}.
The calculation was performed in the \(G_\mu\) scheme, ensuring an optimal
description of pure electroweak interactions at the electroweak scale.

\input{sherpa_scale_pdf.tex}


\subsection[Vgamma (NLO, sliced)]{\(V\gamma\) (NLO, sliced)}
%\label{sec:MB-sherpa-vgamma-nlo}

The descriptions below correspond to the samples in
\cref{tab:MB-sherpa-vynlo}.

\begin{table}[htbp]
  \caption{NLO \(V\gamma\) samples with \SHERPA.}%
  \label{tab:MB-sherpa-vynlo}
  \centering
  \begin{tabular}{l l}
    \toprule
    DSID range & Description \\
    \midrule
    364500--364535   & sliced in \pTX[\gamma]\\
    345887--345900   & sliced in \(m_{\ell\ell}\)\\
    \bottomrule
  \end{tabular}
\end{table}

\paragraph{Description:}

The production of \(V\gamma\) final states was simulated with the
\SHERPA[2.2.2]~\cite{Bothmann:2019yzt} generator.  Matrix elements at
NLO QCD accuracy for up to one additional parton and LO accuracy for
up to three additional parton emissions were matched and merged with
the \SHERPA parton shower based on Catani--Seymour
dipole factorisation~\cite{Gleisberg:2008fv,Schumann:2007mg} using the \MEPSatNLO
prescription~\cite{Hoeche:2011fd,Hoeche:2012yf,Catani:2001cc,Hoeche:2009rj}.
The virtual QCD corrections for matrix elements at NLO accuracy were
provided by the
\OPENLOOPS library~\cite{Buccioni:2019sur,Cascioli:2011va,Denner:2016kdg}. Samples
were generated using the \NNPDF[3.0nnlo] PDFset~\cite{Ball:2014uwa}, along with
the dedicated set of tuned parton-shower parameters developed by the
\SHERPA authors.


\paragraph{Additional description:}

The ME+PS matching~\cite{Hoeche:2011fd} was employed for different jet
multiplicities which were then merged into an inclusive sample
using an improved CKKW matching
procedure~\cite{Catani:2001cc,Hoeche:2009rj} which was extended to NLO
accuracy using the \MEPSatNLO prescription~\cite{Hoeche:2012yf}.
The virtual QCD corrections for matrix elements at NLO accuracy were
provided by the \OPENLOOPS library~\cite{Buccioni:2019sur,Cascioli:2011va,Denner:2016kdg}.
The calculation was performed in the \(G_\mu\) scheme, ensuring an optimal
description of pure electroweak interactions at the electroweak scale.

\input{sherpa_scale_pdf.tex}


\subsection[Vgamma (LO)]{\(V\gamma\) (LO)}
%\label{sec:MB-sherpa-vgamma-lo}

The descriptions below correspond to the samples in
\cref{tab:MB-sherpa-vylo}.

\begin{table}[htbp]
  \caption{LO \(V\gamma\) samples with \SHERPA.}%
  \label{tab:MB-sherpa-vylo}
  \centering
  \begin{tabular}{l l}
    \toprule
    DSID range & Description \\
    \midrule
    366140--366154   & \SHERPA[2.2.4], \(Z(\to ee/\mu\mu/\tau\tau)\gamma\), sliced in \pTX[\gamma]\\
    \bottomrule
  \end{tabular}
\end{table}

\paragraph{Description:}

The production of \(V\gamma\) final states was simulated with the
\SHERPA[2.2.4]~\cite{Bothmann:2019yzt} generator. Matrix elements at LO
accuracy in QCD for up to three additional parton emissions were
matched and merged with the \SHERPA parton shower based on
Catani--Seymour dipole factorisation~\cite{Gleisberg:2008fv,Schumann:2007mg}
using the \MEPSatLO
prescription~\cite{Hoeche:2011fd,Hoeche:2012yf,Catani:2001cc,Hoeche:2009rj}.
Samples were generated using the \NNPDF[3.0nnlo] PDF set~\cite{Ball:2014uwa},
along with the dedicated set of tuned parton-shower parameters
developed by the \SHERPA authors.


\paragraph{Additional description:}

The ME+PS matching~\cite{Hoeche:2011fd} was employed for different jet
multiplicities which were then merged into an inclusive sample using an improved CKKW matching
procedure~\cite{Catani:2001cc,Hoeche:2009rj}.
The calculation was performed in the \(G_\mu\) scheme, ensuring an optimal
description of pure electroweak interactions at the electroweak scale.

\input{sherpa_scale_pdf.tex}


\subsection{Tribosons (NLO)}
%\label{sec:MB-sherpa-vvv-nlo}

The descriptions below correspond to the samples in
\cref{tab:MB-sherpa-vvvnlo}.

\begin{table}[htbp]
  \caption{NLO \(VVV\) samples (factorised decays) with \SHERPA.}%
  \label{tab:MB-sherpa-vvvnlo}
  \centering
  \begin{tabular}{l l}
    \toprule
    DSID range & Description \\
    \midrule
    363507--363509   & \(3\ell1\nu2j\), \(4\ell2j\)\\
    364242--364249   & fully leptonic decays\\
    364336--364339   & \(WWW\to 2\ell2\nu jj\)\\
    \bottomrule
  \end{tabular}
\end{table}

\paragraph{Description:}

The production of triboson (\(VVV\)) events was simulated with the
\SHERPA[2.2.2]~\cite{Bothmann:2019yzt} generator using factorised gauge-boson decays.
Matrix elements, accurate to NLO for the inclusive process and to LO for up to
two additional parton emissions, were matched and merged with the \SHERPA parton
shower based on Catani--Seymour dipole factorisation~\cite{Gleisberg:2008fv,Schumann:2007mg}
using the \MEPSatNLO prescription~\cite{Hoeche:2011fd,Hoeche:2012yf,Catani:2001cc,Hoeche:2009rj}.
The virtual QCD corrections for matrix elements at NLO accuracy were
provided by the \OPENLOOPS library~\cite{Buccioni:2019sur,Cascioli:2011va,Denner:2016kdg}.
Samples were generated using the \NNPDF[3.0nnlo] PEF set~\cite{Ball:2014uwa}, along with
the dedicated set of tuned parton-shower parameters developed by the \SHERPA authors.


\paragraph{Additional description:}

The ME+PS matching~\cite{Hoeche:2011fd} was employed for different jet
multiplicities which were then merged into an inclusive sample
using an improved CKKW matching procedure~\cite{Catani:2001cc,Hoeche:2009rj} which is extended to NLO
accuracy using the \MEPSatNLO prescription~\cite{Hoeche:2012yf}.  The
calculation was performed in the \(G_\mu\) scheme, ensuring an optimal description of pure electroweak interactions at the
electroweak scale.

\input{sherpa_scale_pdf.tex}


\subsection{Tribosons (LO)}
%\label{sec:MB-sherpa-vvv-lo}

The descriptions below correspond to the samples in
\cref{tab:MB-sherpa-vvvlo}.

\begin{table}[htbp]
  \caption{LO \(VVV\) samples with \SHERPA.}%
  \label{tab:MB-sherpa-vvvlo}
  \centering
  \begin{tabular}{l l}
    \toprule
    DSID range & Description \\
    \midrule
    407311--407315   & on- and off-shell contributions to 6-lepton production\\
    \bottomrule
  \end{tabular}
\end{table}

\paragraph{Description:}

The production of triboson (\(VVV\)) events was simulated with the
\SHERPA[2.2.1]~\cite{Bothmann:2019yzt} generator. Matrix elements accurate to LO in QCD
for up to one additional parton emission were matched and merged with the \SHERPA parton shower based on Catani--Seymour
dipole factorisation~\cite{Gleisberg:2008fv,Schumann:2007mg} using the \MEPSatLO
prescription~\cite{Hoeche:2011fd,Hoeche:2012yf,Catani:2001cc,Hoeche:2009rj}.
Samples were generated using the \NNPDF[3.0nnlo] PDF set~\cite{Ball:2014uwa},
along with the dedicated set of tuned parton-shower parameters
developed by the \SHERPA authors.

\paragraph{Additional description:}

The ME+PS matching~\cite{Hoeche:2011fd} was employed for different jet
multiplicities which were then merged into an inclusive sample
using an improved CKKW matching
procedure~\cite{Catani:2001cc,Hoeche:2009rj}.  The calculation was
performed in the \(G_\mu\) scheme, ensuring an optimal description
of pure electroweak interactions at the electroweak scale.

\input{sherpa_scale_pdf.tex}


==> template/MC_snippets/MJ.tex <==
\chapter{Jet processes}
%\label{sec:MJ}

This section describes the MC samples used for the modelling of multijet production.
\Cref{subsec:jets-pythia} describes the \PYTHIA[8] samples,
\cref{subsec:jets-herwig} describes the \HERWIG[7] samples,
\cref{subsec:jets-powheg} describes the \POWPY[8] samples,
and finally \cref{subsec:jets-sherpa} describes the \SHERPA samples.

\section[Pythia 8]{\PYTHIA[8]}
\label{subsec:jets-pythia}

The descriptions below correspond to the samples in \cref{tab:mj_pythia}.

\begin{table}[!htbp]
  \caption{Nominal multijet samples produced with \PYTHIA.}%
  \label{tab:mj_pythia}
  \centering
  \begin{tabular}{l l}
    \toprule
    DSID range & Description \\
    \midrule
    364700--364712 & \PYTHIA with shower weights \\
    \bottomrule
  \end{tabular}
\end{table}

\paragraph{Description:}

Multijet production was generated using \PYTHIA[8.230]~\cite{Sjostrand:2014zea} with leading-order matrix elements
for dijet production which were matched to the parton shower.
%  supplemented by matrix element corrections (MEC) for the hardest
%  emission.

The renormalisation and factorisation scales were set to the geometric
mean of the squared transverse masses of the two outgoing particles in the matrix element,
\(\pTHatPythia = \sqrt{(\pTX[2][1] + m_1^2) (\pTX[2][2] + m_2^2)}\).
The \NNPDF[2.3lo] PDF set~\cite{Ball:2012cx} was used in
the ME generation, the parton shower, and the simulation of the
multi-parton interactions. The A14~\cite{ATL-PHYS-PUB-2014-021}
set of tuned parameters was used. Perturbative uncertainties were estimated
through event weights~\cite{Mrenna:2016sih} that encompass variations
of the scales at which the strong coupling constant is evaluated in
the initial- and final-state shower as well as the PDF uncertainty in
the shower and the non-singular part of the splitting functions.


\paragraph{Additional description:}

The modelling of fragmentation and
hadronisation was based on the Lund string
model~\cite{Andersson:1983ia,Sjostrand:1984ic}. To populate the
inclusive jet \pT spectrum efficiently, the sample used a biased
phase-space sampling which was compensated for by a continuously decreasing
weight for the event. Specifically, events at a scale
\pTHatPythia scale were oversampled by a factor of
\((\pTHatPythia/\SI{10}{\GeV})^4\).


\section[Herwig 7.1]{\HERWIG[7.1]}
\label{subsec:jets-herwig}

The descriptions below correspond to the samples in \cref{tab:mj_herwig}.

\begin{table}[!htbp]
  \caption{Multijet samples produced with \HERWIG[7].}%
  \label{tab:mj_herwig}
  \centering
  \begin{tabular}{l l}
    \toprule
    DSID range & Description \\
    \midrule
    364922--364929 & angular ordering in shower \HERWIG[7] \\
    364902--364909 & dipole shower \HERWIG[7] \\
    \bottomrule
  \end{tabular}
\end{table}

\paragraph{Description:}

Multijet production at next-to-leading order (NLO) was generated using \HERWIG[7.1.3]~\cite{Bellm:2017jjp}.
The renormalisation and factorisation scales were set to the \pT of the leading jet. The
\MMHT[nlo]~\cite{Harland-Lang:2014zoa} PDF set was used for the matrix element calculation.
Two sets of samples were generated, where one makes use of the default parton shower with angular ordering,
and the other uses the dipole shower as an alternative. The description of
hadronisation was based on the cluster model~\cite{Winter:2003tt} for both of these samples.
Two different samples with the same matrix elements and hadronisation allow the effects of using different
parton shower models to be investigated. These samples include variations from the hard scattering and shower.


\section[Powheg+Pythia8]{\POWPY[8]}
\label{subsec:jets-powheg}

The descriptions below correspond to the samples in \cref{tab:mj_powheg}.

\begin{table}[!htbp]
  \caption{Multijet samples produced with \POWHEGBOX[v2].}%
  \label{tab:mj_powheg}
  \centering
  \begin{tabular}{l l}
    \toprule
    DSID range & Description \\
    \midrule
    361281--361289 & \POWPY[8] \\
    \bottomrule
  \end{tabular}
\end{table}

\paragraph{Description:}

Alternative samples of multijet production at NLO accuracy were produced with \POWHEGBOX[v2]~\cite{Nason:2004rx, Frixione:2007vw}
interfaced to \PYTHIA[8]. These were generated with the dijet process as implemented in \POWHEGBOX[v2]~\cite{Alioli:2010xd}.
The \pT of the underlying Born configuration was taken as the renormalisation and factorisation scales
and the \NNPDF[3.0nlo]~\cite{Ball:2014uwa} parton distribution function (PDF) was used. \PYTHIA with the A14 tune and the
\NNPDF[2.3lo]~\cite{Ball:2012cx} PDF was used for the shower and multi-parton interactions.
These samples included per-event weight variations for different perturbative scales in the matrix element,
different parton distribution functions and their uncertainties, and the \PYTHIA perturbative
shower uncertainties.


\section[Sherpa 2.2]{\SHERPA[2.2]}
\label{subsec:jets-sherpa}

The descriptions below correspond to the samples in \cref{tab:mj_sherpa}.

\begin{table}[!htbp]
  \caption{Multijet samples produced with \SHERPA.}%
  \label{tab:mj_sherpa}
  \centering
  \begin{tabular}{l l}
    \toprule
    DSID range & Description \\
    \midrule
    364677--364685 & \SHERPA AHADIC \\
    364686--364694 & \SHERPA Lund \\
    \bottomrule
  \end{tabular}
\end{table}

\paragraph{Description:}

Multijet production samples were also generated using the \SHERPA[2.2.5]~\cite{Bothmann:2019yzt} generator.
The matrix element calculation was included for the \(2\rightarrow2\) process at leading order, and the default \SHERPA parton
shower~\cite{Schumann:2007mg} based on Catani--Seymour dipole factorisation was used for the showering with \pT
ordering, using the \CT[14nnlo] PDF set~\cite{Dulat:2015mca}.
The first of these samples made use of the dedicated \SHERPA AHADIC model for hadronisation~\cite{Winter:2003tt},
based on cluster fragmentation ideas. A second sample was generated with the same configuration but using the \SHERPA interface to
the Lund string fragmentation model of \PYTHIA[6]~\cite{Sjostrand:2006za} and its decay tables.
These two sets of samples were used to evaluate uncertainties stemming from the hadronisation modelling.

% need to comment on the slicing of these samples. JZ1 to JZ4 are JZW filtered to improve statistics for and an equal number of simulated events, while slices JZ9-JZ12 have been combined into a single JZ9 plus slice.


==> template/MC_snippets/Pileup.tex <==
\chapter{\Pileup overlay}

\paragraph{Description:}

The effect of multiple interactions in the same and neighbouring bunch
crossings (\pileup) was modelled by overlaying the simulated hard-scattering event with
inelastic proton--proton (\(pp\)) events generated with \PYTHIA[8.186]~\cite{Sjostrand:2007gs}
using the \NNPDF[2.3lo] set of parton distribution functions (PDF)~\cite{Ball:2012cx} and the
A3 set of tuned parameters~\cite{ATL-PHYS-PUB-2016-017}.

\paragraph{Optional description:}

The Monte Carlo (MC) events were weighted to reproduce the
distribution of the average number of interactions per bunch crossing
(\(\left<\mu \right>\)) observed in the data. The \(\left<\mu \right>\)
value in data was rescaled by a factor of \(1.03\pm 0.04\) to improve
agreement between data and simulation in the visible inelastic
proton--proton (\(pp\)) cross-section~\cite{STDM-2015-05}.



==> template/MC_snippets/RT.tex <==
\chapter{Rare top-quark processes}
%\label{sec:RT}

This chapter describes the samples used for rare top-quark processes.
\Cref{subsec:ttH} describes the \ttH\ samples.
\Cref{subsec:ttV} describes the \ttV\ (\(V=W/Z\)) samples.
\Cref{subsec:ttgamma} describes the \ttgamma\ samples.
\Cref{subsec:tHq} describes the \tH\ samples.
\Cref{subsec:tZq} describes the \tZq\ samples.
\Cref{subsec:tWZ} describes the \tWZ\ samples.
%\tgamma\ samples are described in \cref{subsec:tgamma}.
Finally, \cref{subsec:tttt} describes the \tttt\ samples.

\input{ttH}
\input{ttV}
\input{ttgamma}
\input{tHq}
\input{tHW}
\input{tZq}
\input{tWZ}
%\input{tgamma}
\input{tttt}


==> template/MC_snippets/TQ.tex <==
% !TEX root = MC_snippets.tex

\chapter{Top-quark processes}
%\label{sec:TQ}

This chapter describes the samples used for top-quark processes.
The \ttbar\ samples are described in \cref{subsec:ttbar}.
Single-top samples are described in \cref{subsec:tW} for \(tW\) associated production,
in \cref{subsec:tchan} for \(t\)-channel production,
and in \cref{subsec:schan} for \(s\)-channel production.
Finally, \ttHF\ samples are described in \cref{subsec:ttHF}.

\input{ttbar}
\input{sgtop}
\input{ttHF}


==> template/MC_snippets/sgtop.tex <==
% !TEX root = MC_snippets.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%              tW                     %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Single-top \texorpdfstring{\(tW\)}{tW} associated production}
\label{subsec:tW}

This section describes the MC samples used for the modelling of single-top \(tW\) associated production.
\Cref{subsubsec:tW_PP8} describes the \POWPY[8] samples -- both for the diagram removal (DR) set-ups,
which are used for the nominal prediction as well as uncertainties due to additional radiation and PDFs,
and for the diagram subtraction (DS) set-ups, which are used for the uncertainty due to the treatment
of the overlap with \ttbar production.
\Cref{subsubsec:tW_PH7} describes the \POWHER[7] samples used for the uncertainty
due to parton showering and hadronisation modelling, and \cref{subsubsec:tW_aMCP8} describes the
\MGNLOPY[8] samples used for the uncertainty due to the choice of matching scheme.

The reference cross-section values are extracted from Ref.~\cite{LHCTopWGsgtopXsec}.

\subsection[Powheg+Pythia8]{\POWPY[8]}
\label{subsubsec:tW_PP8}

\paragraph{Samples}
%\label{par:tW_PP8_samples}

\Cref{tab:tW_PP8} gives the DSIDs of the \(tW\) \POWPY[8] samples, for both the DR and DS schemes.
Single-top and single-anti-top (\(tW^-\) and \(\bar{t}W^+\)) events were generated in different samples.
The dileptonic samples overlap with the inclusive ones.

\begin{table}[htbp]
  \caption{Single-top \(tW\) associated production samples produced with \POWPY[8].}%
  \label{tab:tW_PP8}
  \centering
  \begin{tabular}{l l}
    \toprule
    DSID & Description \\
    \midrule
    410646 & \(tW^-\) (DR) inclusive \\
    410647 & \(\bar{t}W^+\) (DR) inclusive \\
    410648 & \(tW^-\) (DR) dileptonic \\
    410649 & \(\bar{t}W^+\) (DR) dileptonic \\
    \midrule
    410654 & \(tW^-\) (DS) inclusive \\
    410655 & \(\bar{t}W^+\) (DS) inclusive \\
    410656 & \(tW^-\) (DS) dileptonic \\
    410657 & \(\bar{t}W^+\) (DS) dileptonic \\
    \bottomrule
  \end{tabular}
\end{table}

\paragraph{Short description:}

The associated production of top quarks with \(W\) bosons (\(tW\)) was
modelled by the
\POWHEGBOX[v2]~\cite{Re:2010bp,Nason:2004rx,Frixione:2007vw,Alioli:2010xd}
generator at NLO in QCD using the five-flavour scheme and the
\NNPDF[3.0nlo] set of PDFs~\cite{Ball:2014uwa}.
The diagram removal scheme~\cite{Frixione:2008yi} was used to
remove interference and overlap with \ttbar production.
The related uncertainty was estimated by comparison with an alternative sample
generated using the diagram subtraction scheme~\cite{Frixione:2008yi,ATL-PHYS-PUB-2016-020}.\footnote{Analyses which do not use this approach
should obviously not use this sentence in their description.}
The events were interfaced to \PYTHIA[8.230]~\cite{Sjostrand:2014zea} using the A14
tune~\cite{ATL-PHYS-PUB-2014-021} and the \NNPDF[2.3lo] set of
PDFs~\cite{Ball:2012cx}.

\input{top_isrfsr_powpy_short}


\paragraph{Long description:}

Single-top \(tW\) associated production was modelled using the
\POWHEGBOX[v2]~\cite{Re:2010bp,Nason:2004rx,Frixione:2007vw,Alioli:2010xd}
generator, which provided matrix elements at next-to-leading
order~(NLO) in the strong coupling constant \alphas\ in the five-flavour
scheme with the \NNPDF[3.0nlo]~\cite{Ball:2014uwa} parton
distribution function~(PDF) set.  The functional form of the
renormalisation and factorisation scales was set to the default scale,
which is equal to the top-quark mass (\(\mtop = \SI{172.5}{\GeV}\)).
The diagram removal scheme~\cite{Frixione:2008yi} was employed to handle the interference
with \ttbar production~\cite{ATL-PHYS-PUB-2016-020}.  The events were
interfaced with \PYTHIA[8.230]~\cite{Sjostrand:2014zea} using the A14
tune~\cite{ATL-PHYS-PUB-2014-021} and the \NNPDF[2.3lo] PDF set.  The
decays of bottom and charm hadrons were simulated using the
\EVTGEN[1.6.0] program~\cite{Lange:2001uf}.

The inclusive cross-section was corrected to the theory prediction
calculated at NLO in QCD with NNLL soft-gluon
corrections~\cite{Kidonakis:2010ux,Kidonakis:2013zqa}.  For proton--proton
collisions at a centre-of-mass energy of \(\rts = \SI{13}{\TeV}\), this
cross-section corresponds to \(\sigma(tW)_{\text{NLO+NNLL}} = 71.7 \pm 3.8\,\si{\pb}\),
using a top-quark mass of \(\mtop = \SI{172.5}{\GeV}\).  The uncertainty in
the cross-section due to the PDF was calculated using the \MSTW[nnlo] 90\%
CL~\cite{Martin:2009iq,Martin:2009bu} PDF set, and was added in
quadrature to the effect of the scale uncertainty.

\input{top_isrfsr_powpy_long}

The nominal \POWPY[8] sample was compared with an alternative
sample generated using the diagram subtraction
scheme~\cite{Frixione:2008yi,ATL-PHYS-PUB-2016-020} to estimate the
uncertainty arising from the interference with \ttbar production.

To evaluate the PDF uncertainties for the nominal PDF, the 100
variations for \NNPDF[3.0nlo] were taken into account.
In addition, the central value of this PDF was compared with the
central values of the \CT[14nnlo]~\cite{Dulat:2015mca} and
\MMHT[nnlo]~\cite{Harland-Lang:2014zoa} PDF sets.


\subsection[Powheg+Herwig7]{\POWHER[7]}
\label{subsubsec:tW_PH7}

\paragraph{Samples}
%\label{par:tW_PH7_samples}

\Cref{tab:tW_PH7} gives the DSIDs of the \(tW\) \POWHER[7] DR samples.
Single-top and single-anti-top (\(tW^-\) and \(\bar{t}W^+\)) events were generated in different samples.
The dileptonic samples overlap with the inclusive ones.

\begin{table}[htbp]
  \caption{Single-top \(tW\) associated production samples produced with \POWHER[7].}%
  \label{tab:tW_PH7}
  \centering
  \begin{tabular}{l l}
    \toprule
    DSID & Description \\
    \midrule
    411036 & \(tW^-\) (DR) inclusive \\
    411037 & \(\bar{t}W^+\) (DR) inclusive \\
    411038 & \(tW^-\) (DR) dileptonic \\
    411039 & \(\bar{t}W^+\) (DR) dileptonic \\
    \bottomrule
  \end{tabular}
\end{table}

\paragraph{Short description:}

The uncertainty due to the parton shower and hadronisation model was
evaluated by comparing the nominal sample of events with a sample where
events generated with the
\POWHEGBOX[v2]~\cite{Re:2010bp,Nason:2004rx,Frixione:2007vw,Alioli:2010xd}
generator were interfaced to
\HERWIG[7.04]~\cite{Bahr:2008pv,Bellm:2015jjp}, using the H7UE set
of tuned parameters~\cite{Bellm:2015jjp} and the \MMHT[lo] PDF set~\cite{Harland-Lang:2014zoa}.


\paragraph{Long description:}

The impact of using a different parton shower and hadronisation model was evaluated
by comparing the nominal \(tW\) sample with another sample produced with the
\POWHEGBOX[v2]~\cite{Re:2010bp,Nason:2004rx,Frixione:2007vw,Alioli:2010xd}
generator but interfaced with \HERWIG[7.04]~\cite{Bahr:2008pv,Bellm:2015jjp},
using the H7UE set of tuned parameters~\cite{Bellm:2015jjp} and the
\MMHT[lo] PDF set \cite{Harland-Lang:2014zoa}.
\POWHEGBOX provided matrix elements at next-to-leading order~(NLO) in the
strong coupling constant \alphas in the five-flavour scheme with the
\NNPDF[3.0nlo]~\cite{Ball:2014uwa} parton distribution function~(PDF).
The functional form of the renormalisation and factorisation scales was set to
the default scale, which is equal to the top-quark mass.  The diagram removal
scheme~\cite{Frixione:2008yi} was employed to handle the interference
with \ttbar production~\cite{ATL-PHYS-PUB-2016-020}.  The decays of bottom
and charm hadrons are simulated using the \EVTGEN[1.6.0]
program~\cite{Lange:2001uf}.


\subsection[MadGraph5\_aMC@NLO+Pythia8]{\MGNLOPY[8]}
\label{subsubsec:tW_aMCP8}

\paragraph{Samples}
%\label{par:tW_aMCP8_samples}

\Cref{tab:tW_aMCP8} gives the DSIDs of the \(tW\) \MGNLOPY[8] samples.
The dileptonic sample overlaps with the inclusive one.

\begin{table}[htbp]
  \caption{Single-top \(tW\) associated production samples produced with \MGNLOPY[8].}%
  \label{tab:tW_aMCP8}
  \centering
  \begin{tabular}{l l}
    \toprule
    DSID & Description \\
    \midrule
    412002 & \(tW\) inclusive \\
    412003 & \(tW\) dileptonic \\
    \bottomrule
  \end{tabular}
\end{table}

\paragraph{Short description:}

To assess the uncertainty in the matching of NLO matrix elements to the
parton shower, the nominal \(tW\) sample was compared with a sample generated
with the \MGNLO[2.6.2]~\cite{Alwall:2014hca} generator at NLO in QCD using the five-flavour
scheme and the \NNPDF[2.3nlo]~\cite{Ball:2014uwa} PDF set. The events were
interfaced with \PYTHIA[8.230]~\cite{Sjostrand:2014zea}, using the A14
set of tuned parameters~\cite{ATL-PHYS-PUB-2014-021} and the \NNPDF[2.3lo]
PDF.


\paragraph{Long description:}

To assess the uncertainty due to the choice of matching scheme, the nominal \(tW\) sample was compared with a sample generated
with the \MGNLO[2.6.2]~\cite{Alwall:2014hca} generator, which provided matrix elements at next-to-leading order~(NLO) in the strong coupling constant \alphas
in the five-flavour scheme, using the \NNPDF[2.3nlo]~\cite{Ball:2014uwa} PDF set.
The functional form of the renormalisation and factorisation scale was set to the default scale, which is equal to the top-quark mass.
The parton-shower starting scale had the functional form \(\muQ = \HT/2\)~\cite{ATL-PHYS-PUB-2017-007},
where \HT is defined as the scalar sum of the \pT of all outgoing partons.
The diagram removal scheme~\cite{Frixione:2008yi} was employed to handle the interference with \ttbar production~\cite{ATL-PHYS-PUB-2016-020}.
The events were interfaced with \PYTHIA[8.230]~\cite{Sjostrand:2014zea}, using the A14 set of tuned parameters~\cite{ATL-PHYS-PUB-2014-021}
and the \NNPDF[2.3lo] PDF.
The decays of bottom and charm hadrons were simulated using the \EVTGEN[1.6.0] program~\cite{Lange:2001uf}.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%              t-channel              %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Single-top \texorpdfstring{\(t\)}{t}-channel production}
\label{subsec:tchan}

This section describes the MC samples used for the modelling of single-top \(t\)-channel production.
\Cref{subsubsec:tchan_PP8} describes the \POWPY[8] samples used for the nominal prediction
and for the uncertainty from additional radiation and due to PDFs.
\Cref{subsubsec:tchan_PH7} describes the \POWHER[7] samples used for the uncertainty due to the choice of parton shower and hadronisation model,
and \cref{subsubsec:tchan_aMCP8} describes the \MGNLOPY[8] samples used for the uncertainty due to the choice of matching scheme.

The reference cross-section values are extracted from Ref.~\cite{LHCTopWGsgtopXsec}.


\subsection[Powheg+Pythia8]{\POWPY[8]}
\label{subsubsec:tchan_PP8}

\paragraph{Samples}
%\label{par:tchan_PP8_samples}

\Cref{tab:tchan_PP8} gives the DSIDs of the \(t\)-channel \POWPY[8] samples.
Single-top and single-anti-top events were generated in distinct samples.

\begin{table}[!htbp]
  \caption{Single-top \(t\)-channel event samples produced with \POWPY[8].}%
  \label{tab:tchan_PP8}
  \centering
  \begin{tabular}{l l}
    \toprule
    DSID & Description \\
    \midrule
    410658 & \(t\)-channel \(t\) leptonic \\
    410659 & \(t\)-channel \(\bar{t}\) leptonic \\
    \bottomrule
  \end{tabular}
\end{table}

\paragraph{Short description:}

Single-top \(t\)-channel production was modelled using the
\POWHEGBOX[v2]~\cite{Frederix:2012dh,Nason:2004rx,Frixione:2007vw,Alioli:2010xd}
generator at NLO in QCD using the four-flavour scheme and the
corresponding \NNPDF[3.0nlo] set of PDFs~\cite{Ball:2014uwa}.  The events were
interfaced with \PYTHIA[8.230]~\cite{Sjostrand:2014zea} using the A14
tune~\cite{ATL-PHYS-PUB-2014-021} and the \NNPDF[2.3lo] set of
PDFs~\cite{Ball:2012cx}.

\input{top_isrfsr_powpy_short}


\paragraph{Long description:}

Single-top \(t\)-channel production was modelled using the
\POWHEGBOX[v2]~\cite{Frederix:2012dh,Nason:2004rx,Frixione:2007vw,Alioli:2010xd}
generator, which provided matrix elements at next-to-leading-order~(NLO)
accuracy in the strong coupling constant \alphas\ in the four-flavour
scheme with the corresponding \NNPDF[3.0nlo]~\cite{Ball:2014uwa} parton
distribution function~(PDF) set.  The functional form of the
renormalisation and factorisation scales was set to
\(\sqrt{m_b^2 + \pTX[2][b]}\) following the
recommendation of Ref.~\cite{Frederix:2012dh}. Top quarks were decayed at
LO using \MADSPIN~\cite{Frixione:2007zp,Artoisenet:2012st} to preserve
all spin correlations.  The events were interfaced with
\PYTHIA[8.230]~\cite{Sjostrand:2014zea} using the A14
tune~\cite{ATL-PHYS-PUB-2014-021} and the \NNPDF[2.3lo] PDF set.
The decays of bottom and charm hadrons were simulated using the
\EVTGEN[1.6.0] program~\cite{Lange:2001uf}.

The inclusive cross-section was corrected to the theory prediction calculated at NLO in QCD with
\HATHOR[2.1]~\cite{Aliev:2010zk,Kant:2014oha}.
For proton--proton collisions at a centre-of-mass energy of \(\rts = \SI{13}{\TeV}\), this cross-section corresponds to
\(\sigma(t,t\text{-chan})_\text{NLO}= 136.02^{+5.40}_{-4.57}\)\,pb (\(\sigma(\bar{t},t\text{-chan})_\text{NLO}=80.95^{+4.06}_{-3.61}\)\,pb)
for single-top (single-anti-top) production, using a top-quark mass of \(\mtop = \SI{172.5}{\GeV}\).
The uncertainties in the cross-section due to the PDF and \alphas were calculated using the \PDFforLHC prescription~\cite{Butterworth:2015oua}
with the \MSTW[nlo] 68\% CL~\cite{Martin:2009iq,Martin:2009bu}, \CT[10nlo]~\cite{Lai:2010vv}
and \NNPDF[2.3nlo]~\cite{Ball:2012cx} PDF sets,
and were added in quadrature to the effect of the scale uncertainty.

\input{top_isrfsr_powpy_long}

To evaluate the PDF uncertainties for the nominal PDF, the 100 variations for \NNPDF[3.0nlo] were taken into account.
In addition, the central value of this PDF was compared with the central values of the \CT[14nnlo]~\cite{Dulat:2015mca}
and \MMHT[nnlo]~\cite{Harland-Lang:2014zoa} PDF sets.


\subsection[Powheg+Herwig7]{\POWHER[7]}
\label{subsubsec:tchan_PH7}

\paragraph{Samples}
%\label{par:tchan_PH7_samples}

\Cref{tab:tchan_PH7} gives the DSIDs of the \(t\)-channel \POWHER[7] samples.
Single-top and single-anti-top events were generated in distinct samples.

\begin{table}[htbp]
  \caption{Single-top \(t\)-channel event samples produced with \POWHER[7].}%
  \label{tab:tchan_PH7}
  \centering
  \begin{tabular}{l l}
    \toprule
    DSID & Description \\
    \midrule
    411032 & \(t\)-channel \(\bar t\) leptonic \\
    411033 & \(t\)-channel \(t\) leptonic \\
    \bottomrule
  \end{tabular}
\end{table}

\paragraph{Short description:}

The uncertainty due to the parton shower and hadronisation model was
evaluated by comparing the nominal sample of events with a sample where
the events generated with the
\POWHEGBOX[v2]~\cite{Frederix:2012dh,Nason:2004rx,Frixione:2007vw,Alioli:2010xd}
generator were interfaced to
\HERWIG[7.04]~\cite{Bahr:2008pv,Bellm:2015jjp}, using the H7UE set
of tuned parameters~\cite{Bellm:2015jjp} and the \MMHT[lo] PDF set
\cite{Harland-Lang:2014zoa}.


\paragraph{Long description:}

The impact of using a different parton shower and hadronisation model was evaluated by comparing the nominal sample
with another sample produced with the \POWHEGBOX[v2]~\cite{Frederix:2012dh,Nason:2004rx,Frixione:2007vw,Alioli:2010xd}
generator but interfaced with \HERWIG[7.04]~\cite{Bahr:2008pv,Bellm:2015jjp}, using the H7UE set of
tuned parameters~\cite{Bellm:2015jjp} and the \MMHT[lo] PDF set \cite{Harland-Lang:2014zoa}.
\POWHEGBOX provided matrix elements at next-to-leading order~(NLO) in the strong coupling constant \alphas
in the four-flavour scheme with the corresponding \NNPDF[3.0nlo]~\cite{Ball:2014uwa} parton distribution function~(PDF).
The functional form of the renormalisation and factorisation scales was set to \(\sqrt{m_b^2 + \pTX[2][b]}\)
following the recommendation of Ref.~\cite{Frederix:2012dh}.
Top quarks were decayed at LO using \MADSPIN~\cite{Frixione:2007zp,Artoisenet:2012st} to preserve all spin correlations.
The decays of bottom and charm hadrons were simulated using the \EVTGEN[1.6.0] program~\cite{Lange:2001uf}.


\subsection[MadGraph5\_aMC@NLO+Pythia8]{\MGNLOPY[8]}
\label{subsubsec:tchan_aMCP8}

\paragraph{Samples}
%\label{par:tchan_aMCP8_samples}

\Cref{tab:tchan_aMCP8} gives the DSIDs of the \(t\)-channel \MGNLOPY[8] samples.

\begin{table}[htbp]
  \caption{Single-top \(t\)-channel event samples produced with \MGNLOPY[8].}%
  \label{tab:tchan_aMCP8}
  \centering
  \begin{tabular}{l l}
    \toprule
    DSID & Description \\
    \midrule
    412004 & \(t\)-channel leptonic \\
    \bottomrule
  \end{tabular}
\end{table}

\paragraph{Short description:}

To assess the uncertainty in the matching of NLO matrix elements to the
parton shower, the nominal sample was compared with a sample generated
with the \MGNLO[2.6.2]~\cite{Alwall:2014hca} generator at NLO in QCD using the five-flavour
scheme and the \NNPDF[2.3nlo]~\cite{Ball:2014uwa} PDF set. The events were
interfaced with \PYTHIA[8.230]~\cite{Sjostrand:2014zea}, using the A14
set of tuned parameters~\cite{ATL-PHYS-PUB-2014-021} and the \NNPDF[2.3lo] PDF set.


\paragraph{Long description:}

To assess the uncertainty due to the choice of matching scheme, the nominal sample was compared with a sample generated
with the \MGNLO[2.6.2]~\cite{Alwall:2014hca} generator, which provided matrix elements at next-to-leading order~(NLO) in the strong coupling constant \alphas
in the four-flavour scheme, using the corresponding \NNPDF[3.0nlo]~\cite{Ball:2014uwa} PDF set.
The functional form of the renormalisation and factorisation scales was set to \(\sqrt{m_b^2 + \pTX[2][b]}\)
following the recommendation of Ref.~\cite{Frederix:2012dh}.
The parton-shower starting scale had the functional form \(\muQ = \HT/2\)~\cite{ATL-PHYS-PUB-2017-007},
where \HT is defined as the scalar sum of the \pT of all outgoing partons.
Top quarks were decayed at LO using \MADSPIN~\cite{Frixione:2007zp,Artoisenet:2012st} to preserve all spin correlations.
The events were interfaced with \PYTHIA[8.230]~\cite{Sjostrand:2014zea}, using the A14 set of tuned parameters~\cite{ATL-PHYS-PUB-2014-021}
and the \NNPDF[2.3lo] PDF set.
The decays of bottom and charm hadrons were simulated using the \EVTGEN[1.6.0] program~\cite{Lange:2001uf}.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%              s-channel              %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Single-top \texorpdfstring{\(s\)}{s}-channel production}
\label{subsec:schan}

This section describes the MC samples used for the modelling of single-top \(s\)-channel production.
\Cref{subsubsec:schan_PP8} describes the \POWPY[8] samples used for the nominal prediction
and for the uncertainty from additional radiation and due to PDFs.
\Cref{subsubsec:schan_PH7} describes the \POWHER[7] samples used for the uncertainty due to the parton shower and hadronisation model,
and \cref{subsubsec:schan_aMCP8} describes the \MGNLOPY[8] samples used for the uncertainty due to the choice of matching scheme.

The reference cross-section values are extracted from Ref.~\cite{LHCTopWGsgtopXsec}.

\subsection[Powheg+Pythia8]{\POWPY[8]}
\label{subsubsec:schan_PP8}

\paragraph{Samples}
%\label{par:schan_PP8_samples}

\Cref{tab:schan_PP8} gives the DSIDs of the \(s\)-channel \POWPY[8] samples.
Single-top and single-anti-top events were generated in distinct samples.

\begin{table}[htbp]
  \caption{Single-top \(s\)-channel event samples produced with \POWPY[8].}%
  \label{tab:schan_PP8}
  \centering
  \begin{tabular}{l l}
    \toprule
    DSID & Description \\
    \midrule
    410644 & \(s\)-channel \(t\) leptonic \\
    410645 & \(s\)-channel \(\bar{t}\) leptonic \\
    \bottomrule
  \end{tabular}
\end{table}

\paragraph{Short description:}

Single-top \(s\)-channel production was modelled using the \POWHEGBOX[v2]~\cite{Alioli:2009je,Nason:2004rx,Frixione:2007vw,Alioli:2010xd}
generator at NLO in QCD in the five-flavour scheme with the \NNPDF[3.0nlo]~\cite{Ball:2014uwa} parton distribution function~(PDF) set.
The events were interfaced with \PYTHIA[8.230]~\cite{Sjostrand:2014zea} using the A14 tune~\cite{ATL-PHYS-PUB-2014-021} and the
\NNPDF[2.3lo] PDF set.

\input{top_isrfsr_powpy_short}


\paragraph{Long description:}

Single-top \(s\)-channel production was modelled using the \POWHEGBOX[v2]~\cite{Alioli:2009je,Nason:2004rx,Frixione:2007vw,Alioli:2010xd}
generator, which provided matrix elements at next-to-leading order~(NLO) in the strong coupling constant \alphas in the
five-flavour scheme with the \NNPDF[3.0nlo]~\cite{Ball:2014uwa} parton distribution function~(PDF) set.
The functional form of the renormalisation and factorisation scales was set to the default scale, which was equal to the top-quark mass.
The events were interfaced with \PYTHIA[8.230]~\cite{Sjostrand:2014zea} using the A14 tune~\cite{ATL-PHYS-PUB-2014-021} and the
\NNPDF[2.3lo] PDF set.
The decays of bottom and charm hadrons were simulated using the \EVTGEN[1.6.0] program~\cite{Lange:2001uf}.

The inclusive cross-section was corrected to the theory prediction calculated at NLO in QCD with
\HATHOR[2.1]~\cite{Aliev:2010zk,Kant:2014oha}.
For proton--proton collisions at a centre-of-mass energy of \(\rts = \SI{13}{\TeV}\), this cross-section corresponds to
\(\sigma(t,s\text{-chan})_{\text{NLO}} = 6.35^{+0.23}_{-0.20}\,\si{\pb}\)
(\(\sigma(\bar{t},s\text{-chan})_{\text{NLO}} = 3.97^{+0.19}_{-0.17}\,\si{\pb}\))
for single-top (single-anti-top) production, using a top-quark mass of \(\mtop = \SI{172.5}{\GeV}\).
The uncertainties in the cross-section due to the PDF and \alphas were calculated using the \PDFforLHC prescription~\cite{Butterworth:2015oua}
with the \MSTW[nlo] 68\% CL~\cite{Martin:2009iq,Martin:2009bu}, \CT[10nlo]~\cite{Lai:2010vv} and \NNPDF[2.3nlo]~\cite{Ball:2012cx} PDF sets,
and were added in quadrature to the effect of the scale uncertainty.

\input{top_isrfsr_powpy_long}

To evaluate the PDF uncertainties for the nominal PDF, the 100 variations for \NNPDF[3.0nlo] were taken into account.
In addition, the central value of this PDF was compared with the central values of the
\CT[14nnlo]~\cite{Dulat:2015mca} and \MMHT[nnlo]~\cite{Harland-Lang:2014zoa} PDF sets.


\subsection[Powheg+Herwig7]{\POWHER[7]}
\label{subsubsec:schan_PH7}

\paragraph{Samples}
%\label{par:schan_PH7_samples}

\Cref{tab:schan_PH7} gives the DSIDs of the \(s\)-channel \POWHER[7] samples.
Single-top and single-anti-top events were generated in distinct samples.

\begin{table}[htbp]
  \caption{Single-top \(s\)-channel event samples produced with \POWHER[7].}%
  \label{tab:schan_PH7}
  \centering
  \begin{tabular}{l l}
    \toprule
    DSID & Description \\
    \midrule
    411034 & \(s\)-channel \(t\) leptonic \\
    411035 & \(s\)-channel \(\bar{t}\) leptonic \\
    \bottomrule
  \end{tabular}
\end{table}

\paragraph{Short description:}

The impact of using a different parton shower and hadronisation model was evaluated by comparing the nominal sample
with another sample produced with the \POWHEGBOX[v2]~\cite{Alioli:2009je,Nason:2004rx,Frixione:2007vw,Alioli:2010xd}
generator at NLO in the strong coupling constant \alphas in the five-flavour scheme using the
\NNPDF[3.0nlo]~\cite{Ball:2014uwa} parton distribution function~(PDF).
Events in the latter sample were interfaced with \HERWIG[7.04]~\cite{Bahr:2008pv,Bellm:2015jjp}, using the H7UE set of
tuned parameters~\cite{Bellm:2015jjp} and the \MMHT[lo] PDF set \cite{Harland-Lang:2014zoa}.


\paragraph{Long description:}

The impact of using a different parton shower and hadronisation model was evaluated by comparing the nominal sample
with another sample produced with the \POWHEGBOX[v2]~\cite{Alioli:2009je,Nason:2004rx,Frixione:2007vw,Alioli:2010xd}
generator but interfaced with \HERWIG[7.04]~\cite{Bahr:2008pv,Bellm:2015jjp}, using the H7UE set of
tuned parameters~\cite{Bellm:2015jjp} and the \MMHT[lo] PDF set \cite{Harland-Lang:2014zoa}.
\POWHEGBOX provided matrix elements at next-to-leading order~(NLO) in the strong coupling constant \alphas
in the five-flavour scheme with the \NNPDF[3.0nlo]~\cite{Ball:2014uwa} parton distribution function~(PDF).
The functional form of the renormalisation and factorisation scales was set to the default scale, which is equal to the top-quark mass.
The decays of bottom and charm hadrons were simulated using the \EVTGEN[1.6.0] program~\cite{Lange:2001uf}.


\subsection[MadGraph5\_aMC@NLO+Pythia8]{\MGNLOPY[8]}
\label{subsubsec:schan_aMCP8}

\paragraph{Samples}
%\label{par:schan_aMCP8_samples}

\Cref{tab:schan_aMCP8} gives the DSIDs of the \(s\)-channel \MGNLOPY[8] samples.

\begin{table}[htbp]
  \caption{Single-top \(s\)-channel event samples produced with \MGNLOPY[8].}%
  \label{tab:schan_aMCP8}
  \centering
  \begin{tabular}{l l}
    \toprule
    DSID & Description \\
    \midrule
    412005 & \(s\)-channel leptonic \\
    \bottomrule
  \end{tabular}
\end{table}

\paragraph{Short description:}

%% the MG5_aMC@NLO version was double checked in the tag collector
To assess the uncertainty due to the choice of matching scheme, the nominal sample was compared with a sample generated
with the \MGNLO[2.6.2]~\cite{Alwall:2014hca} generator at NLO in the strong coupling constant \alphas in the five-flavour scheme,
using the \NNPDF[3.0nlo]~\cite{Ball:2014uwa} PDF set.
The events were interfaced with \PYTHIA[8.230]~\cite{Sjostrand:2014zea}, using the A14 set of tuned parameters~\cite{ATL-PHYS-PUB-2014-021}
and the \NNPDF[2.3lo] PDF set.


\paragraph{Long description:}

To assess the uncertainty due to the choice of matching scheme, the nominal sample was compared with a sample generated
with the \MGNLO[2.6.2]~\cite{Alwall:2014hca} generator, which provided matrix elements at next-to-leading order~(NLO) in the strong coupling constant \alphas
in the five-flavour scheme with the \NNPDF[3.0nlo]~\cite{Ball:2014uwa} parton distribution function~(PDF).
The functional form of the renormalisation and factorisation scales was set to the default scale, which is equal to the top-quark mass.
The parton-shower starting scale had the functional form \(\muQ = \HT/2\)~\cite{ATL-PHYS-PUB-2017-007},
where \HT is defined as the scalar sum of the \pT of all outgoing partons.
Top quarks were decayed at LO using \MADSPIN~\cite{Frixione:2007zp,Artoisenet:2012st} to preserve all spin correlations.
The events were interfaced with \PYTHIA[8.230]~\cite{Sjostrand:2014zea}, using the A14 set of tuned parameters~\cite{ATL-PHYS-PUB-2014-021}
and the \NNPDF[2.3lo] PDF set.
The decays of bottom and charm hadrons were simulated using the \EVTGEN[1.6.0] program~\cite{Lange:2001uf}.


==> template/MC_snippets/sherpa_scale_pdf.tex <==
Uncertainties from missing higher orders were
evaluated~\cite{Bothmann:2016nao} using seven variations of the QCD
factorisation and renormalisation scales in the matrix elements by
factors of \(0.5\) and \(2\), avoiding variations in opposite directions.

Uncertainties in the nominal PDF set were evaluated using 100 replica
variations. Additionally, the results were cross-checked using the
central values of the \CT[14nnlo]~\cite{Dulat:2015mca} and
\MMHT[nnlo]~\cite{Harland-Lang:2014zoa} PDF sets. The effect of the uncertainty
in the strong coupling constant \(\alphas\) was assessed by variations of \(\pm 0.001\).






==> template/MC_snippets/tHW.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%              tHW                    %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section[\tHW]{\tHW}
\label{subsec:tHW}

This section describes the MC samples used for the modelling of \tHW\ production.
\Cref{subsubsec:tHW_aMCP8} describes the \MGNLOPY[8] samples.

\subsection[MadGraph5\_aMC@NLO+Pythia8]{\MGNLOPY[8]}
\label{subsubsec:tHW_aMCP8}

\paragraph{Samples}

The descriptions below correspond to the samples in \cref{tab:tHW_aMCP8}.

\begin{table}
  \caption{Nominal \tHW\ samples produced with \MGNLOPY[8].}%
  \label{tab:tHW_aMCP8}
  \centering
  \begin{tabular}{l l}
    \toprule
    DSID & Description \\
    \midrule
    346486 & \tHW\, \Hgg\ \\
    346511 & \tHW\, \Hllll \\
    346678 & \tHW\, \(H\rightarrow\) inclusive, UFO model \\
    346759 & \tHW\, \Hgg{}, UFO model \\
    \bottomrule
  \end{tabular}
\end{table}

\paragraph{Short description:}

The \tHW{} production is modelled using the \MGNLO[2.6.2]~\cite{Alwall:2014hca} generator at NLO with the \NNPDF[3.0nlo]~\cite{Ball:2014uwa} parton distribution function~(PDF). The overlap with the \ttH{} production is removed using the diagram removal scheme~\cite{Frixione:2008yi,Demartin:2016axk}. The events are interfaced with \PYTHIA[8.235]~\cite{Sjostrand:2014zea} using the A14 parameter set~\cite{ATL-PHYS-PUB-2014-021} and the \NNPDF[2.3lo]~\cite{Ball:2014uwa} PDF set.
The decays of bottom and charm hadrons are simulated using the \EVTGEN[1.6.0] program~\cite{Lange:2001uf}.


\paragraph{Long description:}

The \tHW{} samples were simulated using the \MGNLO[2.6.2]~\cite{Alwall:2014hca}
generator at NLO with the \NNPDF[3.0nlo]~\cite{Ball:2014uwa} parton distribution function~(PDF). The events were interfaced with
\PYTHIA[8.235]~\cite{Sjostrand:2014zea}~ using the A14 tune~\cite{ATL-PHYS-PUB-2014-021} and the \NNPDF[2.3lo]~\cite{Ball:2014uwa} PDF set.
The top quark was decayed at LO using \MADSPIN~\cite{Frixione:2007zp,Artoisenet:2012st} to preserve spin correlations,
whereas the Higgs boson was decayed by \PYTHIA in the parton shower. The samples
were generated in the five-flavour scheme.
The functional form of the renormalisation and factorisation scales was set to the
default scale \(0.5\times \sum_i \sqrt{m^2_i+p^2_{\text{T},i}}\), where the sum runs over
all the particles generated from the matrix element calculation.
The decays of bottom and charm hadrons were simulated using the \EVTGEN[1.6.0] program~\cite{Lange:2001uf}.


==> template/MC_snippets/tHq.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%              tH                    %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section[\tHq]{\tHq}
\label{subsec:tHq}

This section describes the MC samples used for the modelling of \tH\ production.
\Cref{subsubsec:tHq_aMCP8} describes the \MGNLOPY[8] samples,

\subsection[MadGraph5\_aMC@NLO+Pythia8]{\MGNLOPY[8]}
\label{subsubsec:tHq_aMCP8}

\paragraph{Samples}
%\label{par:tHq_aMCP8_samples}

The descriptions below correspond to the samples in \cref{tab:tHq_aMCP8}.

\begin{table}[htbp]
  \caption{Nominal \tH\ samples produced with \MGNLOPY[8].}%
  \label{tab:tHq_aMCP8}
  \centering
  \begin{tabular}{l l}
    \toprule
    DSID range & Description \\
    \midrule
    346188 & \tHq\, \Hgg\, four flavour \\
    346229 & \tHq\, \Hbb\, four flavour \\
    346230 & \tHq\, \Htautau/\HZZ/\HWW\, four flavour \\
    346414 & \tHq\, \Hllll, four flavour \\
    \midrule
    346676 & \tHq\, \(H\rightarrow\) inclusive, four flavour, UFO model \\
    346677 & \tHq\, \Hgg, four flavour, UFO model \\
    346799 & \tHq\, \Htautau/\HZZ/\HWW\ + Nleptons=2 filter, four flavour, UFO model \\
    \bottomrule
  \end{tabular}
\end{table}

\paragraph{Exceptions:}
If and only if you are using the UFO model sample: the correct version is \MGNLO[2.6.2].

\paragraph{Short description:}

The production of \tHq events was modelled using the \MGNLO[2.6.0]~\cite{Alwall:2014hca}
generator at NLO with the \NNPDF[3.0nlo]~\cite{Ball:2014uwa} parton distribution function~(PDF).
The events were interfaced with \PYTHIA[8.230]~\cite{Sjostrand:2014zea} using the A14 tune~\cite{ATL-PHYS-PUB-2014-021} and the
\NNPDF[2.3lo]~\cite{Ball:2014uwa} PDF set.
The decays of bottom and charm hadrons were simulated using the \EVTGEN[1.6.0] program~\cite{Lange:2001uf}.


\paragraph{Long description:}

The \tHq samples were simulated using the \MGNLO[2.6.0]~\cite{Alwall:2014hca}
generator at NLO with the \NNPDF[3.0nlo]~\cite{Ball:2014uwa} parton distribution function~(PDF). The events were interfaced with
\PYTHIA[8.230]~\cite{Sjostrand:2014zea}~ using the A14 tune~\cite{ATL-PHYS-PUB-2014-021} and the \NNPDF[2.3lo]~\cite{Ball:2014uwa} PDF set.
The top quark was decayed at LO using \MADSPIN~\cite{Frixione:2007zp,Artoisenet:2012st} to preserve spin correlations,
whereas the Higgs boson was decayed by \PYTHIA in the parton shower. The samples
were generated in the four-flavour scheme.
The functional form of the renormalisation and factorisation scales was set to the
default scale \(0.5\times \sum_i \sqrt{m^2_i+p^2_{\text{T},i}}\), where the sum runs over
all the particles generated from the matrix element calculation.
The decays of bottom and charm hadrons were simulated using the \EVTGEN[1.6.0] program~\cite{Lange:2001uf}.


==> template/MC_snippets/tWZ.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%              tWZ                    %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section[\tWZ]{\tWZ}
\label{subsec:tWZ}

This section describes the MC samples used for the modelling of \tWZ\ production.
\Cref{subsubsec:tWZ_aMCP8} describes the \MGNLOPY[8] samples,

\subsection[MadGraph5\_aMC@NLO+Pythia8]{\MGNLOPY[8]}
\label{subsubsec:tWZ_aMCP8}

\paragraph{Samples}
%\label{par:tWZ_aMCP8_samples}

The descriptions below correspond to the samples in \cref{tab:tWZ_aMCP8}.

\begin{table}[htbp]
  \caption{Nominal \tWZ\ samples produced with \MGNLOPY[8].}%
  \label{tab:tWZ_aMCP8}
  \centering
  \begin{tabular}{l l}
    \toprule
    DSID range & Description \\
    \midrule
    410408 & \tWZ\, DR1 \\
    410409 & \tWZ\, DR2 \\
    \bottomrule
  \end{tabular}
\end{table}

\paragraph{Short description:}

The production of \tWZ\ events was modelled using the \MGNLO[2.3.3]~\cite{Alwall:2014hca}
generator at NLO with the \NNPDF[3.0nlo]~\cite{Ball:2014uwa} parton distribution function~(PDF).
The events were interfaced with \PYTHIA[8.212]~\cite{Sjostrand:2014zea}~ using the A14 tune~\cite{ATL-PHYS-PUB-2014-021} and the
\NNPDF[2.3lo]~\cite{Ball:2014uwa} PDF set.
The decays of bottom and charm hadrons were simulated using the \EVTGEN[1.2.0] program~\cite{Lange:2001uf}.


\paragraph{Long description:}

The production of \tWZ events was modelled using the \MGNLO[2.3.3]~\cite{Alwall:2014hca}
generator at NLO with the \NNPDF[3.0nlo]~\cite{Ball:2014uwa} parton distribution function~(PDF).
The events were interfaced with
\PYTHIA[8.212]~\cite{Sjostrand:2014zea} using the A14 tune~\cite{ATL-PHYS-PUB-2014-021} and the \NNPDF[2.3lo]~\cite{Ball:2014uwa} PDF set.
The top quark and the \(Z\) boson were decayed at LO using \MADSPIN~\cite{Frixione:2007zp,Artoisenet:2012st} to preserve spin correlations.
While the top quark was allowed to decay inclusively, the \(Z\) boson decay was restricted to a pair of charged leptons.
The five-flavour scheme was used, where all the quark masses are set to zero, except the top quark.
The renormalisation and factorisation scales were set to the top-quark mass.
The diagram removal scheme described in Ref.~\cite{Frixione:2008yi} was employed to handle the interference
between \tWZ and \ttZ, and was applied to the \tWZ sample.
A sample with the alternative scheme described in Ref.~\cite{Demartin:2016axk} was produced to assess the associated systematic uncertainty.
The decays of bottom and charm hadrons were simulated using the \EVTGEN[1.2.0] program~\cite{Lange:2001uf}.



==> template/MC_snippets/tZq.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%              tZq                    %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section[\tZq]{\tZq}
\label{subsec:tZq}

This section describes the MC samples used for the modelling of \tZq production.
\Cref{subsubsec:tZq_aMCP8} describes the \MGNLOPY[8] samples,

\subsection[MadGraph5\_aMC@NLO+Pythia8]{\MGNLOPY[8]}
\label{subsubsec:tZq_aMCP8}

\paragraph{Samples}
%\label{par:tZq_aMCP8_samples}

The descriptions below correspond to the samples in \cref{tab:tZq_aMCP8,tab:tZq_aMCP8_addRad}.

\begin{table}[htbp]
  \caption{Nominal \tZq samples produced with \MGNLOPY[8].}%
  \label{tab:tZq_aMCP8}
  \centering
  \begin{tabular}{l l}
    \toprule
    DSID range & Description \\
    \midrule
    412063 & \tZq \\
    \bottomrule
  \end{tabular}
\end{table}

\begin{table}[htbp]
  \caption{\tZq samples produced with \MGNLOPY[8] used to estimate initial-state radiation systematic uncertainties.}%
  \label{tab:tZq_aMCP8_addRad}
  \centering
  \begin{tabular}{l l}
    \toprule
    DSID range & Description \\
    \midrule
    412065 & \tZq, A14Var3c up \\
    410064 & \tZq, A14Var3c down \\
    \bottomrule
  \end{tabular}
\end{table}

\paragraph{Short description:}

The production of \tZq events was modelled using the \MGNLO[2.3.3]~\cite{Alwall:2014hca}
generator at NLO with the \NNPDF[3.0nlo]~\cite{Ball:2014uwa} parton distribution function~(PDF).
The events were interfaced with \PYTHIA[8.230]~\cite{Sjostrand:2014zea} using the A14 tune~\cite{ATL-PHYS-PUB-2014-021} and the
\NNPDF[2.3lo]~\cite{Ball:2014uwa} PDF set.

The uncertainty due to initial-state radiation (ISR) was estimated by comparing the nominal \tZq sample with two additional samples,
which had the same settings as the nominal one, but employed the Var3c up and down variations of the A14 tune.


\paragraph{Long description:}

The \tZq sample was simulated using the \MGNLO[2.3.3]~\cite{Alwall:2014hca}
generator at NLO with the \NNPDF[3.0nlo]~\cite{Ball:2014uwa} parton distribution function~(PDF). The events were interfaced with
\PYTHIA[8.230]~\cite{Sjostrand:2014zea} using the A14 tune~\cite{ATL-PHYS-PUB-2014-021}
and the \NNPDF[2.3lo]~\cite{Ball:2014uwa} PDF set. Off-resonance events away from the \(Z\) mass peak were included.
The top quark was decayed at LO using \MADSPIN~\cite{Frixione:2007zp,Artoisenet:2012st} to preserve spin correlations.
The four-flavour scheme was used, where all the quark masses are set to zero, except for the top and bottom quarks.
Following the discussion in Ref.~\cite{Frederix:2012dh}, the functional form of the renormalisation and factorisation scales
was set to \(4\sqrt{m_b^2+\pTX[2][b]}\), where the \(b\)-quark was the one produced by a gluon splitting in the event.
The decays of bottom and charm hadrons were simulated using the \EVTGEN program~\cite{Lange:2001uf}.

The \tZq total cross-section, calculated at next-to-leading order (NLO) using \MGNLO[2.3.3] with the \NNPDF[3.0nlo] PDF set,
is \(\SI{800}{\fb}\), with an uncertainty of \(^{+6.1}_{-7.4}\)\%. The uncertainty was computed by varying the renormalisation and
factorisation scales by a factor of two and by a factor of 0.5.

The uncertainty due to initial-state radiation (ISR) was estimated by comparing the nominal \tZq sample with two additional samples,
which have the same settings as the nominal one, but employed the Var3c up or down variation of the A14 tune, which
corresponds to the variation of \alphas for ISR in the A14 tune.

To evaluate the effect of renormalisation and factorisation scale uncertainties, the two scales were varied simultaneously by factors 2.0 and 0.5.
To evaluate the PDF uncertainties for the nominal PDF, the 100 variations for \NNPDF[2.3lo] were taken into account.


==> template/MC_snippets/tgamma.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%              tgamma                    %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section[tgamma production]{\tgamma production}
\label{subsec:tgamma}

This section describes the MC samples used for the modelling of \tgamma production.
For now, it will be empty since the sample is still in production.


==> template/MC_snippets/top_isrfsr_powpy_long.tex <==
The uncertainty due to initial-state radiation (ISR) was estimated by
comparing the nominal \ttbar sample with two additional
samples~\cite{ATL-PHYS-PUB-2017-007}.  To simulate higher parton
radiation, the factorisation and renormalisation scales were reduced by
a factor of 0.5 while simultaneously increasing the \hdamp value to
3.0\,\mtop and using the Var3c up variation from the A14 tune. For
lower parton radiation, \muR and \muF were increased by a factor of two
while keeping the \hdamp value set to 1.5\,\mtop and using the Var3c down
variation in the parton shower.  The Var3c A14 tune
variation~\cite{ATL-PHYS-PUB-2014-021} largely corresponds to the variation of
\alphas for ISR in the A14 tune.
The impact of final-state radiation (FSR) was evaluated by
varying the renormalisation scale for emissions from the
parton shower up and down by a factor of two.


==> template/MC_snippets/top_isrfsr_powpy_short.tex <==
The uncertainty due to initial-state radiation (ISR) was estimated by
simultaneously varying the \hdamp parameter and the \muR and
\muF scales, and choosing the Var3c up/down variants of the A14 tune
as described in Ref.~\cite{ATL-PHYS-PUB-2017-007}. The impact of
final-state radiation (FSR) was evaluated by varying the renormalisation scale
for emissions from the parton shower up or down by a factor two.


==> template/MC_snippets/ttH.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%              ttH                    %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section[\ttH production]{\ttH}
\label{subsec:ttH}

\subsection[Powheg+Pythia8]{\POWPY[8]}
%\label{subsubsec:ttH_PP8}

Nominal \(t\bar{t}H\) samples are produced with \POWPY[8].
The \hdamp value is set to \(\SI{352.5}{\GeV} = 3/4 \cdot (\mH+2\mtop)\).

\paragraph{Samples}
%\label{par:ttH_PP8_samples}
\Cref{tab:ttH_PP8} gives the nominal \ttH samples.

\begin{table}[htbp]
  \caption{Nominal \ttH samples produced with \POWPY[8].}%
  \label{tab:ttH_PP8}
  \centering
  \begin{tabular}{l l}
    \toprule
    DSID range & Description \\
    \midrule
    346343 & \ttH, \(H\to\) all, \(\ttbar\to\) all-hadronic \\
    346344 & \ttH, \(H\to\) all, \(\ttbar\to\) semileptonic \\
    346345 & \ttH, \(H\to\) all, \(\ttbar\to\) dileptonic \\
    346525 & \ttH, \(H\to \gamma\gamma\), \(\ttbar\to\) all \\
    \bottomrule
  \end{tabular}
\end{table}

\paragraph{Short description:}

The production of \ttH events was modelled using the
\POWHEGBOX[v2]~\cite{Frixione:2007nw,Nason:2004rx,Frixione:2007vw,Alioli:2010xd,Hartanto:2015uka}
generator at NLO with the \NNPDF[3.0nlo]~\cite{Ball:2014uwa} PDF set.
The events were interfaced to \PYTHIA[8.230]~\cite{Sjostrand:2014zea}~using
the A14 tune~\cite{ATL-PHYS-PUB-2014-021} and the
\NNPDF[2.3lo]~\cite{Ball:2014uwa} PDF set. The decays of bottom and charm hadrons
were performed by \EVTGEN[1.6.0]~\cite{Lange:2001uf}.

\paragraph{Long description:}

The production of \ttH events was modelled using the
\POWHEGBOX[v2]~\cite{Frixione:2007nw,Nason:2004rx,Frixione:2007vw,Alioli:2010xd,Hartanto:2015uka}
generator, which provided matrix elements at next-to-leading order (NLO) in the strong coupling
constant \alphas in the five-flavour scheme with the \NNPDF[3.0nlo]~\cite{Ball:2014uwa} PDF set.
The functional form of the renormalisation and factorisation scales was
set to \(\sqrt[3]{m_\text{T}(t)\cdot m_\text{T}(\bar{t}) \cdot m_\text{T}(H)}\).
The events were interfaced to \PYTHIA[8.230]~\cite{Sjostrand:2014zea}
using the A14 tune~\cite{ATL-PHYS-PUB-2014-021} and the
\NNPDF[2.3lo]~\cite{Ball:2014uwa} PDF set. The decays of bottom and charm hadrons
were performed by \EVTGEN[1.6.0]~\cite{Lange:2001uf}.

The cross-section was calculated at NLO QCD and NLO EW accuracy using
\MGNLO as reported in Ref.~\cite{deFlorian:2016spz}.
The predicted value at \(\rts = \SI{13}{\TeV}\) is
\(507^{+35}_{-50}\,\si{\fb}\), where the uncertainties were estimated from
variations of \alphas and the renormalisation and factorisation scales.

The uncertainty in the initial-state radiation (ISR) was estimated using the Var3c
up/down variations of the A14 tune. Uncertainties due to missing
higher-order corrections were evaluated through simultaneous variations of the
renormalisation and factorisation scales by factors of
2.0 and 0.5. Uncertainties in the PDFs were evaluated using the 100
variations of the \NNPDF[3.0nlo] set.


\subsection[Powheg+Herwig7]{\POWHER[7]}
%\label{subsubsec:ttH_PH7}

\paragraph{Samples}
%\label{par:ttH_PH7_samples}

\Cref{tab:ttH_PH7} presents alternative \ttH samples.

\begin{table}[htbp]
  \caption{Alternative \ttH \POWHER[7] samples produced to evaluate systematic uncertainties
  due to different MC models for parton showering and hadronisation.}%
  \label{tab:ttH_PH7}
  \centering
  \begin{tabular}{l l}
    \toprule
    DSID range & Description \\
    \midrule
    346346 & \ttH, \(H\to\) all, \(\ttbar\to\) all-hadronic \\
    346347 & \ttH, \(H\to\) all, \(\ttbar\to\) semileptonic \\
    346348 & \ttH, \(H\to\) all, \(\ttbar\to\) dileptonic \\
    346526 & \ttH, \(H\to\gamma\gamma\), \(\ttbar\to\) all \\
    \bottomrule
  \end{tabular}
\end{table}

\paragraph{Short description:}

The impact of using a different parton shower and hadronisation model was evaluated by showering the nominal hard-scatter events with
\HERWIG[7.04]~\cite{Bahr:2008pv,Bellm:2015jjp} using the H7UE set of tuned parameters~\cite{Bellm:2015jjp} and
the \MMHT[lo] PDF set~\cite{Harland-Lang:2014zoa}.

\paragraph{Long description:}

The impact of using a different parton shower and hadronisation model was evaluated
by comparing the nominal sample with another sample produced with
the \POWHEGBOX[v2]~\cite{Frixione:2007nw,Nason:2004rx,Frixione:2007vw,Alioli:2010xd}
generator but interfaced with \HERWIG[7.04]~\cite{Bahr:2008pv,Bellm:2015jjp}, using the
H7UE set of tuned parameters~\cite{Bellm:2015jjp} and
the \MMHT[lo] PDF set~\cite{Harland-Lang:2014zoa}.
\POWHEGBOX provided matrix elements at next-to-leading
order~(NLO) in the strong coupling constant \alphas with the
\NNPDF[3.0nlo]~\cite{Ball:2014uwa} parton distribution function~(PDF).
The functional form of the renormalisation and factorisation scales was
set to \(\sqrt[3]{m_\text{T}(t)\cdot m_\text{T}(\bar{t}) \cdot m_\text{T}(H)}\).
The decays of bottom and charm hadrons
were simulated using the \EVTGEN[1.6.0] program~\cite{Lange:2001uf}.


==> template/MC_snippets/ttHF.tex <==
% !TEX root = MC_snippets.tex

\section[\ttHF]{\ttHF}
\label{subsec:ttHF}

In the following subsections, the set-ups of the current baseline samples for the production of \ttbar quark pairs in association with
\(b\)-quarks (\ttHF) are described. NLO predictions with massive \(b\)-quarks in the matrix element and matched to parton shower
programs are available within the \SHERPAOL, \MGNLO and, more recently, \POWHEGBOX frameworks.

\subsection[Sherpa]{\SHERPA}
%\label{subsubsec:ttHF_sherpa}
The descriptions below refer to the \SHERPA[2.2.1] samples.
Details of the set-up are given in Ref.~\cite{ATL-PHYS-PUB-2016-016} and reported below.

\paragraph{Samples}
%\label{par:ttHF_sherpa_samples}

The descriptions below correspond to the samples in \cref{tab:ttHF_Sh}.

\begin{table}[htbp]
  \caption{Nominal \ttbar+HF samples produced with \SHERPA.
      Variation samples are not explicitly listed.}%
  \label{tab:ttHF_Sh}
  \centering
  \begin{tabular}{l l}
    \toprule
    DSID range & Description \\
    \midrule
    410323--4 & \ttbar single lepton \\
    410325 & \ttbar dilepton \\
    410369 & \ttbar all-hadronic \\
    \bottomrule
  \end{tabular}
\end{table}

\paragraph{Description:}

Samples for \ttHF processes were produced with the \SHERPA[2.2.1]~\cite{Bothmann:2019yzt} generator,
using the MEPS@NLO prescription~\cite{Hoeche:2012yf} and interfaced with \OPENLOOPS~\cite{Buccioni:2019sur,Cascioli:2011va,Denner:2016kdg}
to provide the virtual corrections for matrix elements at NLO accuracy.
The four-flavour scheme is used with the \(b\)-quark mass set to \SI{4.75}{\GeV}.
The renormalisation scale \muR has the functional form
\(\sqrt[4]{m_\text{T}(t) \cdot m_{\text{T}}(\bar{t}) \cdot m_{\text{T}}(b) \cdot m_{\text{T}}(\bar{b})}\). The
factorisation scale \muF was set to \(\HT/2\), where \HT is the transverse-mass sum of the
partons in the matrix element, and this value was also the resummation scale \muQ of the parton shower.
The \CT[10nlo] PDF set was used in conjunction with a dedicated PS tune developed by the \SHERPA authors.


\subsection[MadGraph5\_aMC@NLO+Pythia8]{\MGNLOPY[8]}
%\label{subsubsec:ttHF_aMCP8}
In the following, set-ups are described for \PYTHIA only.
Details of the set-up are given in Ref.~\cite{ATL-PHYS-PUB-2016-016} and reported below.

\paragraph{Samples}
%\label{par:ttHF_aMCP8_samples}

The descriptions below correspond to the samples in \cref{tab:ttHF_amc}.

\begin{table}[htbp]
  \caption{Nominal \ttbar+HF samples produced with \MGNLOPY[8].}%
  \label{tab:ttHF_amc}
  \centering
  \begin{tabular}{l l}
    \toprule
    DSID range & Description \\
    \midrule
    410265 & \ttbar non-all-hadronic \\
    410266 & \ttbar dileptonic \\
    410267 & \ttbar all-hadronic \\
    \bottomrule
  \end{tabular}
\end{table}

\paragraph{Description:}

Samples for \ttHF processes were produced with the \MGNLO generator
with the \NNPDF[3.0nlo]~\cite{Ball:2014uwa} PDF set. It was interfaced with \PYTHIA[8.230]~\cite{Sjostrand:2014zea},
using the A14 set of tuned parameters~\cite{ATL-PHYS-PUB-2014-021} and the \NNPDF[2.3lo] PDF.
The four-flavour scheme was used with the \(b\)-quark mass set to \SI{4.75}{\GeV}.
The renormalisation scale \muR has the functional form
\(\sqrt[4]{m_\text{T}(t) \cdot m_\text{T}(\bar{t}) \cdot m_\text{T}(b) \cdot m_\text{T}(\bar{b})}\). The
factorisation scale \muF was set to \(\HT/2\), where \HT is the transverse-mass sum of the partons in the matrix
element.
The resummation scale \muQ has the form \(\muQ = f_\text{Q} \sqrt{\hat{s}}\), where
the prefactor \(f_\text{Q}\) is an external parameter randomly distributed in the
range \([f^\text{min}_\text{Q}\), \(f^\text{max}_\text{Q}]=[0.1,0.25]\).


\subsection[PowhegBoxRes+Pythia8]{\POWHEGBOXRES+\PYTHIA[8]}
%\label{subsubsec:ttHF_PP8}
In the following, set-ups are described for \PYTHIA[8] only.

\paragraph{Samples}
%\label{par:ttHF_PP8_samples}
The descriptions below correspond to the samples in \cref{tab:ttHF_pp8}.

\begin{table}[htbp]
  \caption{Nominal \ttbar+HF samples produced with \POWHEGBOXRES+\PYTHIA[8].}%
  \label{tab:ttHF_pp8}
  \centering
  \begin{tabular}{l l}
    \toprule
    DSID range & Description \\
    \midrule
    411179--80 & \ttbar non-all-hadronic \\
    411178    & \ttbar dileptonic \\
    411275    & \ttbar all-hadronic \\
    \bottomrule
  \end{tabular}
\end{table}

\paragraph{Description:}

Samples for \ttHF processes were produced with the \POWHEGBOXRES~\cite{Jezo:2018yaf}
generator and \OPENLOOPS~\cite{Buccioni:2019sur,Cascioli:2011va,Denner:2016kdg}, using a pre-release
of the implementation of this process in \POWHEGBOXRES provided by the authors~\cite{ttbbPowheg},
with the \NNPDF[3.0nlo]~\cite{Ball:2014uwa} PDF set. It was interfaced with \PYTHIA[8.240]~\cite{Sjostrand:2014zea},
using the A14 set of tuned parameters~\cite{ATL-PHYS-PUB-2014-021} and the \NNPDF[2.3lo] PDF set.
The four-flavour scheme was used with the \(b\)-quark mass set to \SI{4.95}{\GeV}.
The factorisation scale was set to \(0.5\times\Sigma_{i=t,\bar{t},b,\bar{b},j}m_{\mathrm{T},i}\),
the renormalisation scale was set to \(\sqrt[4]{m_{\text{T}}(t)\cdot m_{\text{T}}(\bar{t})\cdot m_{\text{T}}(b)\cdot m_{\text{T}}(\bar{b})}\),
and the \hdamp parameter was set to \(0.5\times\Sigma_{i=t,\bar{t},b,\bar{b}}m_{\mathrm{T},i}\).


==> template/MC_snippets/ttV.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%              ttV                    %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section[\ttV production]{\ttV production}
\label{subsec:ttV}

This section describes the MC samples used for the modelling of \ttV (\(V=W/Z\)) production.
\Cref{subsubsec:ttV_aMCP8} describes the \MGNLOPY[8] samples,
and \cref{subsubsec:ttV_sherpa} describes the \SHERPA samples.
(NOTE: this section is not frozen as the \SHERPA samples are likely to be updated and become the nominal samples in the near future.)

\subsection[MadGraph5\_aMC@NLO+Pythia8]{\MGNLOPY[8]}
\label{subsubsec:ttV_aMCP8}

\paragraph{Samples}
%\label{par:ttV_aMCP8_samples}

The descriptions below correspond to the samples in \cref{tab:ttV_aMCP8,tab:ttV_aMCP8_addRad}.

\begin{table}[htbp]
  \caption{Nominal \ttV samples produced with \MGNLOPY[8].}%
  \label{tab:ttV_aMCP8}
  \centering
  \begin{tabular}{l l}
    \toprule
    DSID range & Description \\
    \midrule
    410155 & \ttW \\
    410156 & \ttZnunu \\
    410157 & \ttZqq \\
    410218 & \ttee, \(m_{\ell\ell} > \SI{5}{\GeV}\) \\
    410219 & \ttmumu, \(m_{\ell\ell} > \SI{5}{\GeV}\) \\
    410220 & \tttautau, \(m_{\ell\ell} > \SI{5}{\GeV}\) \\
    410276 & \ttee, \(m_{\ell\ell} \in \SI[parse-numbers=false]{[1,5]}{\GeV}\)\\
    410277 & \ttmumu, \(m_{\ell\ell} \in \SI[parse-numbers=false]{[1,5]}{\GeV}\)\\
    410278 & \tttautau, \(m_{\ell\ell} \in \SI[parse-numbers=false]{[1,5]}{\GeV}\)\\
    \bottomrule
  \end{tabular}
\end{table}

\begin{table}[htbp]
  \caption{\ttV samples produced with \MGNLOPY[8] used to estimate initial-state radiation systematic uncertainties.}%
  \label{tab:ttV_aMCP8_addRad}
  \centering
  \begin{tabular}{l l}
    \toprule
    DSID range & Description \\
    \midrule
    410376 & \ttW\ A14Var3c up \\
    410377 & \ttW\ A14Var3c down \\
    410378 & \ttZnunu\ A14Var3c up \\
    410379 & \ttZnunu\ A14Var3c down \\
    410380 & \ttZqq\ A14Var3c up \\
    410381 & \ttZqq\ A14Var3c down \\
    410370 & \ttee\ A14Var3c up \\
    410371 & \ttee\ A14Var3c down \\
    410372 & \ttmumu\ A14Var3c up \\
    410373 & \ttmumu\ A14Var3c down \\
    410374 & \tttautau\ A14Var3c up \\
    410375 & \tttautau\ A14Var3c down \\
    \bottomrule
  \end{tabular}
\end{table}

\paragraph{Short description:}

The production of \ttV\ events was modelled using the
\MGNLO[2.3.3]~\cite{Alwall:2014hca} generator at NLO with the
\NNPDF[3.0nlo]~\cite{Ball:2014uwa} parton distribution function~(PDF).
The events were interfaced to \PYTHIA[8.210]~\cite{Sjostrand:2014zea}
using the A14 tune~\cite{ATL-PHYS-PUB-2014-021} and the
\NNPDF[2.3lo]~\cite{Ball:2014uwa} PDF set. The decays of bottom and charm
hadrons were simulated using the \EVTGEN[1.2.0] program~\cite{Lange:2001uf}.

The uncertainty due to initial-state radiation (ISR) was estimated by
comparing the nominal event sample with two samples where the Var3c
up/down variations of the A14 tune were employed.


\paragraph{Long description:}

The production of \ttV events was modelled using the \MGNLO[2.3.3]
\cite{Alwall:2014hca} generator, which provided matrix elements at
next-to-leading order~(NLO) in the strong coupling constant \alphas
with the \NNPDF[3.0nlo]~\cite{Ball:2014uwa} parton distribution
function~(PDF). The functional form of the renormalisation and
factorisation scales was set to the default of
\(0.5 \times \sum_i \sqrt{m^2_i+p^2_{\text{T},i}}\),
where the sum runs over all the particles
generated from the matrix element calculation. Top quarks were decayed
at LO using \MADSPIN~\cite{Frixione:2007zp,Artoisenet:2012st} to
preserve spin correlations. The events were interfaced with
\PYTHIA[8.210]~\cite{Sjostrand:2014zea} for the parton shower and
hadronisation, using the A14 set of tuned
parameters~\cite{ATL-PHYS-PUB-2014-021} and the
\NNPDF[2.3lo]~\cite{Ball:2014uwa} PDF set.
The decays of bottom and charm hadrons were simulated using the \EVTGEN[1.2.0] program~\cite{Lange:2001uf}.

% Note : The cross-section is supplemented with an off-shell (down to \SI{5}{\GeV}) correction calculated in Ref.~\cite{ATLASPMGttVNLOXsec}.
The cross-sections were calculated at NLO QCD and NLO EW accuracy using
\MGNLO as reported in Ref.~\cite{deFlorian:2016spz}.
In the case of \ttll the cross-section was scaled by
an off-shell correction estimated at one-loop level in \alphas.
(\emph{Optionally:})
The predicted values at \(\rts = \SI{13}{\TeV}\) are \(0.88^{+0.09}_{-0.11}\,\si{\pb}\) and
\(0.60^{+0.08}_{-0.07}\,\si{\pb}\) for \ttZ and \ttW, respectively, where the
uncertainties were estimated from variations of \alphas and the renormalisation and
factorisation scales.

The uncertainty due to initial-state radiation (ISR) was estimated by
comparing the nominal \ttV sample with two additional samples, which
have the same settings as the nominal one, but employed the Var3c up or down
variation of the A14 tune, which corresponds
to the variation of \alphas for initial-state radiation
(ISR) in the A14 tune.

Uncertainties due to missing higher-order corrections were evaluated
by simultaneously varying the renormalisation and factorisation scales
by factors of 2.0 and 0.5. Uncertainties in the PDFs
were evaluated using the 100 replicas of the \NNPDF[3.0nlo] set.


\subsection[Sherpa]{\SHERPA}
\label{subsubsec:ttV_sherpa}

\paragraph{Samples}
%\label{par:ttV_sherpa_samples}

The descriptions below correspond to the samples in \cref{tab:ttV_sherpa}.

\begin{table}[htbp]
  \caption{\ttV samples produced with \SHERPA.}%
  \label{tab:ttV_sherpa}
  \centering
  \begin{tabular}{l l}
    \toprule
    DSID range & Description \\
    \midrule
    410142 & \ttll \\
    410143 & \ttZqq, \ttZnunu \\
    410144 & \ttW \\
    \bottomrule
  \end{tabular}
\end{table}

\paragraph{Description:}

Additional \ttV samples were produced with the
\SHERPA[2.2.0]~\cite{Bothmann:2019yzt} generator at LO accuracy, using
the \MEPSatLO set-up~\cite{Catani:2001cc,Hoeche:2009rj} with up to one
additional parton for the \ttll sample and two additional partons for the
others. A dynamic renormalisation scale was used and is defined
similarly to that of the nominal \ttV samples. The CKKW matching
scale of the additional emissions was set to \SI{30}{\GeV}. The default
\SHERPA[2.2.0] parton shower was used along with the
\NNPDF[3.0nnlo]~\cite{Ball:2014uwa} PDF set.


==> template/MC_snippets/ttbar.tex <==
% !TEX root = MC_snippets.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%              ttbar                  %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section[\ttbar production]{\ttbar production}
\label{subsec:ttbar}

This section describes the MC samples used for the modelling of \ttbar production.
\Cref{subsubsec:ttbar_PP8} describes the \POWPY[8] samples,
\cref{subsubsec:ttbar_PH7} describes the \POWHER[7] samples,
\cref{subsubsec:ttbar_aMCP8} describes the \MGNLOPY[8] samples,
and finally \cref{subsubsec:ttbar_sherpa} describes the \SHERPA samples.

The reference cross-section values are extracted from Ref.~\cite{LHCTopWGttbarXsec}.
Studies of MC simulation performance including comparisons with unfolded data
are collected in the PUB notes~\cite{ATL-PHYS-PUB-2018-009,ATL-PHYS-PUB-2017-007,ATL-PHYS-PUB-2016-020}.

\subsection[Powheg+Pythia8]{\POWPY[8]}
\label{subsubsec:ttbar_PP8}

\paragraph{Samples}
%\label{par:ttbar_PP8_samples}

The descriptions below correspond to the samples in \cref{tab:ttbar_PP8,tab:ttbar_PP8_addRad,tab:ttbar_PP8_hdampvar}.

\begin{table}[htbp]
  \caption{Nominal \ttbar samples produced with \POWPY[8].
    The \hdamp\ value is set to 1.5\,\mtop.}%
  \label{tab:ttbar_PP8}
  \centering
  \begin{tabular}{l l}
    \toprule
    DSID range & Description \\
    \midrule
    410470 & \ttbar non-all-hadronic \\
    410471 & \ttbar dileptonic \\
    410472 & \ttbar all-hadronic \\
    \bottomrule
  \end{tabular}
\end{table}

\begin{table}[htbp]
  \caption{\ttbar samples produced with \POWPY[8]
    used to estimate initial-state radiation systematic uncertainties.
    The \hdamp value is set to 3.0\,\mtop.}%
  \label{tab:ttbar_PP8_addRad}
  \centering
  \begin{tabular}{l l}
    \toprule
    DSID range & Description \\
    \midrule
    410480 & \ttbar single lepton \\
    410481 & \ttbar all-hadronic \\
    410482 & \ttbar dileptonic \\
    \bottomrule
  \end{tabular}
\end{table}

\begin{table}[htbp]
  \caption{\ttbar samples produced with \POWPY[8] with alternative \hdamp values
    which can be used to estimate the uncertainty due to the \POWPY[8] matching scheme.}%
  \label{tab:ttbar_PP8_hdampvar}
  \centering
  \begin{tabular}{l l l l}
    \toprule
    DSID (1.3\,\mtop) & DSID (1.8\,\mtop) & DSID (2.0\,\mtop) & Description \\
    \midrule
    411350 & 411353 & 411356 & \ttbar single lepton \\
    411351 & 411354 & 411357 & \ttbar all-hadronic \\
    411352 & 411355 & 411358 & \ttbar dileptonic \\
    \bottomrule
  \end{tabular}
\end{table}

\paragraph{Short description:}

The production of \ttbar events was modelled using the
\POWHEGBOX[v2]~\cite{Frixione:2007nw,Nason:2004rx,Frixione:2007vw,Alioli:2010xd}
generator at NLO with the \NNPDF[3.0nlo]~\cite{Ball:2014uwa} PDF set
and the \hdamp parameter\footnote{The
  \hdamp parameter is a resummation damping factor and one of the
  parameters that controls the matching of \POWHEG matrix elements to
  the parton shower and thus effectively regulates the
  high-\pT radiation against which the \ttbar system recoils.} set
to 1.5\,\mtop~\cite{ATL-PHYS-PUB-2016-020}.  The events were interfaced
to \PYTHIA[8.230]~\cite{Sjostrand:2014zea} to model the parton shower,
hadronisation, and underlying event, with parameters set according
to the A14 tune~\cite{ATL-PHYS-PUB-2014-021} and using the \NNPDF[2.3lo]
set of PDFs~\cite{Ball:2012cx}. The decays of bottom and charm hadrons
were performed by \EVTGEN[1.6.0]~\cite{Lange:2001uf}.

\input{top_isrfsr_powpy_short}


\paragraph{Long description:}

The production of \ttbar events was modelled using the
\POWHEGBOX[v2]~\cite{Frixione:2007nw,Nason:2004rx,Frixione:2007vw,Alioli:2010xd}
generator, which provided matrix elements at next-to-leading
order~(NLO) in the strong coupling constant \alphas, and the
\NNPDF[3.0nlo]~\cite{Ball:2014uwa} parton distribution function~(PDF).
The \hdamp parameter, which controls the matching in \POWHEG and
effectively regulates the high-\pT radiation against which the
\ttbar system recoils, was set to 1.5\,\mtop~\cite{ATL-PHYS-PUB-2016-020}.
The functional form of the renormalisation and factorisation scales was
set to the default scale \(\sqrt{\mtop^{2} + \pTX[2]}\).
The events were interfaced with
\PYTHIA[8.230]~\cite{Sjostrand:2014zea} for the parton shower and
hadronisation, using the A14 set of tuned
parameters~\cite{ATL-PHYS-PUB-2014-021} and the \NNPDF[2.3lo]
set of PDFs~\cite{Ball:2012cx}.
The decays of bottom and charm hadrons were simulated using the
\EVTGEN[1.6.0] program~\cite{Lange:2001uf}.

The \ttbar sample was normalised to the cross-section prediction at next-to-next-to-leading order (NNLO)
in QCD including the resummation of next-to-next-to-leading logarithmic (NNLL) soft-gluon terms calculated using
\TOPpp[2.0]~\cite{Beneke:2011mq,Cacciari:2011hy,Baernreuther:2012ws,Czakon:2012zr,Czakon:2012pz,Czakon:2013goa,Czakon:2011xx}.
For proton--proton collisions at a centre-of-mass energy of \(\rts = \SI{13}{\TeV}\), this cross-section corresponds to
\(\sigma(\ttbar)_{\text{NNLO+NNLL}} = 832 \pm 51\,\si{\fb}\) using a top-quark mass of \(\mtop = \SI{172.5}{\GeV}\).
The uncertainties in the cross-section due to the PDF and \alphas were calculated using the \PDFforLHC[15] prescription~\cite{Butterworth:2015oua}
with the \MSTW[nnlo]~\cite{Martin:2009iq,Martin:2009bu}, \CT[10nnlo]~\cite{Lai:2010vv,Gao:2013xoa}
and \NNPDF[2.3lo]~\cite{Ball:2012cx} PDF sets in the five-flavour scheme, and were added in quadrature to the effect of the scale uncertainty.

\input{top_isrfsr_powpy_long}

The \NNPDF[3.0lo] replicas were used to evaluate the PDF uncertainties for the nominal PDF.
In addition, the central value of this PDF was compared with the central values of the
\CT[14nnlo]~\cite{Dulat:2015mca} and \MMHT[nnlo]~\cite{Harland-Lang:2014zoa} PDF sets.


\subsection[Powheg+Herwig7.04]{\POWHER[7.04]}
\label{subsubsec:ttbar_PH7}

\paragraph{Samples}
%\label{par:ttbar_PH7_samples}

The descriptions below correspond to the samples in \cref{tab:ttbar_PH7}.

\begin{table}[htbp]
  \caption{\ttbar samples produced with \POWHER[7].}%
  \label{tab:ttbar_PH7}
  \centering
  \begin{tabular}{l l}
    \toprule
    DSID range & Description \\
    \midrule
    410557 & \ttbar single lepton  \\
    410558 & \ttbar dileptonic  \\
    410559 & \ttbar all-hadronic  \\
    \bottomrule
  \end{tabular}
\end{table}

\paragraph{Short description:}

The impact of using a different parton shower and hadronisation model was evaluated
by comparing the nominal \ttbar sample with another event sample produced with the
\POWHEGBOX[v2]~\cite{Frixione:2007nw,Nason:2004rx,Frixione:2007vw,Alioli:2010xd}
generator using the \NNPDF[3.0nlo]~\cite{Ball:2014uwa} parton distribution function~(PDF).
Events in the latter sample were interfaced with \HERWIG[7.04]~\cite{Bahr:2008pv,Bellm:2015jjp},
using the H7UE set of tuned parameters~\cite{Bellm:2015jjp} and the
\MMHT[lo] PDF set~\cite{Harland-Lang:2014zoa}.
The decays of bottom and charm hadrons
were simulated using the \EVTGEN[1.6.0] program~\cite{Lange:2001uf}.

\paragraph{Long description:}

The impact of using a different parton shower and hadronisation model was evaluated
by comparing the nominal \ttbar sample with an event sample also produced with the
\POWHEGBOX[v2]~\cite{Frixione:2007nw,Nason:2004rx,Frixione:2007vw,Alioli:2010xd}
generator but interfaced with \HERWIG[7.04]~\cite{Bahr:2008pv,Bellm:2015jjp}, using the H7UE set
of tuned parameters~\cite{Bellm:2015jjp} and the \MMHT[lo] PDF set~\cite{Harland-Lang:2014zoa}.
\POWHEGBOX provided matrix elements at next-to-leading order~(NLO) in the
strong coupling constant \alphas, and used the \NNPDF[3.0nlo]~\cite{Ball:2014uwa}
parton distribution function~(PDF) and an \hdamp parameter value of \(1.5\,\mtop\)~\cite{ATL-PHYS-PUB-2016-020}.
The functional form of the renormalisation and factorisation scales was
set to the default scale \(\sqrt{\mtop^{2} + \pT^2}\).
The decays of bottom and charm hadrons
were simulated using the \EVTGEN[1.6.0] program~\cite{Lange:2001uf}.


\subsection[Powheg+Herwig7.13]{\POWHER[7.13]}
%\label{subsubsec:ttbar_PH713}

\paragraph{Samples}
%\label{par:ttbar_PH713_samples}

The descriptions below correspond to the samples in \cref{tab:ttbar_PH713}.

\begin{table}[htbp]
  \caption{\ttbar samples produced with \POWHER[7.13].}%
  \label{tab:ttbar_PH713}
  \centering
  \begin{tabular}{l l}
    \toprule
    DSID range & Description \\
    \midrule
    411233 & \ttbar single lepton  \\
    411234 & \ttbar dileptonic  \\
    411316 & \ttbar all-hadronic  \\
    \bottomrule
  \end{tabular}
\end{table}

\paragraph{Short description:}

The impact of using a different parton shower and hadronisation model was evaluated
by comparing the nominal \ttbar sample with another event sample produced with the
\POWHEGBOX[v2]~\cite{Frixione:2007nw,Nason:2004rx,Frixione:2007vw,Alioli:2010xd}
generator using the \NNPDF[3.0nlo]~\cite{Ball:2014uwa} parton distribution function~(PDF).
Events in the latter sample were interfaced with \HERWIG[7.13]~\cite{Bahr:2008pv,Bellm:2015jjp},
using the \HERWIG[7.1] default set of tuned parameters~\cite{Bellm:2015jjp,Bellm:2017jjp}
and the \MMHT[lo] PDF set~\cite{Harland-Lang:2014zoa}.
The decays of bottom and charm hadrons
were simulated using the \EVTGEN[1.6.0] program~\cite{Lange:2001uf}.


\paragraph{Long description:}

The impact of using a different parton shower and hadronisation model was evaluated
by comparing the nominal \ttbar sample with an event sample also produced with the
\POWHEGBOX[v2]~\cite{Frixione:2007nw,Nason:2004rx,Frixione:2007vw,Alioli:2010xd}
generator but interfaced with \HERWIG[7.13]~\cite{Bahr:2008pv,Bellm:2015jjp}, using the
\HERWIG[7.1] default set of tuned parameters~\cite{Bellm:2015jjp,Bellm:2017jjp} and the
\MMHT[lo] PDF set~\cite{Harland-Lang:2014zoa}.
\POWHEGBOX provided matrix elements at next-to-leading
order~(NLO) in the strong coupling constant \alphas, and used the
\NNPDF[3.0nlo]~\cite{Ball:2014uwa} parton distribution function~(PDF) and
an \hdamp parameter value of 1.5\,\mtop~\cite{ATL-PHYS-PUB-2016-020}.
The functional form of the renormalisation and factorisation scales was
set to the default scale \(\sqrt{\mtop^{2} + \pTX[2]}\).
The decays of bottom and charm hadrons
were simulated using the \EVTGEN[1.6.0] program~\cite{Lange:2001uf}.


\subsection[MadGraph5\_aMC@NLO+Pythia8]{\MGNLOPY[8]}
\label{subsubsec:ttbar_aMCP8}

\paragraph{Samples}
%\label{par:ttbar_aMCP8_samples}

The descriptions below correspond to the samples in \cref{tab:ttbar_aMCP8}.
\begin{table}[htbp]
  \caption{\ttbar samples produced with \MGNLOPY[8].}%
  \label{tab:ttbar_aMCP8}
  \centering
  \begin{tabular}{l l}
  \toprule
  DSID range & Description \\
  \midrule
  410464 & \ttbar single lepton \\
  410465 & \ttbar dileptonic \\
  410466 & \ttbar all-hadronic \\
  \bottomrule
  \end{tabular}
\end{table}

\paragraph{Short description:}

To assess the uncertainty in the matching of NLO matrix elements to the
parton shower, the \POWHEG sample was compared with a sample of events
generated with \MGNLO[2.6.0]~\cite{Alwall:2014hca} interfaced with
\PYTHIA[8.230]~\cite{Sjostrand:2014zea}. The \MGNLO calculation used the
\NNPDF[3.0nlo] set of PDFs~\cite{Ball:2014uwa} and \PYTHIA[8] used
the A14 set of tuned parameters~\cite{ATL-PHYS-PUB-2014-021} and
the \NNPDF[2.3lo] set of PDFs~\cite{Ball:2012cx}.
The decays of bottom and charm hadrons
were simulated using the \EVTGEN[1.6.0] program~\cite{Lange:2001uf}.

\paragraph{Long description:}

To assess the uncertainty due to the choice of matching scheme,
the \POWHEG sample was compared with a sample generated by
\MGNLOPY[8]. For the calculation of the hard-scattering,
\MGNLO[2.6.0]~\cite{Alwall:2014hca} with the \NNPDF[3.0nlo]~\cite{Ball:2014uwa} PDF set was
used. The events were interfaced with
\PYTHIA[8.230]~\cite{Sjostrand:2014zea}, using the A14 set of tuned
parameters~\cite{ATL-PHYS-PUB-2014-021} and the \NNPDF[2.3lo] set of PDFs~\cite{Ball:2012cx}.
Top quarks were decayed at LO using
\MADSPIN~\cite{Frixione:2007zp,Artoisenet:2012st} to preserve spin
correlations. The decays of bottom and charm hadrons were simulated
using the \EVTGEN[1.6.0] program~\cite{Lange:2001uf}.  The parton-shower starting
scale had the functional form \(\muQ = \HT/2\)~\cite{ATL-PHYS-PUB-2017-007},
where \HT is defined as the scalar sum of the \pT of all outgoing partons.
The renormalisation and factorisation scale choice was the same as for the
\POWHEGBOX set-up.

\subsection[MadGraph5\_aMC@NLO+Herwig7.13]{\MGNLOHER[7.13]}
%\label{subsubsec:ttbar_aMCH713}

\paragraph{Samples}
%\label{par:ttbar_aMCH713_samples}

The descriptions below correspond to the samples in \cref{tab:ttbar_aMCH713}.
\begin{table}[htbp]
  \caption{\ttbar samples produced with \MGNLOHER[7.13].}%
  \label{tab:ttbar_aMCH713}
  \centering
  \begin{tabular}{l l}
    \toprule
    DSID range & Description \\
    \midrule
    412116 & \ttbar single lepton \\
    412117 & \ttbar dileptonic \\
    412175 & \ttbar all-hadronic \\
    \bottomrule
  \end{tabular}
\end{table}

\paragraph{Short description:}

To assess the uncertainty in the matching of NLO matrix elements to the
parton shower, a sample produced with the
\POWHEGBOX[v2]
generator was compared with a sample generated with \MGNLO[2.6.0]~\cite{Alwall:2014hca}, both using the
\NNPDF[3.0nlo]~\cite{Ball:2014uwa} parton distribution function~(PDF) and interfaced with
\HERWIG[7.13]~\cite{Bahr:2008pv,Bellm:2015jjp}, using the \HERWIG[7.1] default set of
tuned parameters~\cite{Bellm:2015jjp} and the \MMHT[lo] PDF set~\cite{Harland-Lang:2014zoa}.
The decays of bottom and charm hadrons
were simulated using the \EVTGEN[1.6.0] program~\cite{Lange:2001uf}.


\paragraph{Long description:}

To assess the uncertainty in the matching of NLO matrix elements to the parton shower,
a \POWHEG sample was compared with a sample generated by \MGNLO~\cite{Alwall:2014hca}.
The first sample was produced with the same hard-scatter set-up as the nominal sample using the
\POWHEGBOX[v2]~\cite{Frixione:2007nw,Nason:2004rx,Frixione:2007vw,Alioli:2010xd}
generator, which provided matrix elements at next-to-leading
order~(NLO) in the strong coupling constant \alphas, with the
\NNPDF[3.0nlo]~\cite{Ball:2014uwa} parton distribution function~(PDF) and
the \hdamp parameter set to 1.5\,\mtop~\cite{ATL-PHYS-PUB-2016-020}.
The functional form of the renormalisation and factorisation scales was
set to the default scale \(\sqrt{\mtop^{2} + \pTX[2]}\).
The second sample used \MGNLO[2.6.0] with the
\NNPDF[3.0nlo]~\cite{Ball:2014uwa} PDF set for the calculation of the hard-scattering.
Top quarks were decayed at LO using
\MADSPIN~\cite{Frixione:2007zp,Artoisenet:2012st} to preserve spin
correlations. The parton-shower starting
scale had the functional form \(\muQ = \HT/2\)~\cite{ATL-PHYS-PUB-2017-007},
where \HT is defined
as the scalar sum of the \pT of all outgoing partons.
The events from both generators were interfaced with
\HERWIG[7.13]~\cite{Bahr:2008pv,Bellm:2015jjp}, using the \HERWIG[7.1] default set
of tuned parameters~\cite{Bellm:2015jjp} and the \MMHT[lo] PDF set
\cite{Harland-Lang:2014zoa}.
The renormalisation and factorisation scale choice in the \MGNLO set-up was the same as for the
\POWHEGBOX set-up. The decays of bottom and charm hadrons were simulated
using the \EVTGEN[1.6.0] program~\cite{Lange:2001uf} in both set-ups.


\subsection[Sherpa 2.2.1]{\SHERPA[2.2.1]}
\label{subsubsec:ttbar_sherpa}

\paragraph{Samples}
%\label{par:ttbar_sherpa_samples}

The descriptions below correspond to the samples in \cref{tab:ttbar_sherpa}.
\begin{table}[htbp]
  \caption{\ttbar samples produced with \SHERPA[2.2.1].}%
  \label{tab:ttbar_sherpa}
  \centering
  \begin{tabular}{l l}
  \toprule
  DSID range & Description \\
  \midrule
  410249 & \ttbar all-hadronic  \\
  410250 & \ttbar single lepton  \\
  410251 & \ttbar single lepton  \\
  410252 & \ttbar dileptonic  \\
  \bottomrule
  \end{tabular}
\end{table}

\paragraph{Short description:}

Additional samples of \ttbar events were produced with the
\SHERPA[2.2.1]~\cite{Bothmann:2019yzt} generator using NLO-accurate
matrix elements for up to one additional parton, and LO-accurate
matrix elements for up to four additional partons calculated with the
Comix~\cite{Gleisberg:2008fv} and
\OPENLOOPS~\cite{Buccioni:2019sur,Cascioli:2011va,Denner:2016kdg} libraries. They were
matched with the \SHERPA parton shower~\cite{Schumann:2007mg} using
the \MEPSatNLO
prescription~\cite{Hoeche:2011fd,Hoeche:2012yf,Catani:2001cc,Hoeche:2009rj}
and the set of tuned parameters developed by the \SHERPA authors
to match the \NNPDF[3.0nnlo] set of PDFs~\cite{Ball:2014uwa}.

\textbf{Additional information}: The central scale had the functional
form \(\mu^{2} = \mtop^{2} + 0.5\times(\pTX[2][t]p + \pTX[2][\bar{t}])\).
The CKKW matching scale of the
additional emissions was set to \SI{30}{\GeV}.


==> template/MC_snippets/ttgamma.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%              ttgamma                    %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section[\ttgamma production]{\ttgamma production}
\label{subsec:ttgamma}

This section describes the MC samples used for the modelling of \ttgamma\ production.
\Cref{subsubsec:ttgamma_aMCP8} describes the \MGNLOPY[8] samples,
and \cref{subsubsec:ttgamma_aMCH7} describes the \MGNLOHER[7] samples.

\subsection[MadGraph5\_aMC@NLO+Pythia8]{\MGNLOPY[8]}
\label{subsubsec:ttgamma_aMCP8}

\paragraph{Samples}
%\label{par:ttgamma_aMCP8_samples}

The descriptions below correspond to the samples in \cref{tab:ttgamma_aMCP8,tab:ttgamma_aMCP8_addRad}.

\begin{table}[htbp]
  \caption{Nominal \ttgamma\ samples produced with \MGNLOPY[8].}%
  \label{tab:ttgamma_aMCP8}
  \centering
  \begin{tabular}{l l}
    \toprule
    DSID range & Description \\
    \midrule
    410389 & \ttgamma, non-all-hadronic \\
    410394 & \ttgamma, all-hadronic \\
    \bottomrule
  \end{tabular}
\end{table}

\begin{table}[htbp]
  \caption{\ttgamma\ samples produced with \MGNLOPY[8] used to estimate initial-state radiation systematic uncertainties.}%
  \label{tab:ttgamma_aMCP8_addRad}
  \centering
  \begin{tabular}{l l}
    \toprule
    DSID range & Description \\
    \midrule
    410404 & \ttgamma\, non-all-hadronic, A14Var3c up \\
    410405 & \ttgamma\, non-all-hadronic, A14Var3c down \\
    410410 & \ttgamma\, all-hadronic, A14Var3c up \\
    410411 & \ttgamma\, all-hadronic, A14Var3c down \\
    \bottomrule
  \end{tabular}
\end{table}

\paragraph{Short description:}

The production of \ttgamma events was modelled using the \MGNLO[2.3.3]~\cite{Alwall:2014hca}
generator at LO with the \NNPDF[2.3lo]~\cite{Ball:2014uwa} parton distribution function~(PDF).
The events were interfaced with \PYTHIA[8.212]~\cite{Sjostrand:2014zea} using the A14 tune~\cite{ATL-PHYS-PUB-2014-021} and the
\NNPDF[2.3lo]~\cite{Ball:2014uwa} PDF set.
The decays of bottom and charm hadrons were simulated using the \EVTGEN[1.6.0] program~\cite{Lange:2001uf}.

The uncertainty due to initial-state radiation (ISR) was estimated by
comparing the nominal \ttgamma sample with two additional samples,
where the Var3c up/down variations of the A14 tune were employed.


\paragraph{Long description:}

The \ttgamma sample was simulated as a 2\(\to\)7 process at LO including the decay of the top quarks by
\MGNLO[2.3.3]~\cite{Alwall:2014hca} with the \NNPDF[2.3lo]~\cite{Ball:2014uwa} parton distribution function~(PDF), interfaced with
\PYTHIA[8.212]~\cite{Sjostrand:2014zea}, using the A14 set of tuned parameters~\cite{ATL-PHYS-PUB-2014-021} and the
\NNPDF[2.3lo]~\cite{Ball:2014uwa} PDF set. The photon could be radiated from an initial charged parton, an intermediate top quark,
or any of the charged final-state particles. The top-quark mass, top-quark decay width, \(W\)-boson decay width,
and fine structure constant were set to \SI{172.5}{\GeV}, \SI{1.320}{\GeV}, \SI{2.085}{\GeV}, and 1/137, respectively.
The five-flavour scheme was used, where all the quark masses are set to zero, except for the top quark. The renormalisation and the
factorisation scales were set to \(0.5\times \sum_i \sqrt{m^2_i+p^2_{\text{T},i}}\), where the sum runs over all the particles generated
from the matrix element calculation.
The decays of bottom and charm hadrons were simulated using the \EVTGEN[1.6.0] program~\cite{Lange:2001uf}.

The cross-section was calculated at NLO in QCD as reported in Ref.~\cite{Melnikov:2011ta}, resulting in a \(K\)-factor of 1.24 which was applied
to the samples, with a relative uncertainty of 14\% from variations of renormalisation and factorisation scales as well
as the choice of PDF set.

The uncertainty due to initial-state radiation (ISR) was estimated by comparing the nominal \ttV\ sample with two additional samples,
 which had the same settings as the nominal one, but employed the Var3c up or down variation of the A14 tune, which
corresponds to the variation of \alphas for initial-state radiation (ISR) in the A14 tune.

To evaluate the effect of renormalisation and factorisation scale uncertainties, the two scales were varied simultaneously by factors 2.0 and 0.5.
To evaluate the PDF uncertainties for the nominal PDF, the 100 replicas for \NNPDF[2.3lo] were taken into account.


\subsection[MadGraph5\_aMC@NLO+Herwig7]{\MGNLOHER[7]}
\label{subsubsec:ttgamma_aMCH7}

\paragraph{Samples}
%\label{par:ttgamma_aMCH7_samples}

The descriptions below correspond to the samples in \cref{tab:ttgamma_aMCH7}.

\begin{table}[htbp]
  \caption{\ttgamma\ samples produced with \MGNLOHER[7].}%
  \label{tab:ttgamma_aMCH7}
  \centering
  \begin{tabular}{l l}
    \toprule
    DSID range & Description \\
    \midrule
    410395 & \ttgamma non-all-hadronic \\
    410396 & \ttgamma all-hadronic \\
    \bottomrule
  \end{tabular}
\end{table}

\paragraph{Short description:}

Additional \ttgamma samples were produced with the parton shower of the nominal samples replaced by
\HERWIG[7.04]~\cite{Bahr:2008pv,Bellm:2015jjp} to evaluate the impact of using using a different parton shower and hadronisation model.
The H7UE set of tuned parameters~\cite{Bellm:2015jjp} and the \MMHT[lo] PDF set~\cite{Harland-Lang:2014zoa} were used.


==> template/MC_snippets/tttt.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%              tttt                    %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section[\tttt production]{\tttt production}
\label{subsec:tttt}

This section describes the MC samples used for the modelling of \tttt\ production.
\Cref{subsubsec:tttt_aMCP8} describes the \MGNLOPY[8] samples,
and \cref{subsubsec:tttt_aMCH7} describes the \MGNLOHER[7] samples.

\subsection[MadGraph5\_aMC@NLO+Pythia8]{\MGNLOPY[8]}
\label{subsubsec:tttt_aMCP8}

\paragraph{Samples}
%\label{par:tttt_aMCP8_samples}

The descriptions below correspond to the samples in \cref{tab:tttt_aMCP8}.

\begin{table}[htbp]
  \caption{Nominal \tttt\ samples produced with \MGNLOPY[8].}%
  \label{tab:tttt_aMCP8}
  \centering
  \begin{tabular}{l l}
    \toprule
    DSID range & Description \\
    \midrule
    412043 & \tttt \\
    \bottomrule
  \end{tabular}
\end{table}

\paragraph{Short description:}

The production of \tttt\ events was modelled using the \MGNLO[2.3.3]~\cite{Alwall:2014hca}
generator at NLO with the \NNPDF[3.1nlo]~\cite{Ball:2014uwa} parton distribution function~(PDF).
The events were interfaced with \PYTHIA[8.230]~\cite{Sjostrand:2014zea}~ using the A14 tune~\cite{ATL-PHYS-PUB-2014-021} and the
\NNPDF[2.3lo]~\cite{Ball:2014uwa} PDF set.
The decays of bottom and charm hadrons were simulated using the \EVTGEN[1.6.0] program~\cite{Lange:2001uf}.


\paragraph{Long description:}

The production of \tttt\ events was modelled using the \MGNLO[2.3.3]~\cite{Alwall:2014hca}
generator, which provided matrix elements at next-to-leading order~(NLO) in the strong coupling constant \alphas
with the \NNPDF[3.1nlo]~\cite{Ball:2014uwa} parton distribution function~(PDF).
The functional form of the renormalisation and factorisation scales was set to \(0.25\times \sum_i \sqrt{m^2_i+p^2_{\text{T},i}}\),
where the sum runs over all the particles generated from the matrix element calculation, following the Ref.~\cite{Frederix:2017wme}.
Top quarks were decayed at LO using \MADSPIN~\cite{Frixione:2007zp,Artoisenet:2012st} to preserve all spin correlations.
The events were interfaced with \PYTHIA[8.230]~\cite{Sjostrand:2014zea} for the parton shower and hadronisation,
using the A14 set of tuned parameters~\cite{ATL-PHYS-PUB-2014-021} and the \NNPDF[2.3lo]~\cite{Ball:2014uwa} PDF set.
The decays of bottom and charm hadrons were simulated using the \EVTGEN[1.6.0] program~\cite{Lange:2001uf}.


\subsection[MadGraph5\_aMC@NLO+Herwig7]{\MGNLOHER[7]}
\label{subsubsec:tttt_aMCH7}

\paragraph{Samples}
%\label{par:tttt_aMCH7_samples}

The descriptions below correspond to the samples in \cref{tab:tttt_aMCH7}.

\begin{table}[htbp]
  \caption{\tttt\ samples produced with \MGNLOHER[7].}%
  \label{tab:tttt_aMCH7}
  \centering
  \begin{tabular}{l l}
    \toprule
    DSID range & Description \\
    \midrule
    412044 & \tttt \\
    \bottomrule
  \end{tabular}
\end{table}

\paragraph{Description:}

Additional \tttt\ samples were produced with the parton shower of the nominal samples replaced by
\HERWIG[7.04]~\cite{Bahr:2008pv,Bellm:2015jjp} to evaluate the impact of using a different parton shower and hadronisation model. The H7UE set of
tuned parameters~\cite{Bellm:2015jjp} and the \MMHT[lo] PDF set~\cite{Harland-Lang:2014zoa} were used.


==> template/SUSY/executive_summary.tex <==
\section{Executive Summary}

This section, ideally less than two pages, should be placed at the beginning of the supporting note.
It should give a high-level overview of the analysis including (but not limited to):
\begin{itemize}
\item physics target and the general characteristics of the signal;
\item analysis strategy;
\item general characteristics of the control, validation, and signal regions;
\item a background estimation strategy overview;
\item highlights of major or most important points of the analysis;
\item a table or list of all critical tasks and who is responsible for each.
\end{itemize}

This section should include explicit pointers to the items required for the PAR and FAR\@.  For reference, those items are listed below. Please feel free to modify these lists into references to document sections.

For a PAR (ed board request), the SUSY group looks for:
\begin{itemize}
\item A definition of the target scenarios
\item A brief run-down of the signal grids, in particular pointing to any production problems or places where the production has not yet begun
\item A discussion of any non-standard object definitions in the analysis, and any on-going development that might affect the object definition
\item A discussion of the derivations: whether any reprocessing is needed, and whether the required samples have been requested
\item Data/MC comparisons in some inclusive regions (demonstrating the technical ability to use the data from all periods in the team's framework)
\item Any signal region definitions that are available, with some preliminary optimization in place and some description of the optimization procedure
\item Plans for further optimization (e.g.\ optimization for different model space regions, or use of an MVA or multi-bin fit)
\item An outline of the plans to get from here to a paper (plan of work, noting if person power is insufficient for any of the areas), as a part of this summary
\item An explicit list of differences in object definitions from the recommendations of the \href{https://gitlab.cern.ch/atlas-phys-susy-wg/Combinations/readme/wikis/home}{Combination Team}, with justification.
\item The location of the analysis code in GIT and demonstration that you have set up containers (\href{https://recast-docs.web.cern.ch/recast-docs/building_images_on_ci/}{described here}).
\end{itemize}

If you are using SUSYTools, please include the current configuration file in the \href{http://gitlab.cern.ch/atlas-phys-susy-wg/AnalysisSUSYToolsConfigurations}{archive}.

For a FAR, the SUSY group looks for:
\begin{itemize}
\item Definitions of SR, CR, VR, including expected yields with the targeted luminosity for all backgrounds that will be estimated with transfer factors or pure MC\@.
    Include signal contamination in CR and VR\@.
\item Cutflow for the background and for representative signal points.
\item Outline of background estimation strategies, including validation and closure tests for data-driven estimations. Statistical uncertainties for transfer-factor (TF) estimated and data-driven estimated backgrounds.
\item Comparison of data and MC with the relevant dataset in CR and VR\@. Strategy for mitigation of mis-modelling wherever needed with proof of feasibility.
\item Estimate of the detector level systematic uncertainties through propagation of CP recommendations.
\item A clear statement on how all others systematic uncertainties will be evaluated, including theory uncertainties on both backgrounds and signal: all the procedures need to be defined before unblinding.
\item A clear plan for ``discovery regions'' as well as the statistical treatment of the signal regions.
\item Background only fit with pull plot for the nuisance parameters.
\item Estimated exclusion, including depth of exclusion within the normal exclusion contour, with Asimov fit.
\item To-do list for achieving final result and possible bottlenecks (can the rest of the SUSY WG help with anything?)
\item For analyses using machine learning methods, additional diagnostics are required, which are explained \href{https://twiki.cern.ch/twiki/bin/view/AtlasProtected/SusyMachineLearning}{here}.
\item The location in GIT where your code is using containers and the first implementation of workflows towards recast (\href{https://recast-docs.web.cern.ch/recast-docs/workflowauthoring/intro/}{described here}).
\end{itemize}

The background forum recommends the following diagnostic plots:
\begin{itemize}
\item Standard occupancy maps and plots that can reveal detector or non-collision background issues --- plot for CRs, VRs and SRs of MET phi, the leading jet and/or leading lepton eta vs.\ phi 2D map, and the leading jet and/or leading lepton phi distributions
\item Selection efficiencies as a function of mu (VR, SR, and CR): to check how dependent the analysis is on pileup (primarily for MC)
\item Run number and data period dependencies: plot lumi-normalized yields in CRs, VRs and SRs as a function of the run number and data period (data only).
    This is to check for potential temporary issues in the data present only for certain runs, and to reveal potential chunks of data not processed by mistake.
    You should normalize the per-run yield using the lumi as reported from an independent source (not the in-file metadata!),
    e.g.\ simply use \href{https://svnweb.cern.ch/trac/atlasoff/browser/PhysicsAnalysis/SUSYPhys/SUSYTools/trunk/scripts/ilumi2histo.py}{this script in SUSYTools} to build the luminosity-vs-run histogram from your \texttt{iLumiCalc} file.
\item In particular, for Full Run 2 dataset analyses, a plot of data from 2018 vs period, specifically to compare the efficiencies for the period with two dead tile modules to the periods without.
\item Check for missing data: Compare the total number of processed data events and compare to the reference numbers for the combination of GRL and derivation you're running over in \href{https://docs.google.com/spreadsheets/d/1LMioo0nvALkKgoCKRW_ihQThHyVwcOQVRJe4aXiENUs/edit#gid=424865170}{this spreadsheet}. If your total does not match this reference number, feel free to contact BG forum conveners and derivation contacts for help with debugging.
\item Check for duplicated events: several bugs in MC and DAOD production have caused duplicated events to appear in the derivations in the past. This can potentially happen in both MC and data. Please check that there are no duplicated events in your CRs, VRs or SRs. If you notice duplicated events in your derivations, please get in touch with the Background Forum conveners immediately.
\item Comparisons of data and MC in the CRs and VRs, as well as MC in the SRs, for 2015+2016, 2017, and 2018 separately, for key distributions and yields.
\item Debug stream yields in SR and CR\@. The full name of the debug stream is \texttt{debugrec\_hlt}, and derivation datasets can be found for both 2015 and 2016 data with a query like \texttt{rucio ls --short --filter type=container data*\_13TeV.00*.debugrec\_hlt*DAOD\_SUSY1*p2709*}.
\item Pileup reweighting check: plot the nvtx distribution before and after pileup reweighting (data Vs MC). Purpose: check that the pileup reweighting works as intended.
\end{itemize}

Again, if you are using SUSYTools, please include the current configuration file in the \href{http://gitlab.cern.ch/atlas-phys-susy-wg/AnalysisSUSYToolsConfigurations}{archive}.  Please also take care that you have looked into the \href{https://twiki.cern.ch/twiki/bin/viewauth/Atlas/DataPreparationCheckListForPhysicsAnalysis}{items recommended by DataPrep}.


==> template/atlas-auxmat.tex <==
\part*{Auxiliary material}
\addcontentsline{toc}{part}{Auxiliary material}
%-------------------------------------------------------------------------------

In an ATLAS paper, auxiliary plots and tables that are supposed to be made public 
should be collected in an appendix that has the title \enquote{Auxiliary material}.
This information will appear on the public webpage, but will not be included
in the document submitted to arXiv and to the journal.


==> template/atlas-detector.tex <==
% Footnote with ATLAS coordinate system
\newcommand{\AtlasCoordFootnote}{%
ATLAS uses a right-handed coordinate system with its origin at the nominal interaction point (IP)
in the centre of the detector and the \(z\)-axis along the beam pipe.
The \(x\)-axis points from the IP to the centre of the LHC ring,
and the \(y\)-axis points upwards.
Cylindrical coordinates \((r,\phi)\) are used in the transverse plane, 
\(\phi\) being the azimuthal angle around the \(z\)-axis.
The pseudorapidity is defined in terms of the polar angle \(\theta\) as \(\eta = -\ln \tan(\theta/2)\).
Angular distance is measured in units of \(\Delta R \equiv \sqrt{(\Delta\eta)^{2} + (\Delta\phi)^{2}}\).}

%-------------------------------------------------------------------------------
\subsection{Run 2 ATLAS detector example for a Letter}
\label{sec:atlas2a}
%-------------------------------------------------------------------------------

The ATLAS experiment~\cite{PERF-2007-01} at the LHC is a multipurpose particle detector
with a forward--backward symmetric cylindrical geometry and a near \(4\pi\) coverage in 
solid angle.\footnote{\AtlasCoordFootnote}
It consists of an inner tracking detector surrounded by a thin superconducting solenoid
providing a \SI{2}{\tesla} axial magnetic field, electromagnetic and hadron calorimeters, and a muon spectrometer.
The inner tracking detector covers the pseudorapidity range \(|\eta| < 2.5\).
It consists of silicon pixel, silicon microstrip, and transition radiation tracking detectors.
Lead/liquid-argon (LAr) sampling calorimeters provide electromagnetic (EM) energy measurements
with high granularity.
A steel/scintillator-tile hadron calorimeter covers the central pseudorapidity range (\(|\eta| < 1.7\)).
The endcap and forward regions are instrumented with LAr calorimeters
for both the EM and hadronic energy measurements up to \(|\eta| = 4.9\).
The muon spectrometer surrounds the calorimeters and is based on
three large superconducting air-core toroidal magnets with eight coils each.
The field integral of the toroids ranges between \num{2.0} and \SI{6.0}{\tesla\metre}
across most of the detector. 
The muon spectrometer includes a system of precision tracking chambers and fast detectors for triggering.
A two-level trigger system is used to select events.
The first-level trigger is implemented in hardware and uses a subset of the detector information
to accept events at a rate below \SI{100}{\kHz}.
This is followed by a software-based trigger that
reduces the accepted event rate to \SI{1}{\kHz} on average
depending on the data-taking conditions.
An extensive software suite~\cite{ATL-SOFT-PUB-2021-001} is used in the reconstruction and analysis of real
and simulated data, in detector operations, and in the trigger and data acquisition systems of the experiment.

%-------------------------------------------------------------------------------
\subsection{Run 2 ATLAS detector example for a paper making use of the whole detector}
\label{sec:atlas2b}
%-------------------------------------------------------------------------------

The ATLAS detector~\cite{PERF-2007-01} at the LHC covers nearly the entire solid angle around the collision point.\footnote{\AtlasCoordFootnote}
It consists of an inner tracking detector surrounded by a thin superconducting solenoid, electromagnetic and hadron calorimeters,
and a muon spectrometer incorporating three large superconducting air-core toroidal magnets.

The inner-detector system (ID) is immersed in a \SI{2}{\tesla} axial magnetic field 
and provides charged-particle tracking in the range \(|\eta| < 2.5\).
The high-granularity silicon pixel detector covers the vertex region and typically provides four measurements per track, 
the first hit normally being in the insertable B-layer (IBL) installed before Run~2~\cite{ATLAS-TDR-19,PIX-2018-001}.
It is followed by the silicon microstrip tracker (SCT), which usually provides eight measurements per track.
These silicon detectors are complemented by the transition radiation tracker (TRT),
which enables radially extended track reconstruction up to \(|\eta| = 2.0\). 
The TRT also provides electron identification information 
based on the fraction of hits (typically 30 in total) above a higher energy-deposit threshold corresponding to transition radiation.

The calorimeter system covers the pseudorapidity range \(|\eta| < 4.9\).
Within the region \(|\eta|< 3.2\), electromagnetic calorimetry is provided by barrel and 
endcap high-granularity lead/liquid-argon (LAr) calorimeters,
with an additional thin LAr presampler covering \(|\eta| < 1.8\)
to correct for energy loss in material upstream of the calorimeters.
Hadron calorimetry is provided by the steel/scintillator-tile calorimeter,
segmented into three barrel structures within \(|\eta| < 1.7\), and two copper/LAr hadron endcap calorimeters.
The solid angle coverage is completed with forward copper/LAr and tungsten/LAr calorimeter modules
optimised for electromagnetic and hadronic energy measurements respectively.

The muon spectrometer (MS) comprises separate trigger and
high-precision tracking chambers measuring the deflection of muons in a magnetic field generated by the superconducting air-core toroidal magnets.
The field integral of the toroids ranges between \num{2.0} and \SI{6.0}{\tesla\metre}
across most of the detector. 
Three layers of precision chambers, each consisting of layers of monitored drift tubes, covers the region \(|\eta| < 2.7\),
complemented by cathode-strip chambers in the forward region, where the background is highest.
The muon trigger system covers the range \(|\eta| < 2.4\) with resistive-plate chambers in the barrel, and thin-gap chambers in the endcap regions.

Interesting events are selected by the first-level trigger system implemented in custom hardware,
followed by selections made by algorithms implemented in software in the high-level trigger~\cite{TRIG-2016-01}. 
The first-level trigger accepts events from the \SI{40}{\MHz} bunch crossings at a rate below \SI{100}{\kHz},
which the high-level trigger further reduces in order to record events to disk at about \SI{1}{\kHz}.

An extensive software suite~\cite{ATL-SOFT-PUB-2021-001} is used in the reconstruction and analysis of real
and simulated data, in detector operations, and in the trigger and data acquisition systems of the experiment.

%-------------------------------------------------------------------------------
\subsection{Run 1 ATLAS detector example for a Letter}
\label{sec:atlas1a}
%-------------------------------------------------------------------------------

The ATLAS experiment~\cite{PERF-2007-01} at the LHC is a multipurpose particle detector
with a forward--backward symmetric cylindrical geometry and a near \(4\pi\) coverage in 
solid angle.\footnote{\AtlasCoordFootnote}
It consists of an inner tracking detector surrounded by a thin superconducting solenoid
providing a \SI{2}{\tesla} axial magnetic field, electromagnetic and hadron calorimeters, and a muon spectrometer.
The inner tracking detector covers the pseudorapidity range \(|\eta| < 2.5\).
It consists of silicon pixel, silicon microstrip, and transition radiation tracking detectors.
Lead/liquid-argon (LAr) sampling calorimeters provide electromagnetic (EM) energy measurements
with high granularity.
A steel/scintillator-tile hadron calorimeter covers the central pseudorapidity range (\(|\eta| < 1.7\)).
The endcap and forward regions are instrumented with LAr calorimeters
for both the EM and hadronic energy measurements up to \(|\eta| = 4.9\).
The muon spectrometer surrounds the calorimeters and is based on
three large superconducting air-core toroidal magnets with eight coils each.
The field integral of the toroids ranges between \num{2.0} and \SI{6.0}{\tesla\metre}
across most of the detector. 
The muon spectrometer includes a system of precision tracking chambers and fast detectors for triggering.
A three-level trigger system is used to select events.
The first-level trigger is implemented in hardware and uses a subset of the detector information
to accept events at a rate of at most \SI{75}{\kilo\hertz}.
This is followed by two software-based trigger levels that
together reduce the accepted event rate to \SI{400}{\hertz} on average
depending on the data-taking conditions during 2012.
An extensive software suite~\cite{ATL-SOFT-PUB-2021-001} is used in the reconstruction and analysis of real
and simulated data, in detector operations, and in the trigger and data acquisition systems of the experiment.


%-------------------------------------------------------------------------------
\subsection{Run 1 ATLAS detector example for a paper making use of the whole detector}
\label{sec:atlas1b}
%-------------------------------------------------------------------------------

The ATLAS detector~\cite{PERF-2007-01} at the LHC covers nearly the entire solid angle around the collision point.\footnote{\AtlasCoordFootnote}
It consists of an inner tracking detector surrounded by a thin superconducting solenoid, electromagnetic and hadron calorimeters,
and a muon spectrometer incorporating three large superconducting air-core toroidal magnets.

The inner-detector system (ID) is immersed in a \SI{2}{\tesla} axial magnetic field 
and provides charged-particle tracking in the range \(|\eta| < 2.5\).
The high-granularity silicon pixel detector covers the vertex region and typically provides three measurements per track, 
the first hit normally being in the innermost layer.
It is followed by the silicon microstrip tracker (SCT) which usually provides eight measurements per track.
These silicon detectors are complemented by the transition radiation tracker (TRT),
which enables radially extended track reconstruction up to \(|\eta| = 2.0\). 
The TRT also provides electron identification information 
based on the fraction of hits (typically 30 in total) above a higher energy-deposit threshold corresponding to transition radiation.

The calorimeter system covers the pseudorapidity range \(|\eta| < 4.9\).
Within the region \(|\eta|< 3.2\), electromagnetic calorimetry is provided by barrel and 
endcap high-granularity lead/liquid-argon (LAr) calorimeters,
with an additional thin LAr presampler covering \(|\eta| < 1.8\)
to correct for energy loss in material upstream of the calorimeters.
Hadron calorimetry is provided by the steel/scintillator-tile calorimeter,
segmented into three barrel structures within \(|\eta| < 1.7\), and two copper/LAr hadron endcap calorimeters.
The solid angle coverage is completed with forward copper/LAr and tungsten/LAr calorimeter modules
optimised for electromagnetic and hadronic energy measurements respectively.

The muon spectrometer (MS) comprises separate trigger and
high-precision tracking chambers measuring the deflection of muons in a magnetic field generated by the superconducting air-core toroidal magnets.
The field integral of the toroids ranges between \num{2.0} and \SI{6.0}{\tesla\metre}
across most of the detector. 
A set of precision chambers covers the region \(|\eta| < 2.7\) with three layers of monitored drift tubes,
complemented by cathode-strip chambers in the forward region, where the background is highest.
The muon trigger system covers the range \(|\eta| < 2.4\) with resistive-plate chambers in the barrel, and thin-gap chambers in the endcap regions.

A three-level trigger system is used to select interesting events~\cite{PERF-2011-02}.
The first-level trigger is implemented in hardware and uses a subset of detector information
to accept events at a design value rate of at most \SI{75}{\kHz}.
This is followed by two software-based trigger levels which together reduce the event rate to about \SI{400}{\Hz}.

An extensive software suite~\cite{ATL-SOFT-PUB-2021-001} is used in the reconstruction and analysis of real
and simulated data, in detector operations, and in the trigger and data acquisition systems of the experiment.



==> template/atlas-hepdata.tex <==
\section{HepData material}
%-------------------------------------------------------------------------------

This file is available for detailed tables etc.\ that are going to be
submitted to HepData or other similar destinations.

==> template/atlas-note-metadata.tex <==
%-------------------------------------------------------------------------------
% This file contains the title, author and abstract.
% It also contains all relevant document numbers used for an ATLAS note.
%-------------------------------------------------------------------------------

% Title
\AtlasTitle{AtlasTitle: Bare bones ATLAS note}

% Draft version:
% Should be 1.0 for the first circulation, and 2.0 for the second circulation.
% If given, adds draft version on front page, a 'DRAFT' box on top of each other page, 
% and line numbers.
% Comment or remove in the final version.
\AtlasVersion{0.1}

% Abstract - % directly after { is important for correct indentation.
\AtlasAbstract{%
  This is a bare bones ATLAS note. Put the abstract for the document here.
}

% Author - this does not work with revtex (add it after \begin{document})
\author{The ATLAS Collaboration}

% Authors and list of contributors to the analysis.
% \AtlasAuthorContributor also adds the name to the author list.
% Include package latex/atlascontribute to use this.
% Use authblk package if there are multiple authors, which is included by latex/atlascontribute.
% \usepackage{authblk}
% Use the following 3 lines to have all institutes on one line.
% \makeatletter
% \renewcommand\AB@affilsepx{, \protect\Affilfont}
% \makeatother
% \renewcommand\Authands{, } % avoid ``. and'' for last author
% \renewcommand\Affilfont{\itshape\small} % affiliation formatting
% \AtlasAuthorContributor{First AtlasAuthorContributor}{a}{Author's contribution.}
% \AtlasAuthorContributor{Second AtlasAuthorContributor}{b}{Author's contribution.}
% \AtlasAuthorContributor{Third AtlasAuthorContributor}{a}{Author's contribution.}
% \AtlasContributor{Fourth AtlasContributor}{Contribution to the analysis.}
% \author[a]{First Author}
% \author[a]{Second Author}
% \author[b]{Third Author}
% \affil[a]{One Institution}
% \affil[b]{Another Institution}

% If a special author list should be indicated via a link use the following code:
% Include the two lines below if you do not use atlasstyle:
% \usepackage[marginal,hang]{footmisc}
% \setlength{\footnotemargin}{0.5em}
% Use the following lines in all cases:
% \usepackage{authblk}
% \author{The ATLAS Collaboration%
% \thanks{The full author list can be found at:\newline
%   \url{https://atlas.web.cern.ch/Atlas/PUBNOTES/ATL-PHYS-PUB-2021-XXX/authorlist.pdf}}
% }

% ATLAS reference code, to help ATLAS members to locate the paper.
\AtlasRefCode{GROUP-2021-XX}

% ATLAS note number. Can be an COM, INT, PUB or CONF note.
% \AtlasNote{ATLAS-CONF-2021-XXX}
% \AtlasNote{ATL-PHYS-PUB-2021-XXX}
% \AtlasNote{ATL-COM-PHYS-2021-XXX}


==> template/atlas-paper-metadata.tex <==
%-------------------------------------------------------------------------------
% This file contains the title, author and abstract.
% It also contains all relevant document numbers used by the different cover pages.
%-------------------------------------------------------------------------------

% Title
\AtlasTitle{AtlasTitle: Bare bones ATLAS document}

% Draft version:
% Should be 1.0 for the first circulation, and 2.0 for the second circulation.
% If given, adds draft version on front page, a 'DRAFT' box on top of every other page, 
% and line numbers.
% Comment or remove in the final version.
\AtlasVersion{0.1}

% Abstract - % directly after { is important for correct indentation
\AtlasAbstract{%
  This is a bare bones ATLAS document. Put the abstract for the document here.
}

% Author - this does not work with revtex (add it after \begin{document})
% This has to be commented out for TDR etc.
% For PUB notes, add package authblk and use \thanks if an ACE/STA should be added.
% See Section 4.2 of ATLAS LaTeX guide for more details.
% \author{The ATLAS Collaboration}

% ATLAS reference code, to help ATLAS members to locate the paper
\AtlasRefCode{GROUP-2021-XX}

% CERN preprint number
% \PreprintIdNumber{CERN-EP-2021-XX}

% ATLAS date - arXiv submission; usually filled in by the Physics Office
% \AtlasDate{\today}

% ATLAS heading - heading at top of title page. Set for TDR etc.
% \AtlasHeading{ATLAS ABC TDR}

% arXiv identifier
% \arXivId{21XX.YYYY}

% HepData record
% \HepDataRecord{ZZZZZZZZ}

% Submission journal and final reference
% \AtlasJournal{Phys.\ Lett.\ B.}
% \AtlasJournalRef{\PLB 789 (2021) 123}
% \AtlasDOI{}

%-------------------------------------------------------------------------------
% The following information is needed for the cover page. The commands are only defined
% if you use the coverpage option in atlasdoc or use the atlascover package
%-------------------------------------------------------------------------------

% List of supporting notes  (leave as null \AtlasCoverSupportingNote{} if you want to skip this option)
% \AtlasCoverSupportingNote{Short title note 1}{https://cds.cern.ch/record/XXXXXXX}
% \AtlasCoverSupportingNote{Short title note 2}{https://cds.cern.ch/record/YYYYYYY}
%
% OR (the 2nd option is deprecated, especially for CONF and PUB notes)
%
% Supporting material TWiki page  (leave as null \AtlasCoverTwikiURL{} if you want to skip this option)
% \AtlasCoverTwikiURL{https://twiki.cern.ch/twiki/bin/view/Atlas/WebHome}

% Comment deadline
% \AtlasCoverCommentsDeadline{DD Month 2021}

% Analysis team members - contact editors should no longer be specified
% as there is a generic email list name for the editors
% \AtlasCoverAnalysisTeam{Peter Analyser, Susan Editor1, Jenny Editor2, Alphonse Physicien}

% Editorial Board Members - indicate the Chair by a (chair) after his/her name
% Give either all members at once (then they appear on one line), or separately
% \AtlasCoverEdBoardMember{EdBoard~Chair~(chair), EB~Member~1, EB~Member~2, EB~Member~3}
% \AtlasCoverEdBoardMember{EdBoard~Chair~(chair)}
% \AtlasCoverEdBoardMember{EB~Member~1}
% \AtlasCoverEdBoardMember{EB~Member~2}
% \AtlasCoverEdBoardMember{EB~Member~3}

% A PUB note has readers and not an EdBoard -- give their names here (one line or several entries)
% \AtlasCoverReaderMember{Reader~1, Reader~2}
% \AtlasCoverReaderMember{Reader~1}
% \AtlasCoverReaderMember{Reader~2}

% Editors egroup
% \AtlasCoverEgroupEditors{atlas-GROUP-2021-XX-editors@cern.ch}

% EdBoard egroup
% \AtlasCoverEgroupEdBoard{atlas-GROUP-2021-XX-editorial-board@cern.ch}

